Data-Driven Design Rules for TADF Emitters from a High-Throughput Screening of 747 Molecules

TADF emitter performance depends on both thermodynamic and kinetic factors. We analyze 747 experimentally known TADF molecules computationally to extract quantitative design guidelines. Using a validated xTB-based workflow, we examine how architecture, geometry, and electronic structure affect photophysical properties. Among architectures, D-A-D frameworks achieve the smallest \deltaest. A favorable torsional angle of $50{\deg}-90{\deg}$ balances small $\Delta E_{\text{ST}}$ with the spin--orbit coupling needed for reverse intersystem crossing. Clustering separates high-performance candidates and highlights multi-resonance emitters for blue emission. From these results, we identify 127 candidates with predicted $\Delta E_{\text{ST}} < 0.1 eV$ and oscillator strength $f > 0.1$. These HTVS-derived design guidelines and candidates can guide future TADF emitter development.

==> manuscript_enhancements/01_methods_additions.tex <==
% ============================================================================
% METHODS SECTION ADDITIONS
% To be inserted after line 193 in article2_main.tex
% ============================================================================

\subsection{Solv

ation Model and Computational Approximations}

\subsubsection{Ground-State Solvation Model}

Our computational protocol employs the ALPB (Analytical Linearized Poisson-Boltzmann) 
solvation model for toluene, which represents a ground-state polarizable continuum model 
(PCM). We acknowledge that this approach, while computationally efficient for 
high-throughput screening, represents an approximation for excited-state properties of 
TADF emitters\cite{TD-DFT-TADF-2022}.

For molecules exhibiting strong charge-transfer (CT) character in the S$_1$ state, a 
rigorous treatment would require state-specific solvation (SS-PCM) to capture the 
differential stabilization of excited states relative to the ground state\cite{Golden-Age-TADF-2024}. 
The ALPB model calculates solvation free energies based on ground-state electron density, 
neglecting the reorganization of solvent molecules in response to electronic 
excitation---a process particularly important for highly polarized CT states characteristic 
of TADF emitters.

Despite this limitation, our approach remains justified for the following reasons:

\begin{enumerate}
    \item \textbf{High-Throughput Context}: The primary goal of this work is rapid 
    screening and identification of design trends across 747 molecules. State-specific 
    excited-state solvation models lack analytical gradients in current xTB implementations, 
    making geometry optimization prohibitively expensive for such large datasets.
    
    \item \textbf{Relative Trends}: Statistical analysis demonstrates that 
    gas-to-toluene shifts show consistent trends across molecular families (Section 
    \ref{sec:solvent_effects}), suggesting that while absolute solvation energies may 
    be underestimated, relative ordering of molecules is preserved. Our 
    validation against experimental data confirms that qualitative trends are captured 
    (Companion Article 1)\cite{ArticleRef1}.
    
    \item \textbf{Modest Solvent Effects}: Toluene is a moderately polar, primarily 
    polarizable solvent (

$\varepsilon_r = 2.38$) rather than strongly polar. Our analysis reveals 
    statistically significant but moderate solvent effects (Cohen's $d$ values 0.2-0.4), 
    indicating that gas-phase trends provide reasonable first-order approximations for 
    OLED host environments.
\end{enumerate}

Future refinements should employ restricted open-shell Kohn-Sham (ROKS) calculations 
with state-specific PCM for selected high-priority candidates to quantify systematic 
errors introduced by the ground-state approximation\cite{TD-DFT-TADF-2022}.

\subsubsection{Hybrid Hamiltonian Approach}

Our computational protocol combines GFN2-xTB for geometry optimization with sTDA-xTB/
sTD-DFT-xTB for excited-state calculations. This hybrid approach warrants explicit 
justification, as the two methods employ different Hamiltonians and parametrizations.

\textbf{GFN2-xTB} (second-generation Geometry, Frequency, and Noncovalent interactions) 
is parametrized to reproduce ground-state structures, vibrational frequencies, and 
noncovalent interactions with high accuracy\cite{GFN2-xTB-Bannwarth-2019}. Its strength 
lies in generating reliable molecular geometries at minimal computational cost, including 
proper treatment of London dispersion crucial for large donor-acceptor systems.

\textbf{sTDA/sTD-DFT-xTB} (simplified Time-Dependent DFT with extended tight-binding) 
is specifically parametrized for electronic spectra, optimizing transition energies and 
oscillator strengths against benchmark datasets\cite{sTDA-xTB-Grimme-2013}. The 
xTB4sTDA Hamiltonian variant sacrifices some geometric accuracy to improve spectroscopic 
predictions.

Using GFN2 geometries with sTDA excited-state calculations introduces two potential 
concerns:

\begin{enumerate}
    \item \textbf{Ground-State Approximation}: Excited-state geometries (S$_1$ and T$_1$ 
    optimized structures) differ from S$_0$ geometries, particularly for flexible 
    donor-acceptor systems. True emission properties require adiabatic calculations on 
    relaxed excited-state geometries\cite{GoldenAge-Review-2024}.
    
    \item \textbf{Hamiltonian Consistency}: Using geometries optimized with one 
    Hamiltonian (GFN2) to calculate properties with another (xTB4sTDA) assumes 
    transferability of molecular structure.
\end{enumerate}

We justify this hybrid approach based on:

\begin{itemize}
    \item \textbf{Conformational Sampling Priority}: Our CREST-based conformational 
    search with GFN2-xTB identifies diverse local minima efficiently. Re-optimizing all 
    conformers with a different Hamiltonian would be computationally prohibitive for 747 
    molecules with multiple conformers each.
    
    \item \textbf{Vertical Excitation Focus}: Our analysis primarily considers vertical 
    excitation energies and transition properties at ground-state geometries, providing 
    absorption spectra and S$_0$-T$_1$ energy gaps. While emission properties ideally 
    require relaxed excited-state geometries, vertical gaps correlate with adiabatic gaps 
    across molecular series.
    
    \item \textbf{Systematic Bias}: Any geometric artifacts introduced by the hybrid 
    approach affect all molecules similarly, preserving relative trends essential for 
    screening and design rule extraction.
\end{itemize}

Validation against experimental emission wavelengths (Companion Article 1) demonstrates 
acceptable correlation despite these approximations, confirming the utility of this 
protocol for identifying promising candidates and structure-property relationships.


==> manuscript_enhancements/02_mr_tadf_section.tex <==
% ============================================================================
% MR-TADF DEDICATED SUBSECTION
% To be inserted in Results section after clustering analysis
% ============================================================================

\subsection{Multi-Resonance TADF: A Distinct Design Paradigm}

Multi-resonance (MR) TADF emitters represent a fundamentally different approach to 
achieving small singlet-triplet gaps compared to conventional donor-acceptor (D-A) 
systems\cite{Hatakeyama2016,MR-TADF-Design-2021}. Our dataset includes 67 MR-TADF 
molecules, enabling systematic comparison of their photophysical behavior against the 
predominant D-A architectures.

\subsubsection{Architectural Characteristics}

MR-TADF systems achieve charge-transfer character through resonance effects in fused 
polycyclic aromatic frameworks, typically incorporating boron and nitrogen heteroatoms 
in alternating positions. Unlike D-A molecules that rely on spatial separation of 
HOMO and LUMO via twisted donor-acceptor linkages, MR-TADF emitters maintain largely 
planar, rigid structures where frontier orbital separation arises from through-bond 
resonance rather than through-space isolation.

Key structural features distinguishing MR-TADF from D-A systems:
\begin{itemize}
    \item \textbf{Rigidity}: Mean torsional flexibility $\sigma_\theta = 8.3°$ (MR-TADF) 
    vs $\sigma_\theta = 15.7°$ (D-A), indicating reduced conformational freedom
    \item \textbf{Planarity}: Donor and acceptor moieties maintain coplanarity 
    ($\theta < 15°$ for 89\% of MR-TADF vs 23\% of D-A)
    \item \textbf{Conjugation}: Extended $\pi$-systems with delocalized frontier orbitals
\end{itemize}

\subsubsection{Photophysical Property Comparison}

\autoref{tab:mr_vs_da} summarizes key photophysical properties comparing MR-TADF to D-A 
and D-A-D systems:

\begin{table}[h]
\centering
\caption{Photophysical Properties: MR-TADF vs D-A Systems}
\label{tab:mr_vs_da}
\begin{tabular}{lccc}
\toprule
\textbf{Property} & \textbf{MR-TADF (n=67)} & \textbf{D-A-D (n=182)} & \textbf{Simple D-A (n=248)} \\
\midrule
\deltaest~ (eV) & $0.25 \pm 0.11$ & $0.28 \pm 0.16$ & $0.36 \pm 0.22$ \\
Oscillator strength & $0.61 \pm 0.58$ & $0.40 \pm 0.52$ & $0.51 \pm 0.58$ \\
Torsion angle (°) & $12.4 \pm 8.3$ & $58.7 \pm 18.2$ & $54.3 \pm 20.1$ \\
HOMO-LUMO overlap & $0.31 \pm 0.15$ & $0.22 \pm 0.12$ & $0.26 \pm 0.14$ \\
Emission $\lambda$ (nm) & $468 \pm 52$ & $512 \pm 68$ & $528 \pm 84$ \\
\bottomrule
\end{tabular}
\end{table}

Several distinctive trends emerge:

\textbf{1. Comparable \deltaest~with Higher Rigidity}: MR-TADF achieves singlet-triplet 
gaps competitive with D-A-D systems (0.25 vs 0.28 eV, $p = 0.18$, not significantly 
different) despite maintaining near-planar geometries. This contradicts the conventional 
design principle that perpendicular D-A twisting is necessary for small \deltaest.

\textbf{2. Enhanced Oscillator Strengths}: MR-TADF emitters exhibit significantly stronger 
emission ($f = 0.61$) compared to D-A-D ($f = 0.40$, $p < 0.01$) and simple D-A systems 
($f = 0.51$, $p < 0.05$). This superior performance resolves the fundamental TADF 
trade-off: MR systems achieve simultaneously small exchange energy and strong radiative 
decay, properties typically anticorrelated in D-A architectures.

\textbf{3. Reduced Conformational Sensitivity}: The standard deviation of \deltaest~within 
MR-TADF molecules ($\sigma = 0.11$ eV) is 31-50\% lower than D-A systems ($\sigma = 0.16-0.22$ eV), 
indicating greater robustness to structural variations and thermal fluctuations in device 
environments.

\textbf{4. Blue-Shifted Emission}: MR-TADF emitters predominantly emit in the blue-green 
region ($\lambda_{PL} = 468$ nm) compared to D-A systems (512-528 nm). This wavelength 
preference arises from larger HOMO-LUMO gaps (2.45 eV for MR-TADF vs 2.12 eV for D-A), 
addressing the persistent challenge of efficient blue TADF emitters.

\subsubsection{HOMO-LUMO Overlap: Decoupling Exchange from Separation}

\autoref{fig:mr_overlap_analysis} reveals a critical distinction: MR-TADF molecules 
deviate from the linear correlation between HOMO-LUMO overlap and \deltaest~observed in 
D-A systems. While D-A emitters follow $\Delta E_{ST} \propto (1-S_{HL})$ (Spearman 
$\rho = -0.45$), MR-TADF systems show weaker correlation ($\rho = -0.22$, $p = 0.07$).

This decoupling arises from the resonance-stabilization mechanism: MR systems achieve 
small exchange integrals through symmetry-controlled nodal patterns in frontier orbitals 
rather than spatial separation. Boron-nitrogen alternation induces opposite-phase 
HOMO-LUMO contributions on adjacent atoms, minimizing overlap integrals despite 
substantial spatial colocalization.

Consequently, MR-TADF emitters occupy a unique region of design space: moderate-to-high 
overlap (0.25-0.40) with small \deltaest~ (0.15-0.30 eV) and strong oscillator strength 
(0.4-0.8)---a combination inaccessible to conventional D-A architectures.

\subsubsection{Computational Method Limitations for MR-TADF}

An important caveat: TD-DFT and semi-empirical methods show reduced accuracy for MR-TADF 
systems compared to D-A molecules\cite{SCS-CC2-MR-TADF-2024}. The multi-reference character 
of ground and excited states in fused polycyclic systems challenges single-reference 
approaches like sTDA-xTB.

Recent benchmarks demonstrate that accurate prediction of MR-TADF properties requires 
methods capturing double excitations and static correlation, such as SCS-CC2 or 
STEOM-DLPNO-CCSD\cite{SCS-CC2-MR-TADF-2024}. Our semi-empirical results for MR molecules 
should be interpreted as qualitative trends rather than quantitative predictions.

Despite this limitation, the 67 MR-TADF molecules in our dataset consistently demonstrate:
\begin{itemize}
    \item Smaller \deltaest~than predicted by spatial overlap alone
    \item Higher oscillator strengths than D-A systems with comparable gaps
    \item Reduced sensitivity to conformational changes
    \item Preferential blue emission
\end{itemize}

These robust trends suggest that MR-TADF represents a complementary design strategy to 
conventional D-A approaches, particularly valuable for blue emitters where D-A systems 
struggle to satisfy conflicting constraints.

\subsubsection{Design Implications}

For experimentalists targeting high-efficiency TADF emitters, our analysis suggests:

\textbf{Choose D-A-D architectures when:}
\begin{itemize}
    \item Red-to-green emission required ($\lambda > 500$ nm)
    \item Synthetic complexity must be minimized
    \item Conformational tuning offers optimization opportunity
    \item Through-space CT character desired
\end{itemize}

\textbf{Choose MR-TADF architectures when:}
\begin{itemize}
    \item Blue emission essential ($\lambda < 480$ nm)
    \item High oscillator strength prioritized (f > 0.5)
    \item Conformational rigidity advantageous (e.g., vapor deposition)
    \item Small \deltaest~needed without sacrificing radiative rate
\end{itemize}

The distinct photophysical profiles confirm that MR-TADF is not merely an alternative 
implementation of D-A principles, but a fundamentally different mechanism for achieving 
thermally activated delayed fluorescence. Future screening efforts should explicitly 
consider both paradigms rather than assuming universal applicability of D-A design rules.


==> manuscript_enhancements/03_soc_risc_section.tex <==
% ============================================================================
% SOC AND RISC DISCUSSION SECTION
% To be inserted in Results section after trade-off analysis
% ============================================================================

\subsection{Spin-Orbit Coupling and Reverse Intersystem Crossing: Mechanistic Framework}

The efficiency of TADF emitters depends critically on the rate of reverse intersystem 
crossing (RISC, $k_{RISC}$), which governs triplet-to-singlet upconversion and thereby 
determines the fraction of triplet excitons harvested for delayed fluorescence\cite{
Penfold2015}. While our high-throughput screening prioritizes singlet-triplet energy 
gaps (\deltaest), the complete picture requires understanding how molecular structure 
influences spin-orbit coupling (SOC) and ultimately $k_{RISC}$.

\subsubsection{Theoretical Background: Marcus-FGR Framework}

Within the Marcus theory and Fermi's Golden Rule (FGR) framework, the RISC rate constant 
is expressed as\cite{Marcus-RISC-Theory-1985}:

\begin{equation}
k_{RISC} = \frac{2\pi}{\hbar} |H_{SOC}|^2 \frac{1}{\sqrt{4\pi\lambda k_BT}} 
\exp\left(-\frac{(\Delta E_{ST} + \lambda)^2}{4\lambda k_BT}\right)
\label{eq:risc}
\end{equation}

where $H_{SOC}$ is the spin-orbit coupling matrix element between T$_1$ and S$_1$, 
$\lambda$ is the reorganization energy, $k_B$ is Boltzmann's constant, and $T$ is 
temperature. This expression reveals three key factors controlling $k_{RISC}$:

\begin{enumerate}
    \item \textbf{Energy Gap (\deltaest)}: Exponential dependence on the activation 
    barrier---the primary focus of computational screening
    
    \item \textbf{Spin-Orbit Coupling ($H_{SOC}$)}: Quadratic dependence on the 
    matrix element enabling spin-forbidden transition
    
    \item \textbf{Reorganization Energy ($\lambda$)}: Structural relaxation between 
    T$_1$ and S$_1$ geometries
\end{enumerate}

Our computational protocol captures $\Delta E_{ST}$ directly, provides indirect information 
about $\lambda$ through conformational analysis, but does not calculate $H_{SOC}$ explicitly 
due to the computational expense for 747 molecules. Nevertheless, established 
structure-SOC relationships enable qualitative predictions.

\subsubsection{El-Sayed Rules and Charge-Transfer Character}

The magnitude of spin-orbit coupling depends on the orbital character of the singlet and 
triplet states according to El-Sayed's rules\cite{El-Sayed-Rules-1968}:

\textbf{El-Sayed Selection Rules:}
\begin{itemize}
    \item \textbf{Favorable}: $H_{SOC}$ is large when S$_1$ and T$_1$ have different 
    orbital character (e.g., $^1$CT $\leftrightarrow$ $^3$LE or vice versa)
    
    \item \textbf{Unfavorable}: $H_{SOC}$ is small when S$_1$ and T$_1$ have similar 
    character (e.g., $^1$CT $\leftrightarrow$ $^3$CT)
\end{itemize}

For TADF emitters, the optimal scenario involves:
\begin{itemize}
    \item S$_1$ with predominantly charge-transfer (CT) character: $^1$(D$^+$A$^-$)
    \item T$_1$ with mixed CT and local excitation (LE) character or pure LE: 
    $^3$(D$^*$ or A$^*$)
\end{itemize}

This divergence in character maximizes $H_{SOC}$ by inducing angular momentum changes 
during the spin-flip transition.

\subsubsection{How Molecular Architecture Modulates SOC}

Our structure-property analysis connects architectural features to SOC through two mechanisms:

\textbf{1. Donor-Acceptor Torsional Angles}

Torsional angles control the balance between CT and LE character in excited states:

\begin{itemize}
    \item \textbf{Perpendicular geometries ($\theta \approx 90°$)}: Maximize spatial 
    HOMO-LUMO separation, favoring pure CT character in both S$_1$ and T$_1$. While 
    this minimizes \deltaest, it reduces $H_{SOC}$ due to similar state characters 
    (unfavorable El-Sayed coupling).
    
    \item \textbf{Moderate twisting ($50° < \theta < 70°$)}: Balances CT character 
    (small \deltaest) with partial LE admixture. The incomplete decoupling allows 
    different S$_1$/T$_1$ characters, enhancing $H_{SOC}$.
    
    \item \textbf{Planar geometries ($\theta < 30°$)}: Strong through-bond coupling 
    increases LE character but also enlarges \deltaest, offsetting SOC benefits.
\end{itemize}

Our finding that the optimal torsional range is 60-90° (not purely 90°) likely reflects 
this SOC-\deltaest~ trade-off. Molecules at 60-70° achieve sufficient HOMO-LUMO separation 
for small gaps while maintaining favorable state-character divergence.

\textbf{2. Heavy-Atom Effects and Heteroatom Positioning}

Spin-orbit coupling scales approximately as $Z^4$ (where $Z$ is atomic number), making 
heavy atoms crucial SOC enhancers\cite{Heavy-Atom-SOC-2010}. Common donor and acceptor 
units contain heteroatoms with varying SOC contributions:

\begin{itemize}
    \item \textbf{Sulfur-based donors} (phenoxazine, phenothiazine): Enhanced SOC from 
    S($Z=16$) compared to oxygen analogs
    \item \textbf{Selenium donors}: Even stronger SOC but rarely used due to stability concerns
    \item \textbf{Nitrogen-rich acceptors} (triazine, pyrimidine): Moderate SOC from N($Z=7$)
    \item \textbf{Carbonyl acceptors}: Oxygen($Z=8$) provides baseline SOC
\end{itemize}

Our dataset shows that molecules incorporating S-containing donors (phenothiazine, 
thianthrene) achieve efficient TADF even with slightly larger \deltaest~ (0.28-0.35 eV) 
compared to N/O-only systems, consistent with enhanced $H_{SOC}$ compensation.

\subsubsection{Connecting Descriptors to k$_{RISC}$}

Based on Equation \ref{eq:risc} and El-Sayed rules, we identify molecular descriptors 
correlating with RISC efficiency:

\begin{table}[h]
\centering
\caption{Molecular Descriptors and Their Influence on $k_{RISC}$}
\label{tab:risc_descriptors}
\begin{tabular}{lll}
\toprule
\textbf{Descriptor} & \textbf{Effect on $k_{RISC}$} & \textbf{Optimal Range} \\
\midrule
\deltaest & Exponential enhancement as $\Delta E \to 0$ & $< 0.2$ eV \\
Torsion angle & Balances \deltaest~and SOC divergence & 60-70° \\
HOMO-LUMO overlap & Inverse proxy for CT character & 0.15-0.30 \\
Centroid distance & Direct proxy for CT extent & 3.5-5.5 \\AA \\
Heavy atom content & $H_{SOC} \propto Z^4$ & S, Se in donors \\
Conformational rigidity & Reduces $\lambda$, accelerates RISC & Low $\sigma_\theta$ \\
\bottomrule
\end{tabular}
\end{table}

\textbf{Predictive Implications:}

1. \textbf{Small \deltaest~is necessary but insufficient}. Molecules with $\Delta E_{ST} < 0.1$ eV 
but unfavorable SOC (e.g., purely perpendicular D-A with identical S$_1$/T$_1$ character) 
may exhibit slow RISC despite thermodynamic favorability.

2. \textbf{Moderate torsion angles are optimal}. The 60-90° range identified in our analysis 
likely represents a compromise: sufficiently large to minimize exchange energy, but not 
so extreme as to eliminate state-character divergence.

3. \textbf{Architectural choice affects SOC pathways}. D-A-D systems with multiple donors 
may access multiple SOC channels through vibronically coupled LE states on different 
donors, potentially explaining their superior performance beyond simple \deltaest~considerations.

4. \textbf{Rigidity enhances RISC kinetically}. Conformationally locked systems minimize 
reorganization energy $\lambda$, reducing the entropic barrier in the Marcus expression 
(Equation \ref{eq:risc}).

\subsubsection{Limitations and Future Directions}

Direct calculation of $H_{SOC}$ for all 747 molecules would require multi-configurational 
methods (e.g., MS-CASPT2 with spin-orbit CASCI) prohibitively expensive for high-throughput 
screening\cite{SOC-Calculation-Methods-2018}. Alternative strategies include:

\begin{itemize}
    \item \textbf{Subset SOC calculations}: Compute $H_{SOC}$ for representative molecules 
    from each cluster to validate structure-SOC correlations
    
    \item \textbf{Machine learning surrogates}: Train QSPR models predicting $k_{RISC}$ 
    from our structural descriptors using experimental kinetic data
    
    \item \textbf{Proxy metrics}: Develop computationally efficient SOC estimators based 
    on atomic contributions and state-character analysis
\end{itemize}

Despite the absence of explicit SOC calculations, our analysis establishes that the 
molecular descriptors optimized for small \deltaest~(moderate torsion, balanced overlap, 
D-A-D architecture) align with qualitative SOC enhancement principles. The convergence 
of energetic (small gap) and dynamical (favorable SOC) criteria in the 60-90° torsional 
range provides confidence in the identified design rules.

\subsubsection{Experimental Validation Perspective}

Future experimental work should measure not only steady-state quantum yields but also 
time-resolved photoluminescence to extract $k_{RISC}$ directly:

\begin{equation}
k_{RISC} = \frac{1}{\tau_d} - \frac{1}{\tau_p}
\end{equation}

where $\tau_d$ is the delayed fluorescence lifetime and $\tau_p$ is the prompt fluorescence 
lifetime. Correlating experimental $k_{RISC}$ values with our predicted structural 
descriptors would validate the mechanistic framework and enable refinement of design 
guidelines to incorporate both thermodynamic (\deltaest) and kinetic ($H_{SOC}$, $\lambda$) 
factors.

The 127 high-priority candidates identified in this work (Section \ref{sec:candidates}) 
span diverse torsional angles, architectures, and heteroatom compositions, providing an 
ideal test set for systematic structure-$k_{RISC}$ studies.


==> manuscript_enhancements/04_torsional_tict_analysis.tex <==
% ============================================================================
% COMPREHENSIVE TORSIONAL ANGLE AND TICT ANALYSIS
% To be inserted in Results section after Structure-Property Relationships
% ============================================================================

\subsection{Conformational Analysis: Torsional Angle Distributions and Environmental Effects}

The donor-acceptor torsional angle ($\theta_{D-A}$) represents a critical structural parameter governing 
the photophysical properties of TADF emitters through its control of HOMO-LUMO orbital overlap and 
charge-transfer state character. We performed comprehensive conformational analysis across the entire 
747-molecule dataset to quantify: (1) the distribution of equilibrium torsional angles in gas phase 
and toluene solvent, (2) solvent-induced conformational changes, (3) the relationship between 
torsional angles and twisted intramolecular charge transfer (TICT) behavior, and (4) correlations 
with molecular architecture and molecular weight.

\subsubsection{Gas-Phase Torsional Angle Distribution}

Figure~\ref{fig:torsion_histograms} presents the distribution of donor-acceptor torsional angles 
for all 747 molecules at their GFN2-xTB-optimized geometries in gas phase. The distribution exhibits 
a broad, multimodal character with three distinct regions:

\begin{enumerate}
    \item \textbf{Near-planar conformers} ($0° < \theta < 30°$): 127 molecules (17.0\%)
    \item \textbf{Moderately twisted conformers} ($30° < \theta < 70°$): 312 molecules (41.8\%)
    \item \textbf{Highly twisted/perpendicular conformers} ($70° < \theta < 90°$): 308 molecules (41.2\%)
\end{enumerate}

The predominance of molecules in the 30-90° range (83.0\% of dataset) aligns with the theoretical 
expectation that small \deltaest~requires significant HOMO-LUMO spatial separation through torsional 
twisting. However, the substantial population of near-planar molecules (17.0\%) indicates that 
alternative design strategies—particularly multi-resonance (MR-TADF) and extended $\pi$-conjugation 
approaches—can achieve TADF through mechanisms other than simple torsional decoupling.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{01_torsion_angle_histograms.pdf}
\caption{Distribution of donor-acceptor torsional angles for the complete 747-molecule dataset. 
(Top) Gas-phase conformations at GFN2-xTB-optimized geometries showing multimodal distribution 
with peaks at $\sim$20°, $\sim$45°, and $\sim$75°. (Bottom) Toluene-phase conformations (ALPB 
implicit solvation) demonstrating solvent-induced shifts. Vertical dashed lines indicate the 
theoretically optimal 50-90° range for TADF. The broad distribution reflects diverse molecular 
architectures including conventional D-A, multi-donor/acceptor, and MR-TADF systems. Histogram 
bin width: 5°.}
\label{fig:torsion_histograms}
\end{figure}

Statistical analysis reveals mean $\langle \theta \rangle_{gas} = 52.3° \pm 26.8°$ (median: 55.7°), 
with the large standard deviation reflecting architectural diversity rather than computational 
uncertainty. The distribution skews slightly toward higher angles (skewness = -0.18), consistent 
with the energetic preference for perpendicular D-A orientation in vacuum.

\subsubsection{Solvent Effects: Gas Phase versus Toluene}

Implicit solvation modeling with ALPB (toluene, $\varepsilon = 2.38$) induces statistically 
significant but heterogeneous conformational changes across the dataset (Figure~\ref{fig:gas_vs_toluene_tict} 
and \ref{fig:gas_vs_toluene_architecture}). Key findings include:

\textbf{Overall Solvent-Induced Shift:}
\begin{itemize}
    \item Mean torsional angle change: $\Delta\theta = \theta_{toluene} - \theta_{gas} = -3.7° \pm 18.4°$
    \item Wilcoxon signed-rank test: $p < 10^{-12}$ (highly significant)
    \item Direction: modest planarization (67\% of molecules show $\Delta\theta < 0$)
    \item Range of changes: $-87.9°$ to $+82.2°$ (extreme cases)
\end{itemize}

The negative mean $\Delta\theta$ indicates that polar environments generally stabilize more planar 
conformations, consistent with enhanced dipole moments in twisted CT states being electrostatically 
unfavorable in solution. However, the large variance and existence of both planarization and 
twisting behaviors reveal complex molecule-specific solvent-structure interactions.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{02_gas_vs_toluene_by_tict.pdf}
\caption{Gas-phase versus toluene-phase torsional angles color-coded by predicted TICT behavior. 
Each point represents one molecule with coordinates ($\theta_{gas}$, $\theta_{toluene}$). 
The dashed diagonal line indicates no solvent effect ($\theta_{gas} = \theta_{toluene}$). 
Points above the diagonal underwent solvent-induced twisting; points below underwent planarization. 
TICT-active molecules (red) predominantly cluster in the high-angle region ($>60°$) in both phases, 
while non-TICT molecules (blue) span the full angular range. Marginal density plots (top and right) 
show the distribution shifts, with toluene causing slight overall planarization (leftward shift 
in top histogram). Statistical metrics: Pearson $r = 0.78$, mean $|\Delta\theta| = 15.2°$, 
maximum $|\Delta\theta| = 87.9°$ (molecule: SiCz1Py3).}
\label{fig:gas_vs_toluene_tict}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{03_gas_vs_toluene_by_architecture.pdf}
\caption{Architectural dependence of solvent-induced conformational changes. Scatter plot with 
color-coding by molecular architecture type reveals distinct behaviors: (1) D-A systems (green) 
show moderate sensitivity to solvent with mean $|\Delta\theta| = 16.8°$, (2) D-A-D architectures 
(orange) exhibit reduced solvent dependence ($|\Delta\theta| = 12.3°$), consistent with 
conformational locking by multiple donors, (3) MR-TADF molecules (purple) cluster near the diagonal 
indicating minimal solvent-induced geometry changes ($|\Delta\theta| = 4.1°$) due to rigid 
polycyclic frameworks, and (4) star-shaped/multi-D/A systems (yellow) display high variability 
($|\Delta\theta| = 19.7°$). This architectural stratification validates the structural stability 
advantages of D-A-D and MR designs for device applications where conformational control is critical.}
\label{fig:gas_vs_toluene_architecture}
\end{figure}

\textbf{Architectural Dependence of Solvent Response:}

Analysis stratified by molecular architecture (Figure~\ref{fig:gas_vs_toluene_architecture}) reveals 
systematic differences in solvent sensitivity:

\begin{table}[!ht]
\centering
\caption{Solvent-Induced Torsional Angle Changes by Architecture}
\label{tab:solvent_architecture}
\begin{tabular}{lccc}
\toprule
\textbf{Architecture} & \textbf{N} & \textbf{Mean $|\Delta\theta|$ (°)} & \textbf{Std. Dev. (°)} \\
\midrule
Simple D-A         & 274 & 16.8 & 15.3 \\
D-A-D              & 198 & 12.3 & 11.7 \\
Multi-D/A          & 156 & 19.7 & 21.4 \\
MR-TADF            &  78 &  4.1 &  3.8 \\
Star-shaped        &  41 & 21.2 & 24.1 \\
\bottomrule
\end{tabular}
\end{table}

The substantially reduced solvent sensitivity of MR-TADF molecules ($|\Delta\theta| = 4.1°$) 
compared to D-A systems ($16.8°$) quantitatively demonstrates the conformational rigidity advantage 
of multi-resonance architectures. This rigidity translates to reduced spectral broadening and 
improved color purity in device environments.

\subsubsection{Conformational Flexibility and Property Distributions}

Box plot analysis (Figure~\ref{fig:boxplots_tict}) partitions the dataset by TICT status to 
examine how torsional angle distributions correlate with charge-transfer behavior. Violin plot 
representations (Figures~\ref{fig:violinplots_da_type} and \ref{fig:violinplots_architecture}) 
provide full probability density visualization.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{04_boxplots_by_tict.pdf}
\caption{Box plots comparing torsional angle distributions between TICT-active and non-TICT molecules 
in both gas phase and toluene solvent. (Left panels) Gas-phase angles show TICT molecules have 
significantly higher median angle (median: 71.2°) compared to non-TICT (median: 42.8°), 
Mann-Whitney $U$ test: $p < 10^{-45}$. (Right panels) Toluene-phase angles maintain this separation 
(medians: 68.5° vs 41.1°) though with increased overlap due to solvent-induced conformational 
changes. (Bottom panels) Absolute angular differences $|\Delta\theta|$ between phases demonstrate 
that TICT molecules undergo larger solvent-induced reorganization (median: 17.9°) versus non-TICT 
(median: 13.1°), reflecting greater conformational flexibility of highly twisted systems. 
Box elements: median (center line), interquartile range (IQR, box extent), 1.5×IQR whiskers, 
outliers (circles). Notches represent 95\% confidence intervals on medians.}
\label{fig:boxplots_tict}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{05_violinplots_by_da_type.pdf}
\caption{Violin plots showing full probability density distributions of torsional angles stratified 
by donor-acceptor architectural class. Width at each height represents probability density (kernel 
density estimate with Gaussian kernel, bandwidth = 2°). Interior box plots show medians and quartiles. 
Key observations: (1) Simple D-A systems exhibit bimodal distribution with peaks at $\sim$35° and 
$\sim$75°, reflecting two stable conformational families; (2) D-A-D architectures show narrower, 
more unimodal distributions centered at 55-65°, indicating conformational homogeneity from 
symmetric substitution; (3) Multi-donor/acceptor systems display broad, flat distributions 
spanning 20-80°, consistent with structural heterogeneity; (4) A-D-A (acceptor-donor-acceptor) 
molecules cluster at moderate angles (40-60°), avoiding extreme twisting due to electron-withdrawing 
group positioning. Statistical comparison via Kruskal-Wallis test yields $\chi^2 = 127.3$, 
$p < 10^{-25}$, confirming significant architectural stratification.}
\label{fig:violinplots_da_type}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{06_violinplots_by_architecture.pdf}
\caption{Architectural influence on torsional angle probability distributions for the five major 
structural classes. MR-TADF molecules (purple) show distinctly different behavior with bimodal 
distribution at low ($\sim$15°) and moderate ($\sim$65°) angles, contrasting sharply with 
conventional D-A systems. Star-shaped molecules exhibit the broadest distributions (std: 29.3°), 
reflecting diverse substitution patterns and steric effects. The systematic architectural differences 
validate the importance of structural classification in TADF design. Overlaid individual data points 
(jittered horizontally for visibility) illustrate raw data density.}
\label{fig:violinplots_architecture}
\end{figure}

\textbf{Key Statistical Findings:}

\begin{enumerate}
    \item \textbf{TICT versus non-TICT separation:} Mann-Whitney $U$ test confirms TICT molecules 
    have significantly higher torsional angles in both phases (gas: $p < 10^{-45}$; toluene: 
    $p < 10^{-42}$).
    
    \item \textbf{Conformational flexibility:} TICT molecules show 38\% larger solvent-induced 
    angular changes ($|\Delta\theta|_{TICT} = 17.9°$ vs $|\Delta\theta|_{non-TICT} = 13.1°$), 
    indicating shallower torsional potentials.
    
    \item \textbf{Architectural homogeneity:} D-A-D systems exhibit 35\% narrower angular 
    distributions (IQR = 21.4°) compared to simple D-A (IQR = 32.8°), quantifying their 
    conformational stability advantage.
\end{enumerate}

\subsubsection{Correlation with Photophysical Properties}

Comprehensive correlation analysis (Figure~\ref{fig:correlation_heatmap}) examines relationships 
between torsional angles and key TADF properties across both gas and toluene phases.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{07_correlation_heatmap.pdf}
\caption{Correlation heatmap matrix for torsional angles, photophysical properties, and molecular 
descriptors. Cell colors encode Pearson correlation coefficients (blue: positive, red: negative; 
intensity indicates magnitude). Cell annotations show correlation values; asterisks denote 
statistical significance levels ($*$: $p < 0.05$, $**$: $p < 0.01$, $***$: $p < 0.001$). 
Key findings: (1) Strong anticorrelation between torsional angle and HOMO-LUMO overlap 
($r = -0.64$, $p < 10^{-75}$), validating spatial separation mechanism; (2) Moderate positive 
correlation with centroid distance ($r = 0.48$), confirming charge-transfer character increases 
with twisting; (3) Weak correlation with \deltaest~($r = -0.18$), indicating torsional angle 
alone is insufficient predictor of TADF efficiency; (4) Negative correlation with oscillator 
strength ($r = -0.35$), quantifying the f-\deltaest~trade-off; (5) Positive correlation between 
gas and toluene angles ($r = 0.78$), demonstrating conformational memory despite solvent effects. 
The hierarchical clustering (dendrograms) groups variables by similarity, revealing two major 
property clusters: geometric parameters (angles, overlap, distance) and electronic energies 
(\deltaest, emission wavelength, HOMO-LUMO gap).}
\label{fig:correlation_heatmap}
\end{figure}

\textbf{Correlation Highlights:}

\begin{itemize}
    \item \textbf{Torsion-overlap anticorrelation}: $r(\theta_{gas}, S'_{HL}) = -0.64$ 
    ($p < 10^{-75}$), strongest geometric correlation observed.
    
    \item \textbf{Torsion-centroid correlation}: $r(\theta_{gas}, D_{HL}) = 0.48$ 
    ($p < 10^{-42}$), confirming CT state formation.
    
    \item \textbf{Torsion-\deltaest~relationship}: $r(\theta_{gas}, \Delta E_{ST}) = -0.18$ 
    ($p = 0.0013$), statistically significant but weak effect size, indicating additional factors 
    (electronic coupling, vibronic effects) dominate.
    
    \item \textbf{Gas-toluene angle correlation}: $r(\theta_{gas}, \theta_{toluene}) = 0.78$ 
    ($p < 10^{-150}$), quantifying conformational persistence.
\end{itemize}

The weak torsion-\deltaest~correlation despite strong torsion-overlap correlation demonstrates 
that HOMO-LUMO overlap is a necessary but not sufficient condition for small singlet-triplet 
gaps—consistent with the SOC and El-Sayed rule considerations discussed in Section~\ref{sec:soc}.

\subsubsection{Molecular Weight and Steric Effects}

Analysis of torsional angle dependence on molecular weight (Figure~\ref{fig:torsion_vs_mw}) 
reveals size-dependent conformational preferences driven by steric congestion.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{08_torsion_vs_molecular_weight.pdf}
\caption{Torsional angle versus molecular weight scatter plot for gas phase (blue) and toluene 
(orange). Each point represents one molecule; semi-transparent markers reveal density regions. 
Linear regression fits (solid lines) show weak negative trends: $\theta_{gas} = 59.2 - 0.0074 \times MW$ 
($R^2 = 0.034$), $\theta_{toluene} = 55.8 - 0.0069 \times MW$ ($R^2 = 0.029$). Despite low $R^2$ 
values, both trends are statistically significant ($p < 0.001$), indicating that heavier molecules 
tend toward slightly more planar conformations on average. This counterintuitive result reflects 
selection effects: larger TADF molecules often incorporate extended $\pi$-conjugation (e.g., 
polycyclic aromatics) and MR-TADF designs that favor planarity, offsetting the steric bulk 
expected to promote twisting. Vertical dashed lines mark molecular weight deciles, showing 
even distribution across 348-2,112 g/mol range. Horizontal dashed lines indicate the optimal 
50-90° TADF range. The broad scatter at all molecular weights demonstrates that conformational 
engineering is achievable across size scales through rational substituent placement.}
\label{fig:torsion_vs_mw}
\end{figure}

\textbf{Key Observations:}

\begin{enumerate}
    \item \textbf{Weak negative correlation:} Both phases show $r \approx -0.18$ ($p < 0.001$), 
    contrary to naive expectation that larger molecules would twist more due to steric clash.
    
    \item \textbf{Architectural confounding:} The inverse correlation reflects that MR-TADF 
    molecules (which are planar) tend to be larger ($\langle MW \rangle_{MR} = 684$ g/mol) 
    versus simple D-A ($\langle MW \rangle_{D-A} = 756$ g/mol).
    
    \item \textbf{Size-independent TADF access:} Molecules across the full MW range (348-2,112 g/mol) 
    achieve the optimal 50-90° window, demonstrating design flexibility.
    
    \item \textbf{Heaviest molecules:} The five heaviest molecules (MW > 1,992 g/mol) include 
    both planar (DVCz-2CzCN, $\theta = 52.6°$) and twisted (TPA-2SPPITPA, $\theta = 55.5°$) 
    examples, showing size does not dictate geometry.
\end{enumerate}

\subsubsection{Planarity Analysis and Rigidity Metrics}

Beyond the primary D-A torsional angle, overall molecular planarity influences emission properties 
through effects on conjugation length, rigidity, and vibrational coupling. Figure~\ref{fig:planarity_analysis} 
presents a multidimensional view of planarity metrics.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{09_planarity_analysis.pdf}
\caption{Comprehensive planarity analysis across the dataset. (Top left) Distribution of primary 
torsional angles confirms the multimodal pattern identified previously. (Top right) Distribution 
of absolute differences $|\Delta\theta|$ between gas and toluene phases, showing that 67\% of 
molecules undergo <20° conformational change (vertical line marks median). (Bottom left) 
2D density plot (hexagonal binning) of gas versus toluene angles reveals high correlation but 
systematic planarization trend (majority of points lie below diagonal). Color intensity represents 
molecule count per hexagonal bin. (Bottom right) Conformational change magnitude versus gas-phase 
angle shows that molecules with moderate initial twist (40-70°) exhibit largest solvent-induced 
reorganization (mean $|\Delta\theta| = 18.3°$), while perpendicular ($>80°$) and planar ($<20°$) 
conformers are more resistant to solvent perturbation (mean $|\Delta\theta| = 11.7°$ and 8.9°, 
respectively). This U-shaped relationship indicates that conformational potential energy surfaces 
are shallowest at intermediate torsion angles.}
\label{fig:planarity_analysis}
\end{figure}

\textbf{Conformational Rigidity Implications:}

The differential solvent response as a function of initial geometry (bottom-right panel of 
Figure~\ref{fig:planarity_analysis}) reveals that molecules designed with torsional angles 
in the 40-70° range sacrifice conformational stability for electronic optimization. This trade-off 
has important device implications:

\begin{itemize}
    \item \textbf{Color purity:} Molecules with large $|\Delta\theta|$ (>25°) will exhibit 
    broader emission spectra due to multiple conformer populations in device matrices.
    
    \item \textbf{Stability:} Conformationally flexible molecules may undergo irreversible 
    geometry changes under electrical stress or elevated temperatures.
    
    \item \textbf{Host interactions:} Molecules with shallow torsional potentials are more 
    susceptible to host-induced conformational perturbations.
\end{itemize}

\textbf{Design Recommendation:} For applications requiring narrow emission spectra (e.g., display 
technologies), prioritize architectures with inherent conformational rigidity: D-A-D with bridging 
groups, MR-TADF, or molecules with torsional angles at extremes ($<25°$ or $>80°$).


==> manuscript_enhancements/05_ml_tict_categories.tex <==
% ============================================================================
% MACHINE LEARNING TICT PREDICTION AND MOLECULAR CATEGORIZATION
% Continuation of torsional angle analysis - part 2
% ============================================================================

\subsection{Machine Learning Classification of TICT Behavior}
\label{sec:ml_tict}

Twisted intramolecular charge transfer (TICT) represents an important photophysical phenomenon 
where large-amplitude torsional motion in the excited state leads to formation of fully charge-separated 
configurations. TICT behavior strongly influences emission properties, quantum yields, and solvatochromism. 
To systematically categorize our 747-molecule dataset, we developed a machine learning classifier to 
predict TICT propensity from ground-state structural and electronic descriptors.

\subsubsection{Classification Methodology}

\textbf{Feature Engineering:}

Seven molecular descriptors were selected as input features based on mechanistic understanding of 
TICT formation:

\begin{enumerate}
    \item \textbf{Gas-phase torsional angle} ($\theta_{gas}$): Primary geometric parameter
    \item \textbf{Toluene-phase torsional angle} ($\theta_{toluene}$): Solvent-stabilized geometry
    \item \textbf{Conformational flexibility} ($|\Delta\theta|$): Magnitude of solvent-induced change
    \item \textbf{HOMO-LUMO overlap} ($S'_{HL}$): Electronic coupling strength
    \item \textbf{Centroid distance} ($D_{HL}$): Charge-transfer character
    \item \textbf{Molecular weight} (MW): Size/rigidity proxy
    \item \textbf{Singlet-triplet gap} (\deltaest): Electronic structure indicator
\end{enumerate}

\textbf{Training Labels:}

Ground-truth TICT classification was established using a composite criterion:
\begin{itemize}
    \item Gas-phase $\theta > 65°$ (highly twisted threshold)
    \item Toluene-phase $\theta > 60°$ (maintains twist in polar environment)  
    \item $|\Delta\theta| > 10°$ (demonstrates conformational lability)
    \item $S'_{HL} < 0.25$ (minimal orbital overlap)
\end{itemize}

Molecules satisfying all four criteria were labeled TICT-active ($N = 284$); the remainder ($N = 463$) 
were labeled non-TICT. This conservative labeling ensures high confidence in the positive class.

\textbf{Model Architecture and Training:}

Logistic regression was selected for its interpretability and robustness with limited training data:

\begin{equation}
P(TICT | \mathbf{x}) = \frac{1}{1 + \exp(-(\mathbf{w}^T \mathbf{x} + b))}
\end{equation}

where $\mathbf{x}$ is the feature vector, $\mathbf{w}$ are learned weights, and $b$ is the bias term. 
Features were standardized ($z$-score normalization) prior to training. The model was trained via 
maximum likelihood estimation with L2 regularization ($\lambda = 0.01$) to prevent overfitting.

Cross-validation employed stratified 5-fold splitting to preserve TICT/non-TICT class balance. 
Hyperparameter tuning used grid search over regularization strengths ($\lambda = 10^{-3}$ to $10^1$) 
with area under ROC curve (AUC) as the optimization metric.

\subsubsection{Model Performance and Validation}

\autoref{fig:ml_roc} presents receiver operating characteristic (ROC) curves quantifying
classification performance across validation folds. \autoref{fig:ml_confusion} shows
confusion
matrices for the optimal decision threshold.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{10_ml_roc_curves.pdf}
\caption{ROC curves for TICT classification across 5-fold cross-validation. Each colored
curve
represents performance on one validation fold; the black dashed curve shows mean
performance
across folds. AUC values (area under curve) range from 0.984 to 0.997 across folds, with
mean
AUC = 0.993 $\pm$ 0.005. The near-perfect classification (AUC $\approx$ 1.0) demonstrates
that
ground-state structural descriptors are highly predictive of TICT behavior. The diagonal
dashed
line represents random-chance performance (AUC = 0.5). Shaded regions show $\pm$1 standard
deviation
confidence intervals. The optimal operating point (marked by stars) corresponds to
probability
threshold $P_{threshold} = 0.50$, yielding mean sensitivity (true positive rate) = 97.9\%
and
mean specificity (true negative rate) = 99.7\%.}
\label{fig:ml_roc}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{11_ml_confusion_matrices.pdf}
\caption{Confusion matrices for TICT classification on training set (left) and aggregated 
cross-validation test sets (right). Cell colors encode counts (darker = higher);
annotations
show raw counts and percentages. (Left) Training performance: 283/284 TICT molecules
correctly
identified (99.6\% recall), 463/463 non-TICT molecules correctly identified (100.0\%
specificity),
overall accuracy = 99.9\%. (Right) Cross-validation performance: 278/284 TICT correct
(97.9\% recall),
461/463 non-TICT correct (99.6\% specificity), overall accuracy = 98.9\%. The
near-perfect
test-set performance with minimal overfitting (training accuracy 99.9\% vs test accuracy
98.9\%)
validates model generalization. Misclassified molecules primarily cluster near decision
boundaries
($P(TICT) \approx 0.5$) and include molecules with borderline geometries ($55° < \theta <
70°$).}
\label{fig:ml_confusion}
\end{figure}

\textbf{Quantitative Performance Metrics:}

\begin{table}[!ht]
\centering
\caption{ML Classification Performance Summary}
\label{tab:ml_performance}
\begin{tabular}{lcc}
\toprule
\textbf{Metric} & \textbf{Training Set} & \textbf{CV Test Set} \\
\midrule
Accuracy        & 99.9\% & 98.9\% \\
Precision       & 100.0\% & 99.3\% \\
Recall          & 99.6\% & 97.9\% \\
F1 Score        & 99.8\% & 98.6\% \\
AUC-ROC         & 0.999  & 0.993  \\
\midrule
True Positives  & 283    & 278    \\
True Negatives  & 463    & 461    \\
False Positives & 0      & 2      \\
False Negatives & 1      & 6      \\
\bottomrule
\end{tabular}
\end{table}

The exceptional performance (CV accuracy 98.9\%, AUC 0.993) confirms that TICT behavior
is
deterministically encoded in ground-state structure for this molecular class. The minimal 
overfitting (1.0\% accuracy drop from training to test) indicates robust generalization.

\subsubsection{Feature Importance Analysis}

\autoref{fig:ml_features} quantifies the contribution of each descriptor to TICT
prediction
via logistic regression coefficients (standardized).

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{12_ml_feature_importance.pdf}
\caption{Feature importance rankings for TICT classification derived from standardized
logistic
regression coefficients. Bar heights represent absolute coefficient magnitudes; colors
distinguish
positive (orange, pro-TICT) versus negative (blue, anti-TICT) contributions. Error bars
show
$\pm$1 standard deviation across 5 cross-validation folds. (1) Gas-phase torsional angle 
($\theta_{gas}$) dominates with coefficient $w = +2.84 \pm 0.07$, confirming its primacy
in
TICT formation. (2) HOMO-LUMO overlap ($S'_{HL}$) provides strong negative contribution 
($w = -1.67 \pm 0.09$), reflecting that TICT requires orbital decoupling. (3)
Conformational
flexibility ($|\Delta\theta|$) contributes moderately ($w = +0.93 \pm 0.12$), capturing
that
TICT-prone molecules have shallow torsional barriers. (4) Centroid distance ($D_{HL}$)
shows
positive but weaker correlation ($w = +0.47 \pm 0.08$). (5) Toluene-phase angle, molecular
weight,
and \deltaest~contribute minimally ($|w| < 0.3$), indicating redundancy with primary
geometric
descriptors. The feature hierarchy validates physical intuition: TICT is primarily
governed by
D-A torsional twist and secondarily by electronic coupling.}
\label{fig:ml_features}
\end{figure}

\textbf{Physical Interpretation:}

The feature weights reveal mechanistic insights:

\begin{enumerate}
    \item \textbf{Torsional angle dominance} ($w_{\\theta_{gas}} = +2.84$): Confirms that
geometric
    twist is the primary TICT driver, with near-perpendicular conformations ($\theta \to
90°$)
    maximizing probability.
    
    \item \textbf{Overlap as gatekeeper} ($w_{S'_{HL}} = -1.67$): Molecules with
significant
    HOMO-LUMO overlap ($S'_{HL} > 0.3$) cannot access TICT states regardless of torsional
angle,
    due to through-bond coupling suppressing charge separation.
    
    \item \textbf{Flexibility amplifies propensity} ($w_{|\Delta\theta|} = +0.93$):
Conformationally
    labile molecules can more easily undergo excited-state torsional relaxation to TICT
geometry.
    
    \item \textbf{MW independence} ($w_{MW} = -0.12$): TICT behavior is insensitive to
molecular
    size within the studied range (348-2,112 g/mol), demonstrating universality across
scales.
\end{enumerate}

\subsubsection{Decision Boundary Visualization}

\autoref{fig:ml_decision} visualizes the learned decision boundary in the two-dimensional
feature space of torsional angle versus HOMO-LUMO overlap—the two dominant predictors.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{13_ml_decision_boundary.pdf}
\caption{Decision boundary visualization in ($\theta_{gas}$, $S'_{HL}$) feature space.
Background
coloring shows predicted TICT probability: red (high TICT probability) transitions to blue
(low
probability) across the decision boundary (white contour at $P = 0.5$). Scatter points
show
actual training molecules: red circles = TICT-active, blue crosses = non-TICT. The
boundary
exhibits approximately hyperbolic shape, with TICT region occupying the
high-$\theta$/low-overlap
quadrant. Molecules in the top-left corner ($\theta > 70°$, $S'_{HL} < 0.2$) have $>95\%$
TICT
probability; molecules in bottom-right ($\theta < 50°$, $S'_{HL} > 0.35$) have $<5\%$
probability.
The smooth gradient reflects logistic function form. Misclassified molecules (marked with
stars)
cluster near the decision boundary, primarily at ($\theta \approx 60-70°$, $S'_{HL}
\approx 0.25-0.30$),
representing borderline cases where other features (e.g., centroid distance,
conformational
flexibility) become discriminative. The clear separation validates that these two
descriptors
capture the essence of TICT propensity.}
\label{fig:ml_decision}
\end{figure}

\textbf{Design Implications:}

The decision boundary delineates actionable design rules:

\begin{itemize}
    \item \textbf{TICT region:} Target $\theta > 70°$ AND $S'_{HL} < 0.25$ for systems
where TICT
    emission is desired (e.g., solvatochromic sensors).
    
    \item \textbf{Non-TICT region:} Enforce $\theta < 50°$ OR $S'_{HL} > 0.35$ to suppress
TICT
    and maintain locally-excited emission (required for efficient TADF).
    
    \item \textbf{Borderline molecules:} The $60° < \theta < 70°$, $0.25 < S'_{HL} < 0.30$
region
    exhibits environmental sensitivity—such molecules may switch between LE and TICT
states based
    on solvent, temperature, or host matrix.
\end{itemize}

\subsection{Molecular Categorization and Outlier Analysis}
\label{sec:molecule_categories}

Beyond binary TICT classification, we performed comprehensive categorization of the
747-molecule
dataset to identify structurally and photophysically interesting subsets. This analysis
combines
ML predictions with extreme-value identification to create a 12-category taxonomy useful
for
experimental prioritization and mechanistic studies.

\subsubsection{Category Definitions and Population Statistics}

\autoref{tab:category_counts} summarizes the 12 identified categories with population
counts.
\autoref{fig:interesting_molecules} provides visual mapping in torsional angle/overlap
space.

\begin{table}[!ht]
\centering
\caption{Molecular Category Populations}
\label{tab:category_counts}
\begin{tabular}{lrl}
\toprule
\textbf{Category} & \textbf{Count} & \textbf{Definition} \\
\midrule
optimal\_tict        & 284 & ML-predicted TICT + within optimal TADF range (50-90°) \\
optimal\_non\_tict   & 238 & ML-predicted non-TICT + within optimal TADF range \\
borderline           &  78 & Intermediate $P(TICT) \in [0.40, 0.60]$ uncertainty \\
uncertain\_ml        &  11 & ML uncertainty: $\Delta P < 0.1$ between folds \\
highest\_gas\_angle  &   5 & Top 5 most twisted gas-phase geometries ($\theta > 89°$) \\
lowest\_gas\_angle   &   5 & Top 5 most planar gas-phase geometries ($\theta < 0.6°$) \\
largest\_difference  &   5 & Top 5 largest $|\Delta\theta|$ ($>78°$) \\
smallest\_difference &   5 & Top 5 smallest $|\Delta\theta|$ ($<0.3°$) \\
heaviest             &   5 & Five heaviest molecules (MW $>$ 1,992 g/mol) \\
lightest             &   5 & Five lightest molecules (MW $<$ 384 g/mol) \\
outliers\_gas        &   0 & Statistical outliers ($>3\sigma$) in gas-phase $\theta$ \\
outliers\_tol        &   0 & Statistical outliers ($>3\sigma$) in toluene $\theta$ \\
outliers\_diff       &   0 & Statistical outliers ($>3\sigma$) in $|\Delta\theta|$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{14_interesting_molecules_map.pdf}
\caption{Molecular categorization map overlaid on ($\theta_{gas}$, $S'_{HL}$) feature
space.
Each colored region/point represents one of the 12 categories from
\autoref{tab:category_counts}.
(Background) Light shading shows ML decision regions as in \autoref{fig:ml_decision}.
(Scatter points) Categories are color-coded: optimal\_tict (red circles), optimal\_non\_tict 
(blue circles), borderline (yellow circles), highest\_gas\_angle (green stars, top-left), 
lowest\_gas\_angle (purple stars, bottom-left), largest\_difference (orange diamonds), 
smallest\_difference (brown diamonds), heaviest (magenta triangles), lightest (cyan triangles), 
uncertain\_ml (gray X). Notable molecules are labeled with identifiers (e.g., SiCz1Py3, DDPA-Ph-Bz). 
The spatial clustering validates category logic: borderline molecules concentrate near the ML 
decision boundary; extreme-angle molecules occupy geometric edges; uncertain cases lie in 
low-density regions where training data is sparse. Molecular weight categories (heaviest/lightest) 
do not cluster spatially, confirming that TICT behavior is size-independent. This map serves as 
a practical tool for selecting validation targets: experimentalists seeking TICT references should 
target red stars in top-left; non-TICT controls should come from blue region bottom-right.}
\label{fig:interesting_molecules}
\end{figure}

\subsubsection{Category Highlights and Representative Molecules}

\textbf{1. Optimal TICT (N=284):}

Molecules predicted as TICT-active ($P(TICT) > 0.90$) with torsional angles in the TADF-optimal 
50-90° range. Representative examples:

\begin{itemize}
    \item \textbf{SiCz1Py3} ($\theta_{gas} = 89.6°$, $\theta_{tol} = 1.7°$): Exhibits largest 
    solvent-induced planarization ($|\Delta\theta| = 87.9°$), indicating extremely shallow 
    torsional potential. Silicon-bridged carbazole donor combined with pyridine acceptor creates 
    highly flexible linker susceptible to environmental perturbation.
    
    \item \textbf{BuCzCF3oB} ($\theta_{gas} = 89.7°$): One of the most twisted gas-phase conformers, 
    maintained even in toluene ($\theta_{tol} = 25.4°$). Trifluoromethyl substituents and 
    tert-butyl groups provide steric bulk enforcing perpendicularity.
    
    \item \textbf{Perylene} ($\theta_{gas} = 71.4°$, MW = 384 g/mol): Lightest TICT molecule, 
    demonstrating that small size does not preclude TICT behavior when appropriate D-A 
    architecture is present.
\end{itemize}

\textbf{2. Optimal Non-TICT (N=238):}

Molecules with $P(TICT) < 0.10$ yet maintaining TADF-favorable geometries ($50° < \theta < 90°$). 
These represent the ideal design space: sufficient HOMO-LUMO separation for small \deltaest~without 
TICT deactivation pathways. Example:

\begin{itemize}
    \item \textbf{2CzPN} ($\theta_{gas} = 55.2°$, $S'_{HL} = 0.38$): Canonical TADF emitter with 
    dicarbazole donors and phthalonitrile acceptor. Moderate twist balances orbital decoupling with 
    through-bond coupling necessary for efficient RISC.
\end{itemize}

\textbf{3. Borderline (N=78):}

Molecules with ambiguous TICT classification ($0.40 < P(TICT) < 0.60$). These systems exhibit 
environmental sensitivity and may show dual LE/TICT emission depending on conditions:

\begin{itemize}
    \item \textbf{DHPZ-2BN} ($\theta_{gas} = 41.0°$, $\theta_{tol} = 76.0°$, $P(TICT) = 0.52$): 
    Undergoes dramatic solvent-induced twisting ($\Delta\theta = +35.1°$), crossing from non-TICT 
    to TICT region. Such molecules are candidates for environment-responsive emitters.
\end{itemize}

\textbf{4. Extreme Geometries:}

\textit{Highest gas-phase angles:} DDPA-Ph-Bz ($89.9°$), BuCzCF3oB ($89.7°$), SiCz1Py3 ($89.6°$), 
DHID-DBS ($89.5°$), 2PXZP ($89.3°$). All five molecules maintain near-perpendicular D-A orientation 
in vacuum, representing the geometric limit for torsional TADF design.

\textit{Lowest gas-phase angles:} CH3OH-CHCl3 ($0.05°$), PCBP ($0.11°$), p-DTPACO ($0.27°$), 
FDQPXZ ($0.38°$), PTZ-DBTO2 ($0.50°$). These near-planar molecules achieve TADF through mechanisms 
other than torsional decoupling (likely MR-TADF or extended conjugation).

\textit{Largest conformational changes:} SiCz1Py3 ($|\Delta\theta| = 87.9°$), C3FLA-2 ($85.1°$), 
CPzPyC ($82.2°$), pDTCz-2DPyS ($78.3°$), BTaz-Ar-PXZ ($77.9°$). These molecules demonstrate 
extreme conformational flexibility, useful as test cases for understanding solvent-geometry coupling.

\textit{Smallest conformational changes:} LiPr ($|\Delta\theta| = 0.10°$), STAC-BP-STAC ($0.12°$), 
NDN ($0.13°$), 2CzPN ($0.17°$), BmPyPhB ($0.23°$). These rigid molecules are insensitive to 
environment, ideal for applications requiring stable emission wavelengths.

\textbf{5. Molecular Weight Extremes:}

\textit{Heaviest:} TPA-2SPPITPA (2,112 g/mol), c-D2T (2,052 g/mol), TPA-2PPITPA (2,016 g/mol), 
DVCz-2CzCN (2,004 g/mol), BPCP-2CPC (1,992 g/mol). Despite large size, all maintain TADF-relevant 
geometries, disproving assumptions that heavy molecules cannot be optimized.

\textit{Lightest:} PyI (348 g/mol), TPTI (360 g/mol), Perylene (384 g/mol), BBCz (384 g/mol), 
TPA-CN-N4 (384 g/mol). These compact molecules demonstrate that TADF is achievable with minimal 
structural complexity.

\subsubsection{Design Insights from Categorization}

The systematic categorization enables several actionable insights:

\begin{enumerate}
    \item \textbf{Validation target selection:} Experimentalists should prioritize the 238 
    optimal\_non\_tict molecules for synthesis, as they combine predicted TADF efficiency with 
    suppressed TICT deactivation.
    
    \item \textbf{Mechanistic probes:} The 78 borderline molecules are ideal for studying 
    LE-TICT equilibria and environment-dependent photophysics through systematic solvent/temperature 
    studies.
    
    \item \textbf{Rigidity benchmarks:} Smallest-difference molecules (e.g., 2CzPN with 
    $|\Delta\theta| = 0.17°$) serve as conformational stability standards for comparison.
    
    \item \textbf{Flexibility benchmarks:} Largest-difference molecules (e.g., SiCz1Py3 with 
    $|\Delta\theta| = 87.9°$) exemplify maximum environmental responsiveness, useful for 
    sensor applications.
    
    \item \textbf{Computational validation:} The 11 uncertain\_ml molecules with high model variance 
    indicate regions where semi-empirical methods may have accuracy limitations—these warrant 
    high-level DFT or CASPT2 benchmarking.
\end{enumerate}

\subsection{Summary of Torsional Angle and TICT Analysis}

This comprehensive conformational and machine learning analysis of 747 TADF emitters establishes 
several key findings:

\begin{enumerate}
    \item \textbf{Torsional distributions:} 83\% of molecules adopt 30-90° D-A twist, with trimodal 
    distribution reflecting architectural diversity. MR-TADF molecules constitute a distinct 
    near-planar population ($<30°$).
    
    \item \textbf{Solvent effects:} Toluene induces modest mean planarization ($\Delta\theta = -3.7°$), 
    but with large molecule-specific variance ($\pm 18.4°$). MR-TADF shows 4× lower solvent 
    sensitivity than D-A, quantifying rigidity advantage.
    
    \item \textbf{TICT prediction:} Logistic regression achieves 98.9\% cross-validated accuracy, 
    with torsional angle ($w = +2.84$) and HOMO-LUMO overlap ($w = -1.67$) as dominant features. 
    Decision boundary at $\theta \approx 65-70°$, $S'_{HL} \approx 0.25-0.30$ delineates 
    LE versus TICT regimes.
    
    \item \textbf{Molecular categorization:} 12-category taxonomy identifies 238 optimal non-TICT 
    candidates (highest synthesis priority), 78 borderline molecules (mechanistic interest), and 
    various extreme-geometry systems (computational benchmarks).
    
    \item \textbf{Structure-property correlations:} Strong $\theta$-$S'_{HL}$ anticorrelation 
    ($r = -0.64$) validates spatial separation mechanism, while weak $\theta$-\deltaest~correlation 
    ($r = -0.18$) confirms that additional factors (SOC, vibronic coupling) dominate TADF efficiency 
    beyond simple geometric twist.
\end{enumerate}

These results provide a comprehensive framework for rational TADF design incorporating conformational 
engineering, environmental robustness, and TICT suppression as key optimization targets alongside 
traditional electronic structure considerations.


==> manuscript_enhancements/table_gas_phase.tex <==
{
\squeezetable
\begin{longtable}[H]{>{\tiny}c<{}S[table-format=1.3]*{2}{S[table-format=3]}*{23}{c}}
\caption{Computational results for molecules in the gas phase. This table includes key electronic and photophysical properties calculated at the sTDA and sTD-DFT levels of theory.}
\label{tab:gas_phase_results} \\
\toprule 
\rotatebox{90}{Molecule Id} & {\rotatebox{90}{HOMO-LUMO gap}} & {\rotatebox{90}{HOMO
index}} & {\rotatebox{90}{LUMO index}} & {\rotatebox{90}{$\Delta E_r(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_v}(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_v}(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_v}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_v}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_r}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_r}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_{ST}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_{ST}}$}} &
{\rotatebox{90}{$\underset{sTDA}{S_{shift}(T_1)}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{S_{shift}(T_1)}$}} &
{\rotatebox{90}{$\underset{sTDA}{S_{shift}(S_1)}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{S_{shift}(S_1)}$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{abs}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{abs}}$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{PL}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{PL}}$}} &
{\rotatebox{90}{$\underset{sTDA}{f_{12}}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{f_{12}}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{shift}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{shift}}$}} &
{\rotatebox{90}{Overlap}} &
{\rotatebox{90}{Centroid}} \\
\midrule 
\endfirsthead 
\multicolumn{27}{c}{{\tablename} \thetable{} -- Continued from previous page} \\ 
\toprule 
\rotatebox{90}{Molecule Id} & {\rotatebox{90}{HOMO-LUMO gap}} & {\rotatebox{90}{HOMO
index}} &
{\rotatebox{90}{LUMO index}} & {\rotatebox{90}{$\Delta E_r(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_v}(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_v}(S_0\to T_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_v}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_v}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_r}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_r}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\Delta E_{ST}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\Delta E_{ST}}$}} &
{\rotatebox{90}{$\underset{sTDA}{S_{shift}(T_1)}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{S_{shift}(T_1)}$}} &
{\rotatebox{90}{$\underset{sTDA}{S_{shift}(S_1)}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{S_{shift}(S_1)}$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{abs}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{abs}}$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{PL}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{PL}}$}} &
{\rotatebox{90}{$\underset{sTDA}{f_{12}}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{f_{12}}(S_0\to S_1)$}} &
{\rotatebox{90}{$\underset{sTDA}{\lambda_{shift}}$}} &
{\rotatebox{90}{$\underset{sTD-DFT}{\lambda_{shift}}$}} &
{\rotatebox{90}{Overlap}} &
{\rotatebox{90}{Centroid}} \\
\midrule 
\endhead 
\midrule 
\multicolumn{27}{r}{{Continued on next page}} \\ 
\endfoot 
\bottomrule 
\endlastfoot 
4CzTPN & 1.658 & 143 & 144 & 1.936 & 2.672 & 2.659 & 2.962 & 2.917 & 2.146 & 2.123 & 0.210 & 0.187 & 0.736 & 0.724 & 0.816 & 0.794 & 418.583 & 425.055 & 577.777 & 583.921 & 0.422 & 0.361 & 159.194 & 158.867 & 0.388 & 0.016 \\ 
DMAC-DPS & 3.035 & 78 & 79 & 1.478 & 3.267 & 3.239 & 3.759 & 3.728 & 1.700 & 1.701 & 0.222 & 0.223 & 1.790 & 1.761 & 2.059 & 2.027 & 329.868 & 332.611 & 729.355 & 729.073 & 0.053 & 0.046 & 399.487 & 396.462 & 0.659 & 1.342 \\ 
PSPCz & 2.844 & 68 & 69 & 3.036 & 3.399 & 3.376 & 3.850 & 3.777 & 3.438 & 3.396 & 0.402 & 0.360 & 0.363 & 0.340 & 0.411 & 0.380 & 322.062 & 328.278 & 360.592 & 365.055 & 0.188 & 0.159 & 38.530 & 36.776 & 0.319 & 4.173 \\ 
Px2BP & 1.450 & 100 & 101 & 1.919 & 2.572 & 2.561 & 2.913 & 2.880 & 2.173 & 2.157 & 0.254 & 0.239 & 0.653 & 0.643 & 0.740 & 0.723 & 425.682 & 430.486 & 570.602 & 574.685 & 0.104 & 0.086 & 144.920 & 144.199 & 0.293 & 2.679 \\ 
CzS2 & 2.669 & 98 & 99 & 2.626 & 3.435 & 3.413 & 3.904 & 3.841 & 2.984 & 2.955 & 0.358 & 0.329 & 0.809 & 0.787 & 0.920 & 0.885 & 317.582 & 322.825 & 415.450 & 419.543 & 0.362 & 0.318 & 97.868 & 96.717 & 0.451 & 2.281 \\ 
2TCz-DPS & 2.312 & 146 & 147 & 2.543 & 3.389 & 3.368 & 3.854 & 3.805 & 2.892 & 2.873 & 0.349 & 0.330 & 0.846 & 0.825 & 0.962 & 0.932 & 321.728 & 325.863 & 428.688 & 431.507 & 0.040 & 0.033 & 106.961 & 105.645 & 0.456 & 3.699 \\ 
TDBA-DI & 2.073 & 163 & 164 & 2.514 & 3.095 & 3.076 & 3.573 & 3.503 & 2.902 & 2.862 & 0.388 & 0.349 & 0.582 & 0.563 & 0.672 & 0.641 & 346.993 & 353.907 & 427.307 & 433.146 & 0.151 & 0.217 & 80.314 & 79.239 & 0.134 & 7.505 \\ 
OPDPO & 1.478 & 102 & 103 & 1.139 & 2.487 & 2.447 & 2.804 & 2.797 & 1.284 & 1.302 & 0.145 & 0.163 & 1.348 & 1.308 & 1.520 & 1.495 & 442.216 & 443.339 & 965.487 & 952.411 & 0.019 & 0.017 & 523.271 & 509.072 & 0.138 & 4.145 \\ 
2CzTPEPCz & 2.290 & 152 & 153 & 1.789 & 3.292 & 3.254 & 3.861 & 3.831 & 2.099 & 2.107 & 0.310 & 0.317 & 1.502 & 1.465 & 1.762 & 1.724 & 321.086 & 323.651 & 590.654 & 588.553 & 1.519 & 1.331 & 269.568 & 264.903 & 0.533 & 5.079 \\ 
TBRb & 1.450 & 146 & 147 & 1.144 & 1.532 & 1.444 & 2.453 & 2.248 & 1.830 & 1.780 & 0.687 & 0.637 & 0.389 & 0.300 & 0.622 & 0.467 & 505.480 & 551.605 & 677.339 & 696.458 & 0.491 & 0.314 & 171.859 & 144.853 & 0.940 & 0.008 \\ 
TBPe & 1.932 & 94 & 95 & 1.573 & 2.215 & 2.149 & 3.218 & 3.059 & 2.285 & 2.239 & 0.712 & 0.666 & 0.642 & 0.576 & 0.933 & 0.820 & 385.247 & 405.310 & 542.553 & 553.722 & 0.878 & 0.618 & 157.305 & 148.412 & 0.944 & 0.000 \\ 
2CzPN & 1.989 & 83 & 84 & 2.369 & 3.123 & 3.103 & 3.443 & 3.414 & 2.611 & 2.606 & 0.243 & 0.237 & 0.754 & 0.734 & 0.831 & 0.808 & 360.116 & 363.164 & 474.777 & 475.761 & 0.205 & 0.182 & 114.662 & 112.597 & 0.460 & 4.229 \\ 
3CzFTFP & 1.800 & 101 & 102 & 2.718 & 3.410 & 3.388 & 3.863 & 3.791 & 3.078 & 3.042 & 0.360 & 0.323 & 0.692 & 0.670 & 0.784 & 0.749 & 320.986 & 327.066 & 402.755 & 407.640 & 0.164 & 0.136 & 81.769 & 80.574 & 0.098 & 6.765 \\ 
DDPhCz-DCPP & 1.324 & 166 & 167 & 1.453 & 3.159 & 3.140 & 3.568 & 3.535 & 1.642 & 1.636 & 0.188 & 0.183 & 1.706 & 1.686 & 1.926 & 1.899 & 347.509 & 350.733 & 755.284 & 757.683 & 0.524 & 0.512 & 407.776 & 406.950 & 0.358 & 6.890 \\ 
ACRXTN & 2.418 & 75 & 76 & 2.236 & 2.963 & 2.933 & 3.596 & 3.542 & 2.714 & 2.701 & 0.478 & 0.464 & 0.727 & 0.696 & 0.882 & 0.841 & 344.745 & 350.080 & 456.756 & 459.111 & 0.906 & 0.785 & 112.011 & 109.032 & 0.494 & 4.375 \\ 
TXO-TPA & 1.187 & 87 & 88 & 1.920 & 3.186 & 3.159 & 3.606 & 3.605 & 2.173 & 2.191 & 0.253 & 0.271 & 1.266 & 1.239 & 1.433 & 1.414 & 343.808 & 343.952 & 570.571 & 565.953 & 0.002 & 0.003 & 226.763 & 222.002 & 0.143 & 8.664 \\ 
PCTXO & 1.502 & 93 & 94 & 2.002 & 3.263 & 3.239 & 3.598 & 3.597 & 2.208 & 2.224 & 0.206 & 0.221 & 1.261 & 1.236 & 1.390 & 1.373 & 344.573 & 344.717 & 561.577 & 557.559 & 0.000 & 0.001 & 217.004 & 212.842 & 0.136 & 9.007 \\ 
IP-PPI & 2.465 & 103 & 104 & 2.225 & 3.261 & 3.229 & 3.837 & 3.798 & 2.618 & 2.617 & 0.393 & 0.392 & 1.036 & 1.005 & 1.219 & 1.182 & 323.145 & 326.412 & 473.631 & 473.813 & 0.913 & 0.867 & 150.486 & 147.401 & 0.538 & 8.861 \\ 
DMDHNP-DPS & 2.673 & 78 & 79 & 1.276 & 2.282 & 2.279 & 2.392 & 2.380 & 1.337 & 1.333 & 0.061 & 0.057 & 1.006 & 1.003 & 1.055 & 1.048 & 518.372 & 520.854 & 927.222 & 930.275 & 0.004 & 0.003 & 408.850 & 409.420 & 0.495 & 1.837 \\ 
4NTAZ-PPI & 2.242 & 131 & 132 & 2.219 & 3.369 & 3.319 & 3.865 & 3.827 & 2.546 & 2.559 & 0.327 & 0.339 & 1.150 & 1.100 & 1.319 & 1.268 & 320.754 & 323.989 & 486.919 & 484.575 & 0.652 & 0.581 & 166.166 & 160.586 & 0.191 & 10.023 \\ 
TAZ-PPI & 2.454 & 122 & 123 & 2.227 & 3.452 & 3.423 & 3.845 & 3.807 & 2.481 & 2.477 & 0.253 & 0.250 & 1.225 & 1.196 & 1.364 & 1.330 & 322.481 & 325.649 & 499.825 & 500.553 & 0.596 & 0.533 & 177.344 & 174.904 & 0.543 & 6.662 \\ 
PTZ-mPYR & 1.319 & 115 & 116 & 1.822 & 2.807 & 2.778 & 3.174 & 3.135 & 2.061 & 2.057 & 0.239 & 0.235 & 0.984 & 0.955 & 1.113 & 1.078 & 390.588 & 395.459 & 601.560 & 602.791 & 0.062 & 0.052 & 210.972 & 207.332 & 0.059 & 8.353 \\ 
pCNBCzoCF3 & 1.874 & 121 & 122 & 2.281 & 3.457 & 3.438 & 3.879 & 3.833 & 2.560 & 2.543 & 0.279 & 0.262 & 1.176 & 1.157 & 1.319 & 1.290 & 319.613 & 323.431 & 484.355 & 487.519 & 0.774 & 0.268 & 164.743 & 164.088 & 0.383 & 2.531 \\ 
PTZTPE-2 & 2.644 & 87 & 88 & 1.687 & 3.070 & 3.033 & 3.873 & 3.810 & 2.129 & 2.120 & 0.441 & 0.432 & 1.383 & 1.345 & 1.744 & 1.690 & 320.091 & 325.418 & 582.381 & 584.879 & 0.701 & 0.579 & 262.289 & 259.461 & 0.908 & 0.222 \\ 
4CzIPN & 1.950 & 143 & 144 & 2.196 & 3.086 & 3.077 & 3.298 & 3.268 & 2.346 & 2.332 & 0.151 & 0.137 & 0.891 & 0.881 & 0.952 & 0.936 & 375.915 & 379.331 & 528.414 & 531.592 & 0.151 & 0.136 & 152.500 & 152.261 & 0.325 & 0.046 \\ 
DMAC-TRZ & 1.529 & 96 & 97 & 1.953 & 3.389 & 3.369 & 3.474 & 3.467 & 2.001 & 2.010 & 0.048 & 0.057 & 1.436 & 1.416 & 1.472 & 1.457 & 356.943 & 357.571 & 619.487 & 616.823 & 0.126 & 0.122 & 262.543 & 259.252 & 0.191 & 6.716 \\ 
TCzTrz & 1.960 & 147 & 148 & 1.994 & 3.409 & 3.390 & 3.717 & 3.693 & 2.174 & 2.173 & 0.180 & 0.178 & 1.415 & 1.396 & 1.542 & 1.520 & 333.596 & 335.718 & 570.242 & 570.639 & 0.353 & 0.318 & 236.646 & 234.920 & 0.305 & 5.539 \\ 
$\delta$-2CbPN & 1.725 & 83 & 84 & 2.334 & 3.161 & 3.140 & 3.514 & 3.482 & 2.594 & 2.588 & 0.261 & 0.254 & 0.827 & 0.806 & 0.920 & 0.894 & 352.789 & 356.072 & 477.876 & 479.072 & 0.236 & 0.209 & 125.087 & 123.001 & 0.154 & 6.363 \\ 
CzDCbTrz & 1.819 & 147 & 148 & 1.955 & 3.363 & 3.341 & 3.666 & 3.642 & 2.131 & 2.131 & 0.176 & 0.176 & 1.409 & 1.386 & 1.535 & 1.511 & 338.209 & 340.448 & 581.937 & 581.921 & 0.360 & 0.320 & 243.728 & 241.474 & 0.165 & 4.937 \\ 
$\alpha$-2CbPN & 2.171 & 83 & 84 & 2.484 & 3.306 & 3.283 & 3.696 & 3.661 & 2.777 & 2.770 & 0.293 & 0.286 & 0.822 & 0.799 & 0.919 & 0.891 & 335.437 & 338.681 & 446.397 & 447.619 & 0.253 & 0.223 & 110.960 & 108.938 & 0.221 & 4.610 \\ 
CN-QP & 0.849 & 122 & 123 & 1.287 & 2.941 & 2.912 & 3.297 & 3.285 & 1.443 & 1.452 & 0.156 & 0.165 & 1.654 & 1.625 & 1.854 & 1.833 & 376.063 & 377.437 & 859.422 & 854.056 & 0.034 & 0.020 & 483.359 & 476.620 & 0.150 & 8.262 \\ 
TFM-QP & 0.818 & 130 & 131 & 1.282 & 2.953 & 2.924 & 3.331 & 3.297 & 1.446 & 1.446 & 0.164 & 0.164 & 1.671 & 1.641 & 1.884 & 1.851 & 372.258 & 376.017 & 857.200 & 857.236 & 0.009 & 0.012 & 484.942 & 481.219 & 0.162 & 7.964 \\ 
NDN & 2.756 & 91 & 92 & 2.730 & 3.445 & 3.427 & 3.837 & 3.771 & 3.040 & 3.005 & 0.310 & 0.275 & 0.715 & 0.697 & 0.796 & 0.767 & 323.153 & 328.757 & 407.796 & 412.640 & 0.048 & 0.038 & 84.643 & 83.883 & 0.611 & 1.228 \\ 
mCP & 3.103 & 75 & 76 & 3.035 & 3.415 & 3.391 & 3.906 & 3.841 & 3.472 & 3.438 & 0.436 & 0.403 & 0.379 & 0.355 & 0.434 & 0.402 & 317.452 & 322.825 & 357.113 & 360.604 & 0.337 & 0.285 & 39.660 & 37.779 & 0.674 & 0.266 \\ 
ZDZ & 2.482 & 91 & 92 & 2.674 & 3.388 & 3.372 & 3.770 & 3.708 & 2.976 & 2.941 & 0.302 & 0.266 & 0.714 & 0.697 & 0.794 & 0.767 & 328.862 & 334.415 & 416.612 & 421.608 & 0.085 & 0.070 & 87.750 & 87.194 & 0.434 & 2.241 \\ 
ZDN & 2.555 & 91 & 92 & 2.695 & 3.425 & 3.402 & 3.831 & 3.770 & 3.015 & 2.987 & 0.320 & 0.291 & 0.729 & 0.706 & 0.816 & 0.783 & 323.617 & 328.905 & 411.165 & 415.102 & 0.104 & 0.086 & 87.548 & 86.196 & 0.405 & 4.151 \\ 
BTCz3CzTPN & 1.585 & 159 & 160 & 1.916 & 2.739 & 2.727 & 3.018 & 2.978 & 2.111 & 2.092 & 0.195 & 0.176 & 0.824 & 0.812 & 0.908 & 0.886 & 410.789 & 416.264 & 587.414 & 592.637 & 0.460 & 0.401 & 176.626 & 176.373 & 0.142 & 6.541 \\ 
2BTCz2CzTPN & 1.517 & 175 & 176 & 1.850 & 2.947 & 2.935 & 3.208 & 3.176 & 2.014 & 2.002 & 0.164 & 0.152 & 1.097 & 1.085 & 1.194 & 1.174 & 386.460 & 390.329 & 615.530 & 619.330 & 0.505 & 0.454 & 229.070 & 229.000 & 0.177 & 1.976 \\ 
APDC-DTPA & 1.104 & 135 & 136 & 1.281 & 2.414 & 2.383 & 2.942 & 2.887 & 1.562 & 1.553 & 0.280 & 0.271 & 1.133 & 1.101 & 1.380 & 1.335 & 421.414 & 429.397 & 793.915 & 798.467 & 1.503 & 1.296 & 372.501 & 369.069 & 0.277 & 8.140 \\ 
BMIM & 1.103 & 135 & 136 & 1.281 & 2.415 & 2.383 & 2.943 & 2.888 & 1.562 & 1.553 & 0.280 & 0.271 & 1.133 & 1.102 & 1.381 & 1.335 & 421.342 & 429.338 & 793.964 & 798.543 & 1.502 & 1.295 & 372.621 & 369.205 & 0.276 & 8.144 \\ 
ADO-TPA & 1.203 & 78 & 79 & 1.317 & 2.099 & 2.098 & 2.098 & 2.097 & 1.316 & 1.316 & -0.001 & -0.001 & 0.782 & 0.782 & 0.782 & 0.781 & 591.048 & 591.217 & 942.166 & 942.211 & 0.000 & 0.000 & 351.118 & 350.994 & 0.158 & 9.369 \\ 
DCzTrz & 2.009 & 117 & 118 & 2.027 & 3.452 & 3.428 & 3.864 & 3.822 & 2.268 & 2.260 & 0.241 & 0.233 & 1.426 & 1.402 & 1.596 & 1.563 & 320.912 & 324.354 & 546.698 & 548.704 & 0.273 & 0.273 & 225.786 & 224.351 & 0.269 & 4.764 \\ 
BDPCC & 2.675 & 147 & 148 & 2.502 & 3.326 & 3.304 & 3.770 & 3.719 & 2.835 & 2.816 & 0.333 & 0.314 & 0.824 & 0.802 & 0.934 & 0.903 & 328.905 & 333.398 & 437.260 & 440.275 & 0.348 & 0.307 & 108.355 & 106.877 & 0.547 & 3.138 \\ 
SpiroAC-TRZ & 1.599 & 117 & 118 & 1.964 & 3.398 & 3.390 & 3.515 & 3.507 & 2.032 & 2.032 & 0.068 & 0.068 & 1.433 & 1.425 & 1.483 & 1.474 & 352.759 & 353.564 & 610.125 & 610.077 & 0.207 & 0.199 & 257.366 & 256.513 & 0.211 & 6.733 \\ 
DBT-BZ-DMAC & 2.128 & 90 & 91 & 1.633 & 2.996 & 2.959 & 3.572 & 3.539 & 1.947 & 1.953 & 0.314 & 0.320 & 1.363 & 1.326 & 1.625 & 1.586 & 347.081 & 350.337 & 636.681 & 634.802 & 0.022 & 0.021 & 289.600 & 284.466 & 0.216 & 3.909 \\ 
DQP & 1.078 & 69 & 70 & 1.008 & 3.202 & 3.138 & 3.262 & 3.261 & 1.027 & 1.048 & 0.019 & 0.040 & 2.194 & 2.130 & 2.235 & 2.214 & 380.086 & 380.156 & 1207.508 & 1183.591 & 0.000 & 0.000 & 827.422 & 803.434 & 0.575 & 0.001 \\ 
TPA-DCPP & 1.217 & 140 & 141 & 1.446 & 3.249 & 3.225 & 3.641 & 3.626 & 1.621 & 1.626 & 0.175 & 0.180 & 1.803 & 1.779 & 2.020 & 2.000 & 340.532 & 341.950 & 765.032 & 762.684 & 0.901 & 0.852 & 424.500 & 420.735 & 0.257 & 8.620 \\ 
2PXZ-OXD & 1.541 & 107 & 108 & 1.987 & 2.812 & 2.802 & 3.099 & 3.088 & 2.190 & 2.189 & 0.203 & 0.202 & 0.825 & 0.815 & 0.909 & 0.898 & 400.026 & 401.542 & 566.150 & 566.314 & 0.867 & 0.812 & 166.123 & 164.772 & 0.339 & 1.552 \\ 
BmPyPhB & 1.452 & 174 & 175 & 1.809 & 3.337 & 3.330 & 3.428 & 3.422 & 1.858 & 1.859 & 0.049 & 0.050 & 1.528 & 1.521 & 1.570 & 1.563 & 361.734 & 362.273 & 667.347 & 666.819 & 0.253 & 0.246 & 305.613 & 304.547 & 0.206 & 3.488 \\ 
MPPA & 0.874 & 152 & 153 & 1.343 & 2.449 & 2.434 & 2.806 & 2.777 & 1.539 & 1.532 & 0.196 & 0.189 & 1.106 & 1.091 & 1.267 & 1.245 & 441.791 & 446.500 & 805.588 & 809.255 & 0.019 & 0.016 & 363.797 & 362.754 & 0.285 & 1.094 \\ 
ACRFLCN & 1.653 & 83 & 84 & 2.277 & 3.479 & 3.472 & 3.480 & 3.479 & 2.278 & 2.282 & 0.000 & 0.005 & 1.202 & 1.195 & 1.202 & 1.197 & 356.307 & 356.358 & 544.372 & 543.308 & 0.000 & 0.000 & 188.065 & 186.950 & 0.136 & 3.748 \\ 
PTZ-DCPP & 1.631 & 116 & 117 & 1.360 & 2.579 & 2.552 & 3.106 & 3.052 & 1.637 & 1.626 & 0.278 & 0.267 & 1.219 & 1.192 & 1.468 & 1.426 & 399.241 & 406.213 & 757.168 & 762.325 & 0.383 & 0.357 & 357.927 & 356.112 & 0.527 & 5.058 \\ 
BBA-Pyr & 1.984 & 130 & 131 & 1.998 & 3.331 & 3.309 & 3.787 & 3.764 & 2.271 & 2.273 & 0.273 & 0.275 & 1.333 & 1.311 & 1.516 & 1.491 & 327.377 & 329.430 & 545.865 & 545.578 & 1.789 & 1.630 & 218.488 & 216.148 & 0.275 & 9.868 \\ 
PhICz-Pyr & 2.126 & 128 & 129 & 2.075 & 3.308 & 3.289 & 3.704 & 3.649 & 2.324 & 2.302 & 0.248 & 0.227 & 1.233 & 1.214 & 1.380 & 1.347 & 334.749 & 339.813 & 533.560 & 538.587 & 0.528 & 0.456 & 198.811 & 198.774 & 0.454 & 2.214 \\ 
PhCz-Pyr & 2.119 & 129 & 130 & 2.031 & 3.409 & 3.387 & 3.825 & 3.768 & 2.279 & 2.259 & 0.248 & 0.229 & 1.378 & 1.356 & 1.546 & 1.509 & 324.125 & 329.054 & 544.090 & 548.831 & 0.368 & 0.300 & 219.965 & 219.778 & 0.480 & 1.544 \\ 
PDA-DP & 1.926 & 172 & 173 & 2.227 & 3.296 & 3.268 & 3.840 & 3.810 & 2.594 & 2.596 & 0.367 & 0.369 & 1.069 & 1.041 & 1.245 & 1.213 & 322.901 & 325.435 & 477.878 & 477.509 & 1.902 & 1.704 & 154.977 & 152.074 & 0.142 & 5.404 \\ 
9CzFDBFDPO & 2.338 & 187 & 188 & 2.849 & 3.411 & 3.388 & 3.861 & 3.789 & 3.225 & 3.187 & 0.376 & 0.337 & 0.562 & 0.539 & 0.636 & 0.603 & 321.153 & 327.178 & 384.484 & 389.091 & 0.212 & 0.177 & 63.331 & 61.912 & 0.012 & 12.702 \\ 
9PhCzFDBFDPO & 2.300 & 201 & 202 & 2.690 & 3.440 & 3.417 & 3.893 & 3.827 & 3.044 & 3.012 & 0.354 & 0.323 & 0.750 & 0.727 & 0.849 & 0.815 & 318.480 & 323.981 & 407.326 & 411.603 & 0.207 & 0.170 & 88.846 & 87.622 & 0.007 & 17.002 \\ 
9PhCzFDBFSPO & 2.564 & 167 & 168 & 2.696 & 3.443 & 3.420 & 3.893 & 3.828 & 3.048 & 3.016 & 0.352 & 0.321 & 0.748 & 0.725 & 0.845 & 0.811 & 318.488 & 323.922 & 406.823 & 411.023 & 0.218 & 0.180 & 88.335 & 87.102 & 0.006 & 16.871 \\ 
9CzFDBFSPO & 2.570 & 153 & 154 & 2.904 & 3.444 & 3.421 & 3.914 & 3.847 & 3.300 & 3.265 & 0.396 & 0.361 & 0.540 & 0.517 & 0.614 & 0.582 & 316.771 & 322.296 & 375.738 & 379.739 & 0.201 & 0.170 & 58.967 & 57.443 & 0.023 & 14.172 \\ 
9ArFDBFxPO & 2.373 & 187 & 188 & 2.833 & 3.429 & 3.406 & 3.870 & 3.802 & 3.197 & 3.163 & 0.364 & 0.330 & 0.596 & 0.573 & 0.672 & 0.640 & 320.406 & 326.085 & 387.763 & 392.024 & 0.200 & 0.169 & 67.357 & 65.938 & 0.013 & 12.832 \\ 
12BTCzTPN & 1.650 & 175 & 176 & 1.904 & 2.722 & 2.709 & 3.001 & 2.961 & 2.099 & 2.080 & 0.196 & 0.177 & 0.818 & 0.806 & 0.902 & 0.880 & 413.088 & 418.795 & 590.654 & 596.020 & 0.360 & 0.311 & 177.566 & 177.225 & 0.358 & 0.536 \\ 
oDTBPZ-DPXZ & 1.105 & 151 & 152 & 1.130 & 2.736 & 2.724 & 2.985 & 2.966 & 1.233 & 1.230 & 0.103 & 0.100 & 1.606 & 1.594 & 1.753 & 1.736 & 415.302 & 418.004 & 1005.642 & 1007.893 & 0.645 & 0.595 & 590.340 & 589.889 & 0.321 & 6.444 \\ 
3DMAC-BP-CN & 1.098 & 172 & 173 & 1.024 & 2.460 & 2.431 & 2.905 & 2.897 & 1.209 & 1.220 & 0.185 & 0.196 & 1.436 & 1.408 & 1.696 & 1.677 & 426.796 & 427.945 & 1025.660 & 1016.422 & 0.019 & 0.004 & 598.864 & 588.478 & 0.239 & 5.617 \\ 
3DMAC-BP-Br & 0.894 & 171 & 172 & 1.030 & 2.768 & 2.762 & 2.822 & 2.818 & 1.051 & 1.051 & 0.020 & 0.021 & 1.738 & 1.731 & 1.772 & 1.767 & 439.302 & 439.972 & 1180.140 & 1179.336 & 0.082 & 0.080 & 740.838 & 739.363 & 0.228 & 4.379 \\ 
TPA-PZCN & 1.082 & 149 & 150 & 1.108 & 3.027 & 2.995 & 3.269 & 3.267 & 1.197 & 1.209 & 0.089 & 0.101 & 1.919 & 1.887 & 2.072 & 2.058 & 379.307 & 379.470 & 1036.156 & 1025.675 & 0.007 & 0.008 & 656.848 & 646.205 & 0.258 & 8.686 \\ 
1PXZ-BP & 1.080 & 84 & 85 & 1.143 & 2.742 & 2.712 & 3.062 & 3.046 & 1.276 & 1.284 & 0.133 & 0.141 & 1.599 & 1.569 & 1.785 & 1.762 & 404.965 & 406.999 & 971.559 & 965.508 & 0.322 & 0.291 & 566.594 & 558.508 & 0.232 & 7.639 \\ 
PTZ-DBTO2 & 2.374 & 70 & 71 & 2.259 & 3.024 & 3.004 & 3.505 & 3.438 & 2.619 & 2.585 & 0.360 & 0.326 & 0.765 & 0.745 & 0.887 & 0.853 & 353.705 & 360.650 & 473.443 & 479.610 & 0.049 & 0.038 & 119.738 & 118.960 & 0.395 & 4.883 \\ 
BACQ & 2.301 & 67 & 68 & 2.223 & 2.499 & 2.465 & 3.215 & 3.102 & 2.859 & 2.797 & 0.636 & 0.574 & 0.276 & 0.242 & 0.355 & 0.305 & 385.691 & 399.704 & 433.627 & 443.232 & 0.531 & 0.395 & 47.936 & 43.528 & 0.709 & 1.063 \\ 
2Cz-DMAC-TXO & 1.214 & 135 & 136 & 1.978 & 2.864 & 2.838 & 3.397 & 3.370 & 2.345 & 2.348 & 0.368 & 0.371 & 0.886 & 0.861 & 1.051 & 1.022 & 365.035 & 367.873 & 528.620 & 528.004 & 0.021 & 0.055 & 163.585 & 160.131 & 0.110 & 6.575 \\ 
2Cz-DMAC-TTR & 2.140 & 145 & 146 & 2.347 & 3.482 & 3.459 & 3.917 & 3.864 & 2.641 & 2.622 & 0.293 & 0.274 & 1.135 & 1.112 & 1.277 & 1.242 & 316.504 & 320.887 & 469.540 & 472.938 & 0.431 & 0.366 & 153.036 & 152.052 & 0.156 & 9.090 \\ 
2Cz-DMAC-BTB & 1.533 & 136 & 137 & 2.348 & 3.362 & 3.333 & 3.743 & 3.733 & 2.615 & 2.630 & 0.266 & 0.282 & 1.014 & 0.985 & 1.129 & 1.103 & 331.225 & 332.095 & 474.197 & 471.340 & 0.080 & 0.098 & 142.972 & 139.246 & 0.143 & 6.285 \\ 
DMAC-BPP & 1.664 & 149 & 150 & 1.840 & 3.530 & 3.502 & 3.712 & 3.705 & 1.934 & 1.947 & 0.094 & 0.107 & 1.691 & 1.662 & 1.778 & 1.759 & 334.045 & 334.622 & 641.048 & 636.899 & 0.016 & 0.016 & 307.003 & 302.276 & 0.114 & 5.892 \\ 
Me-MOC & 1.757 & 79 & 80 & 2.321 & 3.135 & 3.110 & 3.648 & 3.563 & 2.701 & 2.660 & 0.380 & 0.339 & 0.814 & 0.789 & 0.947 & 0.904 & 339.841 & 347.948 & 458.978 & 466.164 & 0.415 & 0.308 & 119.137 & 118.216 & 0.111 & 8.219 \\ 
Me-DOC & 1.672 & 85 & 86 & 2.257 & 2.959 & 2.932 & 3.522 & 3.423 & 2.686 & 2.635 & 0.429 & 0.379 & 0.702 & 0.675 & 0.835 & 0.788 & 352.068 & 362.167 & 461.570 & 470.477 & 0.525 & 0.368 & 109.502 & 108.310 & 0.082 & 8.325 \\ 
3DCPO & 3.131 & 109 & 110 & 3.052 & 3.406 & 3.384 & 3.866 & 3.792 & 3.463 & 3.420 & 0.412 & 0.368 & 0.354 & 0.332 & 0.402 & 0.372 & 320.737 & 326.963 & 357.982 & 362.530 & 0.047 & 0.039 & 37.245 & 35.568 & 0.382 & 6.396 \\ 
TDBA-TPDICz & 1.980 & 161 & 162 & 2.313 & 2.697 & 2.670 & 3.198 & 3.103 & 2.743 & 2.688 & 0.430 & 0.375 & 0.384 & 0.357 & 0.455 & 0.415 & 387.644 & 399.575 & 451.920 & 461.182 & 0.391 & 0.309 & 64.276 & 61.607 & 0.205 & 7.393 \\ 
TRZ-pIC & 1.986 & 161 & 162 & 2.312 & 2.697 & 2.670 & 3.198 & 3.103 & 2.742 & 2.687 & 0.430 & 0.375 & 0.385 & 0.358 & 0.456 & 0.416 & 387.681 & 399.601 & 452.157 & 461.429 & 0.391 & 0.309 & 64.477 & 61.828 & 0.208 & 7.391 \\ 
SBF-PXZ & 1.977 & 124 & 125 & 2.257 & 2.864 & 2.833 & 3.250 & 3.216 & 2.561 & 2.562 & 0.305 & 0.305 & 0.607 & 0.576 & 0.689 & 0.654 & 381.502 & 385.535 & 484.051 & 484.010 & 0.038 & 0.023 & 102.550 & 98.475 & 0.390 & 0.798 \\ 
PtOEP & 0.823 & 110 & 111 & 0.550 & 0.163 & 1.329 & 0.944 & 0.601 & 3.188 & 0.249 & 2.638 & -0.301 & -0.387 & 0.779 & -2.243 & 0.353 & 1312.836 & 2062.279 & 388.940 & 4987.205 & 0.000 & 0.000 & -923.896 & 2924.927 & 0.735 & 0.002 \\ 
PxCYP & 1.250 & 113 & 114 & 1.911 & 2.751 & 2.720 & 3.085 & 3.067 & 2.144 & 2.155 & 0.232 & 0.244 & 0.839 & 0.809 & 0.942 & 0.912 & 401.842 & 404.266 & 578.319 & 575.293 & 0.441 & 0.304 & 176.477 & 171.027 & 0.160 & 7.816 \\ 
AcCYP & 1.314 & 125 & 126 & 2.003 & 3.406 & 3.380 & 3.529 & 3.524 & 2.076 & 2.088 & 0.072 & 0.085 & 1.403 & 1.377 & 1.454 & 1.436 & 351.320 & 351.868 & 597.353 & 593.771 & 0.205 & 0.196 & 246.034 & 241.903 & 0.112 & 7.747 \\ 
BCN & 2.070 & 75 & 76 & 2.194 & 2.602 & 2.572 & 3.097 & 3.038 & 2.611 & 2.590 & 0.417 & 0.397 & 0.409 & 0.379 & 0.486 & 0.447 & 400.336 & 408.178 & 474.942 & 478.663 & 0.291 & 0.243 & 74.606 & 70.485 & 0.554 & 4.111 \\ 
DPPSPF & 2.954 & 96 & 97 & 2.545 & 3.661 & 3.624 & 4.401 & 4.344 & 3.059 & 3.051 & 0.514 & 0.506 & 1.116 & 1.079 & 1.342 & 1.293 & 281.718 & 285.415 & 405.254 & 406.377 & 1.307 & 1.149 & 123.536 & 120.962 & 0.744 & 3.419 \\ 
Me2ACBO & 1.816 & 184 & 185 & 2.175 & 2.981 & 2.959 & 3.412 & 3.375 & 2.489 & 2.480 & 0.314 & 0.305 & 0.806 & 0.784 & 0.923 & 0.895 & 363.398 & 367.371 & 498.120 & 499.884 & 0.468 & 0.426 & 134.722 & 132.513 & 0.215 & 6.353 \\ 
F2AcBO & 1.724 & 205 & 206 & 2.239 & 3.130 & 3.111 & 3.528 & 3.516 & 2.524 & 2.531 & 0.285 & 0.292 & 0.891 & 0.872 & 1.004 & 0.985 & 351.459 & 352.588 & 491.256 & 489.874 & 0.255 & 0.314 & 139.797 & 137.286 & 0.123 & 10.079 \\ 
PSPSF & 2.905 & 95 & 96 & 2.545 & 3.699 & 3.662 & 4.436 & 4.381 & 3.052 & 3.045 & 0.507 & 0.500 & 1.154 & 1.117 & 1.384 & 1.336 & 279.508 & 282.985 & 406.258 & 407.197 & 1.218 & 1.084 & 126.750 & 124.212 & 0.546 & 4.151 \\ 
TXO-P-Si & 1.942 & 101 & 102 & 2.081 & 3.543 & 3.542 & 3.534 & 3.532 & 2.076 & 2.075 & -0.005 & -0.006 & 1.462 & 1.460 & 1.458 & 1.457 & 350.852 & 351.031 & 597.303 & 597.371 & 0.000 & 0.000 & 246.450 & 246.340 & 0.079 & 9.955 \\ 
CzB-FMPIM & 2.152 & 125 & 126 & 2.212 & 3.471 & 3.447 & 3.955 & 3.894 & 2.520 & 2.498 & 0.308 & 0.287 & 1.259 & 1.236 & 1.435 & 1.396 & 313.511 & 318.406 & 492.008 & 496.278 & 0.374 & 0.230 & 178.497 & 177.872 & 0.200 & 10.236 \\ 
CzB-FMPPI & 2.134 & 124 & 125 & 2.196 & 3.436 & 3.408 & 3.857 & 3.815 & 2.465 & 2.458 & 0.269 & 0.262 & 1.240 & 1.212 & 1.392 & 1.356 & 321.444 & 325.025 & 502.922 & 504.367 & 0.660 & 0.592 & 181.478 & 179.341 & 0.173 & 10.419 \\ 
BACF & 2.314 & 66 & 67 & 2.290 & 2.567 & 2.532 & 3.144 & 3.054 & 2.805 & 2.763 & 0.515 & 0.473 & 0.277 & 0.242 & 0.339 & 0.291 & 394.339 & 405.907 & 442.013 & 448.722 & 0.100 & 0.077 & 47.674 & 42.815 & 0.632 & 2.892 \\ 
BACH & 2.439 & 63 & 64 & 2.349 & 2.643 & 2.608 & 3.218 & 3.133 & 2.859 & 2.821 & 0.511 & 0.473 & 0.295 & 0.259 & 0.359 & 0.311 & 385.307 & 395.787 & 433.630 & 439.475 & 0.109 & 0.087 & 48.323 & 43.688 & 0.661 & 2.712 \\ 
PzTDBA & 2.516 & 178 & 179 & 2.064 & 3.209 & 3.192 & 3.653 & 3.601 & 2.349 & 2.328 & 0.285 & 0.265 & 1.145 & 1.128 & 1.304 & 1.273 & 339.422 & 344.276 & 527.837 & 532.515 & 0.045 & 0.056 & 188.414 & 188.239 & 0.349 & 4.943 \\ 
3TCPM & 1.588 & 109 & 110 & 2.235 & 3.340 & 3.315 & 3.732 & 3.703 & 2.497 & 2.496 & 0.262 & 0.261 & 1.105 & 1.080 & 1.235 & 1.207 & 332.219 & 334.812 & 496.537 & 496.667 & 1.529 & 1.326 & 164.318 & 161.855 & 0.116 & 12.811 \\ 
TPA-PPO & 2.035 & 100 & 101 & 2.067 & 2.927 & 2.888 & 3.562 & 3.530 & 2.515 & 2.526 & 0.448 & 0.459 & 0.860 & 0.822 & 1.047 & 1.004 & 348.084 & 351.280 & 492.971 & 490.919 & 2.144 & 1.920 & 144.887 & 139.639 & 0.424 & 7.417 \\ 
CzPh-PPO & 2.164 & 99 & 100 & 2.116 & 2.952 & 2.914 & 3.773 & 3.712 & 2.705 & 2.696 & 0.589 & 0.580 & 0.836 & 0.798 & 1.068 & 1.016 & 328.609 & 333.964 & 458.348 & 459.821 & 1.922 & 1.603 & 129.739 & 125.857 & 0.368 & 7.986 \\ 
m-CF3PIBI & 2.434 & 143 & 144 & 2.241 & 3.487 & 3.458 & 3.920 & 3.884 & 2.519 & 2.517 & 0.278 & 0.276 & 1.247 & 1.217 & 1.401 & 1.367 & 316.270 & 319.218 & 492.240 & 492.596 & 0.391 & 0.350 & 175.970 & 173.379 & 0.451 & 3.002 \\ 
DPTPEA & 2.249 & 93 & 94 & 1.654 & 2.954 & 2.920 & 3.525 & 3.492 & 1.974 & 1.978 & 0.320 & 0.324 & 1.300 & 1.266 & 1.551 & 1.513 & 351.718 & 355.072 & 628.043 & 626.714 & 0.839 & 0.739 & 276.325 & 271.641 & 0.572 & 4.659 \\ 
PICNAnCz & 2.194 & 75 & 76 & 2.303 & 3.428 & 3.398 & 3.855 & 3.812 & 2.590 & 2.584 & 0.287 & 0.281 & 1.125 & 1.094 & 1.265 & 1.228 & 321.586 & 325.256 & 478.660 & 479.787 & 0.234 & 0.221 & 157.074 & 154.531 & 0.311 & 5.122 \\ 
DPA-DPQ & 1.735 & 83 & 84 & 1.569 & 2.568 & 2.538 & 3.128 & 3.052 & 1.911 & 1.886 & 0.342 & 0.318 & 0.999 & 0.969 & 1.217 & 1.166 & 396.331 & 406.226 & 648.712 & 657.243 & 0.436 & 0.366 & 252.381 & 251.017 & 0.579 & 0.765 \\ 
PhQLPXZ & 1.545 & 85 & 86 & 1.923 & 2.718 & 2.694 & 2.912 & 2.896 & 2.060 & 2.066 & 0.137 & 0.144 & 0.796 & 0.771 & 0.852 & 0.829 & 425.770 & 428.196 & 602.002 & 600.020 & 0.192 & 0.174 & 176.232 & 171.824 & 0.288 & 5.444 \\ 
2DPA-DPQ & 1.870 & 114 & 115 & 1.683 & 2.431 & 2.401 & 3.061 & 2.975 & 2.119 & 2.085 & 0.437 & 0.402 & 0.748 & 0.718 & 0.942 & 0.890 & 404.992 & 416.754 & 585.021 & 594.607 & 0.816 & 0.667 & 180.030 & 177.853 & 0.582 & 0.642 \\ 
FDQPXZ & 1.163 & 88 & 89 & 1.325 & 2.270 & 2.259 & 2.488 & 2.466 & 1.453 & 1.447 & 0.128 & 0.122 & 0.944 & 0.934 & 1.035 & 1.019 & 498.289 & 502.713 & 853.370 & 856.851 & 0.232 & 0.208 & 355.081 & 354.138 & 0.340 & 5.346 \\ 
DTRZSFX & 1.981 & 145 & 146 & 1.916 & 3.343 & 3.306 & 3.965 & 3.918 & 2.273 & 2.272 & 0.356 & 0.355 & 1.427 & 1.389 & 1.692 & 1.647 & 312.736 & 316.415 & 545.550 & 545.810 & 2.021 & 1.789 & 232.814 & 229.395 & 0.444 & 2.063 \\ 
E-o-DHMPA & 2.134 & 73 & 74 & 1.749 & 2.220 & 2.148 & 3.224 & 3.038 & 2.540 & 2.474 & 0.791 & 0.725 & 0.472 & 0.399 & 0.685 & 0.565 & 384.507 & 408.058 & 488.222 & 501.230 & 0.386 & 0.266 & 103.715 & 93.173 & 0.931 & 0.093 \\ 
Z-o-DHMPA & 2.133 & 73 & 74 & 1.749 & 2.219 & 2.147 & 3.223 & 3.037 & 2.540 & 2.474 & 0.791 & 0.725 & 0.471 & 0.398 & 0.683 & 0.563 & 384.662 & 408.273 & 488.173 & 501.234 & 0.385 & 0.265 & 103.511 & 92.961 & 0.931 & 0.096 \\ 
p-DHMPA & 2.130 & 73 & 74 & 1.734 & 2.244 & 2.172 & 3.254 & 3.076 & 2.514 & 2.455 & 0.780 & 0.722 & 0.510 & 0.439 & 0.740 & 0.621 & 381.021 & 403.017 & 493.212 & 504.971 & 0.453 & 0.320 & 112.191 & 101.954 & 0.936 & 0.001 \\ 
STAC-BP-STAC & 1.572 & 160 & 161 & 2.043 & 3.274 & 3.267 & 3.412 & 3.406 & 2.128 & 2.130 & 0.086 & 0.087 & 1.232 & 1.224 & 1.283 & 1.276 & 363.409 & 363.985 & 582.513 & 582.064 & 0.320 & 0.311 & 219.104 & 218.079 & 0.225 & 2.933 \\ 
SXAC-BP-SXAC & 1.552 & 160 & 161 & 2.033 & 3.284 & 3.275 & 3.418 & 3.412 & 2.116 & 2.118 & 0.083 & 0.085 & 1.250 & 1.242 & 1.302 & 1.294 & 362.707 & 363.334 & 585.803 & 585.351 & 0.332 & 0.322 & 223.096 & 222.016 & 0.214 & 5.607 \\ 
m-DHMPA & 2.138 & 73 & 74 & 1.738 & 2.248 & 2.177 & 3.258 & 3.076 & 2.519 & 2.456 & 0.781 & 0.718 & 0.510 & 0.439 & 0.739 & 0.620 & 380.576 & 403.030 & 492.138 & 504.760 & 0.435 & 0.306 & 111.561 & 101.730 & 0.936 & 0.000 \\ 
SFAC-BP-SFAC & 1.514 & 154 & 155 & 2.014 & 3.290 & 3.282 & 3.416 & 3.410 & 2.091 & 2.092 & 0.077 & 0.079 & 1.276 & 1.268 & 1.325 & 1.318 & 362.920 & 363.558 & 592.921 & 592.574 & 0.313 & 0.303 & 230.002 & 229.016 & 0.215 & 5.398 \\ 
PBTPA & 1.074 & 106 & 107 & 1.415 & 2.554 & 2.511 & 3.038 & 3.004 & 1.684 & 1.694 & 0.269 & 0.278 & 1.138 & 1.096 & 1.354 & 1.311 & 408.044 & 412.689 & 736.232 & 732.105 & 1.383 & 1.236 & 328.187 & 319.416 & 0.317 & 6.161 \\ 
HDP & 0.887 & 59 & 60 & 1.018 & 2.678 & 2.642 & 2.775 & 2.775 & 1.055 & 1.069 & 0.037 & 0.051 & 1.660 & 1.624 & 1.721 & 1.706 & 446.726 & 446.774 & 1175.529 & 1159.849 & 0.000 & 0.000 & 728.804 & 713.075 & 0.382 & 2.096 \\ 
PY-TPA & 0.865 & 142 & 143 & 1.067 & 2.934 & 2.905 & 3.253 & 3.248 & 1.183 & 1.193 & 0.116 & 0.126 & 1.867 & 1.838 & 2.070 & 2.055 & 381.115 & 381.725 & 1047.897 & 1039.272 & 0.058 & 0.185 & 666.782 & 657.547 & 0.248 & 9.216 \\ 
CN-TPA & 2.891 & 95 & 96 & 2.854 & 3.224 & 3.200 & 3.791 & 3.745 & 3.356 & 3.340 & 0.502 & 0.486 & 0.370 & 0.346 & 0.435 & 0.405 & 327.066 & 331.092 & 369.480 & 371.198 & 0.592 & 0.516 & 42.414 & 40.105 & 0.634 & 2.487 \\ 
DMIC-TRZ & 0.958 & 110 & 111 & 0.727 & 0.942 & 0.765 & 1.615 & 1.484 & 1.246 & 1.410 & 0.519 & 0.683 & 0.215 & 0.038 & 0.368 & 0.073 & 767.942 & 835.755 & 994.815 & 879.188 & 0.231 & 0.146 & 226.873 & 43.434 & 0.778 & 0.919 \\ 
NyDPAc & 1.604 & 130 & 131 & 1.540 & 3.356 & 3.323 & 3.717 & 3.715 & 1.706 & 1.722 & 0.166 & 0.182 & 1.816 & 1.783 & 2.011 & 1.993 & 333.542 & 333.721 & 726.776 & 719.931 & 0.035 & 0.057 & 393.234 & 386.209 & 0.031 & 10.504 \\ 
oCBP & 2.723 & 89 & 90 & 2.796 & 3.378 & 3.356 & 3.858 & 3.790 & 3.193 & 3.158 & 0.398 & 0.362 & 0.582 & 0.560 & 0.665 & 0.633 & 321.344 & 327.101 & 388.280 & 392.638 & 0.135 & 0.113 & 66.936 & 65.538 & 0.380 & 2.909 \\ 
PABP & 2.127 & 127 & 128 & 1.738 & 2.251 & 2.182 & 3.313 & 3.154 & 2.559 & 2.512 & 0.820 & 0.774 & 0.513 & 0.444 & 0.755 & 0.641 & 374.213 & 393.164 & 484.588 & 493.520 & 1.049 & 0.724 & 110.375 & 100.356 & 0.925 & 1.740 \\ 
DHID-DPS & 2.122 & 124 & 125 & 2.314 & 2.855 & 2.822 & 3.530 & 3.457 & 2.862 & 2.835 & 0.548 & 0.521 & 0.541 & 0.508 & 0.669 & 0.623 & 351.180 & 358.605 & 433.275 & 437.383 & 0.192 & 0.161 & 82.094 & 78.778 & 0.461 & 3.771 \\ 
4FBTPI & 1.939 & 185 & 186 & 2.086 & 3.474 & 3.448 & 3.877 & 3.842 & 2.327 & 2.324 & 0.242 & 0.239 & 1.389 & 1.362 & 1.550 & 1.518 & 319.786 & 322.665 & 532.716 & 533.398 & 1.077 & 0.965 & 212.930 & 210.732 & 0.396 & 0.126 \\ 
BCzBMes & 2.737 & 123 & 124 & 2.664 & 3.380 & 3.357 & 3.819 & 3.751 & 3.010 & 2.976 & 0.346 & 0.312 & 0.716 & 0.693 & 0.809 & 0.774 & 324.651 & 330.580 & 411.855 & 416.610 & 0.193 & 0.158 & 87.204 & 86.030 & 0.493 & 6.369 \\ 
CCDMB & 2.113 & 123 & 124 & 2.478 & 3.313 & 3.292 & 3.747 & 3.688 & 2.802 & 2.776 & 0.325 & 0.299 & 0.835 & 0.814 & 0.945 & 0.912 & 330.889 & 336.155 & 442.421 & 446.573 & 0.551 & 0.403 & 111.532 & 110.417 & 0.210 & 8.976 \\ 
PCDMB & 1.554 & 126 & 127 & 2.387 & 2.681 & 2.650 & 3.043 & 3.005 & 2.709 & 2.707 & 0.323 & 0.321 & 0.294 & 0.263 & 0.334 & 0.298 & 407.374 & 412.552 & 457.615 & 457.952 & 0.015 & 0.013 & 50.241 & 45.400 & 0.076 & 10.342 \\ 
BTrztCz & 1.512 & 207 & 208 & 1.657 & 3.369 & 3.358 & 3.543 & 3.529 & 1.742 & 1.741 & 0.086 & 0.085 & 1.712 & 1.702 & 1.801 & 1.788 & 349.951 & 351.290 & 711.721 & 712.131 & 0.073 & 0.068 & 361.769 & 360.842 & 0.113 & 4.543 \\ 
DHID-DBS & 1.862 & 135 & 136 & 2.242 & 2.853 & 2.820 & 3.419 & 3.340 & 2.687 & 2.655 & 0.445 & 0.413 & 0.611 & 0.579 & 0.732 & 0.685 & 362.612 & 371.221 & 461.471 & 467.013 & 0.374 & 0.305 & 98.859 & 95.792 & 0.262 & 5.947 \\ 
CZ-DPS-DMAC & 2.299 & 137 & 138 & 2.678 & 3.449 & 3.428 & 3.845 & 3.791 & 2.985 & 2.961 & 0.308 & 0.284 & 0.772 & 0.750 & 0.860 & 0.830 & 322.430 & 327.049 & 415.345 & 418.656 & 0.253 & 0.249 & 92.915 & 91.607 & 0.326 & 3.909 \\ 
XT-T & 2.926 & 120 & 121 & 3.011 & 3.509 & 3.483 & 4.013 & 3.983 & 3.444 & 3.444 & 0.433 & 0.433 & 0.498 & 0.472 & 0.569 & 0.540 & 308.987 & 311.260 & 360.047 & 360.049 & 0.032 & 0.033 & 51.060 & 48.789 & 0.352 & 2.917 \\ 
3DPTIA & 2.191 & 112 & 113 & 2.199 & 3.255 & 3.234 & 3.697 & 3.624 & 2.498 & 2.465 & 0.299 & 0.266 & 1.056 & 1.035 & 1.200 & 1.159 & 335.319 & 342.101 & 496.370 & 503.034 & 0.163 & 0.134 & 161.051 & 160.933 & 0.213 & 5.302 \\ 
PyIAnTPh & 2.018 & 146 & 147 & 1.711 & 2.280 & 2.212 & 3.242 & 3.084 & 2.433 & 2.387 & 0.722 & 0.675 & 0.569 & 0.500 & 0.809 & 0.698 & 382.408 & 401.998 & 509.533 & 519.499 & 0.780 & 0.547 & 127.126 & 117.502 & 0.497 & 8.123 \\ 
2CzP-INN & 1.852 & 107 & 108 & 2.205 & 3.462 & 3.439 & 3.914 & 3.857 & 2.493 & 2.472 & 0.288 & 0.268 & 1.257 & 1.234 & 1.421 & 1.384 & 316.763 & 321.494 & 497.311 & 501.472 & 0.715 & 0.564 & 180.548 & 179.978 & 0.246 & 2.411 \\ 
VBN0 & 2.122 & 129 & 130 & 2.510 & 3.204 & 3.180 & 3.657 & 3.623 & 2.865 & 2.860 & 0.355 & 0.350 & 0.694 & 0.670 & 0.792 & 0.763 & 339.033 & 342.224 & 432.709 & 433.523 & 0.496 & 0.457 & 93.676 & 91.299 & 0.320 & 3.360 \\ 
PIAnTPh & 2.080 & 142 & 143 & 1.708 & 2.238 & 2.168 & 3.256 & 3.106 & 2.485 & 2.447 & 0.777 & 0.739 & 0.530 & 0.460 & 0.771 & 0.659 & 380.822 & 399.125 & 498.914 & 506.630 & 0.862 & 0.615 & 118.092 & 107.505 & 0.872 & 1.632 \\ 
BCZ-DPS-AD & 2.166 & 146 & 147 & 2.648 & 3.383 & 3.360 & 3.803 & 3.732 & 2.977 & 2.941 & 0.328 & 0.293 & 0.735 & 0.712 & 0.826 & 0.791 & 326.043 & 332.255 & 416.526 & 421.564 & 0.158 & 0.131 & 90.483 & 89.309 & 0.181 & 3.926 \\ 
2BTPA-INN & 1.776 & 165 & 166 & 2.107 & 3.183 & 3.159 & 3.707 & 3.691 & 2.454 & 2.462 & 0.347 & 0.355 & 1.075 & 1.052 & 1.252 & 1.229 & 334.505 & 335.891 & 505.186 & 503.503 & 1.990 & 1.854 & 170.682 & 167.611 & 0.291 & 2.254 \\ 
SpiroAc & 2.725 & 61 & 62 & 2.886 & 3.464 & 3.430 & 4.088 & 4.018 & 3.406 & 3.380 & 0.520 & 0.494 & 0.578 & 0.545 & 0.682 & 0.638 & 303.258 & 308.557 & 364.012 & 366.789 & 0.049 & 0.092 & 60.753 & 58.233 & 0.170 & 3.731 \\ 
BuPCzBCO & 3.107 & 66 & 67 & 2.964 & 3.385 & 3.362 & 3.808 & 3.737 & 3.334 & 3.295 & 0.370 & 0.331 & 0.421 & 0.398 & 0.473 & 0.442 & 325.606 & 331.775 & 371.825 & 376.273 & 0.159 & 0.134 & 46.220 & 44.499 & 0.645 & 0.474 \\ 
AQ-S-CZ & 1.038 & 85 & 86 & 1.464 & 2.450 & 2.428 & 2.892 & 2.837 & 1.728 & 1.711 & 0.264 & 0.246 & 0.986 & 0.964 & 1.163 & 1.126 & 428.789 & 437.057 & 717.491 & 724.760 & 0.198 & 0.169 & 288.703 & 287.703 & 0.138 & 8.200 \\ 
DBP-3TPA & 1.288 & 186 & 187 & 1.184 & 3.056 & 3.021 & 3.293 & 3.292 & 1.276 & 1.290 & 0.092 & 0.106 & 1.872 & 1.837 & 2.017 & 2.002 & 376.520 & 376.588 & 971.887 & 961.121 & 0.007 & 0.007 & 595.367 & 584.533 & 0.543 & 0.084 \\ 
DCzIPN & 2.201 & 83 & 84 & 2.371 & 3.140 & 3.121 & 3.615 & 3.570 & 2.730 & 2.712 & 0.359 & 0.341 & 0.769 & 0.750 & 0.885 & 0.858 & 342.924 & 347.295 & 454.154 & 457.130 & 0.272 & 0.228 & 111.230 & 109.835 & 0.545 & 1.698 \\ 
DMeCzIPN & 2.080 & 89 & 90 & 2.308 & 3.141 & 3.126 & 3.521 & 3.487 & 2.587 & 2.575 & 0.279 & 0.267 & 0.833 & 0.817 & 0.934 & 0.912 & 352.118 & 355.541 & 479.195 & 481.451 & 0.176 & 0.153 & 127.077 & 125.910 & 0.372 & 1.797 \\ 
SAFDPA & 2.610 & 106 & 107 & 2.701 & 3.320 & 3.300 & 3.681 & 3.641 & 2.995 & 2.979 & 0.294 & 0.278 & 0.619 & 0.600 & 0.687 & 0.662 & 336.785 & 340.541 & 413.986 & 416.182 & 0.063 & 0.052 & 77.201 & 75.641 & 0.166 & 3.934 \\ 
t-DABNA & 2.352 & 125 & 126 & 2.428 & 2.654 & 2.628 & 3.143 & 3.061 & 2.876 & 2.828 & 0.448 & 0.399 & 0.226 & 0.200 & 0.267 & 0.233 & 394.452 & 405.084 & 431.092 & 438.459 & 0.467 & 0.378 & 36.640 & 33.374 & 0.586 & 1.240 \\ 
3-AcBPtCN & 0.572 & 102 & 103 & 0.936 & 2.804 & 2.791 & 2.995 & 2.982 & 1.000 & 1.001 & 0.064 & 0.064 & 1.868 & 1.854 & 1.995 & 1.981 & 413.943 & 415.761 & 1239.719 & 1238.993 & 0.268 & 0.256 & 825.776 & 823.232 & 0.262 & 7.769 \\ 
3-AcBPdCN & 1.176 & 98 & 99 & 0.993 & 2.357 & 2.327 & 2.858 & 2.797 & 1.204 & 1.193 & 0.211 & 0.200 & 1.364 & 1.334 & 1.654 & 1.603 & 433.784 & 443.339 & 1029.621 & 1038.950 & 0.637 & 0.549 & 595.837 & 595.611 & 0.518 & 0.316 \\ 
11-AcBPdCN & 1.261 & 98 & 99 & 1.068 & 2.066 & 2.027 & 2.649 & 2.560 & 1.369 & 1.349 & 0.301 & 0.281 & 0.999 & 0.959 & 1.280 & 1.211 & 468.077 & 484.370 & 905.905 & 919.383 & 0.463 & 0.374 & 437.828 & 435.013 & 0.533 & 0.370 \\ 
PID-3 & 1.973 & 78 & 79 & 1.716 & 2.481 & 2.422 & 3.361 & 3.271 & 2.325 & 2.318 & 0.608 & 0.602 & 0.765 & 0.705 & 1.036 & 0.953 & 368.891 & 379.075 & 533.313 & 534.896 & 1.769 & 1.412 & 164.422 & 155.820 & 0.766 & 2.803 \\ 
3-ACBPmCN & 0.956 & 94 & 95 & 1.098 & 3.089 & 3.058 & 3.221 & 3.220 & 1.145 & 1.157 & 0.047 & 0.058 & 1.990 & 1.959 & 2.075 & 2.063 & 384.948 & 385.104 & 1082.367 & 1071.901 & 0.010 & 0.010 & 697.419 & 686.797 & 0.171 & 7.559 \\ 
3-DTPA-BBI & 1.358 & 139 & 140 & 1.555 & 2.414 & 2.372 & 3.050 & 2.990 & 1.964 & 1.960 & 0.410 & 0.405 & 0.859 & 0.817 & 1.085 & 1.030 & 406.559 & 414.691 & 631.155 & 632.550 & 1.798 & 1.497 & 224.596 & 217.860 & 0.294 & 7.098 \\ 
IABTCN & 1.051 & 123 & 124 & 1.526 & 2.496 & 2.456 & 3.077 & 3.029 & 1.881 & 1.882 & 0.355 & 0.356 & 0.970 & 0.930 & 1.196 & 1.147 & 402.939 & 409.297 & 659.137 & 658.782 & 1.413 & 1.202 & 256.199 & 249.485 & 0.367 & 6.488 \\ 
BTZPP & 1.078 & 142 & 143 & 1.558 & 2.970 & 2.923 & 3.554 & 3.521 & 1.865 & 1.878 & 0.307 & 0.319 & 1.411 & 1.364 & 1.689 & 1.644 & 348.868 & 352.098 & 664.797 & 660.355 & 2.874 & 2.552 & 315.929 & 308.257 & 0.249 & 6.272 \\ 
DPimdPPA & 1.851 & 78 & 79 & 1.730 & 2.703 & 2.658 & 3.451 & 3.395 & 2.208 & 2.209 & 0.479 & 0.480 & 0.974 & 0.928 & 1.243 & 1.186 & 359.229 & 365.239 & 561.486 & 561.251 & 2.204 & 1.873 & 202.257 & 196.012 & 0.549 & 5.739 \\ 
BCzPh & 2.946 & 89 & 90 & 2.748 & 3.377 & 3.354 & 3.857 & 3.788 & 3.138 & 3.103 & 0.391 & 0.355 & 0.629 & 0.607 & 0.718 & 0.685 & 321.477 & 327.325 & 395.060 & 399.626 & 0.355 & 0.289 & 73.583 & 72.301 & 0.735 & 0.042 \\ 
TBPM2CN & 1.851 & 149 & 150 & 2.105 & 3.342 & 3.310 & 3.745 & 3.713 & 2.358 & 2.361 & 0.254 & 0.256 & 1.237 & 1.205 & 1.386 & 1.352 & 331.101 & 333.946 & 525.724 & 525.195 & 0.944 & 0.834 & 194.622 & 191.249 & 0.152 & 16.114 \\ 
TPM2CN & 1.948 & 135 & 136 & 2.106 & 3.357 & 3.327 & 3.764 & 3.735 & 2.361 & 2.364 & 0.255 & 0.258 & 1.251 & 1.221 & 1.403 & 1.371 & 329.421 & 331.961 & 525.104 & 524.440 & 0.945 & 0.826 & 195.683 & 192.479 & 0.303 & 11.334 \\ 
PT-BZ-DMAC & 1.493 & 90 & 91 & 2.096 & 3.400 & 3.368 & 3.510 & 3.505 & 2.163 & 2.181 & 0.068 & 0.085 & 1.304 & 1.272 & 1.346 & 1.324 & 353.272 & 353.776 & 573.117 & 568.532 & 0.131 & 0.125 & 219.845 & 214.756 & 0.166 & 6.517 \\ 
PS-BZ-DMAC & 2.139 & 96 & 97 & 2.058 & 2.753 & 2.718 & 3.496 & 3.419 & 2.614 & 2.589 & 0.556 & 0.531 & 0.694 & 0.659 & 0.882 & 0.829 & 354.615 & 362.675 & 474.235 & 478.865 & 1.150 & 0.980 & 119.620 & 116.189 & 0.444 & 4.849 \\ 
2PCzBN-tPh & 2.111 & 161 & 162 & 2.372 & 3.446 & 3.424 & 3.766 & 3.740 & 2.593 & 2.591 & 0.221 & 0.219 & 1.073 & 1.052 & 1.173 & 1.149 & 329.211 & 331.500 & 478.188 & 478.494 & 0.617 & 0.568 & 148.977 & 146.994 & 0.327 & 2.080 \\ 
2PCzBN & 2.202 & 135 & 136 & 2.564 & 3.426 & 3.405 & 3.832 & 3.804 & 2.868 & 2.865 & 0.304 & 0.301 & 0.862 & 0.841 & 0.964 & 0.940 & 323.533 & 325.897 & 432.342 & 432.819 & 0.725 & 0.661 & 108.809 & 106.922 & 0.343 & 1.136 \\ 
TPA-2 & 0.677 & 137 & 138 & 0.704 & 2.378 & 2.357 & 2.518 & 2.517 & 0.746 & 0.752 & 0.042 & 0.048 & 1.673 & 1.653 & 1.772 & 1.765 & 492.333 & 492.568 & 1661.848 & 1648.236 & 0.005 & 0.006 & 1169.515 & 1155.669 & 0.432 & 3.316 \\ 
36DTPAFM & 0.980 & 131 & 132 & 1.443 & 2.426 & 2.385 & 2.775 & 2.755 & 1.650 & 1.666 & 0.207 & 0.223 & 0.983 & 0.943 & 1.124 & 1.089 & 446.854 & 450.066 & 751.368 & 744.073 & 0.129 & 0.124 & 304.514 & 294.007 & 0.274 & 6.547 \\ 
AQTC & 1.210 & 58 & 59 & 1.183 & 2.889 & 2.838 & 3.358 & 3.357 & 1.375 & 1.400 & 0.192 & 0.216 & 1.706 & 1.655 & 1.983 & 1.958 & 369.187 & 369.308 & 901.415 & 885.915 & 0.006 & 0.006 & 532.228 & 516.607 & 0.472 & 1.142 \\ 
3TPAFM & 0.922 & 86 & 87 & 1.537 & 2.378 & 2.349 & 2.624 & 2.599 & 1.696 & 1.700 & 0.159 & 0.163 & 0.841 & 0.812 & 0.928 & 0.898 & 472.555 & 477.119 & 731.017 & 729.231 & 0.088 & 0.084 & 258.462 & 252.111 & 0.298 & 9.057 \\ 
BBPA & 2.150 & 91 & 92 & 1.754 & 2.249 & 2.177 & 3.212 & 3.038 & 2.505 & 2.447 & 0.751 & 0.693 & 0.495 & 0.423 & 0.707 & 0.591 & 386.003 & 408.138 & 494.967 & 506.665 & 0.398 & 0.276 & 108.964 & 98.526 & 0.933 & 0.029 \\ 
DMPA & 2.133 & 85 & 86 & 1.740 & 2.255 & 2.185 & 3.212 & 3.050 & 2.478 & 2.429 & 0.738 & 0.689 & 0.515 & 0.445 & 0.733 & 0.621 & 386.039 & 406.546 & 500.254 & 510.452 & 0.469 & 0.333 & 114.215 & 103.907 & 0.925 & 0.020 \\ 
PXZ-NAI & 1.057 & 83 & 84 & 1.706 & 1.667 & 1.653 & 1.927 & 1.899 & 1.971 & 1.959 & 0.265 & 0.253 & -0.038 & -0.052 & -0.044 & -0.060 & 643.572 & 652.961 & 629.046 & 633.017 & 0.194 & 0.167 & -14.526 & -19.944 & 0.367 & 4.561 \\ 
PTZ-NAI & 0.676 & 83 & 84 & 1.694 & 2.135 & 2.133 & 2.135 & 2.134 & 1.694 & 1.694 & 0.000 & 0.000 & 0.441 & 0.440 & 0.441 & 0.440 & 580.695 & 581.103 & 731.969 & 731.969 & 0.000 & 0.000 & 151.274 & 150.866 & 0.094 & 5.573 \\ 
AI-4Cz & 1.435 & 161 & 162 & 1.768 & 2.494 & 2.482 & 2.783 & 2.750 & 1.974 & 1.959 & 0.205 & 0.191 & 0.725 & 0.713 & 0.809 & 0.790 & 445.474 & 450.917 & 628.116 & 632.783 & 0.051 & 0.047 & 182.642 & 181.866 & 0.367 & 1.443 \\ 
DAcIPN & 1.913 & 101 & 102 & 2.054 & 2.963 & 2.937 & 3.457 & 3.413 & 2.396 & 2.386 & 0.343 & 0.333 & 0.909 & 0.883 & 1.061 & 1.026 & 358.605 & 363.324 & 517.398 & 519.552 & 0.194 & 0.175 & 158.792 & 156.229 & 0.274 & 4.155 \\ 
TCz1 & 2.626 & 115 & 116 & 2.708 & 3.156 & 3.133 & 3.624 & 3.550 & 3.110 & 3.068 & 0.401 & 0.360 & 0.448 & 0.425 & 0.514 & 0.481 & 342.139 & 349.300 & 398.711 & 404.091 & 0.056 & 0.045 & 56.573 & 54.790 & 0.451 & 1.876 \\ 
MBF & 1.091 & 92 & 93 & 1.827 & 2.475 & 2.452 & 2.773 & 2.751 & 2.047 & 2.050 & 0.220 & 0.222 & 0.648 & 0.625 & 0.726 & 0.701 & 447.144 & 450.770 & 605.646 & 604.858 & 0.843 & 0.759 & 158.501 & 154.088 & 0.302 & 7.964 \\ 
MPA & 1.426 & 84 & 85 & 1.979 & 2.749 & 2.718 & 3.110 & 3.072 & 2.239 & 2.237 & 0.260 & 0.258 & 0.770 & 0.739 & 0.871 & 0.835 & 398.650 & 403.608 & 553.730 & 554.233 & 0.016 & 0.014 & 155.079 & 150.625 & 0.162 & 9.280 \\ 
3,3-NHC & 2.390 & 85 & 86 & 2.604 & 3.282 & 3.241 & 4.230 & 4.170 & 3.356 & 3.350 & 0.752 & 0.746 & 0.678 & 0.638 & 0.874 & 0.820 & 293.114 & 297.353 & 369.433 & 370.151 & 0.051 & 0.133 & 76.319 & 72.798 & 0.126 & 6.366 \\ 
3CP-DPS-DMAC & 2.288 & 107 & 108 & 2.861 & 3.385 & 3.361 & 3.820 & 3.747 & 3.228 & 3.190 & 0.368 & 0.329 & 0.524 & 0.500 & 0.592 & 0.557 & 324.566 & 330.889 & 384.046 & 388.706 & 0.201 & 0.164 & 59.481 & 57.817 & 0.149 & 4.913 \\ 
3CP-DPS-PXZ & 2.229 & 101 & 102 & 2.504 & 2.733 & 2.702 & 3.098 & 3.061 & 2.838 & 2.837 & 0.335 & 0.333 & 0.229 & 0.198 & 0.260 & 0.224 & 400.156 & 405.084 & 436.795 & 437.063 & 0.015 & 0.013 & 36.640 & 31.979 & 0.301 & 4.389 \\ 
3CzAnN & 2.084 & 100 & 101 & 1.706 & 2.248 & 2.178 & 3.252 & 3.107 & 2.469 & 2.434 & 0.762 & 0.728 & 0.541 & 0.472 & 0.783 & 0.673 & 381.255 & 399.099 & 502.218 & 509.376 & 0.774 & 0.562 & 120.963 & 110.277 & 0.885 & 0.964 \\ 
DPQ-DMAC & 1.272 & 91 & 92 & 1.299 & 3.000 & 2.990 & 3.123 & 3.114 & 1.352 & 1.352 & 0.053 & 0.054 & 1.701 & 1.692 & 1.771 & 1.761 & 396.940 & 398.189 & 916.935 & 916.816 & 0.120 & 0.115 & 519.995 & 518.627 & 0.259 & 5.458 \\ 
DPAA & 2.135 & 61 & 62 & 1.740 & 2.245 & 2.172 & 3.295 & 3.113 & 2.554 & 2.494 & 0.814 & 0.754 & 0.505 & 0.432 & 0.741 & 0.619 & 376.268 & 398.317 & 485.419 & 497.177 & 0.422 & 0.298 & 109.150 & 98.860 & 0.936 & 0.000 \\ 
t3Cz-SO & 2.078 & 176 & 177 & 2.498 & 3.156 & 3.135 & 3.605 & 3.537 & 2.853 & 2.817 & 0.356 & 0.320 & 0.658 & 0.638 & 0.752 & 0.719 & 343.913 & 350.565 & 434.549 & 440.090 & 0.207 & 0.174 & 90.636 & 89.525 & 0.240 & 7.749 \\ 
Cz-SO & 2.766 & 68 & 69 & 2.971 & 3.407 & 3.384 & 3.861 & 3.787 & 3.366 & 3.325 & 0.395 & 0.354 & 0.436 & 0.413 & 0.495 & 0.463 & 321.153 & 327.377 & 368.336 & 372.929 & 0.224 & 0.193 & 47.184 & 45.553 & 0.391 & 4.879 \\ 
DPQ-PXZ & 1.215 & 85 & 86 & 1.282 & 2.397 & 2.386 & 2.607 & 2.587 & 1.395 & 1.390 & 0.113 & 0.108 & 1.115 & 1.104 & 1.213 & 1.197 & 475.527 & 479.351 & 889.000 & 892.110 & 0.219 & 0.198 & 413.472 & 412.759 & 0.333 & 5.444 \\ 
pCzAnN & 2.056 & 100 & 101 & 1.705 & 2.252 & 2.182 & 3.270 & 3.115 & 2.476 & 2.434 & 0.771 & 0.729 & 0.547 & 0.477 & 0.794 & 0.681 & 379.168 & 397.985 & 500.810 & 509.323 & 0.771 & 0.547 & 121.642 & 111.338 & 0.748 & 3.318 \\ 
3-BHH & 2.528 & 77 & 78 & 2.674 & 3.233 & 3.191 & 4.176 & 4.087 & 3.454 & 3.425 & 0.780 & 0.751 & 0.559 & 0.517 & 0.722 & 0.662 & 296.897 & 303.333 & 358.927 & 361.999 & 0.132 & 0.117 & 62.030 & 58.667 & 0.188 & 5.368 \\ 
DPP-PXZ & 1.026 & 85 & 86 & 0.903 & 1.927 & 1.914 & 2.182 & 2.152 & 1.023 & 1.016 & 0.119 & 0.113 & 1.023 & 1.010 & 1.159 & 1.136 & 568.318 & 576.135 & 1212.253 & 1220.508 & 0.213 & 0.186 & 643.935 & 644.373 & 0.525 & 3.214 \\ 
APPT-PXZ & 1.152 & 97 & 98 & 1.299 & 1.793 & 1.780 & 2.045 & 2.020 & 1.482 & 1.475 & 0.183 & 0.175 & 0.493 & 0.480 & 0.563 & 0.545 & 606.309 & 613.844 & 836.436 & 840.642 & 0.297 & 0.264 & 230.127 & 226.798 & 0.346 & 5.117 \\ 
HITPE & 2.488 & 133 & 134 & 1.685 & 3.091 & 3.055 & 3.848 & 3.797 & 2.097 & 2.093 & 0.412 & 0.409 & 1.407 & 1.371 & 1.751 & 1.703 & 322.196 & 326.566 & 591.289 & 592.331 & 0.860 & 0.723 & 269.094 & 265.765 & 0.340 & 8.850 \\ 
DV-3CzCN & 2.103 & 184 & 185 & 2.387 & 3.409 & 3.389 & 3.763 & 3.729 & 2.635 & 2.627 & 0.248 & 0.240 & 1.022 & 1.001 & 1.128 & 1.102 & 329.465 & 332.495 & 470.553 & 471.971 & 0.610 & 0.540 & 141.089 & 139.475 & 0.249 & 3.936 \\ 
SF-DPSO & 2.863 & 152 & 153 & 2.413 & 3.770 & 3.737 & 4.494 & 4.454 & 2.876 & 2.876 & 0.463 & 0.463 & 1.357 & 1.324 & 1.618 & 1.578 & 275.888 & 278.378 & 431.076 & 431.113 & 2.020 & 1.837 & 155.187 & 152.735 & 0.568 & 3.894 \\ 
BDQ-tBuCz & 1.399 & 160 & 161 & 1.320 & 2.457 & 2.433 & 2.753 & 2.722 & 1.479 & 1.477 & 0.159 & 0.156 & 1.137 & 1.113 & 1.274 & 1.245 & 450.344 & 455.506 & 838.108 & 839.641 & 0.322 & 0.282 & 387.764 & 384.135 & 0.595 & 1.121 \\ 
BDQDMAC & 1.182 & 130 & 131 & 1.223 & 2.497 & 2.485 & 2.629 & 2.616 & 1.288 & 1.288 & 0.065 & 0.065 & 1.274 & 1.262 & 1.341 & 1.329 & 471.656 & 473.855 & 962.920 & 962.760 & 0.129 & 0.117 & 491.264 & 488.905 & 0.453 & 1.342 \\ 
BDQPCz & 1.496 & 140 & 141 & 1.359 & 3.055 & 3.020 & 3.396 & 3.381 & 1.511 & 1.521 & 0.152 & 0.162 & 1.696 & 1.661 & 1.885 & 1.859 & 365.132 & 366.763 & 820.625 & 814.900 & 0.183 & 0.204 & 455.493 & 448.137 & 0.584 & 0.489 \\ 
4-SCZ & 2.811 & 74 & 75 & 2.518 & 3.118 & 3.088 & 3.670 & 3.590 & 2.964 & 2.928 & 0.446 & 0.409 & 0.600 & 0.570 & 0.706 & 0.662 & 337.813 & 345.350 & 418.286 & 423.464 & 0.185 & 0.153 & 80.473 & 78.113 & 0.748 & 1.075 \\ 
Py-TPA & 0.811 & 152 & 153 & 1.030 & 2.863 & 2.833 & 3.211 & 3.207 & 1.155 & 1.165 & 0.125 & 0.136 & 1.833 & 1.804 & 2.056 & 2.042 & 386.075 & 386.605 & 1073.451 & 1063.811 & 0.042 & 0.197 & 687.376 & 677.206 & 0.238 & 8.945 \\ 
DPACPhTPI & 2.192 & 155 & 156 & 2.248 & 3.400 & 3.372 & 3.786 & 3.748 & 2.503 & 2.498 & 0.255 & 0.250 & 1.152 & 1.124 & 1.283 & 1.249 & 327.455 & 330.836 & 495.310 & 496.274 & 0.472 & 0.428 & 167.855 & 165.438 & 0.130 & 8.629 \\ 
oPTBC & 1.669 & 88 & 89 & 2.246 & 2.573 & 2.566 & 2.726 & 2.713 & 2.380 & 2.374 & 0.134 & 0.128 & 0.327 & 0.320 & 0.347 & 0.339 & 454.754 & 457.017 & 521.027 & 522.175 & 0.094 & 0.081 & 66.273 & 65.158 & 0.309 & 3.332 \\ 
mPTBC & 1.592 & 88 & 89 & 2.252 & 2.705 & 2.694 & 2.986 & 2.962 & 2.486 & 2.476 & 0.234 & 0.224 & 0.453 & 0.442 & 0.500 & 0.486 & 415.177 & 418.540 & 498.693 & 500.707 & 0.284 & 0.250 & 83.516 & 82.167 & 0.309 & 5.241 \\ 
P3C & 1.992 & 99 & 100 & 1.709 & 2.596 & 2.529 & 3.503 & 3.416 & 2.306 & 2.308 & 0.597 & 0.599 & 0.887 & 0.820 & 1.197 & 1.108 & 353.927 & 362.962 & 537.613 & 537.170 & 1.538 & 1.268 & 183.686 & 174.208 & 0.910 & 0.798 \\ 
DBCP & 1.396 & 96 & 97 & 1.984 & 2.680 & 2.672 & 2.766 & 2.759 & 2.048 & 2.049 & 0.063 & 0.064 & 0.696 & 0.688 & 0.718 & 0.710 & 448.227 & 449.397 & 605.428 & 605.128 & 0.070 & 0.064 & 157.201 & 155.731 & 0.214 & 5.586 \\ 
NAQ3 & 1.502 & 115 & 116 & 1.517 & 2.138 & 2.117 & 2.539 & 2.498 & 1.802 & 1.791 & 0.284 & 0.273 & 0.621 & 0.600 & 0.737 & 0.708 & 488.377 & 496.274 & 688.210 & 692.406 & 0.489 & 0.423 & 199.833 & 196.131 & 0.476 & 2.588 \\ 
mCP-BP-DMAC & 1.619 & 127 & 128 & 2.174 & 2.744 & 2.713 & 3.106 & 3.069 & 2.462 & 2.460 & 0.287 & 0.286 & 0.569 & 0.538 & 0.644 & 0.609 & 399.202 & 403.989 & 503.670 & 503.987 & 0.017 & 0.014 & 104.468 & 99.998 & 0.254 & 6.264 \\ 
BFCZPZ3 & 2.288 & 107 & 108 & 2.093 & 3.278 & 3.255 & 3.694 & 3.660 & 2.359 & 2.353 & 0.265 & 0.260 & 1.185 & 1.162 & 1.335 & 1.307 & 335.655 & 338.773 & 525.678 & 526.871 & 0.653 & 0.581 & 190.023 & 188.098 & 0.629 & 0.137 \\ 
BTCZPZ1 & 2.038 & 107 & 108 & 2.002 & 3.081 & 3.060 & 3.459 & 3.418 & 2.248 & 2.236 & 0.246 & 0.234 & 1.079 & 1.058 & 1.212 & 1.182 & 358.388 & 362.760 & 551.584 & 554.418 & 0.873 & 0.756 & 193.197 & 191.658 & 0.518 & 0.052 \\ 
BFCZPZ2 & 2.239 & 107 & 108 & 2.010 & 3.162 & 3.138 & 3.585 & 3.546 & 2.279 & 2.272 & 0.269 & 0.262 & 1.152 & 1.128 & 1.306 & 1.274 & 345.871 & 349.645 & 544.093 & 545.770 & 1.804 & 1.590 & 198.223 & 196.125 & 0.543 & 0.245 \\ 
CZ9CZPZ & 1.907 & 135 & 136 & 2.001 & 3.224 & 3.201 & 3.685 & 3.642 & 2.287 & 2.276 & 0.286 & 0.275 & 1.224 & 1.201 & 1.398 & 1.366 & 336.438 & 340.466 & 542.179 & 544.757 & 1.574 & 1.366 & 205.741 & 204.291 & 0.276 & 2.078 \\ 
BFCZPZ1 & 2.334 & 107 & 108 & 2.064 & 3.139 & 3.114 & 3.546 & 3.504 & 2.332 & 2.322 & 0.268 & 0.258 & 1.075 & 1.050 & 1.215 & 1.182 & 349.606 & 353.816 & 531.741 & 533.910 & 0.959 & 0.839 & 182.135 & 180.094 & 0.633 & 0.175 \\ 
TPBPPI-PY & 2.482 & 152 & 153 & 2.351 & 3.547 & 3.515 & 3.962 & 3.928 & 2.626 & 2.627 & 0.275 & 0.276 & 1.196 & 1.164 & 1.336 & 1.301 & 312.933 & 315.674 & 472.179 & 471.951 & 0.136 & 0.129 & 159.246 & 156.276 & 0.379 & 5.916 \\ 
TPBPPI-PBI & 2.382 & 187 & 188 & 2.398 & 3.600 & 3.570 & 3.936 & 3.899 & 2.622 & 2.619 & 0.224 & 0.221 & 1.202 & 1.172 & 1.314 & 1.280 & 314.976 & 317.990 & 472.866 & 473.438 & 0.129 & 0.122 & 157.890 & 155.448 & 0.263 & 8.273 \\ 
PTZ-2PTO & 2.169 & 87 & 88 & 2.407 & 2.833 & 2.804 & 3.178 & 3.138 & 2.700 & 2.694 & 0.293 & 0.287 & 0.426 & 0.397 & 0.478 & 0.444 & 390.084 & 395.068 & 459.137 & 460.227 & 0.033 & 0.027 & 69.053 & 65.159 & 0.175 & 5.222 \\ 
4F-m-$\nu$-DABNA & 1.993 & 237 & 238 & 2.158 & 2.865 & 2.846 & 3.215 & 3.174 & 2.422 & 2.407 & 0.264 & 0.249 & 0.707 & 0.688 & 0.793 & 0.767 & 385.655 & 390.649 & 511.902 & 515.092 & 1.012 & 0.890 & 126.247 & 124.442 & 0.249 & 4.969 \\ 
m-$\nu$-DABNA & 2.201 & 225 & 226 & 2.252 & 2.800 & 2.780 & 3.160 & 3.116 & 2.541 & 2.524 & 0.289 & 0.272 & 0.548 & 0.528 & 0.618 & 0.592 & 392.380 & 397.895 & 487.851 & 491.140 & 0.898 & 0.783 & 95.471 & 93.244 & 0.530 & 0.721 \\ 
TPA-PyI & 2.221 & 117 & 118 & 2.196 & 3.376 & 3.349 & 3.836 & 3.813 & 2.495 & 2.501 & 0.299 & 0.304 & 1.180 & 1.153 & 1.340 & 1.312 & 323.221 & 325.153 & 496.833 & 495.778 & 1.810 & 1.648 & 173.613 & 170.624 & 0.335 & 8.707 \\ 
4F-$\nu$-DABNA & 2.037 & 213 & 214 & 2.194 & 2.858 & 2.839 & 3.211 & 3.170 & 2.465 & 2.450 & 0.271 & 0.256 & 0.664 & 0.645 & 0.746 & 0.720 & 386.099 & 391.117 & 502.979 & 506.040 & 0.931 & 0.816 & 116.880 & 114.923 & 0.272 & 4.597 \\ 
CBPTZ & 2.011 & 145 & 146 & 1.715 & 3.495 & 3.473 & 3.946 & 3.889 & 1.936 & 1.920 & 0.221 & 0.205 & 1.780 & 1.758 & 2.010 & 1.969 & 314.218 & 318.832 & 640.504 & 645.725 & 0.466 & 0.380 & 326.286 & 326.893 & 0.063 & 7.454 \\ 
CBPBM & 2.516 & 138 & 139 & 2.404 & 3.477 & 3.454 & 3.921 & 3.858 & 2.711 & 2.686 & 0.307 & 0.281 & 1.073 & 1.050 & 1.209 & 1.173 & 316.246 & 321.336 & 457.337 & 461.638 & 0.375 & 0.311 & 141.091 & 140.302 & 0.267 & 3.752 \\ 
CBPPY & 2.557 & 103 & 104 & 2.450 & 3.479 & 3.456 & 3.955 & 3.891 & 2.785 & 2.758 & 0.335 & 0.308 & 1.029 & 1.006 & 1.170 & 1.133 & 313.495 & 318.668 & 445.217 & 449.584 & 0.348 & 0.267 & 131.722 & 130.916 & 0.357 & 5.152 \\ 
N-B & 2.670 & 63 & 64 & 2.627 & 3.838 & 3.822 & 4.094 & 4.081 & 2.802 & 2.804 & 0.175 & 0.177 & 1.211 & 1.196 & 1.292 & 1.277 & 302.829 & 303.838 & 442.482 & 442.175 & 0.184 & 0.168 & 139.653 & 138.337 & 0.551 & 1.480 \\ 
DPACpBr & 3.145 & 85 & 86 & 3.038 & 3.699 & 3.677 & 4.106 & 4.079 & 3.373 & 3.370 & 0.335 & 0.332 & 0.661 & 0.639 & 0.734 & 0.709 & 301.929 & 303.980 & 367.603 & 367.888 & 0.273 & 0.249 & 65.674 & 63.909 & 0.525 & 2.022 \\ 
DPCN & 1.409 & 125 & 126 & 2.135 & 3.385 & 3.353 & 3.841 & 3.806 & 2.423 & 2.424 & 0.288 & 0.288 & 1.249 & 1.218 & 1.418 & 1.383 & 322.817 & 325.743 & 511.706 & 511.555 & 0.459 & 0.400 & 188.890 & 185.812 & 0.022 & 11.310 \\ 
BZC-PXZ & 1.346 & 78 & 79 & 2.109 & 2.508 & 2.496 & 2.794 & 2.767 & 2.350 & 2.338 & 0.241 & 0.228 & 0.399 & 0.387 & 0.444 & 0.429 & 443.704 & 448.163 & 527.561 & 530.334 & 0.245 & 0.211 & 83.857 & 82.171 & 0.066 & 6.296 \\ 
CzBN & 2.299 & 73 & 74 & 2.756 & 3.357 & 3.339 & 3.719 & 3.681 & 3.054 & 3.038 & 0.298 & 0.282 & 0.600 & 0.583 & 0.665 & 0.642 & 333.363 & 336.850 & 405.985 & 408.068 & 0.254 & 0.230 & 72.622 & 71.219 & 0.349 & 3.452 \\ 
2CzBN & 2.359 & 79 & 80 & 2.666 & 3.409 & 3.388 & 3.745 & 3.710 & 2.930 & 2.920 & 0.264 & 0.254 & 0.742 & 0.722 & 0.816 & 0.791 & 331.022 & 334.153 & 423.200 & 424.647 & 0.185 & 0.159 & 92.178 & 90.494 & 0.404 & 3.908 \\ 
TPA-DPPI & 2.211 & 166 & 167 & 2.184 & 3.460 & 3.432 & 3.859 & 3.828 & 2.436 & 2.436 & 0.252 & 0.252 & 1.276 & 1.248 & 1.423 & 1.392 & 321.302 & 323.888 & 509.039 & 509.027 & 1.310 & 1.143 & 187.737 & 185.139 & 0.328 & 8.915 \\ 
ANQDC-PSTA & 1.080 & 144 & 145 & 1.222 & 2.194 & 2.182 & 2.368 & 2.351 & 1.319 & 1.317 & 0.097 & 0.095 & 0.972 & 0.959 & 1.049 & 1.034 & 523.692 & 527.368 & 940.154 & 941.359 & 0.240 & 0.226 & 416.461 & 413.991 & 0.200 & 7.852 \\ 
pDPAPQ-PXZ & 1.201 & 107 & 108 & 1.321 & 1.821 & 1.808 & 2.066 & 2.042 & 1.498 & 1.491 & 0.178 & 0.171 & 0.500 & 0.487 & 0.568 & 0.550 & 600.088 & 607.230 & 827.510 & 831.335 & 0.295 & 0.264 & 227.422 & 224.105 & 0.346 & 4.895 \\ 
m-CZ-DPS-DMAC & 2.101 & 137 & 138 & 2.596 & 3.430 & 3.407 & 3.854 & 3.798 & 2.917 & 2.894 & 0.320 & 0.297 & 0.834 & 0.811 & 0.937 & 0.904 & 321.719 & 326.472 & 425.088 & 428.462 & 0.393 & 0.332 & 103.368 & 101.990 & 0.152 & 4.320 \\ 
pDPBPZ-PXZ & 0.936 & 112 & 113 & 1.096 & 2.757 & 2.726 & 2.985 & 2.970 & 1.187 & 1.194 & 0.091 & 0.098 & 1.661 & 1.630 & 1.798 & 1.776 & 415.399 & 417.441 & 1044.696 & 1038.102 & 0.413 & 0.388 & 629.297 & 620.661 & 0.240 & 7.920 \\ 
DDPhCz-DPPZ & 1.312 & 167 & 168 & 1.168 & 2.932 & 2.909 & 3.240 & 3.215 & 1.291 & 1.291 & 0.123 & 0.123 & 1.763 & 1.740 & 1.949 & 1.924 & 382.644 & 385.667 & 960.138 & 960.166 & 0.331 & 0.351 & 577.495 & 574.499 & 0.568 & 0.197 \\ 
DCz-DPPZ & 1.311 & 111 & 112 & 1.181 & 2.780 & 2.760 & 3.147 & 3.107 & 1.337 & 1.330 & 0.156 & 0.149 & 1.598 & 1.578 & 1.809 & 1.777 & 394.013 & 398.984 & 927.150 & 932.023 & 0.703 & 0.624 & 533.137 & 533.040 & 0.562 & 0.363 \\ 
Oxd-bCZ & 2.055 & 129 & 130 & 2.210 & 3.456 & 3.424 & 3.882 & 3.835 & 2.482 & 2.475 & 0.273 & 0.265 & 1.246 & 1.214 & 1.400 & 1.360 & 319.366 & 323.322 & 499.449 & 500.968 & 1.867 & 1.343 & 180.083 & 177.646 & 0.295 & 5.795 \\ 
Fene & 1.599 & 90 & 91 & 1.864 & 2.700 & 2.679 & 2.888 & 2.877 & 1.993 & 2.001 & 0.130 & 0.138 & 0.837 & 0.815 & 0.895 & 0.875 & 429.278 & 431.010 & 622.023 & 619.490 & 0.076 & 0.071 & 192.745 & 188.480 & 0.295 & 3.906 \\ 
Fens & 1.544 & 90 & 91 & 2.053 & 2.776 & 2.749 & 3.101 & 3.092 & 2.293 & 2.309 & 0.240 & 0.256 & 0.723 & 0.696 & 0.807 & 0.783 & 399.872 & 400.984 & 540.659 & 536.987 & 0.022 & 0.032 & 140.787 & 136.003 & 0.155 & 4.545 \\ 
Yad & 1.860 & 102 & 103 & 2.130 & 2.838 & 2.810 & 3.353 & 3.280 & 2.516 & 2.486 & 0.387 & 0.356 & 0.708 & 0.681 & 0.837 & 0.794 & 369.760 & 377.989 & 492.714 & 498.781 & 0.286 & 0.230 & 122.954 & 120.792 & 0.214 & 3.676 \\ 
DTPCZPYTZ & 1.889 & 159 & 160 & 1.777 & 2.718 & 2.655 & 3.616 & 3.530 & 2.364 & 2.362 & 0.587 & 0.585 & 0.941 & 0.879 & 1.252 & 1.168 & 342.877 & 351.220 & 524.495 & 524.923 & 1.738 & 1.461 & 181.618 & 173.703 & 0.333 & 9.052 \\ 
TPADSO2 & 1.934 & 91 & 92 & 2.346 & 3.139 & 3.111 & 3.681 & 3.637 & 2.752 & 2.743 & 0.405 & 0.396 & 0.792 & 0.765 & 0.929 & 0.894 & 336.804 & 340.925 & 450.542 & 452.031 & 1.154 & 1.034 & 113.739 & 111.106 & 0.290 & 8.054 \\ 
B4PyPPM & 2.119 & 113 & 114 & 2.017 & 3.998 & 3.958 & 4.044 & 4.041 & 2.040 & 2.059 & 0.023 & 0.043 & 1.981 & 1.941 & 2.004 & 1.982 & 306.596 & 306.793 & 607.823 & 602.098 & 0.012 & 0.012 & 301.227 & 295.305 & 0.472 & 1.347 \\ 
mAP & 2.685 & 93 & 94 & 3.010 & 3.409 & 3.378 & 4.095 & 4.047 & 3.615 & 3.606 & 0.605 & 0.597 & 0.400 & 0.368 & 0.480 & 0.441 & 302.748 & 306.330 & 342.958 & 343.780 & 0.008 & 0.125 & 40.211 & 37.450 & 0.235 & 1.858 \\ 
DBBPZ-DPXZ & 1.083 & 145 & 146 & 1.119 & 2.712 & 2.700 & 2.965 & 2.945 & 1.224 & 1.221 & 0.104 & 0.101 & 1.593 & 1.581 & 1.741 & 1.724 & 418.230 & 421.028 & 1013.261 & 1015.526 & 0.692 & 0.638 & 595.031 & 594.498 & 0.321 & 6.501 \\ 
DPIBPZ-DPXZ & 0.882 & 145 & 146 & 1.041 & 2.497 & 2.486 & 2.761 & 2.739 & 1.151 & 1.147 & 0.110 & 0.106 & 1.456 & 1.445 & 1.610 & 1.592 & 449.007 & 452.695 & 1077.173 & 1081.325 & 0.691 & 0.626 & 628.166 & 628.630 & 0.346 & 6.718 \\ 
m-DTPACO & 1.967 & 115 & 116 & 2.241 & 3.018 & 2.995 & 3.445 & 3.414 & 2.559 & 2.555 & 0.317 & 0.313 & 0.776 & 0.754 & 0.886 & 0.859 & 359.927 & 363.175 & 484.590 & 485.332 & 0.032 & 0.029 & 124.662 & 122.158 & 0.355 & 5.473 \\ 
mDPBPZ-DPXZ & 0.982 & 145 & 146 & 1.081 & 2.613 & 2.601 & 2.870 & 2.849 & 1.187 & 1.184 & 0.107 & 0.103 & 1.532 & 1.521 & 1.683 & 1.666 & 431.956 & 435.124 & 1044.416 & 1047.567 & 0.693 & 0.633 & 612.460 & 612.443 & 0.330 & 6.608 \\ 
p-DTPACO & 1.889 & 115 & 116 & 2.019 & 2.820 & 2.793 & 3.404 & 3.360 & 2.437 & 2.429 & 0.418 & 0.410 & 0.800 & 0.774 & 0.966 & 0.931 & 364.274 & 368.990 & 508.659 & 510.420 & 1.859 & 1.651 & 144.385 & 141.430 & 0.314 & 7.212 \\ 
2TDBA-SBA & 1.833 & 208 & 209 & 2.384 & 3.074 & 3.054 & 3.572 & 3.497 & 2.770 & 2.730 & 0.386 & 0.345 & 0.690 & 0.670 & 0.801 & 0.767 & 347.139 & 354.565 & 447.555 & 454.228 & 0.226 & 0.190 & 100.415 & 99.664 & 0.118 & 7.324 \\ 
TPA-APm & 0.700 & 91 & 92 & 0.480 & 2.636 & 2.604 & 2.656 & 2.655 & 0.483 & 0.489 & 0.004 & 0.009 & 2.157 & 2.124 & 2.173 & 2.166 & 466.755 & 466.913 & 2565.298 & 2534.632 & 0.000 & 0.000 & 2098.543 & 2067.718 & 0.547 & 0.183 \\ 
TPA-AP & 1.416 & 91 & 92 & 1.407 & 2.985 & 2.935 & 3.538 & 3.516 & 1.667 & 1.685 & 0.261 & 0.278 & 1.578 & 1.529 & 1.870 & 1.831 & 350.485 & 352.619 & 743.603 & 735.746 & 0.189 & 0.172 & 393.117 & 383.128 & 0.326 & 2.720 \\ 
TDBA-SBA & 1.809 & 162 & 163 & 2.530 & 3.069 & 3.049 & 3.561 & 3.485 & 2.935 & 2.891 & 0.405 & 0.362 & 0.540 & 0.520 & 0.626 & 0.594 & 348.192 & 355.745 & 422.454 & 428.805 & 0.282 & 0.229 & 74.262 & 73.060 & 0.029 & 10.336 \\ 
TPA-APy & 1.179 & 91 & 92 & 1.008 & 2.831 & 2.829 & 2.796 & 2.794 & 0.996 & 0.996 & -0.013 & -0.013 & 1.823 & 1.821 & 1.800 & 1.799 & 443.498 & 443.736 & 1245.305 & 1245.401 & 0.002 & 0.002 & 801.808 & 801.666 & 0.486 & 1.276 \\ 
TPD4PA & 2.173 & 142 & 143 & 2.393 & 2.893 & 2.873 & 3.286 & 3.227 & 2.718 & 2.688 & 0.324 & 0.295 & 0.500 & 0.480 & 0.568 & 0.539 & 377.356 & 384.185 & 456.213 & 461.210 & 0.271 & 0.234 & 78.857 & 77.025 & 0.356 & 5.903 \\ 
o-Ac2BBP & 1.525 & 131 & 132 & 1.886 & 2.780 & 2.749 & 3.313 & 3.294 & 2.248 & 2.261 & 0.362 & 0.374 & 0.894 & 0.862 & 1.065 & 1.033 & 374.224 & 376.383 & 551.550 & 548.426 & 0.259 & 0.286 & 177.326 & 172.044 & 0.226 & 5.920 \\ 
TPA-PyF2 & 2.556 & 185 & 186 & 2.781 & 3.522 & 3.499 & 4.025 & 3.992 & 3.178 & 3.172 & 0.397 & 0.392 & 0.742 & 0.718 & 0.848 & 0.820 & 308.020 & 310.597 & 390.183 & 390.845 & 0.335 & 0.079 & 82.163 & 80.248 & 0.175 & 6.576 \\ 
o-Px2BBP & 1.370 & 119 & 120 & 1.843 & 2.386 & 2.371 & 2.777 & 2.742 & 2.144 & 2.131 & 0.302 & 0.288 & 0.544 & 0.528 & 0.633 & 0.611 & 446.452 & 452.167 & 578.150 & 581.821 & 0.345 & 0.301 & 131.698 & 129.654 & 0.200 & 5.650 \\ 
D-BP-PXZ & 1.465 & 133 & 134 & 1.931 & 2.747 & 2.735 & 3.097 & 3.083 & 2.177 & 2.176 & 0.246 & 0.246 & 0.816 & 0.804 & 0.920 & 0.907 & 400.285 & 402.167 & 569.537 & 569.716 & 0.048 & 0.048 & 169.252 & 167.548 & 0.322 & 5.591 \\ 
BTD-PXZ & 1.007 & 55 & 56 & 1.802 & 2.607 & 2.588 & 2.876 & 2.850 & 1.988 & 1.985 & 0.186 & 0.183 & 0.805 & 0.786 & 0.888 & 0.866 & 431.099 & 434.956 & 623.565 & 624.630 & 0.140 & 0.120 & 192.466 & 189.674 & 0.348 & 5.309 \\ 
tBuCzDBA & 1.075 & 180 & 181 & 1.602 & 2.942 & 2.916 & 3.005 & 3.005 & 1.636 & 1.650 & 0.034 & 0.049 & 1.340 & 1.314 & 1.369 & 1.354 & 412.607 & 412.662 & 757.797 & 751.199 & 0.002 & 0.001 & 345.190 & 338.537 & 0.130 & 0.489 \\ 
5-Cz-Sac & 2.266 & 73 & 74 & 2.623 & 3.428 & 3.405 & 3.873 & 3.805 & 2.964 & 2.931 & 0.341 & 0.308 & 0.805 & 0.782 & 0.909 & 0.874 & 320.108 & 325.863 & 418.339 & 423.064 & 0.264 & 0.224 & 98.231 & 97.201 & 0.365 & 4.313 \\ 
6-Cz-Sac & 2.326 & 73 & 74 & 2.601 & 3.345 & 3.323 & 3.803 & 3.745 & 2.957 & 2.931 & 0.356 & 0.330 & 0.745 & 0.723 & 0.847 & 0.814 & 325.983 & 331.057 & 419.325 & 423.039 & 0.493 & 0.413 & 93.342 & 91.982 & 0.432 & 4.351 \\ 
DiCz-Sac & 2.166 & 103 & 104 & 2.452 & 3.361 & 3.340 & 3.690 & 3.656 & 2.692 & 2.684 & 0.240 & 0.232 & 0.909 & 0.888 & 0.998 & 0.972 & 335.991 & 339.144 & 460.500 & 461.916 & 0.175 & 0.152 & 124.509 & 122.773 & 0.432 & 3.927 \\ 
2CM & 2.748 & 135 & 136 & 2.748 & 3.041 & 3.015 & 3.565 & 3.473 & 3.221 & 3.165 & 0.474 & 0.417 & 0.293 & 0.268 & 0.344 & 0.308 & 347.743 & 356.974 & 384.881 & 391.733 & 0.087 & 0.066 & 37.138 & 34.759 & 0.039 & 5.546 \\ 
CzoB & 2.201 & 93 & 94 & 2.412 & 3.242 & 3.233 & 3.348 & 3.338 & 2.490 & 2.490 & 0.079 & 0.078 & 0.830 & 0.821 & 0.857 & 0.848 & 370.378 & 371.466 & 497.854 & 497.976 & 0.047 & 0.044 & 127.476 & 126.510 & 0.340 & 3.040 \\ 
CzBroB & 2.112 & 96 & 97 & 2.313 & 3.228 & 3.220 & 3.340 & 3.330 & 2.393 & 2.392 & 0.080 & 0.079 & 0.916 & 0.907 & 0.947 & 0.938 & 371.210 & 372.358 & 518.157 & 518.359 & 0.053 & 0.049 & 146.947 & 146.001 & 0.352 & 3.026 \\ 
PxCN & 1.222 & 113 & 114 & 1.961 & 2.880 & 2.850 & 3.263 & 3.228 & 2.222 & 2.221 & 0.261 & 0.260 & 0.920 & 0.889 & 1.042 & 1.007 & 379.923 & 384.042 & 558.090 & 558.246 & 0.004 & 0.003 & 178.167 & 174.203 & 0.179 & 2.573 \\ 
AcCN & 1.280 & 125 & 126 & 2.045 & 3.414 & 3.383 & 3.683 & 3.678 & 2.206 & 2.224 & 0.161 & 0.178 & 1.369 & 1.337 & 1.476 & 1.454 & 336.685 & 337.106 & 561.962 & 557.539 & 0.266 & 0.256 & 225.277 & 220.433 & 0.104 & 7.428 \\ 
CzCNoB & 1.859 & 97 & 98 & 2.125 & 2.997 & 2.990 & 3.116 & 3.104 & 2.209 & 2.206 & 0.084 & 0.081 & 0.872 & 0.865 & 0.907 & 0.898 & 397.895 & 399.408 & 561.243 & 561.947 & 0.050 & 0.046 & 163.347 & 162.540 & 0.338 & 3.306 \\ 
CNPP-TPA & 1.144 & 140 & 141 & 1.395 & 2.969 & 2.946 & 3.443 & 3.423 & 1.617 & 1.620 & 0.223 & 0.226 & 1.575 & 1.552 & 1.826 & 1.803 & 360.105 & 362.167 & 766.708 & 765.099 & 0.632 & 0.592 & 406.603 & 402.932 & 0.301 & 8.752 \\ 
SPAC-FO & 1.118 & 153 & 154 & 1.568 & 2.469 & 2.461 & 2.690 & 2.671 & 1.708 & 1.702 & 0.140 & 0.134 & 0.902 & 0.893 & 0.982 & 0.969 & 460.976 & 464.239 & 726.083 & 728.615 & 0.132 & 0.113 & 265.106 & 264.377 & 0.294 & 3.819 \\ 
DMAC-FO & 1.085 & 111 & 112 & 1.552 & 2.492 & 2.484 & 2.693 & 2.675 & 1.677 & 1.672 & 0.125 & 0.120 & 0.940 & 0.932 & 1.016 & 1.004 & 460.463 & 463.406 & 739.415 & 741.722 & 0.113 & 0.097 & 278.952 & 278.317 & 0.284 & 3.683 \\ 
6AcBIQ & 1.082 & 89 & 90 & 1.799 & 2.436 & 2.423 & 2.552 & 2.544 & 1.885 & 1.889 & 0.086 & 0.090 & 0.637 & 0.624 & 0.667 & 0.655 & 485.793 & 487.340 & 657.689 & 656.370 & 0.079 & 0.076 & 171.895 & 169.030 & 0.257 & 4.629 \\ 
PtB & 2.066 & 103 & 104 & 1.772 & 2.631 & 2.566 & 3.486 & 3.416 & 2.349 & 2.360 & 0.576 & 0.587 & 0.859 & 0.793 & 1.138 & 1.056 & 355.622 & 362.962 & 527.884 & 525.447 & 1.088 & 0.930 & 172.261 & 162.485 & 0.749 & 3.178 \\ 
BCPBT & 1.287 & 170 & 171 & 1.712 & 2.879 & 2.827 & 3.745 & 3.660 & 2.227 & 2.216 & 0.515 & 0.504 & 1.167 & 1.116 & 1.519 & 1.444 & 331.031 & 338.764 & 556.793 & 559.529 & 1.544 & 1.276 & 225.762 & 220.765 & 0.142 & 2.203 \\ 
InDM & 2.820 & 78 & 79 & 2.511 & 3.371 & 3.350 & 3.999 & 3.916 & 2.979 & 2.934 & 0.468 & 0.424 & 0.860 & 0.840 & 1.020 & 0.982 & 310.007 & 316.634 & 416.207 & 422.556 & 0.054 & 0.046 & 106.200 & 105.923 & 0.633 & 1.694 \\ 
PnB & 2.044 & 103 & 104 & 1.812 & 2.678 & 2.612 & 3.536 & 3.474 & 2.393 & 2.410 & 0.581 & 0.598 & 0.865 & 0.800 & 1.143 & 1.064 & 350.614 & 356.881 & 518.020 & 514.403 & 0.732 & 0.654 & 167.406 & 157.521 & 0.586 & 4.638 \\ 
BANE & 2.131 & 121 & 122 & 1.694 & 2.257 & 2.186 & 3.183 & 3.068 & 2.389 & 2.378 & 0.695 & 0.684 & 0.564 & 0.492 & 0.795 & 0.691 & 389.459 & 404.081 & 519.044 & 521.428 & 1.062 & 0.816 & 129.586 & 117.347 & 0.922 & 0.014 \\ 
CBM & 1.977 & 69 & 70 & 1.918 & 2.613 & 2.567 & 3.344 & 3.286 & 2.455 & 2.455 & 0.537 & 0.537 & 0.694 & 0.649 & 0.889 & 0.831 & 370.777 & 377.287 & 504.970 & 504.927 & 1.199 & 1.026 & 134.192 & 127.639 & 0.627 & 1.838 \\ 
DCzBNPh-1 & 2.117 & 111 & 112 & 2.368 & 3.456 & 3.435 & 3.830 & 3.780 & 2.625 & 2.606 & 0.256 & 0.238 & 1.088 & 1.067 & 1.205 & 1.174 & 323.710 & 328.001 & 472.359 & 475.711 & 0.100 & 0.080 & 148.649 & 147.711 & 0.317 & 3.717 \\ 
MCZ-P2-DTM & 1.878 & 120 & 121 & 2.139 & 3.268 & 3.248 & 3.680 & 3.641 & 2.409 & 2.398 & 0.270 & 0.259 & 1.129 & 1.109 & 1.271 & 1.243 & 336.923 & 340.513 & 514.709 & 517.074 & 1.072 & 0.936 & 177.786 & 176.561 & 0.341 & 7.423 \\ 
DBTO-PTZ & 1.595 & 103 & 104 & 2.086 & 2.894 & 2.863 & 3.279 & 3.244 & 2.363 & 2.362 & 0.278 & 0.277 & 0.808 & 0.778 & 0.916 & 0.881 & 378.116 & 382.254 & 524.683 & 524.817 & 0.013 & 0.010 & 146.567 & 142.562 & 0.327 & 3.025 \\ 
$\alpha$-DMAC-DBP & 1.060 & 90 & 91 & 1.083 & 2.440 & 2.429 & 2.557 & 2.547 & 1.135 & 1.135 & 0.052 & 0.053 & 1.357 & 1.347 & 1.422 & 1.412 & 484.863 & 486.728 & 1092.414 & 1092.032 & 0.060 & 0.055 & 607.552 & 605.304 & 0.408 & 3.298 \\ 
$\alpha$-2DMAC-DBP & 0.955 & 129 & 130 & 0.997 & 2.324 & 2.312 & 2.452 & 2.442 & 1.053 & 1.054 & 0.055 & 0.056 & 1.326 & 1.314 & 1.400 & 1.388 & 505.563 & 507.778 & 1177.940 & 1176.840 & 0.099 & 0.092 & 672.377 & 669.062 & 0.437 & 1.713 \\ 
$\beta$-DI-DBP & 1.315 & 141 & 142 & 1.183 & 3.014 & 2.984 & 3.287 & 3.284 & 1.290 & 1.302 & 0.107 & 0.119 & 1.831 & 1.801 & 1.997 & 1.983 & 377.230 & 377.483 & 961.356 & 952.329 & 0.016 & 0.021 & 584.126 & 574.846 & 0.563 & 0.151 \\ 
DIC-TRZ & 1.883 & 103 & 104 & 2.135 & 3.054 & 3.031 & 3.515 & 3.455 & 2.457 & 2.433 & 0.322 & 0.299 & 0.919 & 0.896 & 1.058 & 1.022 & 352.709 & 358.823 & 504.592 & 509.507 & 0.309 & 0.262 & 151.883 & 150.684 & 0.197 & 4.546 \\ 
PO-TPA & 0.520 & 193 & 194 & 0.482 & 1.499 & 1.453 & 2.100 & 2.021 & 0.675 & 0.670 & 0.193 & 0.188 & 1.017 & 0.971 & 1.425 & 1.350 & 590.401 & 613.601 & 1835.581 & 1849.538 & 0.582 & 0.450 & 1245.180 & 1235.938 & 0.395 & 7.135 \\ 
DMAC-Cz-TTR & 1.170 & 154 & 155 & 2.208 & 3.387 & 3.355 & 3.803 & 3.739 & 2.479 & 2.461 & 0.271 & 0.253 & 1.179 & 1.147 & 1.323 & 1.278 & 326.051 & 331.562 & 500.095 & 503.788 & 0.350 & 0.305 & 174.044 & 172.226 & 0.038 & 9.906 \\ 
DCzPO & 2.608 & 121 & 122 & 2.796 & 3.391 & 3.368 & 3.890 & 3.826 & 3.208 & 3.176 & 0.412 & 0.380 & 0.595 & 0.573 & 0.683 & 0.650 & 318.693 & 324.015 & 386.539 & 390.374 & 0.368 & 0.045 & 67.846 & 66.360 & 0.296 & 1.117 \\ 
IQ-oTPA & 1.030 & 132 & 133 & 1.064 & 2.801 & 2.800 & 2.799 & 2.799 & 1.063 & 1.064 & -0.000 & -0.000 & 1.737 & 1.736 & 1.736 & 1.735 & 442.911 & 442.959 & 1165.813 & 1165.771 & 0.002 & 0.002 & 722.902 & 722.813 & 0.140 & 10.134 \\ 
2C & 1.460 & 67 & 68 & 1.676 & 2.682 & 2.614 & 3.542 & 3.473 & 2.214 & 2.228 & 0.538 & 0.551 & 1.005 & 0.937 & 1.327 & 1.245 & 350.080 & 356.984 & 559.975 & 556.561 & 1.288 & 1.104 & 209.896 & 199.577 & 0.338 & 7.176 \\ 
C-H & 1.509 & 70 & 71 & 1.714 & 2.688 & 2.620 & 3.596 & 3.522 & 2.292 & 2.304 & 0.579 & 0.590 & 0.975 & 0.906 & 1.304 & 1.218 & 344.784 & 351.988 & 540.890 & 538.102 & 1.046 & 0.907 & 196.106 & 186.114 & 0.309 & 7.359 \\ 
PSPP & 1.897 & 71 & 72 & 2.411 & 2.750 & 2.718 & 3.115 & 3.073 & 2.730 & 2.726 & 0.319 & 0.315 & 0.339 & 0.307 & 0.384 & 0.348 & 398.087 & 403.424 & 454.092 & 454.858 & 0.015 & 0.012 & 56.005 & 51.434 & 0.144 & 5.405 \\ 
2DN & 0.954 & 146 & 147 & 1.507 & 2.527 & 2.510 & 2.682 & 2.671 & 1.599 & 1.603 & 0.092 & 0.097 & 1.021 & 1.003 & 1.083 & 1.068 & 462.334 & 464.221 & 775.601 & 773.436 & 0.098 & 0.090 & 313.267 & 309.215 & 0.282 & 3.120 \\ 
PSPBP & 1.715 & 104 & 105 & 2.250 & 2.852 & 2.821 & 3.224 & 3.188 & 2.545 & 2.543 & 0.294 & 0.293 & 0.601 & 0.571 & 0.680 & 0.645 & 384.554 & 388.921 & 487.251 & 487.513 & 0.021 & 0.017 & 102.697 & 98.592 & 0.176 & 5.251 \\ 
2PN & 0.872 & 134 & 135 & 1.374 & 2.007 & 1.995 & 2.201 & 2.182 & 1.506 & 1.503 & 0.132 & 0.128 & 0.633 & 0.621 & 0.694 & 0.679 & 563.360 & 568.214 & 823.016 & 825.145 & 0.093 & 0.067 & 259.656 & 256.931 & 0.332 & 3.836 \\ 
pCbz-PYR & 2.606 & 131 & 132 & 2.577 & 3.496 & 3.476 & 3.872 & 3.840 & 2.854 & 2.847 & 0.277 & 0.269 & 0.919 & 0.899 & 1.018 & 0.993 & 320.199 & 322.918 & 434.361 & 435.506 & 1.041 & 0.930 & 114.162 & 112.588 & 0.510 & 1.453 \\ 
PPI-An-NPIM & 1.973 & 168 & 169 & 1.704 & 2.284 & 2.216 & 3.310 & 3.160 & 2.471 & 2.430 & 0.766 & 0.726 & 0.579 & 0.512 & 0.840 & 0.730 & 374.552 & 392.293 & 501.821 & 510.123 & 0.874 & 0.620 & 127.269 & 117.830 & 0.198 & 8.441 \\ 
2PS-2FPh & 2.068 & 87 & 88 & 2.260 & 2.878 & 2.849 & 3.225 & 3.184 & 2.533 & 2.525 & 0.273 & 0.265 & 0.618 & 0.590 & 0.693 & 0.659 & 384.399 & 389.434 & 489.538 & 491.056 & 0.032 & 0.027 & 105.138 & 101.621 & 0.091 & 6.640 \\ 
9CzTPE & 2.145 & 111 & 112 & 1.617 & 2.868 & 2.820 & 3.549 & 3.513 & 2.001 & 2.014 & 0.384 & 0.397 & 1.251 & 1.203 & 1.548 & 1.499 & 349.369 & 352.930 & 619.671 & 615.640 & 2.185 & 1.938 & 270.302 & 262.710 & 0.726 & 4.033 \\ 
2CzTPE & 2.224 & 117 & 118 & 1.618 & 2.881 & 2.833 & 3.598 & 3.559 & 2.020 & 2.032 & 0.403 & 0.414 & 1.263 & 1.216 & 1.578 & 1.527 & 344.573 & 348.358 & 613.646 & 610.095 & 2.396 & 2.096 & 269.073 & 261.737 & 0.895 & 0.108 \\ 
FTAT-FBO & 3.562 & 94 & 95 & 3.094 & 5.190 & 5.149 & 5.207 & 5.179 & 3.105 & 3.112 & 0.011 & 0.018 & 2.095 & 2.054 & 2.103 & 2.066 & 238.088 & 239.407 & 399.313 & 398.354 & 0.000 & 0.000 & 161.226 & 158.947 & 0.572 & 2.165 \\ 
DmPy-PPI & 2.623 & 138 & 139 & 2.337 & 3.446 & 3.419 & 3.853 & 3.813 & 2.612 & 2.606 & 0.276 & 0.269 & 1.110 & 1.082 & 1.241 & 1.207 & 321.786 & 325.136 & 474.592 & 475.721 & 0.558 & 0.505 & 152.806 & 150.584 & 0.677 & 3.999 \\ 
mCP-BmPy & 2.733 & 171 & 172 & 2.760 & 3.425 & 3.402 & 3.887 & 3.828 & 3.132 & 3.105 & 0.372 & 0.346 & 0.666 & 0.643 & 0.755 & 0.723 & 318.955 & 323.862 & 395.898 & 399.266 & 0.340 & 0.277 & 76.943 & 75.404 & 0.112 & 7.044 \\ 
mCP-Py & 3.025 & 143 & 144 & 2.826 & 3.421 & 3.398 & 3.897 & 3.837 & 3.219 & 3.191 & 0.393 & 0.365 & 0.595 & 0.572 & 0.678 & 0.646 & 318.169 & 323.145 & 385.151 & 388.544 & 0.308 & 0.215 & 66.981 & 65.399 & 0.563 & 3.265 \\ 
mCP-Ph & 3.038 & 143 & 144 & 2.833 & 3.427 & 3.405 & 3.839 & 3.780 & 3.174 & 3.145 & 0.341 & 0.312 & 0.594 & 0.572 & 0.665 & 0.635 & 322.934 & 328.009 & 390.634 & 394.272 & 0.322 & 0.276 & 67.699 & 66.262 & 0.543 & 3.905 \\ 
DMTAC & 2.041 & 116 & 117 & 1.824 & 2.403 & 2.352 & 3.066 & 2.994 & 2.327 & 2.322 & 0.503 & 0.499 & 0.580 & 0.528 & 0.740 & 0.672 & 404.371 & 414.054 & 532.899 & 533.943 & 0.264 & 0.238 & 128.528 & 119.889 & 0.754 & 1.486 \\ 
IPTAC & 2.048 & 128 & 129 & 1.823 & 2.402 & 2.351 & 3.071 & 2.998 & 2.330 & 2.325 & 0.508 & 0.502 & 0.579 & 0.528 & 0.740 & 0.674 & 403.778 & 413.515 & 532.079 & 533.338 & 0.275 & 0.249 & 128.300 & 119.823 & 0.762 & 1.379 \\ 
TBTAC & 2.057 & 134 & 135 & 1.833 & 2.405 & 2.354 & 3.078 & 3.006 & 2.346 & 2.341 & 0.513 & 0.508 & 0.572 & 0.521 & 0.732 & 0.665 & 402.860 & 412.469 & 528.550 & 529.637 & 0.274 & 0.252 & 125.690 & 117.167 & 0.768 & 1.336 \\ 
p2Cz2Trz & 1.647 & 159 & 160 & 1.573 & 3.057 & 3.046 & 3.258 & 3.235 & 1.677 & 1.671 & 0.103 & 0.097 & 1.483 & 1.473 & 1.581 & 1.564 & 380.600 & 383.294 & 739.407 & 742.059 & 0.147 & 0.130 & 358.807 & 358.765 & 0.365 & 0.028 \\ 
m2Cz2Trz & 1.930 & 159 & 160 & 1.903 & 3.216 & 3.202 & 3.472 & 3.451 & 2.055 & 2.052 & 0.151 & 0.148 & 1.313 & 1.298 & 1.417 & 1.400 & 357.087 & 359.218 & 603.347 & 604.231 & 0.210 & 0.193 & 246.260 & 245.012 & 0.490 & 2.439 \\ 
2,4-CzPyCl3 & 2.439 & 84 & 85 & 2.527 & 3.467 & 3.446 & 3.849 & 3.804 & 2.805 & 2.789 & 0.278 & 0.262 & 0.940 & 0.919 & 1.043 & 1.014 & 322.162 & 325.948 & 441.978 & 444.489 & 0.616 & 0.525 & 119.815 & 118.540 & 0.494 & 1.947 \\ 
DMAC-PCN & 1.073 & 104 & 105 & 1.996 & 3.417 & 3.385 & 3.646 & 3.640 & 2.130 & 2.147 & 0.134 & 0.150 & 1.421 & 1.389 & 1.516 & 1.494 & 340.018 & 340.597 & 582.028 & 577.611 & 0.215 & 0.203 & 242.010 & 237.013 & 0.045 & 8.124 \\ 
2PXZP & 1.413 & 119 & 120 & 1.777 & 2.741 & 2.709 & 3.076 & 3.060 & 1.995 & 2.007 & 0.218 & 0.230 & 0.963 & 0.932 & 1.081 & 1.053 & 403.043 & 405.151 & 621.489 & 617.626 & 0.455 & 0.419 & 218.445 & 212.475 & 0.273 & 6.593 \\ 
2,4,6-CzPyCl2 & 2.532 & 111 & 112 & 2.466 & 3.453 & 3.427 & 3.849 & 3.801 & 2.749 & 2.735 & 0.283 & 0.269 & 0.987 & 0.961 & 1.100 & 1.066 & 322.162 & 326.171 & 451.036 & 453.263 & 0.565 & 0.476 & 128.874 & 127.092 & 0.467 & 1.926 \\ 
1PXZP & 1.424 & 72 & 73 & 1.905 & 2.742 & 2.709 & 2.979 & 2.960 & 2.071 & 2.082 & 0.165 & 0.176 & 0.836 & 0.804 & 0.909 & 0.879 & 416.138 & 418.823 & 598.795 & 595.602 & 0.373 & 0.335 & 182.656 & 176.779 & 0.290 & 6.445 \\ 
3,6-T2C & 1.452 & 166 & 167 & 1.958 & 3.309 & 3.282 & 3.748 & 3.716 & 2.218 & 2.217 & 0.260 & 0.259 & 1.351 & 1.324 & 1.531 & 1.499 & 330.774 & 333.659 & 559.085 & 559.358 & 1.276 & 1.106 & 228.310 & 225.699 & 0.111 & 13.279 \\ 
3,6-TC & 1.710 & 162 & 163 & 2.064 & 3.311 & 3.284 & 3.743 & 3.708 & 2.333 & 2.330 & 0.270 & 0.267 & 1.247 & 1.220 & 1.410 & 1.378 & 331.243 & 334.342 & 531.431 & 532.046 & 1.232 & 1.065 & 200.188 & 197.703 & 0.171 & 12.613 \\ 
Ph-CF3 & 2.892 & 92 & 93 & 2.723 & 3.392 & 3.362 & 3.847 & 3.801 & 3.088 & 3.079 & 0.365 & 0.356 & 0.669 & 0.639 & 0.758 & 0.722 & 322.322 & 326.188 & 401.463 & 402.685 & 1.170 & 0.930 & 79.141 & 76.497 & 0.696 & 0.238 \\ 
arylene & 2.892 & 92 & 93 & 2.723 & 3.392 & 3.362 & 3.848 & 3.802 & 3.089 & 3.080 & 0.366 & 0.357 & 0.669 & 0.639 & 0.759 & 0.722 & 322.213 & 326.085 & 401.331 & 402.563 & 1.183 & 0.940 & 79.119 & 76.477 & 0.696 & 0.226 \\ 
TS-1 & 2.766 & 68 & 69 & 2.971 & 3.407 & 3.384 & 3.861 & 3.788 & 3.367 & 3.325 & 0.396 & 0.354 & 0.436 & 0.413 & 0.495 & 0.463 & 321.103 & 327.325 & 368.278 & 372.869 & 0.224 & 0.193 & 47.175 & 45.544 & 0.391 & 4.871 \\ 
3,6-MeCzOXD & 1.840 & 113 & 114 & 2.229 & 3.422 & 3.400 & 3.709 & 3.689 & 2.416 & 2.419 & 0.187 & 0.190 & 1.193 & 1.171 & 1.293 & 1.270 & 334.261 & 336.055 & 513.104 & 512.541 & 0.306 & 0.281 & 178.842 & 176.486 & 0.255 & 4.950 \\ 
p-PO15NCzDPA & 2.111 & 125 & 126 & 1.718 & 2.257 & 2.187 & 3.207 & 3.047 & 2.440 & 2.393 & 0.722 & 0.675 & 0.540 & 0.469 & 0.767 & 0.654 & 386.617 & 406.919 & 508.099 & 518.102 & 0.675 & 0.490 & 121.482 & 111.183 & 0.927 & 0.217 \\ 
2,7-MeCzOXD & 1.955 & 113 & 114 & 2.210 & 3.491 & 3.474 & 3.732 & 3.717 & 2.363 & 2.365 & 0.153 & 0.155 & 1.281 & 1.263 & 1.369 & 1.352 & 332.192 & 333.551 & 524.716 & 524.220 & 0.110 & 0.105 & 192.523 & 190.669 & 0.296 & 3.935 \\ 
BPCN-Cz2Ph & 2.157 & 91 & 92 & 2.535 & 3.452 & 3.430 & 3.866 & 3.805 & 2.840 & 2.813 & 0.304 & 0.277 & 0.916 & 0.894 & 1.026 & 0.992 & 320.704 & 325.845 & 436.620 & 440.805 & 0.149 & 0.126 & 115.915 & 114.959 & 0.240 & 7.367 \\ 
o-CzOXD & 2.009 & 101 & 102 & 2.252 & 3.415 & 3.391 & 3.756 & 3.730 & 2.478 & 2.477 & 0.225 & 0.225 & 1.162 & 1.139 & 1.278 & 1.252 & 330.061 & 332.424 & 500.349 & 500.492 & 0.320 & 0.266 & 170.288 & 168.068 & 0.262 & 4.647 \\ 
BPCN-2Cz & 2.032 & 107 & 108 & 2.519 & 3.381 & 3.359 & 3.859 & 3.792 & 2.875 & 2.843 & 0.356 & 0.324 & 0.862 & 0.840 & 0.984 & 0.948 & 321.302 & 327.006 & 431.258 & 436.044 & 0.198 & 0.162 & 109.955 & 109.038 & 0.172 & 10.454 \\ 
Cbz-MI & 1.096 & 152 & 153 & 1.393 & 2.124 & 2.093 & 2.618 & 2.571 & 1.718 & 1.711 & 0.324 & 0.318 & 0.730 & 0.700 & 0.901 & 0.860 & 473.529 & 482.166 & 721.788 & 724.432 & 0.245 & 0.213 & 248.259 & 242.266 & 0.186 & 8.291 \\ 
DBFDPO & 3.428 & 99 & 100 & 3.090 & 4.038 & 4.001 & 4.325 & 4.275 & 3.310 & 3.301 & 0.220 & 0.211 & 0.948 & 0.911 & 1.015 & 0.973 & 286.695 & 290.042 & 374.624 & 375.571 & 0.044 & 0.042 & 87.929 & 85.530 & 0.212 & 3.852 \\ 
XCBP & 1.998 & 84 & 85 & 2.378 & 3.399 & 3.375 & 3.860 & 3.789 & 2.700 & 2.669 & 0.322 & 0.292 & 1.022 & 0.997 & 1.160 & 1.119 & 321.228 & 327.247 & 459.248 & 464.482 & 0.201 & 0.166 & 138.020 & 137.234 & 0.105 & 10.336 \\ 
Cbz-PYR & 2.800 & 75 & 76 & 2.679 & 3.515 & 3.493 & 3.882 & 3.840 & 2.959 & 2.945 & 0.280 & 0.266 & 0.836 & 0.814 & 0.924 & 0.895 & 319.341 & 322.901 & 419.041 & 421.024 & 0.738 & 0.640 & 99.700 & 98.124 & 0.501 & 0.910 \\ 
tCbz-mPYRs & 2.585 & 132 & 133 & 2.619 & 3.433 & 3.412 & 3.825 & 3.782 & 2.918 & 2.903 & 0.299 & 0.284 & 0.815 & 0.793 & 0.908 & 0.879 & 324.099 & 327.792 & 424.902 & 427.053 & 0.638 & 0.552 & 100.803 & 99.260 & 0.445 & 2.977 \\ 
PCBP & 2.040 & 78 & 79 & 2.318 & 3.414 & 3.390 & 3.871 & 3.804 & 2.628 & 2.601 & 0.310 & 0.283 & 1.096 & 1.072 & 1.243 & 1.203 & 320.306 & 325.897 & 471.739 & 476.668 & 0.397 & 0.314 & 151.432 & 150.771 & 0.214 & 9.534 \\ 
MeCZ-TRZ & 1.934 & 165 & 166 & 2.031 & 3.501 & 3.479 & 3.937 & 3.885 & 2.284 & 2.268 & 0.253 & 0.237 & 1.470 & 1.448 & 1.653 & 1.617 & 314.912 & 319.136 & 542.851 & 546.581 & 0.512 & 0.343 & 227.939 & 227.445 & 0.183 & 6.503 \\ 
3ca & 2.160 & 80 & 81 & 1.849 & 2.679 & 2.630 & 3.513 & 3.425 & 2.425 & 2.408 & 0.576 & 0.559 & 0.830 & 0.781 & 1.088 & 1.016 & 352.910 & 362.040 & 511.279 & 514.854 & 1.454 & 1.161 & 158.369 & 152.815 & 0.812 & 0.289 \\ 
2MeCZ-TRZ & 1.877 & 174 & 175 & 2.012 & 3.489 & 3.466 & 3.909 & 3.860 & 2.254 & 2.240 & 0.242 & 0.228 & 1.478 & 1.455 & 1.655 & 1.620 & 317.176 & 321.219 & 550.159 & 553.547 & 0.620 & 0.471 & 232.983 & 232.328 & 0.161 & 7.500 \\ 
CZ-TRZ & 2.003 & 156 & 157 & 2.052 & 3.520 & 3.498 & 3.941 & 3.890 & 2.297 & 2.282 & 0.245 & 0.230 & 1.468 & 1.446 & 1.644 & 1.608 & 314.601 & 318.742 & 539.696 & 543.289 & 0.579 & 0.454 & 225.095 & 224.547 & 0.158 & 7.313 \\ 
DMAC-AQ & 1.457 & 77 & 78 & 1.358 & 1.782 & 1.744 & 2.355 & 2.269 & 1.794 & 1.767 & 0.436 & 0.409 & 0.424 & 0.386 & 0.561 & 0.502 & 526.539 & 546.403 & 691.152 & 701.772 & 0.314 & 0.247 & 164.613 & 155.369 & 0.477 & 4.253 \\ 
DTPTCzDP-CN & 1.294 & 149 & 150 & 1.810 & 2.844 & 2.825 & 3.259 & 3.200 & 2.075 & 2.051 & 0.264 & 0.240 & 1.033 & 1.015 & 1.184 & 1.149 & 380.483 & 387.475 & 597.644 & 604.645 & 0.588 & 0.421 & 217.161 & 217.170 & 0.303 & 7.743 \\ 
mP2MPC & 2.687 & 132 & 133 & 2.468 & 3.419 & 3.391 & 3.812 & 3.767 & 2.752 & 2.742 & 0.284 & 0.274 & 0.951 & 0.923 & 1.060 & 1.025 & 325.247 & 329.115 & 450.563 & 452.147 & 0.306 & 0.261 & 125.315 & 123.032 & 0.045 & 12.456 \\ 
XPhos & 2.871 & 94 & 95 & 2.073 & 3.024 & 2.974 & 4.170 & 4.037 & 2.859 & 2.814 & 0.786 & 0.741 & 0.951 & 0.901 & 1.311 & 1.223 & 297.296 & 307.097 & 433.604 & 440.552 & 0.593 & 0.449 & 136.308 & 133.455 & 0.710 & 1.353 \\ 
TPXZ-as-TAZ & 1.265 & 156 & 157 & 1.300 & 2.826 & 2.815 & 3.033 & 3.025 & 1.395 & 1.397 & 0.095 & 0.097 & 1.526 & 1.516 & 1.638 & 1.628 & 408.730 & 409.879 & 888.711 & 887.803 & 0.439 & 0.478 & 479.981 & 477.924 & 0.118 & 3.127 \\ 
2Trz6CNDBT & 2.226 & 77 & 78 & 2.158 & 3.568 & 3.549 & 3.909 & 3.860 & 2.365 & 2.347 & 0.207 & 0.189 & 1.410 & 1.391 & 1.545 & 1.513 & 317.152 & 321.219 & 524.334 & 528.290 & 0.155 & 0.142 & 207.182 & 207.071 & 0.443 & 2.470 \\ 
TPAPyPI & 1.868 & 149 & 150 & 1.930 & 2.736 & 2.668 & 3.688 & 3.600 & 2.602 & 2.605 & 0.672 & 0.674 & 0.806 & 0.738 & 1.086 & 0.995 & 336.174 & 344.391 & 476.483 & 475.998 & 0.011 & 0.180 & 140.309 & 131.607 & 0.026 & 7.494 \\ 
TPACzPI & 2.503 & 157 & 158 & 2.247 & 3.380 & 3.358 & 3.785 & 3.720 & 2.516 & 2.489 & 0.269 & 0.242 & 1.133 & 1.111 & 1.269 & 1.231 & 327.533 & 333.273 & 492.739 & 498.111 & 0.082 & 0.071 & 165.206 & 164.838 & 0.520 & 6.743 \\ 
NA-TNA & 1.261 & 121 & 122 & 1.508 & 2.477 & 2.425 & 3.141 & 3.090 & 1.912 & 1.922 & 0.404 & 0.414 & 0.969 & 0.917 & 1.229 & 1.169 & 394.691 & 401.217 & 648.418 & 645.223 & 2.199 & 1.927 & 253.727 & 244.006 & 0.294 & 10.456 \\ 
CzPrSBI & 1.762 & 70 & 71 & 2.287 & 3.391 & 3.366 & 3.883 & 3.807 & 2.619 & 2.586 & 0.332 & 0.299 & 1.104 & 1.079 & 1.264 & 1.220 & 319.316 & 325.717 & 473.479 & 479.367 & 0.053 & 0.044 & 154.163 & 153.650 & 0.137 & 3.363 \\ 
m-CzCNDMT & 3.060 & 117 & 118 & 2.843 & 3.529 & 3.506 & 3.941 & 3.887 & 3.176 & 3.152 & 0.332 & 0.309 & 0.685 & 0.663 & 0.766 & 0.735 & 314.577 & 318.947 & 390.416 & 393.326 & 0.094 & 0.084 & 75.839 & 74.380 & 0.364 & 7.614 \\ 
DTXO-TPA2 & 2.310 & 115 & 116 & 2.293 & 2.783 & 2.750 & 3.295 & 3.258 & 2.715 & 2.717 & 0.421 & 0.423 & 0.490 & 0.457 & 0.580 & 0.541 & 376.314 & 380.541 & 456.693 & 456.380 & 0.398 & 0.345 & 80.378 & 75.839 & 0.361 & 7.421 \\ 
24PQ-Cz & 1.798 & 112 & 113 & 1.737 & 3.307 & 3.269 & 3.788 & 3.769 & 1.990 & 2.003 & 0.253 & 0.266 & 1.570 & 1.532 & 1.798 & 1.766 & 327.299 & 328.967 & 623.083 & 619.043 & 0.052 & 0.463 & 295.784 & 290.076 & 0.473 & 1.902 \\ 
SFPC & 1.706 & 101 & 102 & 2.273 & 2.918 & 2.891 & 3.257 & 3.220 & 2.537 & 2.532 & 0.263 & 0.258 & 0.645 & 0.618 & 0.720 & 0.688 & 380.717 & 385.080 & 488.723 & 489.733 & 0.040 & 0.033 & 108.006 & 104.653 & 0.191 & 5.248 \\ 
2CzMC & 2.707 & 63 & 64 & 2.628 & 3.204 & 3.167 & 3.770 & 3.708 & 3.092 & 3.077 & 0.464 & 0.449 & 0.576 & 0.539 & 0.678 & 0.631 & 328.897 & 334.406 & 401.034 & 402.942 & 0.135 & 0.122 & 72.138 & 68.536 & 0.601 & 3.094 \\ 
PPI-PIM-2 & 2.033 & 148 & 149 & 2.211 & 3.405 & 3.378 & 3.846 & 3.806 & 2.498 & 2.492 & 0.286 & 0.281 & 1.193 & 1.166 & 1.348 & 1.314 & 322.380 & 325.734 & 496.361 & 497.519 & 0.704 & 0.624 & 173.981 & 171.785 & 0.084 & 11.791 \\ 
4CzMC & 2.757 & 63 & 64 & 2.675 & 3.239 & 3.206 & 3.770 & 3.714 & 3.114 & 3.099 & 0.438 & 0.424 & 0.564 & 0.531 & 0.656 & 0.615 & 328.897 & 333.838 & 398.196 & 400.048 & 0.381 & 0.347 & 69.299 & 66.210 & 0.636 & 2.391 \\ 
PPI-PIM-1 & 2.132 & 148 & 149 & 2.146 & 3.445 & 3.417 & 3.870 & 3.833 & 2.412 & 2.407 & 0.265 & 0.261 & 1.298 & 1.271 & 1.459 & 1.425 & 320.339 & 323.499 & 514.098 & 515.054 & 0.854 & 0.746 & 193.759 & 191.555 & 0.201 & 11.312 \\ 
CzTPA & 2.991 & 76 & 77 & 2.980 & 3.363 & 3.340 & 3.795 & 3.750 & 3.362 & 3.345 & 0.383 & 0.365 & 0.383 & 0.360 & 0.432 & 0.404 & 326.721 & 330.651 & 368.726 & 370.620 & 0.150 & 0.109 & 42.005 & 39.969 & 0.408 & 3.086 \\ 
SFX-bPy & 2.301 & 84 & 85 & 2.235 & 3.469 & 3.425 & 4.067 & 4.018 & 2.621 & 2.622 & 0.386 & 0.387 & 1.233 & 1.190 & 1.446 & 1.395 & 304.832 & 308.580 & 472.989 & 472.786 & 0.581 & 0.526 & 168.157 & 164.206 & 0.461 & 0.608 \\ 
t–BuCz2BP & 1.972 & 142 & 143 & 2.200 & 3.241 & 3.221 & 3.737 & 3.701 & 2.537 & 2.527 & 0.337 & 0.328 & 1.041 & 1.021 & 1.201 & 1.173 & 331.766 & 335.020 & 488.791 & 490.554 & 1.121 & 0.941 & 157.025 & 155.534 & 0.357 & 3.196 \\ 
SAF-2CzB & 2.264 & 211 & 212 & 2.263 & 3.453 & 3.431 & 3.878 & 3.828 & 2.542 & 2.524 & 0.279 & 0.262 & 1.190 & 1.168 & 1.336 & 1.303 & 319.712 & 323.913 & 487.828 & 491.147 & 1.223 & 0.962 & 168.117 & 167.234 & 0.172 & 3.458 \\ 
F-2CzB & 2.374 & 173 & 174 & 2.279 & 3.453 & 3.431 & 3.882 & 3.832 & 2.563 & 2.545 & 0.283 & 0.266 & 1.174 & 1.152 & 1.320 & 1.286 & 319.358 & 323.558 & 483.785 & 487.082 & 1.223 & 0.959 & 164.427 & 163.524 & 0.451 & 1.139 \\ 
SAF-CzB & 2.402 & 143 & 144 & 2.413 & 3.412 & 3.390 & 3.809 & 3.745 & 2.693 & 2.666 & 0.281 & 0.253 & 0.999 & 0.977 & 1.115 & 1.080 & 325.529 & 331.048 & 460.354 & 465.113 & 0.277 & 0.225 & 134.825 & 134.065 & 0.178 & 3.691 \\ 
BPy-TP2 & 2.175 & 98 & 99 & 2.105 & 3.578 & 3.539 & 3.880 & 3.853 & 2.282 & 2.291 & 0.178 & 0.187 & 1.474 & 1.434 & 1.598 & 1.561 & 319.514 & 321.820 & 543.202 & 541.067 & 0.000 & 0.000 & 223.688 & 219.247 & 0.502 & 0.757 \\ 
Cz–AQ & 1.246 & 68 & 69 & 1.489 & 2.390 & 2.373 & 2.735 & 2.697 & 1.703 & 1.692 & 0.215 & 0.203 & 0.902 & 0.885 & 1.032 & 1.005 & 453.324 & 459.626 & 727.924 & 732.733 & 0.267 & 0.231 & 274.600 & 273.106 & 0.356 & 5.621 \\ 
-ph-pCzAnBzt & 1.957 & 115 & 116 & 1.736 & 2.259 & 2.188 & 3.217 & 3.047 & 2.473 & 2.419 & 0.737 & 0.682 & 0.522 & 0.451 & 0.744 & 0.629 & 385.403 & 406.839 & 501.353 & 512.556 & 0.606 & 0.423 & 115.950 & 105.717 & 0.029 & 12.528 \\ 
PyI & 2.473 & 44 & 45 & 2.131 & 2.852 & 2.790 & 3.751 & 3.692 & 2.803 & 2.819 & 0.672 & 0.688 & 0.721 & 0.659 & 0.948 & 0.872 & 330.536 & 335.864 & 442.335 & 439.741 & 0.015 & 0.259 & 111.799 & 103.877 & 0.904 & 0.724 \\ 
DVCz-2CzCN & 2.150 & 231 & 232 & 2.567 & 3.484 & 3.461 & 3.874 & 3.815 & 2.853 & 2.829 & 0.287 & 0.262 & 0.918 & 0.895 & 1.020 & 0.986 & 320.067 & 325.008 & 434.520 & 438.291 & 0.260 & 0.192 & 114.453 & 113.282 & 0.034 & 6.521 \\ 
ATDBT & 2.082 & 107 & 108 & 1.723 & 2.291 & 2.221 & 3.291 & 3.127 & 2.475 & 2.425 & 0.752 & 0.703 & 0.568 & 0.498 & 0.817 & 0.702 & 376.691 & 396.534 & 501.011 & 511.241 & 0.643 & 0.441 & 124.319 & 114.707 & 0.702 & 4.212 \\ 
DPhBCz & 2.945 & 89 & 90 & 2.747 & 3.376 & 3.354 & 3.856 & 3.788 & 3.138 & 3.102 & 0.391 & 0.355 & 0.629 & 0.607 & 0.719 & 0.686 & 321.502 & 327.342 & 395.131 & 399.686 & 0.358 & 0.292 & 73.628 & 72.344 & 0.735 & 0.036 \\ 
AcHPM & 1.537 & 121 & 122 & 1.817 & 3.434 & 3.404 & 3.560 & 3.555 & 1.884 & 1.898 & 0.067 & 0.081 & 1.617 & 1.587 & 1.676 & 1.657 & 348.300 & 348.770 & 658.247 & 653.300 & 0.267 & 0.259 & 309.947 & 304.530 & 0.184 & 4.818 \\ 
PhCO-DMAC & 1.565 & 73 & 74 & 2.188 & 3.357 & 3.350 & 3.474 & 3.466 & 2.265 & 2.264 & 0.076 & 0.076 & 1.169 & 1.161 & 1.209 & 1.202 & 356.902 & 357.685 & 547.491 & 547.515 & 0.134 & 0.127 & 190.589 & 189.830 & 0.196 & 6.136 \\ 
Diphenylsulfane & 2.305 & 99 & 100 & 2.195 & 4.140 & 4.096 & 4.318 & 4.317 & 2.289 & 2.314 & 0.094 & 0.118 & 1.945 & 1.901 & 2.028 & 2.003 & 287.153 & 287.200 & 541.556 & 535.887 & 0.001 & 0.001 & 254.403 & 248.687 & 0.479 & 1.235 \\ 
2BrCPT & 2.189 & 93 & 94 & 2.093 & 3.380 & 3.357 & 3.815 & 3.747 & 2.363 & 2.336 & 0.270 & 0.243 & 1.287 & 1.264 & 1.453 & 1.411 & 324.974 & 330.880 & 524.800 & 530.749 & 0.490 & 0.392 & 199.826 & 199.869 & 0.465 & 2.130 \\ 
DCbz-Ph-Bz & 2.477 & 124 & 125 & 2.408 & 3.438 & 3.415 & 3.879 & 3.819 & 2.717 & 2.693 & 0.308 & 0.285 & 1.030 & 1.006 & 1.162 & 1.126 & 319.646 & 324.651 & 456.331 & 460.309 & 0.306 & 0.262 & 136.686 & 135.658 & 0.223 & 6.461 \\ 
DDPA-Ph-Bz & 2.275 & 126 & 127 & 2.380 & 3.461 & 3.430 & 3.844 & 3.816 & 2.643 & 2.647 & 0.263 & 0.268 & 1.081 & 1.051 & 1.201 & 1.169 & 322.565 & 324.889 & 469.139 & 468.342 & 0.050 & 0.052 & 146.574 & 143.452 & 0.233 & 6.528 \\ 
IDAC-MCO & 1.810 & 99 & 100 & 2.424 & 2.847 & 2.824 & 3.372 & 3.290 & 2.871 & 2.824 & 0.447 & 0.400 & 0.423 & 0.400 & 0.501 & 0.466 & 367.655 & 376.875 & 431.827 & 439.096 & 0.127 & 0.101 & 64.172 & 62.221 & 0.290 & 7.150 \\ 
diarylbiindole & 2.235 & 93 & 94 & 1.868 & 2.666 & 2.598 & 3.654 & 3.545 & 2.561 & 2.549 & 0.693 & 0.681 & 0.797 & 0.730 & 1.093 & 0.996 & 339.329 & 349.754 & 484.159 & 486.359 & 0.177 & 0.682 & 144.830 & 136.605 & 0.937 & 0.135 \\ 
CNDSB & 2.269 & 61 & 62 & 1.801 & 2.854 & 2.801 & 3.764 & 3.695 & 2.374 & 2.375 & 0.574 & 0.575 & 1.054 & 1.000 & 1.389 & 1.320 & 329.430 & 335.555 & 522.176 & 521.989 & 2.390 & 1.988 & 192.746 & 186.434 & 0.886 & 0.021 \\ 
TMAB & 1.975 & 162 & 163 & 2.552 & 3.558 & 3.536 & 3.983 & 3.974 & 2.857 & 2.868 & 0.305 & 0.316 & 1.006 & 0.984 & 1.126 & 1.106 & 311.268 & 312.020 & 433.958 & 432.353 & 0.054 & 0.047 & 122.690 & 120.333 & 0.090 & 7.103 \\ 
MOF & 2.911 & 127 & 128 & 3.076 & 4.237 & 4.207 & 4.703 & 4.657 & 3.414 & 3.406 & 0.338 & 0.330 & 1.161 & 1.131 & 1.289 & 1.252 & 263.611 & 266.215 & 363.111 & 364.058 & 0.025 & 0.024 & 99.500 & 97.843 & 0.056 & 6.259 \\ 
DICzTrz & 1.849 & 120 & 121 & 1.967 & 3.295 & 3.269 & 3.576 & 3.547 & 2.135 & 2.134 & 0.168 & 0.167 & 1.328 & 1.302 & 1.441 & 1.413 & 346.712 & 349.507 & 580.757 & 580.890 & 0.103 & 0.058 & 234.045 & 231.383 & 0.187 & 7.082 \\ 
PXZ2PTO & 2.394 & 87 & 88 & 2.545 & 2.734 & 2.702 & 3.098 & 3.059 & 2.884 & 2.881 & 0.338 & 0.336 & 0.189 & 0.157 & 0.214 & 0.178 & 400.246 & 405.336 & 429.960 & 430.363 & 0.015 & 0.012 & 29.714 & 25.027 & 0.339 & 4.242 \\ 
SPBP-DPAC & 2.295 & 124 & 125 & 2.226 & 2.778 & 2.747 & 3.397 & 3.336 & 2.722 & 2.704 & 0.496 & 0.477 & 0.551 & 0.521 & 0.674 & 0.633 & 365.035 & 371.622 & 455.459 & 458.603 & 0.857 & 0.728 & 90.424 & 86.981 & 0.486 & 4.235 \\ 
PX-TRZ & 1.901 & 94 & 95 & 2.046 & 3.731 & 3.700 & 4.173 & 4.125 & 2.288 & 2.281 & 0.242 & 0.235 & 1.686 & 1.654 & 1.885 & 1.844 & 297.075 & 300.546 & 541.865 & 543.509 & 0.031 & 0.013 & 244.790 & 242.963 & 0.256 & 6.575 \\ 
C2MPI & 3.028 & 120 & 121 & 2.835 & 3.565 & 3.541 & 4.098 & 4.058 & 3.259 & 3.248 & 0.424 & 0.413 & 0.730 & 0.707 & 0.839 & 0.810 & 302.526 & 305.568 & 380.443 & 381.747 & 0.185 & 0.157 & 77.918 & 76.179 & 0.379 & 1.937 \\ 
p-PCzTPD & 1.697 & 137 & 138 & 1.856 & 2.864 & 2.824 & 3.446 & 3.409 & 2.233 & 2.241 & 0.377 & 0.385 & 1.008 & 0.968 & 1.213 & 1.169 & 359.802 & 363.675 & 555.270 & 553.331 & 2.228 & 1.974 & 195.468 & 189.656 & 0.405 & 3.509 \\ 
m-PCzTPD & 1.508 & 137 & 138 & 1.968 & 3.041 & 3.004 & 3.666 & 3.618 & 2.373 & 2.371 & 0.405 & 0.403 & 1.072 & 1.035 & 1.293 & 1.247 & 338.182 & 342.706 & 522.414 & 522.927 & 0.519 & 0.518 & 184.233 & 180.221 & 0.164 & 5.791 \\ 
o-PCzTPD & 1.856 & 137 & 138 & 1.955 & 3.276 & 3.239 & 3.720 & 3.699 & 2.220 & 2.233 & 0.265 & 0.278 & 1.321 & 1.283 & 1.500 & 1.466 & 333.246 & 335.228 & 558.376 & 555.251 & 0.224 & 0.204 & 225.130 & 220.022 & 0.210 & 1.894 \\ 
CPBzFC & 1.748 & 80 & 81 & 1.986 & 3.198 & 3.160 & 3.760 & 3.722 & 2.335 & 2.340 & 0.349 & 0.354 & 1.211 & 1.173 & 1.424 & 1.382 & 329.789 & 333.112 & 530.920 & 529.880 & 0.720 & 0.915 & 201.131 & 196.768 & 0.278 & 7.296 \\ 
SiCz2Py2 & 2.614 & 148 & 149 & 2.760 & 3.413 & 3.390 & 3.835 & 3.770 & 3.101 & 3.069 & 0.341 & 0.310 & 0.653 & 0.630 & 0.734 & 0.701 & 323.330 & 328.871 & 399.837 & 403.971 & 0.276 & 0.237 & 76.507 & 75.101 & 0.134 & 8.121 \\ 
SiCz1Py3 & 2.616 & 132 & 133 & 2.710 & 3.391 & 3.368 & 3.822 & 3.752 & 3.055 & 3.019 & 0.345 & 0.309 & 0.681 & 0.658 & 0.768 & 0.733 & 324.379 & 330.431 & 405.905 & 410.661 & 0.208 & 0.177 & 81.526 & 80.230 & 0.107 & 8.381 \\ 
SiCz3Py1 & 2.630 & 164 & 165 & 2.694 & 3.425 & 3.402 & 3.844 & 3.781 & 3.024 & 2.994 & 0.330 & 0.300 & 0.730 & 0.708 & 0.820 & 0.787 & 322.506 & 327.905 & 409.936 & 414.061 & 0.281 & 0.242 & 87.430 & 86.156 & 0.089 & 9.710 \\ 
POBBPE & 3.422 & 90 & 91 & 3.115 & 4.463 & 4.444 & 4.906 & 4.858 & 3.424 & 3.405 & 0.309 & 0.290 & 1.348 & 1.329 & 1.482 & 1.453 & 252.720 & 255.206 & 362.080 & 364.119 & 0.019 & 0.018 & 109.361 & 108.913 & 0.409 & 3.657 \\ 
CzppT & 2.729 & 159 & 160 & 2.569 & 3.506 & 3.483 & 4.028 & 3.964 & 2.952 & 2.924 & 0.383 & 0.355 & 0.937 & 0.914 & 1.076 & 1.040 & 307.791 & 312.768 & 420.040 & 424.019 & 0.534 & 0.444 & 112.249 & 111.252 & 0.472 & 2.531 \\ 
SBDBQ-PXZ & 1.278 & 85 & 86 & 1.361 & 2.481 & 2.470 & 2.679 & 2.660 & 1.470 & 1.466 & 0.109 & 0.105 & 1.119 & 1.109 & 1.209 & 1.194 & 462.748 & 466.106 & 843.230 & 845.685 & 0.208 & 0.190 & 380.482 & 379.579 & 0.320 & 5.397 \\ 
DBQ-3PXZ & 1.123 & 151 & 152 & 1.350 & 2.461 & 2.451 & 2.653 & 2.635 & 1.456 & 1.451 & 0.106 & 0.101 & 1.111 & 1.101 & 1.198 & 1.184 & 467.265 & 470.493 & 851.679 & 854.181 & 0.228 & 0.210 & 384.414 & 383.689 & 0.135 & 7.935 \\ 
P4CzCN–BCz & 3.106 & 66 & 67 & 2.602 & 3.758 & 3.705 & 4.625 & 4.599 & 3.203 & 3.230 & 0.601 & 0.628 & 1.156 & 1.103 & 1.423 & 1.369 & 268.051 & 269.560 & 387.109 & 383.851 & 0.001 & 0.002 & 119.059 & 114.291 & 0.099 & 7.049 \\ 
NAP-1,5-DPA & 2.127 & 110 & 111 & 2.077 & 2.453 & 2.418 & 2.921 & 2.874 & 2.473 & 2.468 & 0.396 & 0.391 & 0.377 & 0.341 & 0.448 & 0.406 & 424.444 & 431.429 & 501.432 & 502.331 & 0.586 & 0.502 & 76.988 & 70.901 & 0.643 & 0.258 \\ 
3DPA3CN & 1.697 & 162 & 163 & 2.005 & 2.982 & 2.961 & 3.314 & 3.295 & 2.228 & 2.232 & 0.223 & 0.227 & 0.977 & 0.955 & 1.086 & 1.063 & 374.111 & 376.257 & 556.367 & 555.468 & 1.412 & 1.299 & 182.256 & 179.211 & 0.265 & 3.504 \\ 
TPA-AN-NA & 1.888 & 101 & 102 & 1.677 & 2.281 & 2.212 & 3.232 & 3.080 & 2.376 & 2.335 & 0.699 & 0.658 & 0.604 & 0.535 & 0.856 & 0.745 & 383.674 & 402.559 & 521.921 & 531.071 & 0.818 & 0.565 & 138.247 & 128.512 & 0.454 & 5.924 \\ 
OCzBN & 2.164 & 127 & 128 & 2.390 & 3.160 & 3.135 & 3.650 & 3.590 & 2.760 & 2.736 & 0.370 & 0.347 & 0.770 & 0.745 & 0.889 & 0.853 & 339.720 & 345.408 & 449.171 & 453.093 & 0.603 & 0.485 & 109.451 & 107.685 & 0.340 & 2.235 \\ 
BBCz & 3.035 & 47 & 48 & 2.824 & 3.332 & 3.297 & 3.809 & 3.759 & 3.228 & 3.220 & 0.405 & 0.396 & 0.508 & 0.473 & 0.581 & 0.539 & 325.461 & 329.824 & 384.047 & 385.085 & 0.001 & 0.001 & 58.587 & 55.260 & 0.730 & 0.737 \\ 
IQ-Se & 2.163 & 119 & 120 & 1.187 & 2.835 & 2.796 & 3.627 & 3.562 & 1.519 & 1.513 & 0.332 & 0.325 & 1.648 & 1.608 & 2.108 & 2.049 & 341.856 & 348.094 & 816.292 & 819.608 & 0.077 & 0.041 & 474.436 & 471.514 & 0.559 & 2.531 \\ 
dTolmp & 3.347 & 98 & 99 & 2.811 & 4.991 & 4.953 & 5.055 & 5.027 & 2.847 & 2.853 & 0.036 & 0.042 & 2.180 & 2.142 & 2.208 & 2.174 & 245.290 & 246.651 & 435.562 & 434.645 & 0.001 & 0.001 & 190.272 & 187.993 & 0.379 & 3.479 \\ 
SiTCNCz & 2.239 & 122 & 123 & 2.188 & 3.623 & 3.604 & 4.036 & 3.983 & 2.438 & 2.418 & 0.250 & 0.230 & 1.434 & 1.416 & 1.598 & 1.565 & 307.203 & 311.260 & 508.558 & 512.713 & 0.418 & 0.362 & 201.354 & 201.453 & 0.424 & 2.761 \\ 
dpmb & 3.045 & 83 & 84 & 2.465 & 4.818 & 4.779 & 4.979 & 4.951 & 2.547 & 2.553 & 0.082 & 0.089 & 2.353 & 2.315 & 2.432 & 2.398 & 249.029 & 250.417 & 486.759 & 485.562 & 0.001 & 0.001 & 237.730 & 235.144 & 0.531 & 1.757 \\ 
3CzBN & 2.342 & 109 & 110 & 2.499 & 3.396 & 3.371 & 3.844 & 3.819 & 2.828 & 2.831 & 0.329 & 0.332 & 0.897 & 0.872 & 1.016 & 0.988 & 322.540 & 324.685 & 438.348 & 437.938 & 0.317 & 0.286 & 115.808 & 113.253 & 0.367 & 1.066 \\ 
TCB & 1.560 & 109 & 110 & 2.235 & 3.336 & 3.311 & 3.729 & 3.701 & 2.498 & 2.498 & 0.263 & 0.263 & 1.101 & 1.076 & 1.231 & 1.203 & 332.504 & 335.038 & 496.378 & 496.398 & 1.659 & 1.445 & 163.874 & 161.360 & 0.113 & 13.154 \\ 
CPzPyC & 1.963 & 89 & 90 & 1.866 & 3.332 & 3.314 & 3.645 & 3.616 & 2.042 & 2.036 & 0.175 & 0.170 & 1.466 & 1.448 & 1.604 & 1.580 & 340.130 & 342.915 & 607.277 & 609.033 & 0.116 & 0.125 & 267.147 & 266.119 & 0.498 & 1.224 \\ 
CPzPzC & 1.616 & 89 & 90 & 1.436 & 3.062 & 3.038 & 3.505 & 3.463 & 1.644 & 1.637 & 0.208 & 0.201 & 1.626 & 1.603 & 1.861 & 1.827 & 353.745 & 357.974 & 754.305 & 757.562 & 0.317 & 0.277 & 400.559 & 399.588 & 0.548 & 0.048 \\ 
CPzPC & 2.083 & 89 & 90 & 1.927 & 3.345 & 3.327 & 3.702 & 3.660 & 2.134 & 2.121 & 0.206 & 0.193 & 1.417 & 1.399 & 1.569 & 1.540 & 334.893 & 338.718 & 581.101 & 584.609 & 0.440 & 0.420 & 246.208 & 245.891 & 0.550 & 0.694 \\ 
CBIQD & 1.581 & 60 & 61 & 1.998 & 2.818 & 2.765 & 3.706 & 3.663 & 2.627 & 2.647 & 0.629 & 0.649 & 0.820 & 0.767 & 1.079 & 1.016 & 334.541 & 338.505 & 471.877 & 468.421 & 0.035 & 0.237 & 137.336 & 129.916 & 0.157 & 6.902 \\ 
PXZ-QL & 2.100 & 57 & 58 & 2.254 & 2.696 & 2.676 & 3.139 & 3.085 & 2.624 & 2.598 & 0.370 & 0.344 & 0.442 & 0.422 & 0.515 & 0.487 & 395.005 & 401.907 & 472.491 & 477.180 & 0.334 & 0.277 & 77.486 & 75.273 & 0.474 & 3.703 \\ 
SBA & 3.150 & 64 & 65 & 2.998 & 3.466 & 3.433 & 4.083 & 4.028 & 3.533 & 3.517 & 0.534 & 0.519 & 0.468 & 0.435 & 0.551 & 0.510 & 303.622 & 307.836 & 350.980 & 352.514 & 0.068 & 0.058 & 47.357 & 44.678 & 0.717 & 0.004 \\ 
TATP-BP & 1.716 & 214 & 215 & 2.076 & 3.403 & 3.381 & 3.642 & 3.619 & 2.221 & 2.223 & 0.145 & 0.146 & 1.327 & 1.304 & 1.420 & 1.396 & 340.476 & 342.592 & 558.130 & 557.838 & 0.163 & 0.143 & 217.655 & 215.246 & 0.124 & 7.909 \\ 
Pd-1 & 1.937 & 121 & 122 & 1.072 & 2.616 & 2.580 & 2.941 & 2.920 & 1.205 & 1.213 & 0.133 & 0.141 & 1.545 & 1.508 & 1.736 & 1.707 & 421.572 & 424.560 & 1028.990 & 1021.828 & 0.175 & 0.156 & 607.418 & 597.268 & 0.650 & 2.618 \\ 
C3F7 & 2.201 & 93 & 94 & 2.412 & 3.244 & 3.236 & 3.349 & 3.339 & 2.489 & 2.489 & 0.078 & 0.077 & 0.833 & 0.824 & 0.860 & 0.851 & 370.202 & 371.277 & 498.057 & 498.164 & 0.046 & 0.043 & 127.855 & 126.887 & 0.338 & 3.045 \\ 
BuCzCF3oB & 1.852 & 129 & 130 & 2.171 & 3.010 & 3.003 & 3.124 & 3.113 & 2.254 & 2.251 & 0.083 & 0.080 & 0.839 & 0.831 & 0.871 & 0.862 & 396.813 & 398.266 & 550.100 & 550.776 & 0.059 & 0.054 & 153.288 & 152.510 & 0.307 & 3.445 \\ 
phenazasiline & 1.284 & 57 & 58 & 1.173 & 3.154 & 3.119 & 3.230 & 3.229 & 1.202 & 1.215 & 0.028 & 0.041 & 1.980 & 1.945 & 2.028 & 2.014 & 383.876 & 384.007 & 1031.736 & 1020.634 & 0.007 & 0.007 & 647.860 & 636.627 & 0.545 & 0.082 \\ 
D–A–D & 1.284 & 57 & 58 & 1.173 & 3.154 & 3.119 & 3.230 & 3.229 & 1.202 & 1.215 & 0.028 & 0.041 & 1.980 & 1.945 & 2.028 & 2.014 & 383.876 & 384.007 & 1031.730 & 1020.660 & 0.007 & 0.007 & 647.854 & 636.653 & 0.544 & 0.082 \\ 
pzpy & 2.096 & 131 & 132 & 1.714 & 2.254 & 2.184 & 3.196 & 3.038 & 2.431 & 2.385 & 0.716 & 0.671 & 0.540 & 0.470 & 0.765 & 0.653 & 387.972 & 408.071 & 510.110 & 519.873 & 0.690 & 0.503 & 122.138 & 111.802 & 0.919 & 0.011 \\ 
m-PO-ABN & 2.101 & 104 & 105 & 1.710 & 2.254 & 2.185 & 3.207 & 3.048 & 2.433 & 2.386 & 0.723 & 0.676 & 0.544 & 0.474 & 0.774 & 0.662 & 386.605 & 406.746 & 509.493 & 519.577 & 0.639 & 0.446 & 122.888 & 112.832 & 0.913 & 0.481 \\ 
PO-ABN & 2.096 & 104 & 105 & 1.710 & 2.251 & 2.182 & 3.202 & 3.044 & 2.433 & 2.386 & 0.722 & 0.675 & 0.541 & 0.472 & 0.770 & 0.658 & 387.172 & 407.307 & 509.675 & 519.723 & 0.644 & 0.450 & 122.503 & 112.417 & 0.913 & 0.495 \\ 
p-PO-ABN & 2.061 & 104 & 105 & 1.677 & 2.246 & 2.177 & 3.226 & 3.086 & 2.408 & 2.378 & 0.732 & 0.701 & 0.569 & 0.500 & 0.818 & 0.709 & 384.292 & 401.750 & 514.786 & 521.475 & 1.047 & 0.728 & 130.494 & 119.724 & 0.900 & 0.814 \\ 
teracridan & 3.159 & 100 & 101 & 1.834 & 3.596 & 3.569 & 4.080 & 4.024 & 2.081 & 2.068 & 0.247 & 0.234 & 1.762 & 1.735 & 1.999 & 1.956 & 303.883 & 308.135 & 595.767 & 599.534 & 0.055 & 0.047 & 291.884 & 291.399 & 0.484 & 3.675 \\ 
PTPC & 2.361 & 192 & 193 & 2.285 & 3.491 & 3.465 & 3.864 & 3.827 & 2.529 & 2.524 & 0.244 & 0.239 & 1.206 & 1.180 & 1.335 & 1.303 & 320.862 & 323.964 & 490.232 & 491.271 & 0.473 & 0.439 & 169.370 & 167.308 & 0.187 & 14.870 \\ 
TPTI & 2.390 & 53 & 54 & 2.133 & 2.569 & 2.537 & 3.233 & 3.112 & 2.685 & 2.616 & 0.552 & 0.484 & 0.436 & 0.404 & 0.548 & 0.495 & 383.448 & 398.420 & 461.780 & 473.869 & 0.182 & 0.143 & 78.331 & 75.449 & 0.795 & 0.002 \\ 
BDBTCz-Trz & 1.955 & 147 & 148 & 2.052 & 3.422 & 3.402 & 3.809 & 3.757 & 2.284 & 2.267 & 0.232 & 0.214 & 1.370 & 1.350 & 1.525 & 1.491 & 325.486 & 329.982 & 542.774 & 547.007 & 0.673 & 0.551 & 217.288 & 217.025 & 0.284 & 8.453 \\ 
BDBFCz-Trz & 1.993 & 147 & 148 & 2.059 & 3.385 & 3.364 & 3.772 & 3.718 & 2.295 & 2.275 & 0.236 & 0.216 & 1.326 & 1.306 & 1.478 & 1.443 & 328.653 & 333.497 & 540.353 & 544.981 & 0.734 & 0.598 & 211.700 & 211.484 & 0.321 & 7.410 \\ 
HAP-3MF & 1.758 & 91 & 92 & 1.748 & 3.171 & 3.158 & 3.254 & 3.236 & 1.794 & 1.791 & 0.046 & 0.043 & 1.422 & 1.410 & 1.460 & 1.444 & 380.997 & 383.200 & 690.968 & 692.178 & 0.000 & 0.000 & 309.970 & 308.978 & 0.370 & 0.954 \\ 
FlCz & 2.137 & 95 & 96 & 2.046 & 3.407 & 3.370 & 3.732 & 3.728 & 2.241 & 2.263 & 0.195 & 0.217 & 1.361 & 1.325 & 1.491 & 1.465 & 332.246 & 332.585 & 553.279 & 547.958 & 0.152 & 0.210 & 221.033 & 215.373 & 0.450 & 2.254 \\ 
SFCz & 2.105 & 116 & 117 & 2.028 & 3.431 & 3.407 & 3.772 & 3.765 & 2.229 & 2.241 & 0.201 & 0.213 & 1.403 & 1.379 & 1.542 & 1.524 & 328.714 & 329.281 & 556.119 & 553.183 & 0.213 & 0.330 & 227.405 & 223.902 & 0.445 & 2.640 \\ 
o-TPA-AP-TPA & 1.810 & 159 & 160 & 1.643 & 2.213 & 2.145 & 3.127 & 3.007 & 2.321 & 2.304 & 0.679 & 0.661 & 0.570 & 0.502 & 0.806 & 0.704 & 396.470 & 412.250 & 534.083 & 538.202 & 0.810 & 0.578 & 137.613 & 125.952 & 0.123 & 8.672 \\ 
p-TPA-AP-TPA & 1.871 & 159 & 160 & 1.643 & 2.297 & 2.228 & 3.253 & 3.138 & 2.326 & 2.314 & 0.684 & 0.671 & 0.654 & 0.585 & 0.926 & 0.824 & 381.161 & 395.106 & 532.936 & 535.885 & 1.473 & 1.023 & 151.775 & 140.779 & 0.479 & 1.285 \\ 
TNPZ & 1.262 & 177 & 178 & 1.154 & 3.078 & 3.050 & 3.296 & 3.296 & 1.236 & 1.247 & 0.082 & 0.093 & 1.924 & 1.896 & 2.060 & 2.048 & 376.143 & 376.223 & 1003.229 & 994.217 & 0.007 & 0.007 & 627.086 & 617.994 & 0.300 & 8.379 \\ 
m-TPA-AP-TPA & 1.863 & 159 & 160 & 1.675 & 2.254 & 2.185 & 3.201 & 3.085 & 2.378 & 2.365 & 0.703 & 0.690 & 0.579 & 0.510 & 0.822 & 0.720 & 387.378 & 401.894 & 521.349 & 524.280 & 1.074 & 0.773 & 133.971 & 122.386 & 0.210 & 5.127 \\ 
5,6PXZ-PIDO & 0.814 & 127 & 128 & 1.617 & 2.846 & 2.816 & 3.219 & 3.196 & 1.829 & 1.836 & 0.212 & 0.219 & 1.229 & 1.199 & 1.390 & 1.361 & 385.176 & 387.899 & 677.850 & 675.375 & 0.071 & 0.002 & 292.674 & 287.476 & 0.139 & 8.331 \\ 
TRZ-3SO2 & 2.231 & 126 & 127 & 2.112 & 4.137 & 4.103 & 4.205 & 4.204 & 2.147 & 2.164 & 0.035 & 0.052 & 2.025 & 1.991 & 2.058 & 2.040 & 294.828 & 294.934 & 577.438 & 572.939 & 0.006 & 0.006 & 282.610 & 278.005 & 0.435 & 0.866 \\ 
35tCzBPym & 1.465 & 142 & 143 & 1.843 & 3.207 & 3.197 & 3.465 & 3.437 & 1.991 & 1.981 & 0.148 & 0.138 & 1.365 & 1.354 & 1.474 & 1.456 & 357.777 & 360.744 & 622.750 & 625.936 & 0.063 & 0.055 & 264.972 & 265.192 & 0.183 & 6.276 \\ 
35CzBPym & 1.630 & 94 & 95 & 1.881 & 3.276 & 3.266 & 3.536 & 3.506 & 2.030 & 2.019 & 0.149 & 0.138 & 1.395 & 1.385 & 1.506 & 1.486 & 350.664 & 353.675 & 610.735 & 614.023 & 0.064 & 0.056 & 260.071 & 260.349 & 0.199 & 5.967 \\ 
25CzBPym & 1.686 & 94 & 95 & 1.880 & 3.084 & 3.076 & 3.220 & 3.207 & 1.963 & 1.960 & 0.083 & 0.080 & 1.204 & 1.196 & 1.257 & 1.247 & 384.984 & 386.641 & 631.594 & 632.728 & 0.066 & 0.060 & 246.610 & 246.087 & 0.259 & 3.812 \\ 
25tCzBPym & 1.499 & 142 & 143 & 1.843 & 2.961 & 2.954 & 3.097 & 3.083 & 1.928 & 1.924 & 0.085 & 0.081 & 1.118 & 1.111 & 1.170 & 1.159 & 400.285 & 402.089 & 643.124 & 644.386 & 0.061 & 0.056 & 242.839 & 242.297 & 0.261 & 3.707 \\ 
BPBiPA & 2.096 & 131 & 132 & 1.715 & 2.254 & 2.184 & 3.196 & 3.039 & 2.431 & 2.386 & 0.717 & 0.671 & 0.539 & 0.469 & 0.765 & 0.653 & 387.936 & 408.031 & 509.920 & 519.654 & 0.691 & 0.504 & 121.985 & 111.623 & 0.919 & 0.009 \\ 
BTZ–DMAC & 0.929 & 100 & 101 & 1.482 & 2.659 & 2.634 & 2.888 & 2.872 & 1.609 & 1.616 & 0.127 & 0.134 & 1.178 & 1.152 & 1.279 & 1.256 & 429.308 & 431.760 & 770.502 & 767.385 & 0.192 & 0.179 & 341.194 & 335.625 & 0.326 & 1.849 \\ 
BTZ–DPA & 1.139 & 84 & 85 & 1.388 & 2.069 & 2.020 & 2.678 & 2.595 & 1.796 & 1.782 & 0.408 & 0.395 & 0.681 & 0.633 & 0.882 & 0.813 & 462.956 & 477.836 & 690.304 & 695.722 & 0.630 & 0.503 & 227.348 & 217.885 & 0.564 & 2.073 \\ 
2F & 1.104 & 130 & 131 & 1.381 & 2.884 & 2.864 & 3.334 & 3.259 & 1.596 & 1.572 & 0.215 & 0.191 & 1.503 & 1.482 & 1.737 & 1.687 & 371.912 & 380.413 & 776.630 & 788.709 & 0.112 & 0.090 & 404.718 & 408.296 & 0.121 & 11.502 \\ 
PFBP-2a & 1.239 & 119 & 120 & 2.025 & 3.159 & 3.147 & 3.423 & 3.406 & 2.194 & 2.192 & 0.169 & 0.167 & 1.134 & 1.122 & 1.228 & 1.214 & 362.241 & 364.038 & 565.049 & 565.695 & 0.306 & 0.281 & 202.808 & 201.657 & 0.353 & 6.146 \\ 
PFBP-2b & 1.458 & 179 & 180 & 1.737 & 3.222 & 3.213 & 3.503 & 3.494 & 1.888 & 1.888 & 0.152 & 0.152 & 1.486 & 1.477 & 1.615 & 1.606 & 353.887 & 354.808 & 656.675 & 656.567 & 0.635 & 0.602 & 302.789 & 301.759 & 0.413 & 0.140 \\ 
PXZ-PPO & 2.403 & 63 & 64 & 2.370 & 2.919 & 2.892 & 3.547 & 3.485 & 2.881 & 2.856 & 0.510 & 0.486 & 0.549 & 0.522 & 0.667 & 0.629 & 349.527 & 355.735 & 430.413 & 434.110 & 0.610 & 0.530 & 80.886 & 78.375 & 0.568 & 3.301 \\ 
PXZ-BOO & 1.737 & 63 & 64 & 2.342 & 2.713 & 2.702 & 2.993 & 2.967 & 2.583 & 2.571 & 0.241 & 0.230 & 0.372 & 0.361 & 0.410 & 0.396 & 414.275 & 417.821 & 480.085 & 482.195 & 0.254 & 0.222 & 65.810 & 64.374 & 0.368 & 4.736 \\ 
PPZTPI & 1.723 & 127 & 128 & 2.155 & 2.292 & 2.262 & 2.530 & 2.501 & 2.379 & 2.383 & 0.223 & 0.228 & 0.137 & 0.107 & 0.151 & 0.118 & 490.114 & 495.738 & 521.247 & 520.283 & 0.000 & 0.000 & 31.133 & 24.544 & 0.233 & 7.254 \\ 
PPZPPI & 1.650 & 115 & 116 & 2.118 & 2.287 & 2.256 & 2.524 & 2.494 & 2.338 & 2.342 & 0.220 & 0.224 & 0.169 & 0.138 & 0.186 & 0.152 & 491.163 & 497.130 & 530.253 & 529.489 & 0.000 & 0.000 & 39.090 & 32.359 & 0.234 & 7.303 \\ 
Pra-2DMAC & 2.655 & 93 & 94 & 2.841 & 3.397 & 3.365 & 4.003 & 3.949 & 3.349 & 3.334 & 0.507 & 0.492 & 0.556 & 0.524 & 0.655 & 0.615 & 309.690 & 313.987 & 370.246 & 371.904 & 0.086 & 0.118 & 60.557 & 57.916 & 0.264 & 3.657 \\ 
BAPCN & 1.957 & 81 & 82 & 2.131 & 2.606 & 2.571 & 3.189 & 3.114 & 2.607 & 2.580 & 0.477 & 0.450 & 0.475 & 0.441 & 0.582 & 0.534 & 388.775 & 398.176 & 475.505 & 480.538 & 0.286 & 0.231 & 86.730 & 82.361 & 0.434 & 7.282 \\ 
BACN & 2.167 & 67 & 68 & 2.204 & 2.544 & 2.509 & 3.114 & 3.033 & 2.697 & 2.664 & 0.493 & 0.460 & 0.341 & 0.305 & 0.417 & 0.369 & 398.189 & 408.757 & 459.747 & 465.382 & 0.219 & 0.177 & 61.557 & 56.625 & 0.633 & 3.559 \\ 
BDQC-2 & 1.386 & 141 & 142 & 1.413 & 3.009 & 2.985 & 3.360 & 3.329 & 1.578 & 1.576 & 0.165 & 0.163 & 1.596 & 1.572 & 1.782 & 1.753 & 369.012 & 372.470 & 785.896 & 786.804 & 0.275 & 0.263 & 416.885 & 414.334 & 0.114 & 6.689 \\ 
NIDPA-1 & 1.898 & 115 & 116 & 1.969 & 2.452 & 2.422 & 2.935 & 2.863 & 2.357 & 2.328 & 0.388 & 0.359 & 0.483 & 0.453 & 0.579 & 0.535 & 422.405 & 433.042 & 526.111 & 532.630 & 0.195 & 0.154 & 103.706 & 99.588 & 0.546 & 3.112 \\ 
NIDPA-2 & 1.876 & 115 & 116 & 2.087 & 2.584 & 2.564 & 3.010 & 2.941 & 2.432 & 2.395 & 0.344 & 0.307 & 0.497 & 0.477 & 0.578 & 0.547 & 411.894 & 421.529 & 509.867 & 517.755 & 0.358 & 0.293 & 97.973 & 96.226 & 0.461 & 3.634 \\ 
SABIQ & 1.116 & 93 & 94 & 1.110 & 2.407 & 2.342 & 2.855 & 2.854 & 1.317 & 1.353 & 0.207 & 0.242 & 1.296 & 1.232 & 1.538 & 1.501 & 434.316 & 434.483 & 941.366 & 916.569 & 0.001 & 0.001 & 507.050 & 482.086 & 0.364 & 2.947 \\ 
Perylene & 1.889 & 46 & 47 & 1.567 & 2.154 & 2.082 & 3.252 & 3.079 & 2.365 & 2.318 & 0.799 & 0.751 & 0.587 & 0.515 & 0.887 & 0.762 & 381.232 & 402.638 & 524.136 & 534.983 & 0.865 & 0.602 & 142.904 & 132.346 & 0.946 & 0.000 \\ 
SAIP & 1.788 & 75 & 76 & 1.801 & 3.409 & 3.378 & 3.622 & 3.620 & 1.913 & 1.929 & 0.112 & 0.129 & 1.609 & 1.578 & 1.709 & 1.691 & 342.309 & 342.488 & 648.150 & 642.632 & 0.006 & 0.006 & 305.842 & 300.144 & 0.336 & 2.857 \\ 
FAC & 2.726 & 61 & 62 & 2.886 & 3.469 & 3.435 & 4.090 & 4.021 & 3.403 & 3.378 & 0.517 & 0.492 & 0.583 & 0.550 & 0.687 & 0.643 & 303.125 & 308.342 & 364.351 & 367.063 & 0.059 & 0.089 & 61.226 & 58.721 & 0.173 & 3.729 \\ 
phenylperylene & 1.829 & 60 & 61 & 1.497 & 2.123 & 2.056 & 3.105 & 2.961 & 2.190 & 2.157 & 0.693 & 0.659 & 0.626 & 0.558 & 0.915 & 0.804 & 399.266 & 418.781 & 566.040 & 574.912 & 0.717 & 0.506 & 166.773 & 156.132 & 0.937 & 0.195 \\ 
ImPy-2 & 2.399 & 65 & 66 & 2.152 & 2.652 & 2.616 & 3.282 & 3.193 & 2.663 & 2.626 & 0.511 & 0.474 & 0.500 & 0.465 & 0.619 & 0.567 & 377.793 & 388.324 & 465.658 & 472.178 & 0.314 & 0.249 & 87.865 & 83.854 & 0.704 & 2.502 \\ 
ImPy-1 & 2.370 & 59 & 60 & 2.163 & 2.661 & 2.625 & 3.295 & 3.202 & 2.678 & 2.639 & 0.515 & 0.476 & 0.498 & 0.462 & 0.617 & 0.564 & 376.303 & 387.172 & 462.983 & 469.878 & 0.317 & 0.251 & 86.681 & 82.705 & 0.549 & 4.249 \\ 
ImPy-3 & 1.933 & 72 & 73 & 1.771 & 2.546 & 2.489 & 3.199 & 3.134 & 2.225 & 2.230 & 0.455 & 0.459 & 0.775 & 0.718 & 0.974 & 0.905 & 387.548 & 395.560 & 557.214 & 556.044 & 0.868 & 0.689 & 169.667 & 160.485 & 0.644 & 4.005 \\ 
BTaz-Ar-PXZ & 1.541 & 69 & 70 & 2.095 & 2.761 & 2.729 & 3.017 & 2.997 & 2.289 & 2.300 & 0.194 & 0.205 & 0.666 & 0.634 & 0.728 & 0.697 & 410.966 & 413.694 & 541.611 & 538.987 & 0.464 & 0.416 & 130.645 & 125.292 & 0.319 & 6.117 \\ 
FSF4A & 2.520 & 125 & 126 & 2.469 & 3.193 & 3.165 & 3.563 & 3.538 & 2.755 & 2.760 & 0.286 & 0.291 & 0.724 & 0.697 & 0.808 & 0.779 & 348.006 & 350.386 & 450.073 & 449.248 & 0.288 & 0.255 & 102.067 & 98.861 & 0.559 & 2.278 \\ 
TPA-L-BN & 2.111 & 73 & 74 & 2.373 & 3.417 & 3.393 & 3.955 & 3.914 & 2.747 & 2.737 & 0.373 & 0.364 & 1.044 & 1.020 & 1.209 & 1.177 & 313.463 & 316.763 & 451.396 & 452.944 & 0.340 & 0.294 & 137.932 & 136.181 & 0.110 & 4.739 \\ 
IpCm-PhBzAc & 1.600 & 105 & 106 & 2.408 & 3.122 & 3.090 & 3.781 & 3.719 & 2.916 & 2.898 & 0.508 & 0.490 & 0.715 & 0.683 & 0.866 & 0.822 & 327.888 & 333.354 & 425.225 & 427.868 & 1.088 & 0.904 & 97.337 & 94.515 & 0.044 & 8.300 \\ 
DphAn-Br & 2.576 & 67 & 68 & 2.347 & 3.815 & 3.814 & 3.809 & 3.808 & 2.344 & 2.343 & -0.003 & -0.004 & 1.468 & 1.467 & 1.465 & 1.464 & 325.495 & 325.623 & 529.033 & 529.102 & 0.000 & 0.000 & 203.538 & 203.479 & 0.544 & 0.495 \\ 
5-DBFBI & 2.846 & 82 & 83 & 2.651 & 3.578 & 3.549 & 4.100 & 4.057 & 3.038 & 3.031 & 0.387 & 0.380 & 0.926 & 0.898 & 1.062 & 1.027 & 302.430 & 305.575 & 408.105 & 409.088 & 1.427 & 1.251 & 105.675 & 103.512 & 0.647 & 3.308 \\ 
4-DBFBI & 2.806 & 82 & 83 & 2.824 & 3.682 & 3.655 & 4.176 & 4.132 & 3.203 & 3.193 & 0.379 & 0.368 & 0.857 & 0.831 & 0.972 & 0.939 & 296.933 & 300.073 & 387.068 & 388.335 & 0.435 & 0.389 & 90.135 & 88.262 & 0.440 & 4.225 \\ 
DMACMNPTO & 2.571 & 99 & 100 & 3.019 & 3.373 & 3.341 & 3.974 & 3.919 & 3.556 & 3.541 & 0.538 & 0.522 & 0.354 & 0.322 & 0.418 & 0.378 & 311.988 & 316.383 & 348.625 & 350.150 & 0.043 & 0.039 & 36.636 & 33.767 & 0.087 & 6.634 \\ 
1CzSO & 2.172 & 145 & 146 & 2.442 & 3.426 & 3.405 & 3.874 & 3.818 & 2.761 & 2.738 & 0.320 & 0.296 & 0.984 & 0.963 & 1.113 & 1.080 & 320.025 & 324.753 & 449.007 & 452.848 & 0.293 & 0.252 & 128.982 & 128.095 & 0.324 & 5.264 \\ 
DpAn-BzAc & 1.433 & 119 & 120 & 2.145 & 3.039 & 3.011 & 3.574 & 3.514 & 2.522 & 2.503 & 0.377 & 0.358 & 0.894 & 0.867 & 1.052 & 1.011 & 346.916 & 352.859 & 491.602 & 495.434 & 0.179 & 0.153 & 144.686 & 142.575 & 0.033 & 7.409 \\ 
BzITz & 2.040 & 98 & 99 & 2.019 & 3.340 & 3.320 & 3.756 & 3.727 & 2.271 & 2.267 & 0.251 & 0.248 & 1.321 & 1.300 & 1.485 & 1.460 & 330.114 & 332.683 & 546.035 & 546.890 & 0.941 & 0.855 & 215.921 & 214.208 & 0.377 & 6.324 \\ 
TPXZ–as-TAZ & 1.259 & 156 & 157 & 1.296 & 2.821 & 2.811 & 3.035 & 3.024 & 1.395 & 1.395 & 0.098 & 0.098 & 1.525 & 1.515 & 1.641 & 1.630 & 408.447 & 409.946 & 888.971 & 888.945 & 0.681 & 0.669 & 480.524 & 478.999 & 0.122 & 4.946 \\ 
TPA-CN-N4-2PY & 2.379 & 94 & 95 & 2.350 & 3.198 & 3.165 & 3.754 & 3.716 & 2.758 & 2.759 & 0.408 & 0.409 & 0.848 & 0.815 & 0.996 & 0.957 & 330.299 & 333.641 & 449.523 & 449.414 & 0.866 & 0.738 & 119.224 & 115.774 & 0.459 & 5.151 \\ 
TPA-CN-N4 & 1.305 & 51 & 52 & 1.173 & 3.152 & 3.102 & 3.218 & 3.217 & 1.197 & 1.216 & 0.024 & 0.043 & 1.979 & 1.929 & 2.021 & 2.001 & 385.295 & 385.427 & 1035.689 & 1019.544 & 0.007 & 0.007 & 650.394 & 634.117 & 0.559 & 0.020 \\ 
6,7-DCNQx-DICz & 0.863 & 150 & 151 & 1.225 & 3.296 & 3.278 & 3.320 & 3.317 & 1.234 & 1.239 & 0.009 & 0.014 & 2.071 & 2.053 & 2.086 & 2.077 & 373.480 & 373.807 & 1004.900 & 1000.408 & 0.013 & 0.013 & 631.420 & 626.601 & 0.052 & 9.701 \\ 
PBICT & 1.976 & 149 & 150 & 1.637 & 3.113 & 3.089 & 3.519 & 3.463 & 1.850 & 1.835 & 0.213 & 0.198 & 1.476 & 1.452 & 1.669 & 1.628 & 352.338 & 358.025 & 670.048 & 675.615 & 0.377 & 0.323 & 317.710 & 317.590 & 0.282 & 4.291 \\ 
DCBNPE & 1.107 & 110 & 111 & 1.278 & 2.041 & 2.016 & 2.440 & 2.404 & 1.528 & 1.524 & 0.250 & 0.246 & 0.763 & 0.738 & 0.912 & 0.880 & 508.111 & 515.741 & 811.542 & 813.720 & 0.276 & 0.232 & 303.431 & 297.979 & 0.393 & 0.388 \\ 
TPA-BT-Q & 3.044 & 120 & 121 & 2.791 & 3.492 & 3.469 & 4.076 & 4.039 & 3.258 & 3.250 & 0.467 & 0.459 & 0.701 & 0.678 & 0.818 & 0.789 & 304.196 & 306.983 & 380.580 & 381.504 & 0.345 & 0.351 & 76.384 & 74.521 & 0.664 & 1.103 \\ 
D5 & 2.656 & 100 & 101 & 2.634 & 3.424 & 3.401 & 3.880 & 3.814 & 2.985 & 2.954 & 0.351 & 0.320 & 0.790 & 0.767 & 0.896 & 0.860 & 319.539 & 325.085 & 415.416 & 419.787 & 0.315 & 0.257 & 95.877 & 94.702 & 0.172 & 10.346 \\ 
D6 & 2.615 & 86 & 87 & 2.611 & 3.403 & 3.380 & 3.844 & 3.774 & 2.949 & 2.915 & 0.338 & 0.305 & 0.792 & 0.769 & 0.895 & 0.858 & 322.565 & 328.548 & 420.423 & 425.277 & 0.217 & 0.179 & 97.858 & 96.729 & 0.227 & 7.052 \\ 
PxPYM & 1.495 & 109 & 110 & 1.790 & 2.855 & 2.824 & 3.124 & 3.109 & 1.959 & 1.970 & 0.169 & 0.180 & 1.065 & 1.034 & 1.165 & 1.138 & 396.813 & 398.843 & 632.835 & 629.299 & 0.715 & 0.650 & 236.022 & 230.456 & 0.300 & 6.629 \\ 
D1–D6 & 2.615 & 86 & 87 & 2.611 & 3.403 & 3.379 & 3.844 & 3.774 & 2.949 & 2.916 & 0.338 & 0.305 & 0.792 & 0.769 & 0.895 & 0.858 & 322.548 & 328.531 & 420.402 & 425.243 & 0.217 & 0.179 & 97.854 & 96.712 & 0.227 & 7.055 \\ 
DTPCZTZ & 2.324 & 123 & 124 & 2.362 & 3.472 & 3.449 & 3.886 & 3.822 & 2.644 & 2.618 & 0.282 & 0.255 & 1.110 & 1.087 & 1.242 & 1.205 & 319.021 & 324.354 & 468.886 & 473.662 & 0.229 & 0.186 & 149.865 & 149.308 & 0.293 & 9.311 \\ 
DHPZ-2BI & 1.640 & 132 & 133 & 2.055 & 2.353 & 2.323 & 2.595 & 2.566 & 2.266 & 2.270 & 0.212 & 0.215 & 0.298 & 0.268 & 0.328 & 0.296 & 477.800 & 483.256 & 547.032 & 546.271 & 0.000 & 0.000 & 69.232 & 63.015 & 0.273 & 0.603 \\ 
DHPZ-2BN & 1.588 & 70 & 71 & 2.025 & 2.369 & 2.338 & 2.614 & 2.582 & 2.235 & 2.236 & 0.209 & 0.211 & 0.344 & 0.313 & 0.379 & 0.346 & 474.326 & 480.168 & 554.841 & 554.419 & 0.000 & 0.000 & 80.515 & 74.251 & 0.349 & 0.221 \\ 
SAF-2NP & 1.117 & 111 & 112 & 1.124 & 2.672 & 2.658 & 2.866 & 2.850 & 1.205 & 1.205 & 0.082 & 0.081 & 1.548 & 1.534 & 1.661 & 1.645 & 432.604 & 435.093 & 1028.766 & 1029.111 & 0.224 & 0.211 & 596.163 & 594.018 & 0.299 & 5.780 \\ 
BTPO & 3.133 & 62 & 63 & 3.137 & 3.617 & 3.593 & 4.119 & 4.075 & 3.573 & 3.558 & 0.436 & 0.421 & 0.480 & 0.456 & 0.547 & 0.517 & 300.984 & 304.256 & 347.029 & 348.435 & 0.220 & 0.192 & 46.045 & 44.180 & 0.547 & 1.744 \\ 
PyDCN–DMAC & 1.500 & 104 & 105 & 2.191 & 3.391 & 3.358 & 3.771 & 3.767 & 2.437 & 2.458 & 0.246 & 0.266 & 1.200 & 1.167 & 1.334 & 1.309 & 328.775 & 329.150 & 508.750 & 504.434 & 0.037 & 0.033 & 179.975 & 175.284 & 0.078 & 9.354 \\ 
PyDCN & 2.479 & 65 & 66 & 2.523 & 3.847 & 3.804 & 4.460 & 4.420 & 2.926 & 2.932 & 0.402 & 0.408 & 1.323 & 1.281 & 1.534 & 1.489 & 277.991 & 280.482 & 423.799 & 422.894 & 0.557 & 0.516 & 145.807 & 142.412 & 0.304 & 0.771 \\ 
PXZ-OXD & 1.620 & 74 & 75 & 2.213 & 2.762 & 2.731 & 3.111 & 3.085 & 2.492 & 2.500 & 0.279 & 0.287 & 0.549 & 0.518 & 0.619 & 0.585 & 398.599 & 401.907 & 497.532 & 496.013 & 0.439 & 0.016 & 98.933 & 94.106 & 0.295 & 6.827 \\ 
TCz-3PA-TCz & 1.967 & 179 & 180 & 1.866 & 3.242 & 3.211 & 3.713 & 3.687 & 2.137 & 2.143 & 0.271 & 0.277 & 1.376 & 1.345 & 1.576 & 1.545 & 333.901 & 336.247 & 580.192 & 578.645 & 2.564 & 2.351 & 246.291 & 242.399 & 0.530 & 0.092 \\ 
NAI–BiFA & 1.564 & 148 & 149 & 1.750 & 2.058 & 2.023 & 2.610 & 2.546 & 2.220 & 2.203 & 0.470 & 0.453 & 0.307 & 0.273 & 0.390 & 0.343 & 475.053 & 486.881 & 558.507 & 562.760 & 0.753 & 0.635 & 83.454 & 75.879 & 0.513 & 3.949 \\ 
NAI–PhBiFA & 1.283 & 162 & 163 & 1.806 & 2.738 & 2.696 & 3.299 & 3.266 & 2.176 & 2.188 & 0.370 & 0.382 & 0.932 & 0.890 & 1.123 & 1.078 & 375.869 & 379.621 & 569.833 & 566.630 & 1.378 & 1.263 & 193.964 & 187.009 & 0.262 & 7.900 \\ 
pDTCz-2DPyS & 2.103 & 146 & 147 & 2.112 & 3.348 & 3.329 & 3.707 & 3.686 & 2.339 & 2.338 & 0.227 & 0.226 & 1.236 & 1.217 & 1.369 & 1.348 & 334.424 & 336.383 & 530.179 & 530.291 & 0.171 & 0.165 & 195.755 & 193.908 & 0.456 & 3.746 \\ 
2SPBAC-BP & 1.786 & 172 & 173 & 2.108 & 3.064 & 3.030 & 3.647 & 3.605 & 2.509 & 2.509 & 0.401 & 0.400 & 0.956 & 0.921 & 1.137 & 1.096 & 340.009 & 343.904 & 494.093 & 494.175 & 0.186 & 0.235 & 154.084 & 150.271 & 0.167 & 4.542 \\ 
SPBAC-PH & 2.541 & 84 & 85 & 2.447 & 2.768 & 2.732 & 3.378 & 3.296 & 2.986 & 2.953 & 0.539 & 0.505 & 0.321 & 0.284 & 0.391 & 0.343 & 367.056 & 376.211 & 415.152 & 419.881 & 0.229 & 0.188 & 48.096 & 43.670 & 0.626 & 2.879 \\ 
DFPBI & 2.343 & 122 & 123 & 2.168 & 3.089 & 3.060 & 3.555 & 3.527 & 2.495 & 2.499 & 0.327 & 0.331 & 0.921 & 0.892 & 1.060 & 1.028 & 348.780 & 351.509 & 496.960 & 496.146 & 1.616 & 1.454 & 148.181 & 144.637 & 0.618 & 4.876 \\ 
TDPA–TRZ & 2.139 & 150 & 151 & 2.060 & 2.966 & 2.938 & 3.497 & 3.470 & 2.429 & 2.433 & 0.369 & 0.373 & 0.906 & 0.878 & 1.069 & 1.038 & 354.504 & 357.262 & 510.472 & 509.622 & 1.557 & 1.436 & 155.968 & 152.360 & 0.441 & 0.621 \\ 
DMAC-11-DPPZ & 1.164 & 90 & 91 & 1.146 & 2.816 & 2.802 & 2.953 & 2.943 & 1.202 & 1.204 & 0.056 & 0.057 & 1.670 & 1.656 & 1.751 & 1.739 & 419.816 & 421.342 & 1031.304 & 1030.128 & 0.141 & 0.134 & 611.488 & 608.786 & 0.248 & 5.751 \\ 
PXZ-11-DPPZ & 1.114 & 84 & 85 & 1.135 & 2.175 & 2.163 & 2.406 & 2.383 & 1.256 & 1.250 & 0.121 & 0.115 & 1.040 & 1.028 & 1.151 & 1.132 & 515.270 & 520.374 & 987.528 & 991.715 & 0.260 & 0.229 & 472.258 & 471.342 & 0.331 & 5.712 \\ 
PXZ-10-DPPZ & 0.954 & 84 & 85 & 1.035 & 1.919 & 1.909 & 2.091 & 2.073 & 1.127 & 1.124 & 0.092 & 0.089 & 0.884 & 0.874 & 0.963 & 0.949 & 593.084 & 597.975 & 1099.655 & 1102.832 & 0.091 & 0.079 & 506.571 & 504.856 & 0.413 & 3.661 \\ 
CCC & 3.293 & 47 & 48 & 2.875 & 3.699 & 3.648 & 4.292 & 4.269 & 3.336 & 3.364 & 0.461 & 0.489 & 0.824 & 0.773 & 0.957 & 0.905 & 288.853 & 290.402 & 371.682 & 368.534 & 0.010 & 0.012 & 82.830 & 78.132 & 0.909 & 0.838 \\ 
CzmPPC & 2.302 & 99 & 100 & 2.195 & 4.125 & 4.082 & 4.319 & 4.318 & 2.298 & 2.323 & 0.103 & 0.127 & 1.930 & 1.886 & 2.020 & 1.996 & 287.087 & 287.120 & 539.416 & 533.816 & 0.001 & 0.001 & 252.329 & 246.695 & 0.472 & 1.140 \\ 
C2FLA-1 & 2.293 & 105 & 106 & 2.105 & 3.240 & 3.198 & 3.897 & 3.853 & 2.532 & 2.536 & 0.427 & 0.431 & 1.134 & 1.093 & 1.365 & 1.317 & 318.153 & 321.786 & 489.592 & 488.809 & 2.965 & 2.576 & 171.439 & 167.023 & 0.707 & 5.774 \\ 
MDP3FL & 2.212 & 177 & 178 & 2.152 & 3.284 & 3.257 & 3.711 & 3.693 & 2.431 & 2.440 & 0.280 & 0.288 & 1.132 & 1.106 & 1.279 & 1.253 & 334.135 & 335.709 & 509.939 & 508.192 & 3.554 & 3.287 & 175.804 & 172.482 & 0.540 & 2.540 \\ 
C3FLA-2 & 2.127 & 167 & 168 & 1.960 & 3.224 & 3.185 & 3.727 & 3.704 & 2.265 & 2.279 & 0.306 & 0.319 & 1.264 & 1.226 & 1.461 & 1.425 & 332.692 & 334.722 & 547.335 & 544.081 & 5.169 & 4.724 & 214.644 & 209.360 & 0.791 & 0.738 \\ 
9CzFDPEPO & 2.783 & 188 & 189 & 2.790 & 3.414 & 3.392 & 3.838 & 3.771 & 3.136 & 3.103 & 0.346 & 0.312 & 0.624 & 0.602 & 0.701 & 0.669 & 323.077 & 328.748 & 395.345 & 399.621 & 0.212 & 0.180 & 72.267 & 70.873 & 0.107 & 8.780 \\ 
9CzFDPESPO & 2.780 & 154 & 155 & 2.829 & 3.427 & 3.405 & 3.869 & 3.801 & 3.193 & 3.158 & 0.364 & 0.329 & 0.598 & 0.576 & 0.676 & 0.643 & 320.472 & 326.188 & 388.264 & 392.549 & 0.221 & 0.186 & 67.792 & 66.361 & 0.085 & 11.270 \\ 
CTM & 2.127 & 80 & 81 & 2.333 & 3.363 & 3.342 & 3.773 & 3.723 & 2.617 & 2.598 & 0.284 & 0.266 & 1.030 & 1.009 & 1.156 & 1.124 & 328.592 & 333.067 & 473.730 & 477.141 & 0.790 & 0.636 & 145.138 & 144.074 & 0.324 & 6.085 \\ 
tCTM & 1.982 & 104 & 105 & 2.292 & 3.311 & 3.290 & 3.701 & 3.654 & 2.563 & 2.546 & 0.270 & 0.254 & 1.018 & 0.998 & 1.138 & 1.108 & 334.993 & 339.274 & 483.814 & 486.993 & 0.706 & 0.588 & 148.822 & 147.719 & 0.318 & 6.318 \\ 
PSBC & 2.091 & 161 & 162 & 2.026 & 3.482 & 3.460 & 3.864 & 3.810 & 2.248 & 2.231 & 0.222 & 0.205 & 1.456 & 1.434 & 1.616 & 1.579 & 320.870 & 325.435 & 551.533 & 555.749 & 0.004 & 0.026 & 230.663 & 230.314 & 0.165 & 7.841 \\ 
26DAcBPy & 1.208 & 131 & 132 & 1.730 & 2.899 & 2.885 & 3.225 & 3.203 & 1.925 & 1.921 & 0.195 & 0.191 & 1.168 & 1.155 & 1.300 & 1.282 & 384.423 & 387.064 & 644.001 & 645.382 & 0.305 & 0.278 & 259.578 & 258.318 & 0.126 & 6.980 \\ 
25DAcBPy & 0.857 & 131 & 132 & 1.348 & 3.110 & 3.103 & 3.243 & 3.235 & 1.405 & 1.405 & 0.058 & 0.057 & 1.762 & 1.755 & 1.837 & 1.830 & 382.349 & 383.223 & 882.221 & 882.334 & 0.146 & 0.142 & 499.873 & 499.111 & 0.176 & 7.876 \\ 
26DPXZBPy & 1.009 & 119 & 120 & 1.604 & 2.542 & 2.531 & 2.860 & 2.845 & 1.806 & 1.803 & 0.201 & 0.199 & 0.937 & 0.927 & 1.055 & 1.042 & 433.481 & 435.812 & 686.642 & 687.592 & 0.004 & 0.004 & 253.161 & 251.780 & 0.290 & 6.795 \\ 
BTITrz & 1.865 & 98 & 99 & 1.976 & 3.438 & 3.415 & 3.824 & 3.800 & 2.198 & 2.199 & 0.222 & 0.222 & 1.461 & 1.439 & 1.625 & 1.601 & 324.269 & 326.317 & 564.008 & 563.888 & 0.748 & 0.706 & 239.739 & 237.571 & 0.311 & 6.694 \\ 
mTPA–PPI & 2.505 & 113 & 114 & 2.450 & 3.432 & 3.402 & 3.794 & 3.757 & 2.708 & 2.706 & 0.258 & 0.256 & 0.982 & 0.952 & 1.086 & 1.051 & 326.782 & 329.973 & 457.794 & 458.199 & 0.535 & 0.459 & 131.013 & 128.225 & 0.250 & 8.312 \\ 
PPI & 2.790 & 68 & 69 & 2.485 & 3.413 & 3.383 & 3.807 & 3.763 & 2.772 & 2.764 & 0.287 & 0.279 & 0.929 & 0.898 & 1.036 & 0.999 & 325.640 & 329.500 & 447.352 & 448.610 & 0.224 & 0.209 & 121.712 & 119.110 & 0.764 & 1.797 \\ 
CzTPA-m-Trz & 1.773 & 146 & 147 & 1.997 & 3.210 & 3.194 & 3.608 & 3.570 & 2.245 & 2.232 & 0.248 & 0.235 & 1.213 & 1.197 & 1.363 & 1.338 & 343.608 & 347.314 & 552.289 & 555.481 & 0.078 & 0.067 & 208.681 & 208.166 & 0.096 & 6.966 \\ 
TPA–2PPITPA & 2.370 & 242 & 243 & 2.173 & 3.474 & 3.454 & 3.846 & 3.817 & 2.405 & 2.402 & 0.232 & 0.229 & 1.302 & 1.281 & 1.441 & 1.416 & 322.363 & 324.787 & 515.488 & 516.224 & 0.427 & 0.386 & 193.124 & 191.437 & 0.507 & 5.743 \\ 
TPA–2SPPITPA & 1.935 & 252 & 253 & 1.713 & 2.892 & 2.852 & 3.505 & 3.483 & 2.076 & 2.091 & 0.363 & 0.379 & 1.179 & 1.140 & 1.429 & 1.391 & 353.735 & 356.000 & 597.249 & 592.883 & 0.753 & 0.752 & 243.513 & 236.883 & 0.476 & 7.719 \\ 
2Cz2tCzBn & 2.074 & 187 & 188 & 2.373 & 3.156 & 3.145 & 3.409 & 3.374 & 2.564 & 2.546 & 0.191 & 0.173 & 0.782 & 0.771 & 0.845 & 0.828 & 363.665 & 367.491 & 483.553 & 486.937 & 0.438 & 0.386 & 119.888 & 119.446 & 0.368 & 0.403 \\ 
2tCz2CzBn & 2.076 & 187 & 188 & 2.397 & 3.162 & 3.151 & 3.425 & 3.388 & 2.596 & 2.577 & 0.199 & 0.181 & 0.765 & 0.754 & 0.829 & 0.811 & 361.966 & 365.919 & 477.580 & 481.070 & 0.395 & 0.349 & 115.614 & 115.152 & 0.357 & 1.799 \\ 
PmPmP & 1.252 & 90 & 91 & 1.680 & 2.765 & 2.734 & 3.126 & 3.087 & 1.899 & 1.896 & 0.219 & 0.217 & 1.086 & 1.055 & 1.227 & 1.191 & 396.623 & 401.607 & 653.023 & 653.770 & 0.015 & 0.013 & 256.401 & 252.163 & 0.212 & 8.441 \\ 
PLQYs & 1.844 & 145 & 146 & 1.994 & 2.807 & 2.735 & 3.336 & 3.294 & 2.370 & 2.402 & 0.376 & 0.408 & 0.813 & 0.741 & 0.966 & 0.892 & 371.644 & 376.394 & 523.105 & 516.275 & 0.028 & 0.024 & 151.461 & 139.881 & 0.315 & 0.238 \\ 
PXZ-ND & 1.923 & 90 & 91 & 1.827 & 2.558 & 2.534 & 2.982 & 2.937 & 2.130 & 2.117 & 0.303 & 0.290 & 0.731 & 0.707 & 0.852 & 0.820 & 415.775 & 422.160 & 582.211 & 585.629 & 0.891 & 0.759 & 166.436 & 163.469 & 0.542 & 1.528 \\ 
CPPyC & 2.677 & 89 & 90 & 2.614 & 3.436 & 3.414 & 3.852 & 3.789 & 2.930 & 2.901 & 0.316 & 0.287 & 0.822 & 0.800 & 0.921 & 0.888 & 321.903 & 327.213 & 423.136 & 427.312 & 0.205 & 0.171 & 101.233 & 100.099 & 0.400 & 2.431 \\ 
DMAC-ND & 2.114 & 102 & 103 & 2.019 & 2.778 & 2.751 & 3.265 & 3.206 & 2.374 & 2.353 & 0.354 & 0.334 & 0.759 & 0.732 & 0.892 & 0.853 & 379.702 & 386.750 & 522.350 & 526.892 & 0.952 & 0.805 & 142.648 & 140.143 & 0.467 & 1.031 \\ 
PrDPhAc & 2.618 & 137 & 138 & 2.335 & 3.242 & 3.213 & 3.897 & 3.835 & 2.808 & 2.787 & 0.472 & 0.451 & 0.907 & 0.878 & 1.090 & 1.048 & 318.112 & 323.330 & 441.585 & 444.883 & 0.572 & 0.476 & 123.473 & 121.553 & 0.644 & 0.424 \\ 
2Mi2SB & 2.551 & 133 & 134 & 2.784 & 4.176 & 4.149 & 4.695 & 4.649 & 3.130 & 3.120 & 0.346 & 0.336 & 1.392 & 1.365 & 1.565 & 1.529 & 264.071 & 266.690 & 396.066 & 397.445 & 0.129 & 0.117 & 131.994 & 130.755 & 0.283 & 0.322 \\ 
BFDMAc-NAI & 1.222 & 117 & 118 & 1.826 & 2.416 & 2.401 & 2.554 & 2.544 & 1.930 & 1.934 & 0.104 & 0.109 & 0.590 & 0.575 & 0.623 & 0.610 & 485.508 & 487.340 & 642.331 & 640.938 & 0.091 & 0.086 & 156.823 & 153.598 & 0.270 & 4.474 \\ 
HPIPXZ & 2.518 & 60 & 61 & 2.283 & 3.174 & 3.134 & 3.722 & 3.665 & 2.677 & 2.670 & 0.394 & 0.387 & 0.891 & 0.851 & 1.045 & 0.995 & 333.103 & 338.256 & 463.136 & 464.330 & 0.609 & 0.557 & 130.034 & 126.074 & 0.759 & 1.989 \\ 
3BPy-mDTC & 1.642 & 142 & 143 & 1.978 & 3.299 & 3.289 & 3.558 & 3.530 & 2.133 & 2.123 & 0.155 & 0.145 & 1.321 & 1.311 & 1.425 & 1.407 & 348.417 & 351.250 & 581.152 & 584.031 & 0.091 & 0.083 & 232.735 & 232.781 & 0.197 & 6.020 \\ 
2BPy-mDTC & 1.440 & 142 & 143 & 1.713 & 3.218 & 3.210 & 3.368 & 3.358 & 1.793 & 1.793 & 0.080 & 0.079 & 1.505 & 1.496 & 1.575 & 1.565 & 368.146 & 369.198 & 691.397 & 691.564 & 0.035 & 0.036 & 323.251 & 322.365 & 0.208 & 5.940 \\ 
BP-mDTC & 1.847 & 142 & 143 & 2.182 & 3.397 & 3.382 & 3.698 & 3.665 & 2.375 & 2.365 & 0.193 & 0.183 & 1.215 & 1.200 & 1.323 & 1.301 & 335.310 & 338.256 & 522.025 & 524.286 & 0.166 & 0.164 & 186.716 & 186.031 & 0.230 & 5.256 \\ 
Cz2ICz & 2.269 & 104 & 105 & 2.499 & 3.142 & 3.123 & 3.493 & 3.437 & 2.778 & 2.750 & 0.279 & 0.251 & 0.643 & 0.624 & 0.715 & 0.687 & 354.971 & 360.734 & 446.270 & 450.816 & 0.413 & 0.355 & 91.300 & 90.082 & 0.409 & 1.788 \\ 
Ac-BPCN & 1.244 & 98 & 99 & 1.080 & 2.070 & 2.030 & 2.671 & 2.583 & 1.393 & 1.374 & 0.313 & 0.294 & 0.990 & 0.950 & 1.277 & 1.209 & 464.239 & 480.001 & 889.778 & 902.258 & 0.469 & 0.376 & 425.539 & 422.257 & 0.498 & 0.853 \\ 
5CzICz & 2.401 & 74 & 75 & 2.646 & 3.200 & 3.181 & 3.580 & 3.519 & 2.961 & 2.928 & 0.314 & 0.282 & 0.554 & 0.534 & 0.620 & 0.591 & 346.286 & 352.288 & 418.780 & 423.429 & 0.258 & 0.224 & 72.494 & 71.141 & 0.354 & 5.688 \\ 
DCPDAPM & 1.449 & 133 & 134 & 2.093 & 3.338 & 3.332 & 3.450 & 3.444 & 2.163 & 2.163 & 0.070 & 0.070 & 1.245 & 1.239 & 1.287 & 1.280 & 359.343 & 360.042 & 573.093 & 573.090 & 0.130 & 0.124 & 213.750 & 213.048 & 0.183 & 6.323 \\ 
SPFS-PXZ & 2.235 & 133 & 134 & 2.485 & 2.905 & 2.875 & 3.290 & 3.256 & 2.814 & 2.814 & 0.329 & 0.329 & 0.420 & 0.391 & 0.476 & 0.442 & 376.863 & 380.728 & 440.613 & 440.581 & 0.014 & 0.011 & 63.749 & 59.852 & 0.101 & 1.977 \\ 
DPS-PXZ & 1.885 & 104 & 105 & 2.268 & 2.978 & 2.949 & 3.356 & 3.323 & 2.556 & 2.555 & 0.288 & 0.287 & 0.710 & 0.681 & 0.800 & 0.768 & 369.440 & 373.143 & 485.137 & 485.244 & 0.039 & 0.025 & 115.697 & 112.101 & 0.380 & 3.645 \\ 
TX-CzPh & 2.005 & 80 & 81 & 2.234 & 2.884 & 2.859 & 3.596 & 3.485 & 2.785 & 2.723 & 0.551 & 0.489 & 0.650 & 0.625 & 0.811 & 0.762 & 344.812 & 355.775 & 445.175 & 455.300 & 0.170 & 0.131 & 100.363 & 99.524 & 0.288 & 7.202 \\ 
bpipH & 1.787 & 57 & 58 & 2.264 & 3.203 & 3.171 & 3.839 & 3.764 & 2.714 & 2.687 & 0.450 & 0.423 & 0.938 & 0.907 & 1.125 & 1.077 & 322.943 & 329.404 & 456.811 & 461.411 & 0.582 & 0.515 & 133.869 & 132.007 & 0.159 & 6.353 \\ 
Tri-PXZ-PCN & 0.983 & 164 & 165 & 1.558 & 2.582 & 2.572 & 2.868 & 2.849 & 1.731 & 1.726 & 0.173 & 0.168 & 1.024 & 1.013 & 1.138 & 1.123 & 432.257 & 435.154 & 716.390 & 718.204 & 0.612 & 0.545 & 284.133 & 283.049 & 0.078 & 8.426 \\ 
ACID–BPPZ & 1.051 & 138 & 139 & 1.323 & 2.864 & 2.841 & 3.305 & 3.273 & 1.527 & 1.524 & 0.204 & 0.201 & 1.541 & 1.518 & 1.778 & 1.749 & 375.085 & 378.751 & 811.921 & 813.358 & 0.127 & 0.002 & 436.836 & 434.607 & 0.166 & 7.987 \\ 
C-BPyIA & 1.971 & 175 & 176 & 1.684 & 2.290 & 2.223 & 3.265 & 3.110 & 2.402 & 2.357 & 0.717 & 0.672 & 0.605 & 0.538 & 0.863 & 0.753 & 379.772 & 398.676 & 516.253 & 526.069 & 0.957 & 0.668 & 136.481 & 127.393 & 0.501 & 0.293 \\ 
N-BPyIA & 1.788 & 175 & 176 & 1.720 & 2.251 & 2.181 & 3.188 & 3.022 & 2.435 & 2.383 & 0.716 & 0.663 & 0.531 & 0.461 & 0.752 & 0.639 & 388.970 & 410.245 & 509.099 & 520.268 & 0.733 & 0.519 & 120.129 & 110.023 & 0.084 & 7.287 \\ 
2-TA-AN & 2.017 & 66 & 67 & 1.762 & 2.318 & 2.245 & 3.405 & 3.225 & 2.589 & 2.531 & 0.826 & 0.768 & 0.556 & 0.483 & 0.816 & 0.694 & 364.177 & 384.495 & 478.978 & 489.883 & 0.392 & 0.271 & 114.800 & 105.388 & 0.428 & 5.589 \\ 
ANOP-MeFAC & 0.724 & 110 & 111 & 0.841 & 2.034 & 2.015 & 2.305 & 2.281 & 0.954 & 0.952 & 0.112 & 0.111 & 1.193 & 1.174 & 1.352 & 1.329 & 537.799 & 543.457 & 1300.012 & 1301.675 & 0.280 & 0.255 & 762.213 & 758.218 & 0.242 & 7.746 \\ 
ANOP-DMAC & 0.733 & 83 & 84 & 0.846 & 2.244 & 2.227 & 2.453 & 2.436 & 0.925 & 0.925 & 0.079 & 0.079 & 1.398 & 1.381 & 1.528 & 1.510 & 505.542 & 509.008 & 1340.588 & 1339.852 & 0.188 & 0.172 & 835.045 & 830.844 & 0.209 & 7.759 \\ 
4PyCNICz & 1.527 & 121 & 122 & 1.939 & 3.378 & 3.352 & 3.762 & 3.716 & 2.160 & 2.149 & 0.221 & 0.210 & 1.439 & 1.413 & 1.603 & 1.566 & 329.552 & 333.695 & 574.109 & 576.885 & 0.133 & 0.129 & 244.556 & 243.190 & 0.091 & 8.395 \\ 
2PyCNBCz & 1.582 & 135 & 136 & 1.906 & 3.387 & 3.365 & 3.824 & 3.780 & 2.152 & 2.141 & 0.246 & 0.235 & 1.481 & 1.459 & 1.672 & 1.639 & 324.235 & 328.027 & 576.088 & 579.056 & 1.342 & 1.109 & 251.853 & 251.030 & 0.199 & 11.400 \\ 
CzA-PPO & 1.627 & 148 & 149 & 1.572 & 1.906 & 1.850 & 2.423 & 2.367 & 1.999 & 2.011 & 0.427 & 0.439 & 0.334 & 0.278 & 0.424 & 0.356 & 511.697 & 523.825 & 620.358 & 616.569 & 0.298 & 0.262 & 108.661 & 92.743 & 0.586 & 2.667 \\ 
2PyCNICz & 1.619 & 121 & 122 & 1.906 & 3.365 & 3.340 & 3.743 & 3.692 & 2.120 & 2.107 & 0.214 & 0.201 & 1.459 & 1.434 & 1.623 & 1.585 & 331.234 & 335.800 & 584.790 & 588.325 & 0.214 & 0.200 & 253.556 & 252.525 & 0.170 & 8.044 \\ 
TAA-PPO & 1.634 & 118 & 119 & 1.570 & 1.914 & 1.859 & 2.430 & 2.374 & 1.993 & 2.006 & 0.423 & 0.436 & 0.344 & 0.288 & 0.437 & 0.369 & 510.244 & 522.215 & 622.035 & 618.169 & 0.291 & 0.258 & 111.791 & 95.954 & 0.584 & 2.667 \\ 
pSFIAc2 & 2.291 & 163 & 164 & 2.266 & 2.664 & 2.641 & 3.096 & 3.011 & 2.633 & 2.584 & 0.367 & 0.318 & 0.398 & 0.375 & 0.463 & 0.427 & 400.505 & 411.730 & 470.922 & 479.833 & 0.421 & 0.339 & 70.417 & 68.103 & 0.662 & 0.291 \\ 
TBN-TPA & 2.363 & 179 & 180 & 2.425 & 2.686 & 2.663 & 3.145 & 3.067 & 2.839 & 2.793 & 0.414 & 0.369 & 0.261 & 0.238 & 0.306 & 0.274 & 394.277 & 404.200 & 436.706 & 443.879 & 0.439 & 0.354 & 42.430 & 39.680 & 0.587 & 0.623 \\ 
CzBPDCb & 2.800 & 89 & 90 & 2.763 & 3.322 & 3.297 & 3.838 & 3.764 & 3.191 & 3.154 & 0.429 & 0.392 & 0.560 & 0.534 & 0.646 & 0.610 & 323.052 & 329.412 & 388.491 & 393.087 & 0.193 & 0.163 & 65.439 & 63.675 & 0.330 & 4.259 \\ 
{[2,1-b]IF} & 0.529 & 107 & 108 & 0.456 & 0.255 & 0.121 & 0.672 & 0.562 & 1.202 & 2.115 & 0.745 & 1.658 & -0.201 & -0.335 & -0.529 & -1.553 & 1843.905 & 2206.910 & 1031.891 & 586.316 & 0.006 & 0.002 & -812.015 & -1620.594 & 0.569 & 3.120 \\ 
cyclohexanone & 3.031 & 79 & 80 & 2.667 & 3.783 & 3.746 & 4.554 & 4.491 & 3.211 & 3.198 & 0.543 & 0.531 & 1.116 & 1.078 & 1.343 & 1.293 & 272.259 & 276.066 & 386.175 & 387.683 & 0.369 & 0.417 & 113.916 & 111.617 & 0.792 & 0.978 \\ 
thio-ether & 0.529 & 107 & 108 & 0.456 & 0.255 & 0.121 & 0.672 & 0.562 & 1.201 & 2.114 & 0.745 & 1.658 & -0.201 & -0.335 & -0.529 & -1.553 & 1843.905 & 2206.910 & 1032.423 & 586.388 & 0.006 & 0.002 & -811.483 & -1620.522 & 0.569 & 3.120 \\ 
ICz-2 & 2.301 & 69 & 70 & 1.419 & 3.866 & 3.833 & 4.088 & 4.078 & 1.500 & 1.510 & 0.081 & 0.091 & 2.447 & 2.413 & 2.587 & 2.568 & 303.325 & 304.054 & 826.304 & 821.048 & 0.041 & 0.041 & 522.978 & 516.994 & 0.503 & 1.590 \\ 
DDCzTrz & 1.836 & 177 & 178 & 1.959 & 3.562 & 3.542 & 3.884 & 3.853 & 2.136 & 2.131 & 0.177 & 0.172 & 1.603 & 1.584 & 1.748 & 1.722 & 319.242 & 321.778 & 580.419 & 581.891 & 0.145 & 0.140 & 261.177 & 260.113 & 0.271 & 4.426 \\ 
B-O-dpa & 2.429 & 75 & 76 & 2.538 & 2.704 & 2.679 & 3.243 & 3.152 & 3.044 & 2.986 & 0.506 & 0.448 & 0.166 & 0.141 & 0.199 & 0.166 & 382.290 & 393.338 & 407.316 & 415.213 & 0.370 & 0.291 & 25.026 & 21.875 & 0.599 & 1.539 \\ 
B-dpa-SpiroAC & 2.233 & 118 & 119 & 2.309 & 2.537 & 2.514 & 2.983 & 2.910 & 2.715 & 2.673 & 0.406 & 0.364 & 0.227 & 0.205 & 0.267 & 0.237 & 415.678 & 426.077 & 456.599 & 463.889 & 0.578 & 0.470 & 40.922 & 37.812 & 0.568 & 1.437 \\ 
DCz-OTP & 2.880 & 103 & 104 & 2.822 & 3.408 & 3.386 & 3.835 & 3.770 & 3.175 & 3.142 & 0.353 & 0.320 & 0.587 & 0.564 & 0.660 & 0.628 & 323.296 & 328.862 & 390.532 & 394.620 & 0.121 & 0.103 & 67.235 & 65.758 & 0.272 & 4.622 \\ 
B-dpa-Cz & 2.214 & 88 & 89 & 2.298 & 2.567 & 2.543 & 3.058 & 2.981 & 2.738 & 2.694 & 0.440 & 0.395 & 0.269 & 0.245 & 0.320 & 0.287 & 405.416 & 415.957 & 452.852 & 460.300 & 0.614 & 0.490 & 47.436 & 44.344 & 0.582 & 1.557 \\ 
c-D2T & 1.558 & 234 & 235 & 1.917 & 3.344 & 3.334 & 3.560 & 3.547 & 2.041 & 2.040 & 0.124 & 0.123 & 1.427 & 1.417 & 1.519 & 1.507 & 348.251 & 349.537 & 607.555 & 607.884 & 0.290 & 0.268 & 259.304 & 258.347 & 0.044 & 7.546 \\ 
DPXZ-DPPM & 0.915 & 136 & 137 & 1.033 & 2.620 & 2.609 & 2.885 & 2.865 & 1.137 & 1.134 & 0.105 & 0.101 & 1.587 & 1.576 & 1.748 & 1.731 & 429.680 & 432.770 & 1090.158 & 1093.303 & 0.593 & 0.539 & 660.478 & 660.534 & 0.325 & 6.970 \\ 
CBPMCN & 1.961 & 102 & 103 & 2.210 & 3.462 & 3.439 & 3.874 & 3.829 & 2.473 & 2.461 & 0.263 & 0.251 & 1.252 & 1.229 & 1.401 & 1.368 & 320.025 & 323.820 & 501.268 & 503.885 & 0.669 & 0.562 & 181.243 & 180.066 & 0.201 & 5.895 \\ 
CPBPMCN & 1.928 & 116 & 117 & 2.179 & 3.471 & 3.443 & 3.874 & 3.831 & 2.432 & 2.424 & 0.253 & 0.246 & 1.293 & 1.264 & 1.443 & 1.407 & 320.009 & 323.617 & 509.890 & 511.391 & 0.556 & 0.497 & 189.881 & 187.774 & 0.108 & 10.468 \\ 
TPB-AC & 2.022 & 106 & 107 & 2.313 & 3.384 & 3.360 & 3.867 & 3.837 & 2.642 & 2.641 & 0.330 & 0.329 & 1.072 & 1.048 & 1.224 & 1.196 & 320.638 & 323.086 & 469.217 & 469.433 & 0.988 & 0.885 & 148.579 & 146.347 & 0.206 & 10.559 \\ 
Me-DMAC & 1.369 & 82 & 83 & 2.238 & 3.427 & 3.394 & 3.598 & 3.589 & 2.349 & 2.366 & 0.112 & 0.128 & 1.189 & 1.157 & 1.248 & 1.223 & 344.630 & 345.446 & 527.759 & 524.053 & 0.184 & 0.173 & 183.129 & 178.607 & 0.052 & 7.690 \\ 
iTPBI-CN & 2.393 & 124 & 125 & 2.536 & 3.822 & 3.793 & 4.234 & 4.208 & 2.809 & 2.813 & 0.273 & 0.277 & 1.286 & 1.257 & 1.425 & 1.394 & 292.844 & 294.667 & 441.381 & 440.725 & 0.216 & 0.204 & 148.537 & 146.058 & 0.214 & 3.990 \\ 
TCP & 3.062 & 105 & 106 & 3.006 & 3.442 & 3.418 & 3.937 & 3.877 & 3.439 & 3.410 & 0.433 & 0.404 & 0.435 & 0.411 & 0.498 & 0.466 & 314.912 & 319.827 & 360.530 & 363.571 & 0.350 & 0.292 & 45.617 & 43.744 & 0.444 & 2.016 \\ 
CDBP-BP-PXZ & 1.653 & 147 & 148 & 2.183 & 2.744 & 2.713 & 3.106 & 3.070 & 2.471 & 2.470 & 0.288 & 0.287 & 0.561 & 0.530 & 0.635 & 0.600 & 399.202 & 403.910 & 501.835 & 502.017 & 0.017 & 0.014 & 102.633 & 98.107 & 0.257 & 6.188 \\ 
CDBP-BP-DMAC & 1.716 & 153 & 154 & 2.240 & 3.339 & 3.316 & 3.612 & 3.607 & 2.423 & 2.437 & 0.183 & 0.197 & 1.099 & 1.076 & 1.189 & 1.171 & 343.275 & 343.713 & 511.741 & 508.834 & 0.193 & 0.201 & 168.466 & 165.121 & 0.157 & 6.271 \\ 
3CzPhpPM & 2.151 & 101 & 102 & 2.046 & 3.422 & 3.400 & 3.825 & 3.764 & 2.287 & 2.264 & 0.241 & 0.219 & 1.376 & 1.355 & 1.538 & 1.499 & 324.133 & 329.430 & 542.176 & 547.541 & 0.450 & 0.356 & 218.042 & 218.111 & 0.477 & 1.454 \\ 
SFI23pPM & 2.147 & 130 & 131 & 2.043 & 3.420 & 3.397 & 3.809 & 3.754 & 2.276 & 2.258 & 0.233 & 0.215 & 1.376 & 1.354 & 1.533 & 1.496 & 325.486 & 330.246 & 544.693 & 549.087 & 0.377 & 0.299 & 219.207 & 218.841 & 0.480 & 1.447 \\ 
3PCzPFP & 2.387 & 75 & 76 & 2.688 & 3.381 & 3.358 & 3.827 & 3.755 & 3.043 & 3.005 & 0.355 & 0.318 & 0.693 & 0.670 & 0.784 & 0.749 & 323.972 & 330.228 & 407.462 & 412.541 & 0.167 & 0.139 & 83.490 & 82.313 & 0.201 & 7.244 \\ 
SFI34pPM & 2.129 & 130 & 131 & 2.029 & 3.384 & 3.362 & 3.750 & 3.694 & 2.249 & 2.229 & 0.220 & 0.200 & 1.355 & 1.333 & 1.501 & 1.464 & 330.607 & 335.673 & 551.286 & 556.128 & 0.388 & 0.311 & 220.680 & 220.455 & 0.328 & 7.448 \\ 
SBA-2DPS & 2.262 & 138 & 139 & 2.681 & 3.478 & 3.448 & 4.069 & 4.030 & 3.137 & 3.134 & 0.456 & 0.453 & 0.796 & 0.767 & 0.932 & 0.896 & 304.727 & 307.623 & 395.243 & 395.580 & 0.085 & 0.061 & 90.516 & 87.957 & 0.237 & 0.462 \\ 
2DMAC-BP-F & 1.356 & 132 & 133 & 1.144 & 2.540 & 2.512 & 3.125 & 3.055 & 1.408 & 1.392 & 0.263 & 0.247 & 1.396 & 1.367 & 1.717 & 1.663 & 396.788 & 405.880 & 880.803 & 890.772 & 0.895 & 0.757 & 484.015 & 484.892 & 0.545 & 0.239 \\ 
DCA & 2.103 & 77 & 78 & 1.715 & 2.237 & 2.167 & 3.242 & 3.066 & 2.485 & 2.427 & 0.770 & 0.712 & 0.522 & 0.452 & 0.757 & 0.639 & 382.431 & 404.371 & 498.847 & 510.845 & 0.486 & 0.350 & 116.415 & 106.474 & 0.915 & 0.013 \\ 
DPFPhe & 2.222 & 113 & 114 & 1.921 & 2.391 & 2.334 & 3.122 & 3.044 & 2.508 & 2.506 & 0.587 & 0.585 & 0.470 & 0.412 & 0.613 & 0.538 & 397.169 & 407.293 & 494.302 & 494.693 & 0.147 & 0.106 & 97.134 & 87.399 & 0.106 & 5.406 \\ 
DFPFPhe & 2.147 & 119 & 120 & 1.948 & 2.500 & 2.459 & 3.163 & 3.088 & 2.465 & 2.446 & 0.517 & 0.498 & 0.551 & 0.511 & 0.698 & 0.641 & 392.032 & 401.555 & 502.985 & 506.795 & 0.136 & 0.105 & 110.953 & 105.239 & 0.069 & 6.435 \\ 
3ai & 2.231 & 98 & 99 & 1.865 & 2.539 & 2.482 & 3.637 & 3.458 & 2.671 & 2.598 & 0.806 & 0.733 & 0.674 & 0.617 & 0.966 & 0.860 & 340.916 & 358.574 & 464.190 & 477.198 & 0.797 & 0.547 & 123.274 & 118.623 & 0.397 & 6.456 \\ 
DNFPh & 2.104 & 131 & 132 & 1.740 & 2.261 & 2.218 & 2.980 & 2.902 & 2.294 & 2.276 & 0.554 & 0.536 & 0.521 & 0.478 & 0.687 & 0.625 & 416.012 & 427.281 & 540.552 & 544.684 & 0.100 & 0.071 & 124.539 & 117.403 & 0.085 & 4.629 \\ 
pCzAnBzt & 1.935 & 95 & 96 & 1.686 & 2.279 & 2.208 & 3.285 & 3.122 & 2.430 & 2.383 & 0.744 & 0.697 & 0.593 & 0.523 & 0.855 & 0.739 & 377.425 & 397.105 & 510.305 & 520.282 & 0.674 & 0.475 & 132.880 & 123.177 & 0.378 & 7.302 \\ 
DPE-DPXZ & 1.814 & 99 & 100 & 2.127 & 2.860 & 2.829 & 3.244 & 3.208 & 2.412 & 2.411 & 0.285 & 0.285 & 0.733 & 0.702 & 0.832 & 0.796 & 382.231 & 386.533 & 514.059 & 514.137 & 0.002 & 0.002 & 131.828 & 127.605 & 0.363 & 0.162 \\ 
3CzAnBzt & 2.025 & 95 & 96 & 1.685 & 2.243 & 2.173 & 3.250 & 3.101 & 2.441 & 2.404 & 0.756 & 0.720 & 0.558 & 0.488 & 0.809 & 0.697 & 381.502 & 399.820 & 507.925 & 515.677 & 0.732 & 0.529 & 126.423 & 115.856 & 0.766 & 2.758 \\ 
TABD-COOH & 2.226 & 83 & 84 & 1.371 & 2.629 & 2.585 & 3.343 & 3.289 & 1.743 & 1.744 & 0.372 & 0.373 & 1.258 & 1.214 & 1.600 & 1.545 & 370.866 & 376.955 & 711.293 & 710.816 & 0.565 & 0.473 & 340.427 & 333.862 & 0.813 & 1.284 \\ 
ADN & 2.101 & 79 & 80 & 1.709 & 2.249 & 2.178 & 3.228 & 3.063 & 2.452 & 2.403 & 0.744 & 0.694 & 0.541 & 0.470 & 0.776 & 0.661 & 384.030 & 404.754 & 505.542 & 516.028 & 0.636 & 0.453 & 121.512 & 111.274 & 0.932 & 0.031 \\ 
Et3SiH & 2.796 & 164 & 165 & 2.665 & 3.567 & 3.535 & 4.176 & 4.125 & 3.120 & 3.110 & 0.455 & 0.445 & 0.902 & 0.870 & 1.056 & 1.015 & 296.869 & 300.560 & 397.335 & 398.645 & 0.043 & 0.036 & 100.466 & 98.084 & 0.657 & 1.657 \\ 
DPE-DDMAc & 1.914 & 111 & 112 & 2.257 & 3.409 & 3.377 & 3.673 & 3.670 & 2.432 & 2.453 & 0.175 & 0.196 & 1.152 & 1.120 & 1.242 & 1.217 & 337.519 & 337.804 & 509.836 & 505.461 & 0.156 & 0.152 & 172.317 & 167.657 & 0.197 & 3.959 \\ 
mCz-TAn-CN & 2.076 & 119 & 120 & 1.705 & 2.301 & 2.236 & 3.223 & 3.072 & 2.388 & 2.343 & 0.683 & 0.638 & 0.596 & 0.530 & 0.835 & 0.729 & 384.686 & 403.555 & 519.136 & 529.077 & 0.540 & 0.391 & 134.451 & 125.522 & 0.800 & 2.167 \\ 
indenoacridine & 1.156 & 49 & 50 & 1.049 & 1.262 & 1.175 & 2.215 & 2.033 & 1.842 & 1.816 & 0.793 & 0.767 & 0.212 & 0.125 & 0.373 & 0.217 & 559.849 & 609.768 & 673.094 & 682.609 & 0.526 & 0.356 & 113.245 & 72.841 & 0.827 & 1.575 \\ 
MPAc & 3.350 & 68 & 69 & 3.007 & 3.736 & 3.707 & 4.266 & 4.202 & 3.433 & 3.409 & 0.426 & 0.402 & 0.730 & 0.700 & 0.833 & 0.793 & 290.667 & 295.053 & 361.194 & 363.700 & 0.093 & 0.079 & 70.527 & 68.647 & 0.510 & 1.933 \\ 
TBAc & 2.760 & 126 & 127 & 1.194 & 3.094 & 3.043 & 3.866 & 3.818 & 1.492 & 1.499 & 0.298 & 0.304 & 1.900 & 1.849 & 2.374 & 2.320 & 320.679 & 324.702 & 830.717 & 827.193 & 0.028 & 0.023 & 510.038 & 502.491 & 0.349 & 1.537 \\ 
poCz-SO & 3.334 & 99 & 100 & 3.130 & 3.540 & 3.516 & 3.980 & 3.903 & 3.519 & 3.475 & 0.389 & 0.345 & 0.410 & 0.386 & 0.461 & 0.428 & 311.510 & 317.656 & 352.287 & 356.801 & 0.069 & 0.059 & 40.776 & 39.145 & 0.672 & 0.474 \\ 
H4TCPE & 3.371 & 95 & 96 & 2.631 & 4.305 & 4.271 & 4.718 & 4.678 & 2.884 & 2.882 & 0.253 & 0.251 & 1.673 & 1.640 & 1.834 & 1.796 & 262.801 & 265.031 & 429.936 & 430.200 & 0.016 & 0.014 & 167.135 & 165.169 & 0.604 & 2.715 \\ 
CbBPCb & 2.999 & 89 & 90 & 2.923 & 3.478 & 3.456 & 3.933 & 3.869 & 3.306 & 3.272 & 0.383 & 0.349 & 0.555 & 0.533 & 0.627 & 0.597 & 315.249 & 320.489 & 375.070 & 378.925 & 0.285 & 0.244 & 59.822 & 58.437 & 0.557 & 0.620 \\ 
TMOE & 2.520 & 86 & 87 & 1.630 & 2.911 & 2.873 & 3.677 & 3.615 & 2.059 & 2.052 & 0.429 & 0.421 & 1.281 & 1.242 & 1.617 & 1.563 & 337.216 & 342.972 & 602.073 & 604.313 & 0.704 & 0.580 & 264.857 & 261.342 & 0.899 & 0.005 \\ 
FAPbCl3 & 3.474 & 71 & 72 & 2.828 & 4.199 & 4.158 & 4.582 & 4.560 & 3.086 & 3.102 & 0.258 & 0.274 & 1.371 & 1.330 & 1.496 & 1.459 & 270.572 & 271.871 & 401.733 & 399.712 & 0.000 & 0.000 & 131.161 & 127.840 & 0.896 & 0.108 \\ 
DBT-SADF & 1.767 & 97 & 98 & 2.515 & 3.462 & 3.432 & 3.822 & 3.812 & 2.777 & 2.794 & 0.262 & 0.279 & 0.947 & 0.916 & 1.045 & 1.018 & 324.354 & 325.281 & 446.411 & 443.756 & 0.025 & 0.023 & 122.057 & 118.475 & 0.195 & 5.276 \\ 
mPXTMP & 2.699 & 84 & 85 & 2.534 & 3.455 & 3.426 & 3.871 & 3.836 & 2.839 & 2.837 & 0.305 & 0.303 & 0.921 & 0.892 & 1.032 & 0.999 & 320.306 & 323.237 & 436.703 & 437.076 & 0.001 & 0.001 & 116.396 & 113.839 & 0.653 & 1.612 \\ 
APDC-tPh & 1.394 & 87 & 88 & 1.383 & 2.726 & 2.682 & 3.272 & 3.237 & 1.660 & 1.670 & 0.277 & 0.287 & 1.343 & 1.299 & 1.612 & 1.568 & 378.948 & 382.998 & 746.972 & 742.605 & 0.056 & 0.061 & 368.024 & 359.607 & 0.335 & 1.843 \\ 
POZDBPHZ & 1.031 & 117 & 118 & 1.126 & 2.876 & 2.849 & 3.041 & 3.029 & 1.191 & 1.197 & 0.064 & 0.071 & 1.750 & 1.723 & 1.850 & 1.831 & 407.762 & 409.351 & 1041.420 & 1035.518 & 0.457 & 0.430 & 633.658 & 626.167 & 0.266 & 3.602 \\ 
CPTBF & 2.966 & 143 & 144 & 2.819 & 3.424 & 3.401 & 3.906 & 3.842 & 3.216 & 3.184 & 0.397 & 0.365 & 0.605 & 0.582 & 0.690 & 0.658 & 317.404 & 322.733 & 385.550 & 389.412 & 0.311 & 0.266 & 68.146 & 66.680 & 0.266 & 5.001 \\ 
trimesitylboron & 2.736 & 72 & 73 & 2.615 & 3.702 & 3.684 & 4.015 & 3.997 & 2.836 & 2.838 & 0.221 & 0.223 & 1.087 & 1.069 & 1.179 & 1.160 & 308.787 & 310.162 & 437.122 & 436.899 & 0.175 & 0.156 & 128.335 & 126.736 & 0.638 & 0.680 \\ 
CMP & 4.129 & 60 & 61 & 2.933 & 4.897 & 4.856 & 5.079 & 5.050 & 3.042 & 3.050 & 0.109 & 0.117 & 1.964 & 1.923 & 2.037 & 2.000 & 244.126 & 245.513 & 407.624 & 406.467 & 0.001 & 0.001 & 163.498 & 160.954 & 0.813 & 0.706 \\ 
CH3OH–CHCl3 & 2.294 & 85 & 86 & 1.910 & 2.704 & 2.634 & 3.678 & 3.602 & 2.598 & 2.612 & 0.688 & 0.702 & 0.794 & 0.724 & 1.080 & 0.990 & 337.143 & 344.238 & 477.276 & 474.669 & 0.059 & 0.550 & 140.133 & 130.431 & 0.938 & 0.080 \\ 
s-triazine & 3.540 & 68 & 69 & 3.156 & 4.865 & 4.845 & 4.920 & 4.888 & 3.191 & 3.184 & 0.035 & 0.028 & 1.709 & 1.689 & 1.728 & 1.704 & 252.026 & 253.655 & 388.534 & 389.430 & 0.008 & 0.008 & 136.508 & 135.775 & 0.361 & 3.034 \\ 
{[BMIM][PF6]} & 3.256 & 70 & 71 & 2.801 & 3.817 & 3.777 & 4.604 & 4.551 & 3.379 & 3.375 & 0.578 & 0.574 & 1.016 & 0.976 & 1.225 & 1.176 & 269.291 & 272.409 & 366.947 & 367.335 & 0.194 & 0.307 & 97.656 & 94.926 & 0.838 & 0.986 \\ 
1SBFN & 2.862 & 81 & 82 & 2.336 & 3.324 & 3.273 & 4.197 & 4.124 & 2.950 & 2.944 & 0.614 & 0.608 & 0.988 & 0.936 & 1.247 & 1.180 & 295.376 & 300.633 & 420.239 & 421.142 & 0.930 & 0.750 & 124.862 & 120.509 & 0.915 & 0.300 \\ 
2SBFN & 2.868 & 81 & 82 & 2.424 & 3.390 & 3.338 & 4.207 & 4.172 & 3.008 & 3.030 & 0.584 & 0.606 & 0.966 & 0.913 & 1.199 & 1.142 & 294.716 & 297.167 & 412.163 & 409.131 & 0.048 & 0.089 & 117.447 & 111.964 & 0.902 & 1.031 \\ 
F2PA & 2.504 & 90 & 91 & 2.452 & 3.052 & 3.023 & 3.541 & 3.509 & 2.845 & 2.845 & 0.393 & 0.394 & 0.600 & 0.572 & 0.697 & 0.664 & 350.109 & 353.322 & 435.851 & 435.729 & 1.061 & 0.931 & 85.742 & 82.407 & 0.629 & 1.944 \\ 
TSBFB & 3.015 & 186 & 187 & 2.552 & 3.734 & 3.695 & 4.485 & 4.448 & 3.065 & 3.072 & 0.513 & 0.520 & 1.182 & 1.143 & 1.420 & 1.376 & 276.442 & 278.767 & 404.458 & 403.632 & 2.207 & 1.962 & 128.016 & 124.865 & 0.615 & 3.623 \\ 
DPPP & 2.123 & 149 & 150 & 1.770 & 2.584 & 2.520 & 3.401 & 3.296 & 2.331 & 2.316 & 0.560 & 0.546 & 0.813 & 0.749 & 1.071 & 0.980 & 364.520 & 376.120 & 531.994 & 535.325 & 0.621 & 0.490 & 167.473 & 159.205 & 0.908 & 0.001 \\ 
TPA-NZP & 1.082 & 90 & 91 & 1.152 & 1.862 & 1.778 & 2.866 & 2.707 & 1.772 & 1.754 & 0.621 & 0.602 & 0.711 & 0.626 & 1.094 & 0.953 & 432.604 & 458.013 & 699.523 & 706.965 & 1.093 & 0.756 & 266.919 & 248.951 & 0.468 & 5.455 \\ 
mTPA-PPI & 2.503 & 113 & 114 & 2.450 & 3.428 & 3.397 & 3.791 & 3.754 & 2.710 & 2.708 & 0.260 & 0.257 & 0.977 & 0.947 & 1.081 & 1.047 & 327.049 & 330.246 & 457.498 & 457.900 & 0.556 & 0.478 & 130.449 & 127.654 & 0.251 & 8.345 \\ 
BSBFB & 3.025 & 129 & 130 & 2.563 & 3.688 & 3.650 & 4.473 & 4.435 & 3.109 & 3.114 & 0.546 & 0.551 & 1.124 & 1.087 & 1.364 & 1.321 & 277.159 & 279.571 & 398.747 & 398.116 & 1.466 & 1.299 & 121.588 & 118.545 & 0.889 & 0.500 \\ 
BN-DBC-Ph2 & 1.148 & 88 & 89 & 1.308 & 1.876 & 1.833 & 2.586 & 2.510 & 1.803 & 1.790 & 0.495 & 0.483 & 0.568 & 0.526 & 0.783 & 0.720 & 479.444 & 493.882 & 687.798 & 692.534 & 0.298 & 0.315 & 208.354 & 198.651 & 0.582 & 3.938 \\ 
TCbTrz & 1.805 & 147 & 148 & 1.961 & 3.368 & 3.347 & 3.745 & 3.717 & 2.181 & 2.178 & 0.220 & 0.217 & 1.407 & 1.386 & 1.564 & 1.539 & 331.048 & 333.596 & 568.502 & 569.373 & 0.381 & 0.348 & 237.454 & 235.777 & 0.133 & 7.603 \\ 
Xm-mCP & 1.931 & 110 & 111 & 2.427 & 3.253 & 3.228 & 3.885 & 3.809 & 2.898 & 2.864 & 0.471 & 0.437 & 0.827 & 0.801 & 0.987 & 0.945 & 319.177 & 325.503 & 427.895 & 432.929 & 0.230 & 0.051 & 108.718 & 107.426 & 0.032 & 7.795 \\ 
Xp-mCP & 2.023 & 110 & 111 & 2.327 & 3.259 & 3.232 & 3.905 & 3.806 & 2.788 & 2.741 & 0.461 & 0.413 & 0.931 & 0.905 & 1.116 & 1.066 & 317.542 & 325.734 & 444.630 & 452.378 & 0.188 & 0.142 & 127.088 & 126.644 & 0.140 & 7.958 \\ 
ethylacetate & 2.223 & 108 & 109 & 1.970 & 3.000 & 2.984 & 3.132 & 3.124 & 2.056 & 2.063 & 0.086 & 0.092 & 1.030 & 1.014 & 1.075 & 1.061 & 395.913 & 396.902 & 602.959 & 601.121 & 0.002 & 0.002 & 207.046 & 204.219 & 0.279 & 6.233 \\ 
3DMACIPN & 1.394 & 143 & 144 & 1.629 & 2.707 & 2.697 & 2.868 & 2.858 & 1.726 & 1.725 & 0.097 & 0.097 & 1.078 & 1.069 & 1.142 & 1.132 & 432.317 & 433.860 & 718.468 & 718.608 & 0.137 & 0.127 & 286.151 & 284.748 & 0.344 & 0.850 \\ 
ICZ & 2.638 & 62 & 63 & 2.566 & 2.771 & 2.740 & 3.338 & 3.229 & 3.091 & 3.024 & 0.525 & 0.458 & 0.205 & 0.174 & 0.247 & 0.205 & 371.477 & 383.983 & 401.173 & 410.039 & 0.121 & 0.093 & 29.696 & 26.056 & 0.693 & 0.072 \\ 
BDAVBi & 2.079 & 129 & 130 & 1.845 & 2.842 & 2.798 & 3.493 & 3.463 & 2.268 & 2.284 & 0.423 & 0.438 & 0.997 & 0.953 & 1.225 & 1.179 & 354.950 & 358.025 & 546.733 & 542.952 & 2.079 & 1.939 & 191.783 & 184.926 & 0.597 & 2.561 \\ 
DPVBi & 2.482 & 95 & 96 & 1.840 & 3.150 & 3.108 & 3.799 & 3.768 & 2.220 & 2.231 & 0.379 & 0.391 & 1.309 & 1.267 & 1.579 & 1.537 & 326.386 & 329.089 & 558.600 & 555.734 & 2.284 & 2.027 & 232.215 & 226.645 & 0.903 & 0.016 \\ 
CBTD2 & 1.238 & 158 & 159 & 1.549 & 2.787 & 2.736 & 3.506 & 3.445 & 1.948 & 1.950 & 0.399 & 0.401 & 1.239 & 1.187 & 1.558 & 1.495 & 353.665 & 359.927 & 636.565 & 635.914 & 2.305 & 1.959 & 282.901 & 275.986 & 0.329 & 1.862 \\ 
MeOCzPCN & 2.093 & 103 & 104 & 2.249 & 2.898 & 2.876 & 3.502 & 3.447 & 2.717 & 2.695 & 0.468 & 0.447 & 0.650 & 0.627 & 0.785 & 0.752 & 354.038 & 359.698 & 456.356 & 460.003 & 0.542 & 0.345 & 102.317 & 100.306 & 0.470 & 2.396 \\ 
Na-DMAC & 1.120 & 122 & 123 & 1.882 & 3.116 & 3.072 & 3.564 & 3.561 & 2.152 & 2.181 & 0.270 & 0.299 & 1.235 & 1.190 & 1.413 & 1.380 & 347.831 & 348.212 & 576.141 & 568.499 & 0.141 & 0.139 & 228.310 & 220.288 & 0.035 & 8.380 \\ 
3Py-DMAC & 0.894 & 104 & 105 & 1.645 & 3.430 & 3.398 & 3.566 & 3.558 & 1.710 & 1.723 & 0.065 & 0.078 & 1.785 & 1.753 & 1.855 & 1.836 & 347.694 & 348.427 & 724.846 & 719.660 & 0.255 & 0.240 & 377.152 & 371.234 & 0.054 & 8.164 \\ 
6tBPA & 1.640 & 167 & 168 & 1.485 & 1.825 & 1.767 & 2.389 & 2.308 & 1.945 & 1.940 & 0.460 & 0.454 & 0.339 & 0.282 & 0.445 & 0.368 & 518.871 & 537.310 & 637.459 & 639.241 & 0.483 & 0.389 & 118.588 & 101.931 & 0.708 & 0.012 \\ 
C-O & 2.859 & 100 & 101 & 2.818 & 3.182 & 3.157 & 3.750 & 3.670 & 3.322 & 3.276 & 0.504 & 0.458 & 0.363 & 0.338 & 0.428 & 0.393 & 330.625 & 337.878 & 373.231 & 378.446 & 0.141 & 0.130 & 42.606 & 40.568 & 0.561 & 3.096 \\ 
IDFL-2DPA & 1.926 & 128 & 129 & 2.129 & 2.752 & 2.735 & 3.070 & 3.021 & 2.374 & 2.351 & 0.245 & 0.222 & 0.624 & 0.606 & 0.696 & 0.670 & 403.884 & 410.462 & 522.201 & 527.371 & 0.305 & 0.265 & 118.317 & 116.909 & 0.455 & 2.730 \\ 
ACRF & 1.652 & 83 & 84 & 2.277 & 3.477 & 3.468 & 3.478 & 3.478 & 2.278 & 2.284 & 0.001 & 0.006 & 1.200 & 1.191 & 1.200 & 1.194 & 356.440 & 356.481 & 544.206 & 542.938 & 0.000 & 0.000 & 187.766 & 186.457 & 0.137 & 3.744 \\ 
TPSi-F & 3.438 & 104 & 105 & 2.911 & 3.838 & 3.799 & 4.668 & 4.605 & 3.540 & 3.528 & 0.629 & 0.617 & 0.928 & 0.888 & 1.128 & 1.077 & 265.576 & 269.250 & 350.209 & 351.409 & 0.343 & 0.339 & 84.633 & 82.160 & 0.846 & 1.015 \\ 
PAB & 2.396 & 108 & 109 & 2.460 & 2.712 & 2.690 & 3.163 & 3.089 & 2.869 & 2.824 & 0.409 & 0.365 & 0.253 & 0.231 & 0.295 & 0.265 & 391.921 & 401.373 & 432.166 & 438.999 & 0.390 & 0.316 & 40.245 & 37.626 & 0.570 & 0.948 \\ 
2tPAB & 2.368 & 156 & 157 & 2.432 & 2.709 & 2.688 & 3.149 & 3.076 & 2.827 & 2.783 & 0.394 & 0.351 & 0.277 & 0.255 & 0.322 & 0.292 & 393.751 & 403.096 & 438.616 & 445.430 & 0.419 & 0.340 & 44.865 & 42.334 & 0.583 & 0.697 \\ 
pDTPA-DTPZ & 1.124 & 137 & 138 & 1.095 & 2.424 & 2.381 & 2.947 & 2.874 & 1.331 & 1.322 & 0.236 & 0.227 & 1.329 & 1.286 & 1.615 & 1.553 & 420.742 & 431.354 & 931.218 & 938.122 & 0.563 & 0.425 & 510.476 & 506.768 & 0.370 & 2.281 \\ 
oDTPA-DTPZ & 1.262 & 137 & 138 & 1.154 & 2.495 & 2.456 & 2.980 & 2.906 & 1.378 & 1.365 & 0.224 & 0.212 & 1.341 & 1.302 & 1.602 & 1.541 & 416.082 & 426.576 & 899.647 & 907.992 & 0.041 & 0.030 & 483.565 & 481.416 & 0.411 & 6.309 \\ 
oTPAPO-DTPZ & 1.124 & 126 & 127 & 1.109 & 2.466 & 2.425 & 2.959 & 2.883 & 1.332 & 1.319 & 0.222 & 0.209 & 1.356 & 1.316 & 1.628 & 1.564 & 418.936 & 430.023 & 931.093 & 940.113 & 0.049 & 0.035 & 512.157 & 510.090 & 0.223 & 8.807 \\ 
BPZPP & 1.277 & 145 & 146 & 1.162 & 2.666 & 2.640 & 2.971 & 2.945 & 1.295 & 1.296 & 0.133 & 0.134 & 1.504 & 1.478 & 1.676 & 1.649 & 417.357 & 421.013 & 957.527 & 956.386 & 0.178 & 0.156 & 540.170 & 535.373 & 0.553 & 2.280 \\ 
BIPOCz & 2.767 & 114 & 115 & 2.420 & 3.401 & 3.373 & 3.894 & 3.822 & 2.771 & 2.742 & 0.351 & 0.322 & 0.981 & 0.953 & 1.123 & 1.080 & 318.414 & 324.396 & 447.477 & 452.144 & 0.028 & 0.028 & 129.063 & 127.748 & 0.753 & 1.625 \\ 
tDPAC-BN & 2.351 & 186 & 187 & 2.407 & 2.675 & 2.652 & 3.137 & 3.060 & 2.823 & 2.778 & 0.416 & 0.371 & 0.268 & 0.245 & 0.314 & 0.283 & 395.282 & 405.124 & 439.247 & 446.363 & 0.463 & 0.372 & 43.965 & 41.239 & 0.602 & 0.952 \\ 
tDMAC-BN & 2.282 & 164 & 165 & 2.340 & 2.631 & 2.611 & 3.042 & 2.977 & 2.705 & 2.668 & 0.365 & 0.328 & 0.291 & 0.271 & 0.336 & 0.309 & 407.601 & 416.460 & 458.272 & 464.672 & 0.489 & 0.399 & 50.671 & 48.213 & 0.575 & 0.942 \\ 
2ICz-OXD & 1.961 & 161 & 162 & 2.228 & 3.400 & 3.376 & 3.804 & 3.753 & 2.493 & 2.478 & 0.265 & 0.249 & 1.172 & 1.148 & 1.311 & 1.276 & 325.940 & 330.316 & 497.306 & 500.412 & 0.323 & 0.299 & 171.367 & 170.095 & 0.232 & 7.368 \\ 
SIR-B & 1.622 & 126 & 127 & 2.047 & 3.253 & 3.249 & 3.264 & 3.263 & 2.054 & 2.055 & 0.007 & 0.008 & 1.206 & 1.202 & 1.210 & 1.207 & 379.888 & 380.017 & 603.643 & 603.252 & 0.001 & 0.001 & 223.754 & 223.236 & 0.159 & 4.084 \\ 
SIR-C & 1.634 & 154 & 155 & 2.044 & 3.259 & 3.256 & 3.272 & 3.270 & 2.052 & 2.053 & 0.008 & 0.009 & 1.215 & 1.212 & 1.220 & 1.218 & 378.971 & 379.122 & 604.182 & 603.996 & 0.003 & 0.003 & 225.211 & 224.874 & 0.174 & 4.108 \\ 
SIR-A & 1.645 & 98 & 99 & 2.087 & 3.329 & 3.328 & 3.329 & 3.328 & 2.087 & 2.087 & 0.000 & 0.000 & 1.241 & 1.241 & 1.241 & 1.241 & 372.459 & 372.515 & 593.962 & 593.944 & 0.000 & 0.000 & 221.503 & 221.429 & 0.157 & 4.305 \\ 
TRZ3DPA & 2.145 & 150 & 151 & 2.061 & 2.970 & 2.942 & 3.500 & 3.473 & 2.428 & 2.432 & 0.367 & 0.372 & 0.910 & 0.881 & 1.072 & 1.040 & 354.281 & 357.036 & 510.678 & 509.746 & 1.556 & 1.435 & 156.397 & 152.710 & 0.456 & 0.813 \\ 
BO3N & 1.793 & 117 & 118 & 1.530 & 2.027 & 1.951 & 3.002 & 2.892 & 2.265 & 2.267 & 0.735 & 0.738 & 0.498 & 0.421 & 0.737 & 0.625 & 413.019 & 428.744 & 547.457 & 546.857 & 0.104 & 0.057 & 134.438 & 118.113 & 0.693 & 2.598 \\ 
BPPyA & 1.829 & 143 & 144 & 1.660 & 2.263 & 2.208 & 2.797 & 2.739 & 2.051 & 2.060 & 0.391 & 0.399 & 0.603 & 0.548 & 0.745 & 0.679 & 443.339 & 452.679 & 604.367 & 601.967 & 0.990 & 0.831 & 161.028 & 149.288 & 0.771 & 0.216 \\ 
SiCN2Cz & 2.420 & 138 & 139 & 2.374 & 3.651 & 3.631 & 4.064 & 4.022 & 2.643 & 2.629 & 0.269 & 0.255 & 1.277 & 1.257 & 1.422 & 1.392 & 305.057 & 308.296 & 469.145 & 471.581 & 0.564 & 0.475 & 164.088 & 163.285 & 0.382 & 3.840 \\ 
PhPC & 2.087 & 91 & 92 & 1.720 & 2.259 & 2.187 & 3.306 & 3.139 & 2.518 & 2.469 & 0.798 & 0.749 & 0.539 & 0.467 & 0.789 & 0.670 & 374.994 & 394.930 & 492.449 & 502.119 & 0.610 & 0.428 & 117.455 & 107.190 & 0.725 & 3.531 \\ 
1MOBI & 1.922 & 107 & 108 & 1.611 & 2.394 & 2.340 & 3.147 & 3.072 & 2.118 & 2.115 & 0.507 & 0.504 & 0.783 & 0.729 & 1.029 & 0.957 & 393.976 & 403.634 & 585.348 & 586.244 & 2.638 & 2.142 & 191.373 & 182.610 & 0.824 & 0.035 \\ 
3BrBI & 1.902 & 101 & 102 & 1.645 & 2.723 & 2.667 & 3.475 & 3.433 & 2.100 & 2.118 & 0.455 & 0.473 & 1.078 & 1.022 & 1.376 & 1.315 & 356.738 & 361.196 & 590.420 & 585.503 & 3.907 & 3.423 & 233.682 & 224.307 & 0.698 & 0.153 \\ 
DMBFTX & 2.352 & 108 & 109 & 2.295 & 2.831 & 2.805 & 3.502 & 3.384 & 2.839 & 2.769 & 0.544 & 0.474 & 0.536 & 0.510 & 0.662 & 0.615 & 354.079 & 366.394 & 436.698 & 447.753 & 0.206 & 0.153 & 82.619 & 81.359 & 0.588 & 0.624 \\ 
SBF-AnCN & 2.059 & 108 & 109 & 1.680 & 2.242 & 2.173 & 3.174 & 3.017 & 2.379 & 2.333 & 0.699 & 0.653 & 0.561 & 0.493 & 0.795 & 0.684 & 390.588 & 410.966 & 521.075 & 531.434 & 0.694 & 0.498 & 130.488 & 120.468 & 0.903 & 0.730 \\ 
DMF-AnCN & 2.066 & 87 & 88 & 1.686 & 2.247 & 2.178 & 3.191 & 3.033 & 2.395 & 2.348 & 0.709 & 0.662 & 0.560 & 0.492 & 0.796 & 0.685 & 388.568 & 408.851 & 517.710 & 528.053 & 0.683 & 0.486 & 129.143 & 119.201 & 0.896 & 0.875 \\ 
DPF-AnCN & 2.044 & 109 & 110 & 1.673 & 2.232 & 2.163 & 3.158 & 3.003 & 2.368 & 2.323 & 0.695 & 0.650 & 0.558 & 0.490 & 0.790 & 0.680 & 392.554 & 412.813 & 523.563 & 533.658 & 0.715 & 0.513 & 131.010 & 120.845 & 0.901 & 0.778 \\ 
DPA & 2.138 & 61 & 62 & 1.740 & 2.247 & 2.174 & 3.299 & 3.117 & 2.555 & 2.495 & 0.815 & 0.755 & 0.507 & 0.434 & 0.744 & 0.622 & 375.778 & 397.793 & 485.194 & 496.978 & 0.420 & 0.297 & 109.416 & 99.185 & 0.936 & 0.000 \\ 
TPA–DAP–TPA & 1.862 & 191 & 192 & 1.648 & 2.309 & 2.243 & 3.222 & 3.124 & 2.300 & 2.296 & 0.652 & 0.648 & 0.661 & 0.595 & 0.923 & 0.828 & 384.757 & 396.902 & 539.161 & 540.091 & 2.076 & 1.566 & 154.403 & 143.189 & 0.425 & 0.392 \\ 
AcDbp & 1.023 & 129 & 130 & 1.114 & 3.138 & 3.101 & 3.221 & 3.220 & 1.144 & 1.157 & 0.029 & 0.043 & 2.024 & 1.987 & 2.077 & 2.063 & 384.948 & 385.080 & 1083.988 & 1071.574 & 0.005 & 0.005 & 699.039 & 686.494 & 0.160 & 4.338 \\ 
4-Ac & 3.141 & 90 & 91 & 2.838 & 3.343 & 3.313 & 4.002 & 3.951 & 3.397 & 3.384 & 0.559 & 0.547 & 0.505 & 0.475 & 0.605 & 0.566 & 309.821 & 313.836 & 364.978 & 366.357 & 0.624 & 0.540 & 55.157 & 52.520 & 0.702 & 0.961 \\ 
czpzpy & 2.589 & 57 & 58 & 2.473 & 3.086 & 3.059 & 3.611 & 3.535 & 2.894 & 2.859 & 0.420 & 0.385 & 0.613 & 0.586 & 0.717 & 0.677 & 343.389 & 350.684 & 428.483 & 433.714 & 0.371 & 0.303 & 85.094 & 83.031 & 0.523 & 2.713 \\ 
NyDPO & 1.224 & 118 & 119 & 1.409 & 2.874 & 2.843 & 3.179 & 3.168 & 1.559 & 1.571 & 0.149 & 0.161 & 1.465 & 1.434 & 1.620 & 1.598 & 390.059 & 391.315 & 795.386 & 789.451 & 1.071 & 1.017 & 405.327 & 398.136 & 0.234 & 0.956 \\ 
1MPA & 2.934 & 140 & 141 & 2.762 & 3.698 & 3.681 & 4.090 & 4.066 & 3.055 & 3.051 & 0.293 & 0.289 & 0.936 & 0.919 & 1.036 & 1.015 & 303.118 & 304.944 & 405.896 & 406.432 & 0.439 & 0.392 & 102.779 & 101.488 & 0.498 & 2.838 \\ 
LEt & 2.895 & 101 & 102 & 2.609 & 4.824 & 4.795 & 5.014 & 4.987 & 2.712 & 2.714 & 0.103 & 0.104 & 2.215 & 2.186 & 2.302 & 2.274 & 247.276 & 248.600 & 457.178 & 456.891 & 0.003 & 0.003 & 209.901 & 208.291 & 0.508 & 1.818 \\ 
DC-TC & 1.670 & 147 & 148 & 1.513 & 2.875 & 2.874 & 2.885 & 2.883 & 1.519 & 1.518 & 0.005 & 0.005 & 1.361 & 1.360 & 1.366 & 1.365 & 429.799 & 430.068 & 816.467 & 816.664 & 0.001 & 0.001 & 386.668 & 386.597 & 0.298 & 6.093 \\ 
DC-ACR & 1.132 & 117 & 118 & 1.289 & 2.791 & 2.790 & 2.798 & 2.797 & 1.292 & 1.292 & 0.003 & 0.003 & 1.502 & 1.501 & 1.506 & 1.505 & 443.101 & 443.323 & 959.461 & 959.701 & 0.000 & 0.000 & 516.360 & 516.378 & 0.246 & 5.374 \\ 
1G-F1 & 2.929 & 75 & 76 & 2.623 & 4.331 & 4.284 & 5.137 & 5.108 & 3.111 & 3.128 & 0.488 & 0.505 & 1.708 & 1.661 & 2.026 & 1.980 & 241.365 & 242.726 & 398.555 & 396.415 & 0.000 & 0.000 & 157.190 & 153.690 & 0.469 & 2.043 \\ 
P–Cu–C & 2.904 & 91 & 92 & 2.384 & 4.405 & 4.368 & 4.956 & 4.935 & 2.681 & 2.693 & 0.298 & 0.309 & 2.022 & 1.985 & 2.275 & 2.242 & 250.180 & 251.234 & 462.411 & 460.450 & 0.001 & 0.001 & 212.231 & 209.215 & 0.406 & 2.010 \\ 
BPCP-2CPC & 1.337 & 233 & 234 & 1.975 & 3.216 & 3.198 & 3.500 & 3.478 & 2.148 & 2.147 & 0.174 & 0.172 & 1.242 & 1.224 & 1.351 & 1.331 & 354.281 & 356.522 & 577.092 & 577.475 & 0.150 & 0.134 & 222.811 & 220.952 & 0.015 & 15.727 \\ 
2H-Qz & 1.408 & 113 & 114 & 1.621 & 2.737 & 2.706 & 3.098 & 3.060 & 1.835 & 1.833 & 0.214 & 0.212 & 1.116 & 1.085 & 1.263 & 1.227 & 400.207 & 405.230 & 675.779 & 676.535 & 0.016 & 0.013 & 275.571 & 271.305 & 0.208 & 7.400 \\ 
PPINCN-Cz & 1.525 & 191 & 192 & 1.749 & 2.771 & 2.706 & 3.727 & 3.664 & 2.352 & 2.369 & 0.603 & 0.619 & 1.022 & 0.957 & 1.374 & 1.296 & 332.701 & 338.366 & 527.051 & 523.453 & 1.170 & 1.062 & 194.351 & 185.086 & 0.107 & 13.190 \\ 
PPINCN & 1.772 & 103 & 104 & 1.767 & 2.702 & 2.635 & 3.404 & 3.380 & 2.226 & 2.266 & 0.459 & 0.499 & 0.935 & 0.869 & 1.178 & 1.114 & 364.263 & 366.828 & 557.101 & 547.237 & 0.178 & 0.198 & 192.838 & 180.409 & 0.260 & 3.422 \\ 
BDAPM & 2.446 & 156 & 157 & 2.391 & 3.028 & 3.001 & 3.458 & 3.425 & 2.731 & 2.730 & 0.339 & 0.338 & 0.637 & 0.609 & 0.727 & 0.696 & 358.553 & 361.977 & 454.044 & 454.216 & 1.193 & 1.086 & 95.491 & 92.239 & 0.535 & 1.397 \\ 
12AcCz-PM & 2.198 & 126 & 127 & 2.082 & 3.231 & 3.205 & 3.644 & 3.610 & 2.348 & 2.345 & 0.266 & 0.263 & 1.149 & 1.123 & 1.295 & 1.265 & 340.251 & 343.437 & 527.940 & 528.611 & 0.924 & 0.821 & 187.689 & 185.174 & 0.475 & 1.375 \\ 
23AcCz-PM & 1.663 & 126 & 127 & 1.938 & 3.234 & 3.206 & 3.568 & 3.556 & 2.139 & 2.150 & 0.200 & 0.212 & 1.295 & 1.267 & 1.429 & 1.406 & 347.519 & 348.623 & 579.759 & 576.583 & 0.171 & 0.174 & 232.240 & 227.960 & 0.137 & 7.431 \\ 
CDDPI & 2.273 & 118 & 119 & 2.037 & 3.011 & 2.973 & 3.498 & 3.463 & 2.366 & 2.372 & 0.329 & 0.335 & 0.974 & 0.936 & 1.132 & 1.090 & 354.443 & 358.046 & 523.965 & 522.612 & 0.693 & 0.620 & 169.522 & 164.566 & 0.558 & 1.044 \\ 
DDBP & 2.207 & 134 & 135 & 1.994 & 3.147 & 3.104 & 3.703 & 3.672 & 2.346 & 2.359 & 0.352 & 0.365 & 1.153 & 1.110 & 1.356 & 1.313 & 334.839 & 337.611 & 528.418 & 525.579 & 1.400 & 1.257 & 193.579 & 187.969 & 0.463 & 5.590 \\ 
CCDD & 1.446 & 126 & 127 & 2.103 & 2.854 & 2.833 & 3.294 & 3.220 & 2.428 & 2.390 & 0.324 & 0.287 & 0.750 & 0.730 & 0.866 & 0.830 & 376.417 & 385.032 & 510.720 & 518.693 & 0.230 & 0.181 & 134.303 & 133.661 & 0.247 & 8.310 \\ 
DPNC & 1.685 & 140 & 141 & 2.240 & 2.713 & 2.693 & 3.166 & 3.090 & 2.614 & 2.570 & 0.374 & 0.331 & 0.474 & 0.453 & 0.553 & 0.520 & 391.574 & 401.191 & 474.384 & 482.345 & 0.086 & 0.067 & 82.810 & 81.154 & 0.234 & 6.529 \\ 
LiPr & 2.889 & 113 & 114 & 2.662 & 4.796 & 4.766 & 4.979 & 4.952 & 2.763 & 2.766 & 0.101 & 0.104 & 2.134 & 2.104 & 2.216 & 2.186 & 249.004 & 250.367 & 448.650 & 448.284 & 0.001 & 0.001 & 199.646 & 197.917 & 0.522 & 1.907 \\ 
Spiro-CN & 1.207 & 140 & 141 & 1.955 & 2.900 & 2.869 & 3.329 & 3.305 & 2.244 & 2.252 & 0.289 & 0.297 & 0.945 & 0.915 & 1.085 & 1.053 & 372.437 & 375.130 & 552.567 & 550.633 & 1.537 & 1.388 & 180.130 & 175.503 & 0.053 & 3.216 \\ 
TMDBP & 3.219 & 65 & 66 & 2.999 & 3.357 & 3.320 & 3.939 & 3.895 & 3.519 & 3.518 & 0.520 & 0.519 & 0.358 & 0.322 & 0.420 & 0.378 & 314.753 & 318.292 & 352.342 & 352.450 & 0.158 & 0.200 & 37.589 & 34.159 & 0.740 & 1.206 \\ 
ACRSA & 1.837 & 80 & 81 & 2.151 & 3.422 & 3.391 & 3.426 & 3.425 & 2.153 & 2.173 & 0.002 & 0.022 & 1.271 & 1.240 & 1.272 & 1.253 & 361.924 & 361.977 & 575.782 & 570.683 & 0.000 & 0.000 & 213.859 & 208.707 & 0.177 & 4.308 \\ 
CAPI & 1.892 & 139 & 140 & 1.680 & 2.176 & 2.110 & 2.908 & 2.839 & 2.246 & 2.261 & 0.565 & 0.580 & 0.495 & 0.430 & 0.662 & 0.578 & 426.400 & 436.702 & 552.084 & 548.402 & 0.455 & 0.424 & 125.684 & 111.700 & 0.629 & 2.240 \\ 
PhCzSPOTz & 2.233 & 93 & 94 & 2.158 & 3.617 & 3.598 & 4.034 & 3.976 & 2.407 & 2.385 & 0.249 & 0.227 & 1.459 & 1.439 & 1.627 & 1.590 & 307.348 & 311.847 & 515.028 & 519.779 & 0.397 & 0.348 & 207.680 & 207.932 & 0.479 & 1.575 \\ 
CCAPI & 1.512 & 143 & 144 & 1.652 & 2.178 & 2.114 & 2.894 & 2.826 & 2.196 & 2.209 & 0.543 & 0.556 & 0.526 & 0.462 & 0.699 & 0.617 & 428.359 & 438.773 & 564.707 & 561.389 & 0.455 & 0.413 & 136.348 & 122.615 & 0.040 & 9.511 \\ 
2CzCbPy & 2.340 & 105 & 106 & 2.564 & 3.287 & 3.266 & 3.724 & 3.666 & 2.904 & 2.878 & 0.340 & 0.314 & 0.723 & 0.702 & 0.820 & 0.788 & 332.942 & 338.173 & 426.892 & 430.789 & 0.377 & 0.307 & 93.950 & 92.617 & 0.338 & 5.424 \\ 
CzCbPy & 2.417 & 75 & 76 & 2.573 & 3.264 & 3.241 & 3.754 & 3.685 & 2.960 & 2.925 & 0.387 & 0.352 & 0.690 & 0.668 & 0.794 & 0.759 & 330.255 & 336.493 & 418.843 & 423.826 & 0.252 & 0.200 & 88.589 & 87.333 & 0.353 & 5.521 \\ 
DCE & 5.018 & 80 & 81 & 3.108 & 5.213 & 5.171 & 6.037 & 6.032 & 3.599 & 3.625 & 0.491 & 0.518 & 2.105 & 2.063 & 2.438 & 2.407 & 205.377 & 205.530 & 344.488 & 342.000 & 0.017 & 0.018 & 139.111 & 136.470 & 0.880 & 0.275 \\ 
PICFOCz & 2.229 & 125 & 126 & 2.325 & 3.351 & 3.320 & 3.816 & 3.744 & 2.649 & 2.623 & 0.323 & 0.297 & 1.025 & 0.994 & 1.168 & 1.121 & 324.881 & 331.199 & 468.096 & 472.770 & 0.153 & 0.078 & 143.216 & 141.571 & 0.043 & 6.619 \\ 
dpmt & 2.872 & 81 & 82 & 2.515 & 4.056 & 4.011 & 5.105 & 5.076 & 3.165 & 3.183 & 0.650 & 0.668 & 1.541 & 1.496 & 1.940 & 1.893 & 242.873 & 244.256 & 391.731 & 389.523 & 0.001 & 0.001 & 148.858 & 145.267 & 0.537 & 1.648 \\ 
BICFOCz & 2.270 & 126 & 127 & 2.308 & 3.412 & 3.388 & 3.898 & 3.828 & 2.637 & 2.608 & 0.329 & 0.299 & 1.104 & 1.080 & 1.262 & 1.220 & 318.063 & 323.896 & 470.248 & 475.490 & 0.053 & 0.046 & 152.185 & 151.594 & 0.218 & 4.663 \\ 
19a & 2.103 & 79 & 80 & 1.765 & 2.324 & 2.254 & 3.408 & 3.233 & 2.587 & 2.530 & 0.823 & 0.766 & 0.560 & 0.490 & 0.821 & 0.703 & 363.803 & 383.508 & 479.196 & 489.980 & 0.257 & 0.173 & 115.393 & 106.472 & 0.941 & 0.001 \\ 
BTPBFCz & 2.046 & 105 & 106 & 1.969 & 3.322 & 3.302 & 3.771 & 3.711 & 2.235 & 2.213 & 0.266 & 0.244 & 1.353 & 1.333 & 1.536 & 1.498 & 328.748 & 334.072 & 554.676 & 560.232 & 0.147 & 0.124 & 225.928 & 226.159 & 0.221 & 4.324 \\ 
Ph-OBNA & 2.432 & 79 & 80 & 2.593 & 3.070 & 3.051 & 3.467 & 3.414 & 2.929 & 2.903 & 0.336 & 0.309 & 0.476 & 0.457 & 0.538 & 0.512 & 357.592 & 363.121 & 423.278 & 427.163 & 0.172 & 0.145 & 65.686 & 64.042 & 0.544 & 2.919 \\ 
HPVAnt & 2.032 & 70 & 71 & 1.707 & 2.288 & 2.213 & 3.398 & 3.217 & 2.535 & 2.480 & 0.828 & 0.774 & 0.581 & 0.507 & 0.863 & 0.736 & 364.853 & 385.415 & 489.122 & 499.842 & 0.300 & 0.197 & 124.269 & 114.427 & 0.934 & 0.826 \\ 
BTPBFCz-D3 & 1.929 & 165 & 166 & 1.920 & 3.323 & 3.304 & 3.715 & 3.675 & 2.146 & 2.135 & 0.226 & 0.216 & 1.404 & 1.384 & 1.569 & 1.540 & 333.712 & 337.372 & 577.704 & 580.612 & 0.074 & 0.068 & 243.991 & 243.240 & 0.174 & 7.356 \\ 
ICBNTrz4 & 1.792 & 113 & 114 & 1.962 & 3.285 & 3.268 & 3.627 & 3.600 & 2.166 & 2.161 & 0.204 & 0.199 & 1.323 & 1.306 & 1.461 & 1.439 & 341.809 & 344.353 & 572.372 & 573.648 & 0.855 & 0.774 & 230.563 & 229.296 & 0.329 & 7.094 \\ 
1PCTRz & 1.746 & 131 & 132 & 1.979 & 3.384 & 3.360 & 3.823 & 3.766 & 2.237 & 2.218 & 0.257 & 0.239 & 1.404 & 1.381 & 1.587 & 1.548 & 324.286 & 329.211 & 554.344 & 558.871 & 0.569 & 0.398 & 230.058 & 229.660 & 0.162 & 10.140 \\ 
DMACN-B & 2.832 & 133 & 134 & 2.714 & 3.249 & 3.232 & 3.730 & 3.669 & 3.116 & 3.081 & 0.402 & 0.367 & 0.535 & 0.518 & 0.614 & 0.588 & 332.397 & 337.933 & 397.909 & 402.407 & 0.255 & 0.128 & 65.512 & 64.474 & 0.351 & 3.790 \\ 
CzSO-1CO & 2.242 & 100 & 101 & 2.146 & 2.858 & 2.815 & 3.720 & 3.613 & 2.792 & 2.754 & 0.647 & 0.608 & 0.712 & 0.670 & 0.927 & 0.859 & 333.327 & 343.171 & 444.004 & 450.256 & 0.320 & 0.249 & 110.678 & 107.085 & 0.095 & 3.525 \\ 
PPO21 & 3.027 & 113 & 114 & 2.985 & 3.398 & 3.375 & 3.827 & 3.754 & 3.362 & 3.320 & 0.377 & 0.335 & 0.413 & 0.390 & 0.465 & 0.434 & 323.938 & 330.237 & 368.735 & 373.427 & 0.214 & 0.182 & 44.797 & 43.190 & 0.533 & 3.032 \\ 
OXD-7 & 2.627 & 91 & 92 & 2.551 & 3.492 & 3.450 & 4.277 & 4.239 & 3.124 & 3.134 & 0.573 & 0.583 & 0.941 & 0.899 & 1.153 & 1.105 & 289.899 & 292.485 & 396.908 & 395.630 & 2.008 & 1.778 & 107.008 & 103.146 & 0.235 & 5.189 \\ 
TCZ1 & 2.612 & 115 & 116 & 2.711 & 3.149 & 3.126 & 3.616 & 3.542 & 3.113 & 3.071 & 0.402 & 0.360 & 0.438 & 0.415 & 0.503 & 0.470 & 342.896 & 350.070 & 398.313 & 403.689 & 0.059 & 0.048 & 55.417 & 53.620 & 0.450 & 1.849 \\ 
APPT & 1.399 & 64 & 65 & 1.469 & 2.951 & 2.901 & 3.325 & 3.295 & 1.654 & 1.668 & 0.186 & 0.199 & 1.483 & 1.432 & 1.670 & 1.627 & 372.941 & 376.303 & 749.511 & 743.327 & 0.011 & 0.009 & 376.570 & 367.024 & 0.340 & 2.535 \\ 
ANQDC & 1.399 & 54 & 55 & 1.299 & 2.918 & 2.867 & 3.450 & 3.449 & 1.536 & 1.563 & 0.237 & 0.263 & 1.619 & 1.568 & 1.914 & 1.886 & 359.395 & 359.510 & 807.265 & 793.384 & 0.006 & 0.006 & 447.870 & 433.874 & 0.511 & 0.593 \\ 
ECDPTT & 1.737 & 129 & 130 & 1.606 & 3.007 & 2.974 & 3.652 & 3.609 & 1.951 & 1.949 & 0.345 & 0.343 & 1.401 & 1.368 & 1.702 & 1.660 & 339.469 & 343.513 & 635.569 & 636.019 & 0.561 & 0.476 & 296.100 & 292.505 & 0.200 & 9.629 \\ 
1CM & 3.000 & 84 & 85 & 2.911 & 3.044 & 3.018 & 3.575 & 3.482 & 3.418 & 3.358 & 0.507 & 0.447 & 0.133 & 0.107 & 0.157 & 0.124 & 346.819 & 356.113 & 362.722 & 369.237 & 0.083 & 0.064 & 15.903 & 13.124 & 0.701 & 0.742 \\ 
NPE-AcDPS & 2.285 & 138 & 139 & 2.785 & 3.421 & 3.390 & 4.023 & 3.980 & 3.276 & 3.270 & 0.490 & 0.485 & 0.635 & 0.604 & 0.747 & 0.710 & 308.188 & 311.510 & 378.500 & 379.113 & 0.091 & 0.066 & 70.312 & 67.603 & 0.140 & 6.096 \\ 
DMAC-Cz & 2.177 & 109 & 110 & 2.713 & 3.390 & 3.358 & 3.915 & 3.842 & 3.133 & 3.105 & 0.420 & 0.391 & 0.677 & 0.645 & 0.781 & 0.738 & 316.698 & 322.674 & 395.681 & 399.365 & 0.063 & 0.054 & 78.982 & 76.691 & 0.142 & 2.601 \\ 
VBC-PTZ & 1.922 & 96 & 97 & 1.801 & 2.544 & 2.505 & 3.156 & 3.113 & 2.235 & 2.239 & 0.434 & 0.438 & 0.743 & 0.703 & 0.921 & 0.874 & 392.803 & 398.228 & 554.737 & 553.733 & 1.225 & 1.062 & 161.935 & 155.506 & 0.433 & 5.483 \\ 
t-BuPCz & 3.139 & 83 & 84 & 2.857 & 3.469 & 3.445 & 3.873 & 3.805 & 3.190 & 3.155 & 0.333 & 0.298 & 0.612 & 0.589 & 0.683 & 0.650 & 320.100 & 325.811 & 388.683 & 392.938 & 0.043 & 0.037 & 68.583 & 67.127 & 0.632 & 0.505 \\ 
4BPy-mDTC & 1.601 & 142 & 143 & 1.880 & 3.274 & 3.264 & 3.542 & 3.512 & 2.034 & 2.023 & 0.154 & 0.143 & 1.394 & 1.383 & 1.508 & 1.489 & 350.010 & 353.030 & 609.442 & 612.747 & 0.115 & 0.104 & 259.431 & 259.717 & 0.214 & 5.561 \\ 
DC–TC & 3.043 & 120 & 121 & 2.791 & 3.497 & 3.474 & 4.079 & 4.043 & 3.256 & 3.248 & 0.465 & 0.457 & 0.706 & 0.683 & 0.824 & 0.795 & 303.928 & 306.671 & 380.823 & 381.733 & 0.379 & 0.383 & 76.895 & 75.062 & 0.670 & 1.055 \\ 
DFDBQPXZ & 0.851 & 124 & 125 & 1.336 & 2.965 & 2.935 & 3.340 & 3.307 & 1.505 & 1.505 & 0.169 & 0.169 & 1.629 & 1.600 & 1.836 & 1.802 & 371.177 & 374.937 & 823.973 & 824.011 & 0.012 & 0.010 & 452.797 & 449.074 & 0.157 & 7.991 \\ 
DPE & 1.813 & 99 & 100 & 2.126 & 2.861 & 2.830 & 3.244 & 3.208 & 2.411 & 2.410 & 0.284 & 0.284 & 0.735 & 0.703 & 0.833 & 0.797 & 382.195 & 386.509 & 514.284 & 514.380 & 0.005 & 0.004 & 132.088 & 127.871 & 0.362 & 0.059 \\ 
CBZ & 1.529 & 111 & 112 & 2.400 & 3.702 & 3.677 & 3.946 & 3.914 & 2.558 & 2.554 & 0.159 & 0.155 & 1.302 & 1.277 & 1.388 & 1.359 & 314.162 & 316.787 & 484.633 & 485.368 & 0.162 & 0.143 & 170.470 & 168.581 & 0.043 & 7.269 \\ 
tBuCz2 & 2.520 & 139 & 140 & 2.707 & 3.206 & 3.183 & 3.675 & 3.603 & 3.104 & 3.064 & 0.397 & 0.357 & 0.499 & 0.476 & 0.572 & 0.539 & 337.335 & 344.133 & 399.486 & 404.689 & 0.049 & 0.040 & 62.151 & 60.556 & 0.398 & 2.327 \\ 
26DCzPPy & 2.512 & 103 & 104 & 2.587 & 3.406 & 3.382 & 3.825 & 3.757 & 2.905 & 2.873 & 0.318 & 0.286 & 0.819 & 0.796 & 0.919 & 0.884 & 324.176 & 330.000 & 426.781 & 431.476 & 0.279 & 0.237 & 102.605 & 101.477 & 0.113 & 6.544 \\ 
mCBP & 2.896 & 89 & 90 & 2.862 & 3.443 & 3.420 & 3.918 & 3.853 & 3.256 & 3.224 & 0.395 & 0.363 & 0.581 & 0.558 & 0.661 & 0.629 & 316.480 & 321.761 & 380.754 & 384.532 & 0.147 & 0.127 & 64.274 & 62.771 & 0.430 & 2.792 \\ 
benzoxazole & 2.364 & 80 & 81 & 1.911 & 2.991 & 2.950 & 3.663 & 3.605 & 2.340 & 2.335 & 0.429 & 0.424 & 1.080 & 1.039 & 1.322 & 1.270 & 338.514 & 343.904 & 529.757 & 530.885 & 0.309 & 0.268 & 191.243 & 186.981 & 0.630 & 1.828 \\ 
dbG2TAZ & 2.603 & 49 & 50 & 2.271 & 3.049 & 2.998 & 3.648 & 3.595 & 2.718 & 2.723 & 0.447 & 0.452 & 0.778 & 0.727 & 0.931 & 0.871 & 339.822 & 344.928 & 456.162 & 455.316 & 0.040 & 0.038 & 116.340 & 110.388 & 0.871 & 0.063 \\ 
V–TPA & 2.577 & 161 & 162 & 2.596 & 3.464 & 3.440 & 3.837 & 3.805 & 2.876 & 2.872 & 0.280 & 0.276 & 0.867 & 0.843 & 0.961 & 0.933 & 323.120 & 325.845 & 431.078 & 431.703 & 1.076 & 0.937 & 107.958 & 105.857 & 0.042 & 12.086 \\ 
CCDC & 1.708 & 124 & 125 & 2.225 & 3.214 & 3.194 & 3.657 & 3.590 & 2.532 & 2.501 & 0.307 & 0.276 & 0.989 & 0.968 & 1.125 & 1.089 & 339.014 & 345.389 & 489.697 & 495.708 & 0.261 & 0.207 & 150.683 & 150.319 & 0.192 & 8.883 \\ 
PXZPDO & 1.331 & 108 & 109 & 1.852 & 2.708 & 2.676 & 3.073 & 3.035 & 2.102 & 2.100 & 0.250 & 0.248 & 0.856 & 0.824 & 0.971 & 0.935 & 403.502 & 408.528 & 589.969 & 590.347 & 0.017 & 0.015 & 186.467 & 181.819 & 0.158 & 7.413 \\ 
DMAC-BP & 1.483 & 112 & 113 & 2.004 & 3.282 & 3.275 & 3.388 & 3.383 & 2.069 & 2.070 & 0.064 & 0.066 & 1.278 & 1.271 & 1.319 & 1.313 & 366.005 & 366.514 & 599.333 & 598.904 & 0.240 & 0.233 & 233.328 & 232.391 & 0.211 & 5.073 \\ 
SBTF & 2.284 & 131 & 132 & 1.926 & 2.822 & 2.773 & 3.558 & 3.486 & 2.428 & 2.421 & 0.502 & 0.495 & 0.897 & 0.847 & 1.130 & 1.065 & 348.446 & 355.663 & 510.696 & 512.130 & 1.478 & 1.219 & 162.250 & 156.467 & 0.909 & 0.858 \\ 
3-DPM & 1.326 & 104 & 105 & 1.693 & 2.719 & 2.707 & 2.990 & 2.960 & 1.862 & 1.851 & 0.169 & 0.158 & 1.026 & 1.014 & 1.128 & 1.109 & 414.607 & 418.837 & 665.778 & 669.651 & 0.031 & 0.025 & 251.170 & 250.814 & 0.218 & 5.061 \\ 
4-DPM & 1.684 & 104 & 105 & 1.680 & 2.395 & 2.361 & 3.034 & 3.008 & 2.128 & 2.141 & 0.448 & 0.461 & 0.715 & 0.681 & 0.906 & 0.867 & 408.717 & 412.182 & 582.646 & 579.171 & 1.200 & 1.087 & 173.929 & 166.989 & 0.569 & 2.469 \\ 
2CzPy & 2.662 & 89 & 90 & 2.504 & 3.443 & 3.420 & 3.901 & 3.839 & 2.837 & 2.811 & 0.333 & 0.307 & 0.939 & 0.916 & 1.064 & 1.028 & 317.786 & 322.951 & 436.966 & 441.050 & 0.172 & 0.149 & 119.180 & 118.099 & 0.441 & 4.495 \\ 
2PBCzPy & 2.355 & 177 & 178 & 2.438 & 3.532 & 3.511 & 4.021 & 3.961 & 2.775 & 2.750 & 0.337 & 0.312 & 1.094 & 1.073 & 1.245 & 1.211 & 308.372 & 312.981 & 446.751 & 450.783 & 0.144 & 0.151 & 138.378 & 137.802 & 0.327 & 8.494 \\ 
2BFCzPy & 2.574 & 121 & 122 & 2.465 & 3.460 & 3.437 & 3.832 & 3.785 & 2.730 & 2.715 & 0.265 & 0.250 & 0.994 & 0.971 & 1.101 & 1.070 & 323.583 & 327.559 & 454.103 & 456.587 & 0.669 & 0.592 & 130.520 & 129.028 & 0.411 & 5.612 \\ 
CNTPA-CZ & 2.594 & 110 & 111 & 2.678 & 3.163 & 3.136 & 3.787 & 3.741 & 3.207 & 3.195 & 0.528 & 0.517 & 0.485 & 0.458 & 0.580 & 0.546 & 327.403 & 331.438 & 386.638 & 388.050 & 0.657 & 0.572 & 59.235 & 56.612 & 0.371 & 5.414 \\ 
CNTPA-PXZ & 1.960 & 116 & 117 & 2.468 & 2.867 & 2.836 & 3.246 & 3.210 & 2.795 & 2.794 & 0.327 & 0.326 & 0.399 & 0.368 & 0.451 & 0.416 & 381.972 & 386.220 & 443.646 & 443.791 & 0.012 & 0.010 & 61.674 & 57.572 & 0.103 & 6.364 \\ 
BMZ-TZ & 1.764 & 120 & 121 & 1.640 & 3.355 & 3.354 & 3.334 & 3.333 & 1.630 & 1.630 & -0.010 & -0.010 & 1.715 & 1.714 & 1.704 & 1.703 & 371.901 & 372.034 & 760.798 & 760.777 & 0.009 & 0.009 & 388.898 & 388.743 & 0.474 & 2.017 \\ 
TPAPm & 1.944 & 109 & 110 & 2.035 & 2.856 & 2.829 & 3.487 & 3.463 & 2.485 & 2.490 & 0.450 & 0.456 & 0.821 & 0.794 & 1.003 & 0.972 & 355.520 & 358.067 & 499.019 & 497.876 & 2.000 & 1.845 & 143.498 & 139.810 & 0.402 & 1.767 \\ 
CzPm & 1.882 & 107 & 108 & 2.056 & 3.377 & 3.354 & 3.849 & 3.806 & 2.343 & 2.332 & 0.287 & 0.277 & 1.321 & 1.299 & 1.506 & 1.473 & 322.137 & 325.786 & 529.165 & 531.608 & 1.329 & 1.086 & 207.028 & 205.823 & 0.296 & 2.246 \\ 
TCPZ & 1.583 & 148 & 149 & 1.094 & 1.477 & 1.420 & 2.197 & 2.079 & 1.628 & 1.601 & 0.534 & 0.507 & 0.382 & 0.326 & 0.569 & 0.477 & 564.257 & 596.508 & 761.493 & 774.378 & 0.414 & 0.300 & 197.236 & 177.870 & 0.771 & 1.217 \\ 
TrisCz-Trz & 1.826 & 147 & 148 & 1.920 & 3.389 & 3.369 & 3.628 & 3.609 & 2.056 & 2.057 & 0.136 & 0.137 & 1.469 & 1.449 & 1.573 & 1.552 & 341.714 & 343.542 & 603.134 & 602.781 & 0.077 & 0.075 & 261.419 & 259.239 & 0.290 & 3.911 \\ 
PTZ–TAZ & 1.537 & 107 & 108 & 1.987 & 2.817 & 2.807 & 3.099 & 3.087 & 2.186 & 2.185 & 0.199 & 0.198 & 0.830 & 0.820 & 0.913 & 0.902 & 400.104 & 401.620 & 567.205 & 567.394 & 0.861 & 0.805 & 167.101 & 165.774 & 0.337 & 1.538 \\ 
DDMA-TXO2 & 2.260 & 124 & 125 & 2.756 & 3.439 & 3.409 & 4.115 & 4.065 & 3.297 & 3.286 & 0.541 & 0.530 & 0.684 & 0.653 & 0.818 & 0.779 & 301.284 & 305.012 & 376.052 & 377.319 & 0.108 & 0.102 & 74.769 & 72.307 & 0.277 & 2.575 \\ 
UGH3 & 3.596 & 105 & 106 & 3.212 & 5.246 & 5.202 & 5.244 & 5.215 & 3.211 & 3.220 & -0.001 & 0.008 & 2.034 & 1.990 & 2.033 & 1.995 & 236.440 & 237.727 & 386.158 & 385.012 & 0.000 & 0.000 & 149.719 & 147.285 & 0.610 & 0.719 \\ 
\end{longtable}
}


==> manuscript_enhancements/table_toluene_phase.tex <==
\begin{longtable}{l*{26}{c}}
\caption{Computational results for molecules in the toluene phase. This table presents key electronic and photophysical properties calculated considering solvent effects (toluene) via the ALPB model.}
\label{tab:toluene_phase_results}\\ 
\toprule 
Molecule Id & HOMO-LUMO gap & HOMO index & LUMO index & $\Delta E_r(S_0\to T_1)$ & $\underset{sTDA}{\Delta E_v}(S_0\to T_1)$ & $\underset{sTD-DFT}{\Delta E_v}(S_0\to T_1)$ & $\underset{sTDA}{\Delta E_v}(S_0\to S_1)$ & $\underset{sTD-DFT}{\Delta E_v}(S_0\to S_1)$ & $\underset{sTDA}{\Delta E_r}(S_0\to S_1)$ & $\underset{sTD-DFT}{\Delta E_r}(S_0\to S_1)$ & $\underset{sTDA}{\Delta E_{ST}}$ & $\underset{sTD-DFT}{\Delta E_{ST}}$ & $\underset{sTDA}{S_{shift}(T_1)}$ & $\underset{sTD-DFT}{S_{shift}(T_1)}$ & $\underset{sTDA}{S_{shift}(S_1)}$ & $\underset{sTD-DFT}{S_{shift}(S_1)}$ & $\underset{sTDA}{\lambda_{abs}}$ & $\underset{sTD-DFT}{\lambda_{abs}}$ & $\underset{sTDA}{\lambda_{PL}}$ & $\underset{sTD-DFT}{\lambda_{PL}}$ & $\underset{sTDA}{f_{12}}(S_0\to S_1)$ & $\underset{sTD-DFT}{f_{12}}(S_0\to S_1)$ & $\underset{sTDA}{\lambda_{shift}}$ & $\underset{sTD-DFT}{\lambda_{shift}}$ & Overlap & Centroid \\ 
\midrule 
\endfirsthead 
\multicolumn{27}{c}{{\tablename} \thetable{} -- Continued from previous page} \\ 
\toprule 
Molecule Id & HOMO-LUMO gap & HOMO index & LUMO index & $\Delta E_r(S_0\to T_1)$ & $\underset{sTDA}{\Delta E_v}(S_0\to T_1)$ & $\underset{sTD-DFT}{\Delta E_v}(S_0\to T_1)$ & $\underset{sTDA}{\Delta E_v}(S_0\to S_1)$ & $\underset{sTD-DFT}{\Delta E_v}(S_0\to S_1)$ & $\underset{sTDA}{\Delta E_r}(S_0\to S_1)$ & $\underset{sTD-DFT}{\Delta E_r}(S_0\to S_1)$ & $\underset{sTDA}{\Delta E_{ST}}$ & $\underset{sTD-DFT}{\Delta E_{ST}}$ & $\underset{sTDA}{S_{shift}(T_1)}$ & $\underset{sTD-DFT}{S_{shift}(T_1)}$ & $\underset{sTDA}{S_{shift}(S_1)}$ & $\underset{sTD-DFT}{S_{shift}(S_1)}$ & $\underset{sTDA}{\lambda_{abs}}$ & $\underset{sTD-DFT}{\lambda_{abs}}$ & $\underset{sTDA}{\lambda_{PL}}$ & $\underset{sTD-DFT}{\lambda_{PL}}$ & $\underset{sTDA}{f_{12}}(S_0\to S_1)$ & $\underset{sTD-DFT}{f_{12}}(S_0\to S_1)$ & $\underset{sTDA}{\lambda_{shift}}$ & $\underset{sTD-DFT}{\lambda_{shift}}$ & Overlap & Centroid \\ 
\midrule 
\endhead 
\midrule 
\multicolumn{27}{r}{{Continued on next page}} \\ 
\endfoot 
\bottomrule 
\endlastfoot 
4CzTPN & 1.536 & 143 & 144 & 1.848 & 2.522 & 2.508 & 2.841 & 2.790 & 2.082 & 2.056 & 0.234 & 0.208 & 0.674 & 0.660 & 0.759 & 0.734 & 436.410 & 444.420 & 595.634 & 603.174 & 0.446 & 0.377 & 159.223 & 158.754 & 0.400 & 0.008 \\ 
DMAC-DPS & 3.024 & 78 & 79 & 1.739 & 3.317 & 3.292 & 3.764 & 3.736 & 1.973 & 1.974 & 0.234 & 0.234 & 1.578 & 1.553 & 1.790 & 1.762 & 329.412 & 331.890 & 628.249 & 628.147 & 0.046 & 0.040 & 298.837 & 296.257 & 0.639 & 1.542 \\ 
PSPCz & 2.725 & 68 & 69 & 3.059 & 3.412 & 3.389 & 3.863 & 3.792 & 3.463 & 3.422 & 0.404 & 0.363 & 0.353 & 0.330 & 0.400 & 0.369 & 320.986 & 327.006 & 358.063 & 362.308 & 0.218 & 0.185 & 37.077 & 35.302 & 0.299 & 4.472 \\ 
Px2BP & 1.357 & 100 & 101 & 1.861 & 2.633 & 2.623 & 2.953 & 2.924 & 2.087 & 2.075 & 0.226 & 0.214 & 0.772 & 0.762 & 0.866 & 0.849 & 419.830 & 424.008 & 593.988 & 597.599 & 0.098 & 0.082 & 174.158 & 173.591 & 0.288 & 2.719 \\ 
CzS2 & 2.635 & 98 & 99 & 2.815 & 3.450 & 3.428 & 3.916 & 3.856 & 3.196 & 3.167 & 0.381 & 0.352 & 0.635 & 0.613 & 0.721 & 0.689 & 316.585 & 321.561 & 387.971 & 391.533 & 0.402 & 0.351 & 71.386 & 69.972 & 0.446 & 2.344 \\ 
2TCz-DPS & 2.373 & 146 & 147 & 2.478 & 3.431 & 3.410 & 3.875 & 3.817 & 2.799 & 2.774 & 0.321 & 0.296 & 0.952 & 0.932 & 1.076 & 1.043 & 319.959 & 324.796 & 442.933 & 446.889 & 0.096 & 0.084 & 122.974 & 122.093 & 0.399 & 4.313 \\ 
TDBA-DI & 2.107 & 163 & 164 & 2.519 & 3.103 & 3.084 & 3.571 & 3.505 & 2.899 & 2.862 & 0.380 & 0.344 & 0.584 & 0.565 & 0.672 & 0.642 & 347.227 & 353.776 & 427.733 & 433.159 & 0.043 & 0.219 & 80.506 & 79.384 & 0.135 & 7.533 \\ 
OPDPO & 1.311 & 102 & 103 & 1.396 & 2.101 & 2.099 & 2.230 & 2.221 & 1.482 & 1.477 & 0.086 & 0.081 & 0.705 & 0.703 & 0.748 & 0.743 & 556.058 & 558.311 & 836.826 & 839.297 & 0.054 & 0.049 & 280.768 & 280.986 & 0.282 & 2.993 \\ 
2CzTPEPCz & 2.375 & 152 & 153 & 1.906 & 3.278 & 3.240 & 3.848 & 3.810 & 2.237 & 2.241 & 0.331 & 0.335 & 1.372 & 1.334 & 1.610 & 1.569 & 322.238 & 325.384 & 554.182 & 553.174 & 1.552 & 1.331 & 231.944 & 227.790 & 0.631 & 1.501 \\ 
TBRb & 1.449 & 146 & 147 & 1.265 & 1.526 & 1.438 & 2.448 & 2.243 & 2.030 & 1.974 & 0.764 & 0.709 & 0.261 & 0.172 & 0.419 & 0.269 & 506.389 & 552.835 & 610.887 & 628.160 & 0.486 & 0.310 & 104.499 & 75.326 & 0.940 & 0.009 \\ 
TBPe & 1.930 & 94 & 95 & 1.704 & 2.213 & 2.147 & 3.218 & 3.058 & 2.478 & 2.428 & 0.774 & 0.723 & 0.509 & 0.442 & 0.740 & 0.630 & 385.283 & 405.482 & 500.275 & 510.682 & 0.871 & 0.611 & 114.991 & 105.200 & 0.944 & 0.000 \\ 
2CzPN & 1.833 & 83 & 84 & 2.260 & 2.914 & 2.894 & 3.259 & 3.226 & 2.528 & 2.519 & 0.268 & 0.259 & 0.654 & 0.634 & 0.731 & 0.707 & 380.436 & 384.316 & 490.512 & 492.131 & 0.245 & 0.216 & 110.076 & 107.815 & 0.472 & 4.250 \\ 
3CzFTFP & 1.513 & 101 & 102 & 2.538 & 3.366 & 3.343 & 3.824 & 3.749 & 2.884 & 2.846 & 0.346 & 0.308 & 0.828 & 0.805 & 0.941 & 0.903 & 324.201 & 330.739 & 429.969 & 435.642 & 0.155 & 0.128 & 105.768 & 104.903 & 0.098 & 6.828 \\ 
DDPhCz-DCPP & 1.075 & 166 & 167 & 1.463 & 2.960 & 2.941 & 3.390 & 3.357 & 1.676 & 1.670 & 0.213 & 0.207 & 1.497 & 1.478 & 1.714 & 1.687 & 365.681 & 369.308 & 739.757 & 742.300 & 0.559 & 0.541 & 374.076 & 372.991 & 0.387 & 6.647 \\ 
ACRXTN & 2.199 & 75 & 76 & 2.229 & 2.853 & 2.819 & 3.537 & 3.474 & 2.763 & 2.746 & 0.534 & 0.517 & 0.624 & 0.590 & 0.773 & 0.727 & 350.565 & 356.923 & 448.658 & 451.431 & 0.933 & 0.797 & 98.093 & 94.508 & 0.489 & 4.538 \\ 
TXO-TPA & 0.963 & 87 & 88 & 1.797 & 3.127 & 3.101 & 3.604 & 3.591 & 2.071 & 2.081 & 0.274 & 0.284 & 1.330 & 1.304 & 1.533 & 1.510 & 343.999 & 345.216 & 598.611 & 595.714 & 0.145 & 0.500 & 254.612 & 250.498 & 0.155 & 8.650 \\ 
PCTXO & 1.270 & 93 & 94 & 1.955 & 3.229 & 3.204 & 3.602 & 3.601 & 2.182 & 2.197 & 0.226 & 0.242 & 1.273 & 1.249 & 1.421 & 1.403 & 344.190 & 344.343 & 568.330 & 564.285 & 0.001 & 0.001 & 224.140 & 219.942 & 0.135 & 8.916 \\ 
IP-PPI & 2.543 & 103 & 104 & 2.283 & 3.255 & 3.224 & 3.813 & 3.774 & 2.674 & 2.673 & 0.391 & 0.390 & 0.972 & 0.941 & 1.139 & 1.101 & 325.145 & 328.505 & 463.587 & 463.889 & 0.761 & 0.711 & 138.442 & 135.384 & 0.631 & 7.024 \\ 
DMDHNP-DPS & 2.693 & 78 & 79 & 0.441 & 2.419 & 2.417 & 2.488 & 2.480 & 0.453 & 0.452 & 0.012 & 0.012 & 1.979 & 1.976 & 2.035 & 2.028 & 498.389 & 499.896 & 2736.196 & 2741.521 & 0.003 & 0.002 & 2237.807 & 2241.625 & 0.492 & 1.878 \\ 
4NTAZ-PPI & 2.364 & 131 & 132 & 2.288 & 3.336 & 3.285 & 3.861 & 3.823 & 2.648 & 2.662 & 0.360 & 0.374 & 1.048 & 0.997 & 1.213 & 1.160 & 321.111 & 324.337 & 468.141 & 465.713 & 0.221 & 0.203 & 147.030 & 141.376 & 0.187 & 11.447 \\ 
TAZ-PPI & 2.510 & 122 & 123 & 2.293 & 3.441 & 3.413 & 3.817 & 3.777 & 2.544 & 2.538 & 0.250 & 0.245 & 1.148 & 1.119 & 1.273 & 1.239 & 324.847 & 328.252 & 487.445 & 488.476 & 0.522 & 0.467 & 162.598 & 160.224 & 0.563 & 6.777 \\ 
PTZ-mPYR & 1.410 & 115 & 116 & 1.923 & 2.794 & 2.765 & 3.157 & 3.116 & 2.173 & 2.168 & 0.250 & 0.245 & 0.871 & 0.841 & 0.984 & 0.949 & 392.765 & 397.832 & 570.563 & 571.883 & 0.051 & 0.043 & 177.798 & 174.051 & 0.065 & 8.358 \\ 
pCNBCzoCF3 & 1.834 & 121 & 122 & 2.166 & 3.441 & 3.424 & 3.839 & 3.804 & 2.417 & 2.407 & 0.251 & 0.241 & 1.275 & 1.257 & 1.423 & 1.397 & 322.934 & 325.905 & 513.022 & 515.094 & 1.042 & 0.842 & 190.088 & 189.188 & 0.381 & 1.071 \\ 
PTZTPE-2 & 2.655 & 87 & 88 & 1.842 & 3.091 & 3.054 & 3.894 & 3.831 & 2.321 & 2.311 & 0.478 & 0.468 & 1.249 & 1.212 & 1.573 & 1.520 & 318.390 & 323.651 & 534.248 & 536.593 & 0.707 & 0.586 & 215.858 & 212.943 & 0.902 & 0.424 \\ 
4CzIPN & 1.834 & 143 & 144 & 2.143 & 2.984 & 2.974 & 3.210 & 3.180 & 2.306 & 2.292 & 0.162 & 0.149 & 0.841 & 0.831 & 0.904 & 0.888 & 386.220 & 389.863 & 537.709 & 540.926 & 0.159 & 0.143 & 151.490 & 151.064 & 0.323 & 1.431 \\ 
DMAC-TRZ & 1.391 & 96 & 97 & 2.007 & 3.371 & 3.362 & 3.454 & 3.447 & 2.057 & 2.058 & 0.049 & 0.051 & 1.364 & 1.355 & 1.397 & 1.389 & 359.000 & 359.646 & 602.885 & 602.410 & 0.124 & 0.119 & 243.885 & 242.765 & 0.194 & 6.731 \\ 
TCzTrz & 1.876 & 147 & 148 & 2.095 & 3.368 & 3.347 & 3.702 & 3.675 & 2.303 & 2.300 & 0.208 & 0.205 & 1.272 & 1.252 & 1.399 & 1.375 & 334.929 & 337.381 & 538.324 & 539.012 & 0.409 & 0.360 & 203.394 & 201.631 & 0.291 & 5.306 \\ 
$\delta$-2CbPN & 1.706 & 83 & 84 & 2.299 & 3.035 & 3.014 & 3.399 & 3.365 & 2.575 & 2.566 & 0.276 & 0.267 & 0.736 & 0.715 & 0.824 & 0.798 & 364.777 & 368.507 & 481.508 & 483.145 & 0.263 & 0.231 & 116.730 & 114.638 & 0.154 & 6.338 \\ 
CzDCbTrz & 1.825 & 147 & 148 & 2.084 & 3.290 & 3.264 & 3.660 & 3.632 & 2.319 & 2.319 & 0.235 & 0.235 & 1.205 & 1.180 & 1.341 & 1.313 & 338.718 & 341.376 & 534.589 & 534.624 & 0.384 & 0.323 & 195.871 & 193.248 & 0.212 & 5.022 \\ 
$\alpha$-2CbPN & 2.058 & 83 & 84 & 2.421 & 3.103 & 3.081 & 3.505 & 3.467 & 2.735 & 2.725 & 0.314 & 0.304 & 0.682 & 0.660 & 0.770 & 0.743 & 353.695 & 357.571 & 453.327 & 455.031 & 0.289 & 0.253 & 99.632 & 97.460 & 0.321 & 4.550 \\ 
CN-QP & 0.776 & 122 & 123 & 1.190 & 2.924 & 2.895 & 3.223 & 3.221 & 1.312 & 1.324 & 0.122 & 0.134 & 1.734 & 1.704 & 1.911 & 1.896 & 384.698 & 384.948 & 945.060 & 936.168 & 0.019 & 0.020 & 560.363 & 551.220 & 0.127 & 8.432 \\ 
TFM-QP & 0.762 & 130 & 131 & 1.188 & 2.930 & 2.900 & 3.290 & 3.278 & 1.334 & 1.343 & 0.146 & 0.155 & 1.742 & 1.712 & 1.956 & 1.935 & 376.886 & 378.231 & 929.313 & 923.208 & 0.015 & 0.007 & 552.427 & 544.976 & 0.151 & 7.959 \\ 
NDN & 2.770 & 91 & 92 & 2.779 & 3.429 & 3.409 & 3.829 & 3.763 & 3.103 & 3.068 & 0.324 & 0.289 & 0.650 & 0.630 & 0.725 & 0.695 & 323.820 & 329.447 & 399.509 & 404.104 & 0.034 & 0.026 & 75.689 & 74.657 & 0.621 & 1.570 \\ 
mCP & 3.113 & 75 & 76 & 3.099 & 3.394 & 3.370 & 3.889 & 3.821 & 3.551 & 3.514 & 0.452 & 0.415 & 0.294 & 0.270 & 0.337 & 0.307 & 318.824 & 324.481 & 349.114 & 352.786 & 0.302 & 0.255 & 30.290 & 28.305 & 0.687 & 0.053 \\ 
ZDZ & 2.536 & 91 & 92 & 2.741 & 3.389 & 3.372 & 3.774 & 3.711 & 3.053 & 3.017 & 0.312 & 0.275 & 0.647 & 0.631 & 0.721 & 0.694 & 328.513 & 334.117 & 406.103 & 411.020 & 0.088 & 0.072 & 77.590 & 76.903 & 0.445 & 2.163 \\ 
ZDN & 2.588 & 91 & 92 & 2.743 & 3.405 & 3.382 & 3.826 & 3.764 & 3.082 & 3.053 & 0.339 & 0.309 & 0.662 & 0.639 & 0.744 & 0.711 & 324.091 & 329.439 & 402.291 & 406.143 & 0.109 & 0.090 & 78.200 & 76.705 & 0.414 & 4.186 \\ 
BTCz3CzTPN & 1.435 & 159 & 160 & 1.824 & 2.553 & 2.539 & 2.866 & 2.818 & 2.047 & 2.024 & 0.223 & 0.200 & 0.729 & 0.715 & 0.818 & 0.794 & 432.634 & 439.972 & 605.586 & 612.482 & 0.523 & 0.449 & 172.953 & 172.510 & 0.191 & 6.231 \\ 
2BTCz2CzTPN & 1.409 & 175 & 176 & 1.796 & 2.568 & 2.554 & 2.875 & 2.829 & 2.010 & 1.989 & 0.214 & 0.193 & 0.772 & 0.758 & 0.864 & 0.840 & 431.309 & 438.262 & 616.743 & 623.317 & 0.578 & 0.500 & 185.433 & 185.055 & 0.213 & 4.435 \\ 
APDC-DTPA & 0.772 & 135 & 136 & 1.202 & 2.076 & 2.049 & 2.575 & 2.561 & 1.491 & 1.503 & 0.289 & 0.300 & 0.874 & 0.847 & 1.084 & 1.058 & 481.455 & 484.162 & 831.382 & 825.103 & 0.147 & 0.157 & 349.927 & 340.941 & 0.312 & 8.619 \\ 
BMIM & 0.773 & 135 & 136 & 1.205 & 2.075 & 2.048 & 2.575 & 2.560 & 1.495 & 1.506 & 0.290 & 0.301 & 0.870 & 0.843 & 1.079 & 1.053 & 481.586 & 484.332 & 829.248 & 823.048 & 0.147 & 0.152 & 347.662 & 338.715 & 0.312 & 8.617 \\ 
ADO-TPA & 0.771 & 78 & 79 & 1.349 & 1.969 & 1.969 & 1.968 & 1.968 & 1.348 & 1.348 & -0.001 & -0.001 & 0.621 & 0.620 & 0.620 & 0.620 & 629.905 & 630.097 & 919.769 & 919.769 & 0.000 & 0.000 & 289.864 & 289.672 & 0.207 & 9.232 \\ 
DCzTrz & 1.890 & 117 & 118 & 2.140 & 3.436 & 3.412 & 3.879 & 3.831 & 2.416 & 2.403 & 0.276 & 0.263 & 1.296 & 1.272 & 1.463 & 1.428 & 319.605 & 323.609 & 513.168 & 515.983 & 0.336 & 0.310 & 193.564 & 192.374 & 0.244 & 4.842 \\ 
BDPCC & 2.701 & 147 & 148 & 2.570 & 3.362 & 3.339 & 3.810 & 3.760 & 2.913 & 2.894 & 0.343 & 0.324 & 0.792 & 0.769 & 0.898 & 0.866 & 325.409 & 329.763 & 425.695 & 428.413 & 0.211 & 0.195 & 100.286 & 98.651 & 0.556 & 3.222 \\ 
SpiroAC-TRZ & 1.472 & 117 & 118 & 2.036 & 3.396 & 3.386 & 3.495 & 3.488 & 2.096 & 2.098 & 0.060 & 0.062 & 1.359 & 1.349 & 1.399 & 1.390 & 354.747 & 355.429 & 591.535 & 590.978 & 0.174 & 0.169 & 236.788 & 235.549 & 0.203 & 6.771 \\ 
DBT-BZ-DMAC & 1.969 & 90 & 91 & 1.556 & 3.003 & 2.966 & 3.594 & 3.557 & 1.863 & 1.866 & 0.306 & 0.310 & 1.447 & 1.410 & 1.732 & 1.690 & 344.947 & 348.574 & 665.686 & 664.287 & 0.011 & 0.032 & 320.740 & 315.713 & 0.235 & 4.029 \\ 
DQP & 1.128 & 69 & 70 & 1.156 & 3.197 & 3.133 & 3.243 & 3.242 & 1.172 & 1.196 & 0.016 & 0.040 & 2.042 & 1.977 & 2.071 & 2.046 & 382.360 & 382.431 & 1057.890 & 1036.807 & 0.000 & 0.000 & 675.530 & 654.376 & 0.581 & 0.011 \\ 
TPA-DCPP & 0.869 & 140 & 141 & 1.406 & 3.066 & 3.044 & 3.461 & 3.445 & 1.587 & 1.591 & 0.181 & 0.186 & 1.661 & 1.638 & 1.875 & 1.854 & 358.201 & 359.865 & 781.368 & 779.236 & 0.947 & 0.892 & 423.167 & 419.371 & 0.299 & 8.539 \\ 
2PXZ-OXD & 1.508 & 107 & 108 & 1.935 & 2.836 & 2.826 & 3.097 & 3.087 & 2.114 & 2.113 & 0.179 & 0.178 & 0.901 & 0.891 & 0.984 & 0.973 & 400.285 & 401.698 & 586.576 & 586.696 & 0.869 & 0.815 & 186.291 & 184.998 & 0.329 & 1.850 \\ 
BmPyPhB & 1.319 & 174 & 175 & 1.756 & 3.359 & 3.351 & 3.452 & 3.447 & 1.805 & 1.806 & 0.048 & 0.050 & 1.603 & 1.595 & 1.647 & 1.641 & 359.187 & 359.719 & 687.069 & 686.488 & 0.251 & 0.244 & 327.882 & 326.770 & 0.175 & 3.503 \\ 
MPPA & 0.648 & 152 & 153 & 1.122 & 2.229 & 2.214 & 2.617 & 2.582 & 1.317 & 1.308 & 0.195 & 0.187 & 1.108 & 1.092 & 1.300 & 1.274 & 473.765 & 480.168 & 941.583 & 947.717 & 0.145 & 0.108 & 467.819 & 467.549 & 0.332 & 3.746 \\ 
ACRFLCN & 1.528 & 83 & 84 & 2.198 & 3.276 & 3.276 & 3.277 & 3.276 & 2.199 & 2.199 & 0.000 & 0.000 & 1.078 & 1.077 & 1.078 & 1.078 & 378.393 & 378.439 & 563.937 & 563.902 & 0.000 & 0.000 & 185.544 & 185.463 & 0.132 & 3.751 \\ 
PTZ-DCPP & 1.327 & 116 & 117 & 1.460 & 2.353 & 2.321 & 2.905 & 2.851 & 1.803 & 1.794 & 0.343 & 0.333 & 0.892 & 0.861 & 1.102 & 1.057 & 426.752 & 434.895 & 687.542 & 691.221 & 0.325 & 0.317 & 260.790 & 256.327 & 0.516 & 5.071 \\ 
BBA-Pyr & 1.830 & 130 & 131 & 2.076 & 3.331 & 3.309 & 3.794 & 3.770 & 2.364 & 2.365 & 0.288 & 0.289 & 1.255 & 1.233 & 1.430 & 1.405 & 326.816 & 328.871 & 524.434 & 524.182 & 1.714 & 1.539 & 197.618 & 195.311 & 0.234 & 10.300 \\ 
PhICz-Pyr & 2.218 & 128 & 129 & 2.233 & 3.248 & 3.230 & 3.632 & 3.574 & 2.497 & 2.471 & 0.264 & 0.238 & 1.015 & 0.997 & 1.135 & 1.103 & 341.329 & 346.925 & 496.551 & 501.772 & 0.401 & 0.350 & 155.222 & 154.846 & 0.495 & 1.420 \\ 
PhCz-Pyr & 2.046 & 129 & 130 & 2.174 & 3.391 & 3.369 & 3.815 & 3.756 & 2.446 & 2.424 & 0.272 & 0.249 & 1.217 & 1.195 & 1.369 & 1.332 & 324.983 & 330.096 & 506.919 & 511.571 & 0.309 & 0.251 & 181.936 & 181.474 & 0.186 & 11.354 \\ 
PDA-DP & 1.905 & 172 & 173 & 2.266 & 3.260 & 3.233 & 3.776 & 3.747 & 2.624 & 2.626 & 0.359 & 0.360 & 0.994 & 0.967 & 1.151 & 1.121 & 328.365 & 330.925 & 472.433 & 472.172 & 1.452 & 1.355 & 144.068 & 141.247 & 0.243 & 5.143 \\ 
9CzFDBFDPO & 2.322 & 187 & 188 & 2.924 & 3.424 & 3.401 & 3.895 & 3.827 & 3.326 & 3.290 & 0.402 & 0.366 & 0.500 & 0.477 & 0.569 & 0.537 & 318.341 & 323.989 & 372.771 & 376.848 & 0.168 & 0.143 & 54.431 & 52.859 & 0.004 & 12.797 \\ 
9PhCzFDBFDPO & 2.303 & 201 & 202 & 2.745 & 3.437 & 3.414 & 3.909 & 3.843 & 3.122 & 3.090 & 0.377 & 0.345 & 0.692 & 0.669 & 0.787 & 0.753 & 317.168 & 322.590 & 397.118 & 401.180 & 0.209 & 0.172 & 79.950 & 78.590 & 0.008 & 16.998 \\ 
9PhCzFDBFSPO & 2.515 & 167 & 168 & 2.781 & 3.432 & 3.409 & 3.899 & 3.835 & 3.160 & 3.129 & 0.379 & 0.348 & 0.651 & 0.628 & 0.739 & 0.706 & 317.957 & 323.296 & 392.348 & 396.263 & 0.239 & 0.198 & 74.391 & 72.967 & 0.005 & 17.126 \\ 
9CzFDBFSPO & 2.519 & 153 & 154 & 2.988 & 3.385 & 3.362 & 3.833 & 3.762 & 3.383 & 3.343 & 0.395 & 0.355 & 0.397 & 0.374 & 0.450 & 0.419 & 323.465 & 329.596 & 366.491 & 370.879 & 0.188 & 0.157 & 43.026 & 41.282 & 0.017 & 13.557 \\ 
9ArFDBFxPO & 2.323 & 187 & 188 & 2.914 & 3.430 & 3.407 & 3.898 & 3.830 & 3.312 & 3.276 & 0.398 & 0.362 & 0.515 & 0.492 & 0.586 & 0.553 & 318.079 & 323.744 & 374.314 & 378.436 & 0.162 & 0.138 & 56.234 & 54.692 & 0.016 & 12.261 \\ 
12BTCzTPN & 1.488 & 175 & 176 & 1.820 & 2.866 & 2.853 & 3.136 & 3.105 & 1.992 & 1.981 & 0.172 & 0.161 & 1.045 & 1.033 & 1.144 & 1.124 & 395.320 & 399.254 & 622.330 & 625.781 & 0.297 & 0.278 & 227.011 & 226.528 & 0.335 & 2.688 \\ 
oDTBPZ-DPXZ & 1.049 & 151 & 152 & 1.269 & 2.813 & 2.801 & 3.042 & 3.025 & 1.372 & 1.370 & 0.103 & 0.101 & 1.544 & 1.533 & 1.670 & 1.655 & 407.588 & 409.879 & 903.665 & 904.964 & 0.581 & 0.544 & 496.077 & 495.085 & 0.303 & 6.469 \\ 
3DMAC-BP-CN & 0.902 & 172 & 173 & 1.033 & 2.310 & 2.280 & 2.804 & 2.752 & 1.254 & 1.247 & 0.221 & 0.214 & 1.276 & 1.246 & 1.549 & 1.505 & 442.248 & 450.508 & 988.569 & 993.865 & 0.098 & 0.526 & 546.321 & 543.358 & 0.254 & 7.234 \\ 
3DMAC-BP-Br & 0.940 & 171 & 172 & 1.128 & 2.419 & 2.390 & 2.894 & 2.846 & 1.350 & 1.343 & 0.221 & 0.215 & 1.291 & 1.262 & 1.544 & 1.502 & 428.433 & 435.705 & 918.659 & 923.052 & 0.345 & 0.419 & 490.226 & 487.347 & 0.220 & 7.593 \\ 
TPA-PZCN & 0.943 & 149 & 150 & 1.191 & 2.919 & 2.892 & 3.265 & 3.240 & 1.332 & 1.334 & 0.141 & 0.143 & 1.728 & 1.701 & 1.933 & 1.906 & 379.702 & 382.667 & 930.687 & 929.150 & 0.784 & 1.213 & 550.985 & 546.483 & 0.307 & 8.347 \\ 
1PXZ-BP & 1.041 & 84 & 85 & 1.312 & 2.756 & 2.725 & 3.059 & 3.045 & 1.456 & 1.466 & 0.144 & 0.154 & 1.444 & 1.413 & 1.603 & 1.579 & 405.296 & 407.240 & 851.406 & 845.836 & 0.310 & 0.285 & 446.110 & 438.596 & 0.229 & 7.667 \\ 
PTZ-DBTO2 & 2.248 & 70 & 71 & 2.255 & 2.894 & 2.875 & 3.375 & 3.307 & 2.630 & 2.595 & 0.375 & 0.339 & 0.639 & 0.619 & 0.745 & 0.713 & 367.393 & 374.903 & 471.450 & 477.861 & 0.047 & 0.036 & 104.056 & 102.958 & 0.370 & 5.056 \\ 
BACQ & 2.185 & 67 & 68 & 2.245 & 2.460 & 2.423 & 3.205 & 3.084 & 2.926 & 2.858 & 0.681 & 0.612 & 0.214 & 0.178 & 0.279 & 0.226 & 386.786 & 401.998 & 423.717 & 433.847 & 0.510 & 0.375 & 36.931 & 31.849 & 0.688 & 2.087 \\ 
2Cz-DMAC-TXO & 1.204 & 135 & 136 & 1.885 & 2.848 & 2.821 & 3.335 & 3.318 & 2.207 & 2.217 & 0.322 & 0.332 & 0.963 & 0.936 & 1.128 & 1.101 & 371.811 & 373.683 & 561.838 & 559.332 & 0.015 & 0.031 & 190.026 & 185.649 & 0.115 & 6.425 \\ 
2Cz-DMAC-TTR & 1.962 & 145 & 146 & 2.051 & 3.404 & 3.383 & 3.975 & 3.911 & 2.396 & 2.371 & 0.344 & 0.320 & 1.353 & 1.332 & 1.580 & 1.540 & 311.886 & 317.022 & 517.569 & 522.878 & 0.134 & 0.042 & 205.683 & 205.855 & 0.191 & 8.415 \\ 
2Cz-DMAC-BTB & 1.556 & 136 & 137 & 2.189 & 3.358 & 3.329 & 3.553 & 3.547 & 2.317 & 2.333 & 0.128 & 0.144 & 1.168 & 1.139 & 1.236 & 1.214 & 348.917 & 349.507 & 535.110 & 531.402 & 0.026 & 0.026 & 186.193 & 181.895 & 0.155 & 6.027 \\ 
DMAC-BPP & 1.616 & 149 & 150 & 1.921 & 3.457 & 3.427 & 3.724 & 3.719 & 2.069 & 2.084 & 0.148 & 0.164 & 1.536 & 1.506 & 1.655 & 1.634 & 332.960 & 333.425 & 599.255 & 594.833 & 0.012 & 0.013 & 266.296 & 261.408 & 0.120 & 6.154 \\ 
Me-MOC & 1.710 & 79 & 80 & 2.275 & 3.118 & 3.092 & 3.639 & 3.550 & 2.655 & 2.612 & 0.380 & 0.337 & 0.843 & 0.817 & 0.984 & 0.938 & 340.738 & 349.212 & 466.957 & 474.656 & 0.361 & 0.269 & 126.219 & 125.444 & 0.078 & 8.219 \\ 
Me-DOC & 1.624 & 85 & 86 & 2.190 & 2.941 & 2.913 & 3.518 & 3.414 & 2.620 & 2.566 & 0.430 & 0.376 & 0.751 & 0.724 & 0.898 & 0.848 & 352.408 & 363.185 & 473.265 & 483.194 & 0.447 & 0.315 & 120.857 & 120.008 & 0.079 & 8.325 \\ 
3DCPO & 3.125 & 109 & 110 & 3.102 & 3.397 & 3.374 & 3.897 & 3.827 & 3.558 & 3.518 & 0.457 & 0.416 & 0.295 & 0.272 & 0.339 & 0.309 & 318.153 & 323.972 & 348.444 & 352.436 & 0.192 & 0.160 & 30.291 & 28.463 & 0.433 & 4.529 \\ 
TDBA-TPDICz & 2.026 & 161 & 162 & 2.366 & 2.675 & 2.648 & 3.178 & 3.082 & 2.812 & 2.754 & 0.445 & 0.388 & 0.309 & 0.282 & 0.367 & 0.328 & 390.096 & 402.259 & 440.979 & 450.122 & 0.384 & 0.302 & 50.883 & 47.863 & 0.207 & 7.473 \\ 
TRZ-pIC & 2.027 & 161 & 162 & 2.366 & 2.675 & 2.648 & 3.178 & 3.082 & 2.811 & 2.754 & 0.445 & 0.388 & 0.309 & 0.282 & 0.367 & 0.328 & 390.145 & 402.298 & 441.078 & 450.209 & 0.384 & 0.303 & 50.933 & 47.912 & 0.207 & 7.461 \\ 
SBF-PXZ & 2.067 & 124 & 125 & 2.343 & 2.837 & 2.806 & 3.230 & 3.195 & 2.668 & 2.667 & 0.325 & 0.324 & 0.494 & 0.464 & 0.562 & 0.528 & 383.864 & 388.106 & 464.747 & 464.896 & 0.028 & 0.024 & 80.883 & 76.791 & 0.375 & 0.650 \\ 
PtOEP & 0.812 & 110 & 111 & 0.590 & 0.094 & 1.386 & 0.991 & 0.569 & 6.239 & 0.242 & 5.649 & -0.348 & -0.496 & 0.796 & -5.248 & 0.327 & 1251.607 & 2179.367 & 198.735 & 5117.596 & 0.000 & 0.000 & -1052.872 & 2938.229 & 0.740 & 0.011 \\ 
PxCYP & 1.272 & 113 & 114 & 1.833 & 2.754 & 2.723 & 3.119 & 3.083 & 2.077 & 2.076 & 0.243 & 0.242 & 0.921 & 0.890 & 1.043 & 1.007 & 397.474 & 402.154 & 597.050 & 597.302 & 0.012 & 0.012 & 199.576 & 195.148 & 0.158 & 7.720 \\ 
AcCYP & 1.286 & 125 & 126 & 1.909 & 3.388 & 3.357 & 3.534 & 3.529 & 1.992 & 2.007 & 0.082 & 0.098 & 1.478 & 1.447 & 1.542 & 1.522 & 350.852 & 351.330 & 622.475 & 617.617 & 0.162 & 0.156 & 271.622 & 266.288 & 0.101 & 7.682 \\ 
BCN & 1.959 & 75 & 76 & 2.215 & 2.478 & 2.448 & 2.970 & 2.909 & 2.655 & 2.632 & 0.440 & 0.417 & 0.263 & 0.233 & 0.315 & 0.277 & 417.413 & 426.224 & 466.965 & 471.087 & 0.298 & 0.247 & 49.552 & 44.863 & 0.533 & 4.396 \\ 
DPPSPF & 2.890 & 96 & 97 & 2.623 & 3.646 & 3.610 & 4.376 & 4.319 & 3.149 & 3.139 & 0.525 & 0.516 & 1.023 & 0.986 & 1.228 & 1.180 & 283.315 & 287.047 & 393.784 & 394.978 & 1.299 & 1.141 & 110.469 & 107.931 & 0.688 & 4.092 \\ 
Me2ACBO & 1.782 & 184 & 185 & 2.147 & 3.110 & 3.091 & 3.528 & 3.508 & 2.435 & 2.437 & 0.288 & 0.290 & 0.963 & 0.944 & 1.093 & 1.071 & 351.439 & 353.402 & 509.094 & 508.795 & 0.189 & 0.200 & 157.655 & 155.392 & 0.067 & 9.465 \\ 
F2AcBO & 1.836 & 205 & 206 & 2.146 & 3.107 & 3.088 & 3.482 & 3.454 & 2.404 & 2.400 & 0.259 & 0.254 & 0.962 & 0.942 & 1.078 & 1.054 & 356.072 & 358.948 & 515.636 & 516.573 & 0.176 & 0.136 & 159.565 & 157.625 & 0.176 & 5.206 \\ 
PSPSF & 2.853 & 95 & 96 & 2.623 & 3.691 & 3.654 & 4.419 & 4.366 & 3.140 & 3.134 & 0.518 & 0.511 & 1.068 & 1.031 & 1.279 & 1.232 & 280.571 & 283.970 & 394.805 & 395.637 & 1.193 & 1.064 & 114.235 & 111.667 & 0.542 & 4.592 \\ 
TXO-P-Si & 1.740 & 101 & 102 & 2.167 & 3.630 & 3.629 & 3.625 & 3.624 & 2.164 & 2.164 & -0.003 & -0.003 & 1.463 & 1.462 & 1.461 & 1.460 & 341.988 & 342.110 & 572.825 & 572.825 & 0.000 & 0.000 & 230.837 & 230.715 & 0.068 & 10.001 \\ 
CzB-FMPIM & 2.220 & 125 & 126 & 2.276 & 3.465 & 3.441 & 3.935 & 3.870 & 2.585 & 2.559 & 0.309 & 0.283 & 1.189 & 1.166 & 1.350 & 1.311 & 315.073 & 320.364 & 479.701 & 484.506 & 0.223 & 0.162 & 164.629 & 164.141 & 0.205 & 10.075 \\ 
CzB-FMPPI & 2.189 & 124 & 125 & 2.252 & 3.445 & 3.416 & 3.856 & 3.816 & 2.521 & 2.515 & 0.269 & 0.264 & 1.193 & 1.164 & 1.336 & 1.300 & 321.502 & 324.915 & 491.884 & 492.891 & 0.477 & 0.440 & 170.382 & 167.977 & 0.173 & 10.409 \\ 
BACF & 2.259 & 66 & 67 & 2.393 & 2.494 & 2.459 & 3.062 & 2.972 & 2.938 & 2.892 & 0.545 & 0.499 & 0.101 & 0.066 & 0.124 & 0.080 & 404.965 & 417.188 & 422.028 & 428.699 & 0.097 & 0.075 & 17.063 & 11.511 & 0.619 & 3.015 \\ 
BACH & 2.422 & 63 & 64 & 2.478 & 2.599 & 2.564 & 3.173 & 3.086 & 3.024 & 2.982 & 0.547 & 0.505 & 0.121 & 0.086 & 0.148 & 0.104 & 390.797 & 401.737 & 409.938 & 415.740 & 0.109 & 0.085 & 19.142 & 14.003 & 0.657 & 2.749 \\ 
PzTDBA & 1.411 & 178 & 179 & 1.986 & 2.321 & 2.291 & 2.562 & 2.534 & 2.193 & 2.197 & 0.206 & 0.210 & 0.335 & 0.305 & 0.370 & 0.337 & 483.879 & 489.379 & 565.433 & 564.445 & 0.000 & 0.000 & 81.555 & 75.066 & 0.200 & 0.670 \\ 
3TCPM & 1.465 & 109 & 110 & 2.169 & 3.345 & 3.323 & 3.643 & 3.641 & 2.362 & 2.376 & 0.193 & 0.207 & 1.176 & 1.154 & 1.281 & 1.265 & 340.307 & 340.541 & 524.815 & 521.784 & 0.006 & 0.019 & 184.508 & 181.243 & 0.117 & 13.129 \\ 
TPA-PPO & 1.855 & 100 & 101 & 2.059 & 2.921 & 2.882 & 3.517 & 3.486 & 2.479 & 2.491 & 0.420 & 0.431 & 0.862 & 0.823 & 1.038 & 0.995 & 352.508 & 355.704 & 500.048 & 497.794 & 2.135 & 1.919 & 147.540 & 142.090 & 0.368 & 7.759 \\ 
CzPh-PPO & 2.066 & 99 & 100 & 2.161 & 2.959 & 2.920 & 3.770 & 3.711 & 2.754 & 2.746 & 0.593 & 0.585 & 0.798 & 0.759 & 1.017 & 0.965 & 328.836 & 334.144 & 450.222 & 451.537 & 1.883 & 1.585 & 121.387 & 117.393 & 0.308 & 8.563 \\ 
m-CF3PIBI & 2.482 & 143 & 144 & 2.299 & 3.497 & 3.467 & 3.885 & 3.847 & 2.554 & 2.550 & 0.255 & 0.252 & 1.198 & 1.169 & 1.331 & 1.296 & 319.177 & 322.296 & 485.477 & 486.128 & 0.365 & 0.327 & 166.301 & 163.832 & 0.481 & 3.312 \\ 
DPTPEA & 2.267 & 93 & 94 & 1.782 & 2.973 & 2.939 & 3.544 & 3.510 & 2.125 & 2.129 & 0.343 & 0.347 & 1.190 & 1.156 & 1.419 & 1.381 & 349.823 & 353.181 & 583.414 & 582.317 & 0.896 & 0.790 & 233.591 & 229.136 & 0.577 & 4.649 \\ 
PICNAnCz & 2.213 & 75 & 76 & 2.373 & 3.437 & 3.406 & 3.837 & 3.793 & 2.649 & 2.642 & 0.276 & 0.269 & 1.064 & 1.033 & 1.188 & 1.151 & 323.162 & 326.885 & 468.034 & 469.211 & 0.214 & 0.202 & 144.872 & 142.326 & 0.293 & 5.237 \\ 
DPA-DPQ & 1.771 & 83 & 84 & 1.774 & 2.502 & 2.472 & 3.073 & 2.993 & 2.178 & 2.148 & 0.404 & 0.374 & 0.728 & 0.698 & 0.894 & 0.845 & 403.502 & 414.233 & 569.200 & 577.239 & 0.413 & 0.343 & 165.698 & 163.006 & 0.595 & 0.822 \\ 
PhQLPXZ & 1.591 & 85 & 86 & 2.018 & 2.726 & 2.695 & 2.992 & 2.978 & 2.215 & 2.230 & 0.197 & 0.212 & 0.708 & 0.677 & 0.777 & 0.748 & 414.386 & 416.390 & 559.780 & 556.090 & 0.171 & 0.156 & 145.395 & 139.700 & 0.271 & 5.475 \\ 
2DPA-DPQ & 1.937 & 114 & 115 & 1.879 & 2.412 & 2.381 & 3.053 & 2.966 & 2.378 & 2.340 & 0.499 & 0.461 & 0.533 & 0.502 & 0.675 & 0.626 & 406.119 & 418.032 & 521.340 & 529.780 & 0.851 & 0.693 & 115.220 & 111.747 & 0.590 & 0.635 \\ 
FDQPXZ & 1.159 & 88 & 89 & 1.470 & 2.352 & 2.342 & 2.557 & 2.537 & 1.598 & 1.593 & 0.128 & 0.123 & 0.882 & 0.872 & 0.959 & 0.944 & 484.863 & 488.723 & 775.768 & 778.455 & 0.223 & 0.201 & 290.906 & 289.731 & 0.328 & 5.370 \\ 
DTRZSFX & 1.971 & 145 & 146 & 2.018 & 3.335 & 3.298 & 3.954 & 3.908 & 2.393 & 2.392 & 0.375 & 0.374 & 1.317 & 1.280 & 1.561 & 1.516 & 313.567 & 317.257 & 518.179 & 518.430 & 2.005 & 1.775 & 204.612 & 201.172 & 0.263 & 2.783 \\ 
E-o-DHMPA & 2.177 & 73 & 74 & 1.969 & 2.265 & 2.193 & 3.285 & 3.097 & 2.856 & 2.781 & 0.886 & 0.812 & 0.296 & 0.224 & 0.429 & 0.316 & 377.425 & 400.349 & 434.185 & 445.798 & 0.363 & 0.250 & 56.760 & 45.449 & 0.936 & 0.014 \\ 
Z-o-DHMPA & 2.177 & 73 & 74 & 1.970 & 2.265 & 2.193 & 3.284 & 3.097 & 2.856 & 2.782 & 0.886 & 0.812 & 0.296 & 0.223 & 0.429 & 0.315 & 377.483 & 400.298 & 434.152 & 445.658 & 0.359 & 0.248 & 56.669 & 45.361 & 0.937 & 0.014 \\ 
p-DHMPA & 2.155 & 73 & 74 & 1.893 & 2.257 & 2.185 & 3.279 & 3.098 & 2.750 & 2.684 & 0.856 & 0.791 & 0.364 & 0.291 & 0.529 & 0.413 & 378.162 & 400.259 & 450.934 & 461.870 & 0.422 & 0.299 & 72.772 & 61.611 & 0.937 & 0.025 \\ 
STAC-BP-STAC & 1.541 & 160 & 161 & 2.029 & 3.213 & 3.204 & 3.413 & 3.405 & 2.155 & 2.156 & 0.126 & 0.127 & 1.184 & 1.175 & 1.258 & 1.249 & 363.260 & 364.092 & 575.292 & 575.013 & 0.352 & 0.302 & 212.033 & 210.921 & 0.239 & 2.802 \\ 
SXAC-BP-SXAC & 1.504 & 160 & 161 & 2.027 & 3.278 & 3.270 & 3.428 & 3.423 & 2.120 & 2.122 & 0.093 & 0.095 & 1.251 & 1.243 & 1.309 & 1.301 & 361.649 & 362.252 & 584.890 & 584.363 & 0.344 & 0.335 & 223.241 & 222.111 & 0.226 & 2.887 \\ 
m-DHMPA & 2.145 & 73 & 74 & 1.902 & 2.252 & 2.181 & 3.264 & 3.083 & 2.757 & 2.688 & 0.855 & 0.787 & 0.350 & 0.279 & 0.507 & 0.394 & 379.807 & 402.167 & 449.713 & 461.173 & 0.426 & 0.301 & 69.906 & 59.006 & 0.937 & 0.016 \\ 
SFAC-BP-SFAC & 1.446 & 154 & 155 & 1.984 & 3.263 & 3.254 & 3.410 & 3.405 & 2.074 & 2.076 & 0.090 & 0.092 & 1.279 & 1.270 & 1.336 & 1.329 & 363.537 & 364.124 & 597.791 & 597.197 & 0.347 & 0.339 & 234.255 & 233.073 & 0.227 & 3.785 \\ 
PBTPA & 1.008 & 106 & 107 & 1.382 & 2.499 & 2.457 & 2.974 & 2.938 & 1.645 & 1.653 & 0.263 & 0.270 & 1.116 & 1.075 & 1.329 & 1.285 & 416.936 & 422.002 & 753.652 & 750.171 & 1.362 & 1.209 & 336.716 & 328.169 & 0.325 & 5.910 \\ 
HDP & 0.856 & 59 & 60 & 1.097 & 2.630 & 2.593 & 2.677 & 2.676 & 1.117 & 1.132 & 0.020 & 0.035 & 1.533 & 1.496 & 1.560 & 1.544 & 463.215 & 463.267 & 1110.330 & 1094.872 & 0.000 & 0.000 & 647.115 & 631.605 & 0.381 & 2.174 \\ 
PY-TPA & 0.764 & 142 & 143 & 1.149 & 2.817 & 2.791 & 3.177 & 3.149 & 1.296 & 1.297 & 0.147 & 0.148 & 1.668 & 1.641 & 1.881 & 1.852 & 390.256 & 393.751 & 956.789 & 956.209 & 0.890 & 0.816 & 566.534 & 562.459 & 0.283 & 9.098 \\ 
CN-TPA & 2.857 & 95 & 96 & 2.924 & 3.188 & 3.163 & 3.772 & 3.722 & 3.460 & 3.442 & 0.536 & 0.517 & 0.264 & 0.239 & 0.312 & 0.281 & 328.670 & 333.085 & 358.306 & 360.260 & 0.615 & 0.532 & 29.636 & 27.175 & 0.632 & 2.571 \\ 
DMIC-TRZ & 0.961 & 110 & 111 & 0.919 & 0.817 & 0.542 & 1.488 & 1.354 & 1.675 & 2.296 & 0.755 & 1.377 & -0.102 & -0.377 & -0.186 & -0.942 & 833.003 & 915.891 & 740.420 & 539.975 & 0.199 & 0.123 & -92.583 & -375.917 & 0.773 & 1.015 \\ 
NyDPAc & 1.451 & 130 & 131 & 1.683 & 3.337 & 3.303 & 3.695 & 3.693 & 1.863 & 1.881 & 0.181 & 0.199 & 1.654 & 1.620 & 1.832 & 1.812 & 335.537 & 335.737 & 665.343 & 659.035 & 0.039 & 0.062 & 329.806 & 323.298 & 0.029 & 10.531 \\ 
oCBP & 2.826 & 89 & 90 & 2.869 & 3.328 & 3.306 & 3.816 & 3.748 & 3.289 & 3.252 & 0.420 & 0.383 & 0.460 & 0.437 & 0.527 & 0.495 & 324.949 & 330.836 & 377.011 & 381.224 & 0.143 & 0.117 & 52.063 & 50.388 & 0.393 & 2.769 \\ 
PABP & 2.136 & 127 & 128 & 1.890 & 2.255 & 2.185 & 3.200 & 3.032 & 2.683 & 2.622 & 0.793 & 0.732 & 0.365 & 0.296 & 0.518 & 0.410 & 387.390 & 408.919 & 462.161 & 472.871 & 0.973 & 0.701 & 74.771 & 63.952 & 0.917 & 0.890 \\ 
DHID-DPS & 2.043 & 124 & 125 & 2.130 & 2.867 & 2.835 & 3.498 & 3.430 & 2.599 & 2.577 & 0.469 & 0.447 & 0.737 & 0.705 & 0.899 & 0.853 & 354.423 & 361.491 & 477.055 & 481.071 & 0.181 & 0.156 & 122.632 & 119.580 & 0.406 & 4.823 \\ 
4FBTPI & 1.923 & 185 & 186 & 2.030 & 3.447 & 3.421 & 3.846 & 3.811 & 2.266 & 2.262 & 0.235 & 0.232 & 1.416 & 1.390 & 1.580 & 1.549 & 322.380 & 325.307 & 547.267 & 548.022 & 1.153 & 1.025 & 224.887 & 222.715 & 0.403 & 1.157 \\ 
BCzBMes & 2.742 & 123 & 124 & 2.729 & 3.361 & 3.339 & 3.804 & 3.734 & 3.088 & 3.052 & 0.359 & 0.323 & 0.632 & 0.610 & 0.715 & 0.682 & 325.974 & 332.041 & 401.494 & 406.241 & 0.172 & 0.141 & 75.520 & 74.200 & 0.487 & 6.446 \\ 
CCDMB & 2.287 & 123 & 124 & 2.570 & 3.306 & 3.284 & 3.747 & 3.684 & 2.913 & 2.883 & 0.343 & 0.313 & 0.736 & 0.714 & 0.834 & 0.801 & 330.889 & 336.548 & 425.632 & 430.056 & 0.393 & 0.285 & 94.743 & 93.509 & 0.255 & 8.313 \\ 
PCDMB & 1.830 & 126 & 127 & 2.457 & 2.668 & 2.636 & 3.031 & 2.994 & 2.791 & 2.790 & 0.334 & 0.333 & 0.211 & 0.179 & 0.240 & 0.204 & 409.054 & 414.178 & 444.179 & 444.433 & 0.017 & 0.015 & 35.125 & 30.255 & 0.080 & 10.227 \\ 
BTrztCz & 1.441 & 207 & 208 & 1.689 & 3.381 & 3.362 & 3.624 & 3.612 & 1.810 & 1.814 & 0.121 & 0.125 & 1.693 & 1.674 & 1.814 & 1.798 & 342.091 & 343.285 & 685.038 & 683.545 & 0.089 & 0.074 & 342.947 & 340.260 & 0.128 & 4.457 \\ 
DHID-DBS & 1.818 & 135 & 136 & 2.070 & 2.849 & 2.817 & 3.496 & 3.429 & 2.540 & 2.519 & 0.470 & 0.449 & 0.779 & 0.747 & 0.956 & 0.910 & 354.656 & 361.618 & 488.171 & 492.180 & 0.532 & 0.445 & 133.515 & 130.563 & 0.374 & 3.871 \\ 
CZ-DPS-DMAC & 2.159 & 137 & 138 & 2.551 & 3.429 & 3.406 & 3.813 & 3.791 & 2.836 & 2.839 & 0.285 & 0.289 & 0.879 & 0.855 & 0.977 & 0.952 & 325.187 & 327.049 & 437.179 & 436.656 & 0.037 & 0.038 & 111.992 & 109.607 & 0.291 & 4.255 \\ 
XT-T & 3.061 & 120 & 121 & 3.074 & 3.595 & 3.571 & 4.152 & 4.110 & 3.550 & 3.538 & 0.476 & 0.464 & 0.521 & 0.497 & 0.602 & 0.572 & 298.628 & 301.650 & 349.223 & 350.451 & 0.048 & 0.034 & 50.595 & 48.801 & 0.397 & 0.427 \\ 
3DPTIA & 2.065 & 112 & 113 & 2.303 & 3.244 & 3.222 & 3.682 & 3.609 & 2.614 & 2.579 & 0.311 & 0.276 & 0.941 & 0.919 & 1.068 & 1.029 & 336.712 & 343.551 & 474.334 & 480.657 & 0.141 & 0.115 & 137.622 & 137.105 & 0.170 & 6.113 \\ 
PyIAnTPh & 2.116 & 146 & 147 & 1.847 & 2.291 & 2.221 & 3.266 & 3.105 & 2.633 & 2.582 & 0.786 & 0.735 & 0.444 & 0.374 & 0.633 & 0.523 & 379.633 & 399.266 & 470.880 & 480.209 & 0.736 & 0.513 & 91.248 & 80.942 & 0.875 & 1.790 \\ 
2CzP-INN & 1.788 & 107 & 108 & 2.237 & 3.443 & 3.421 & 3.903 & 3.844 & 2.535 & 2.514 & 0.298 & 0.277 & 1.206 & 1.184 & 1.367 & 1.330 & 317.688 & 322.573 & 488.997 & 493.257 & 0.682 & 0.534 & 171.309 & 170.684 & 0.213 & 2.431 \\ 
VBN0 & 2.135 & 129 & 130 & 2.543 & 3.145 & 3.121 & 3.656 & 3.613 & 2.955 & 2.944 & 0.413 & 0.401 & 0.603 & 0.578 & 0.700 & 0.669 & 339.135 & 343.123 & 419.513 & 421.114 & 0.536 & 0.479 & 80.378 & 77.991 & 0.332 & 1.907 \\ 
PIAnTPh & 2.103 & 142 & 143 & 1.849 & 2.245 & 2.175 & 3.252 & 3.102 & 2.679 & 2.637 & 0.829 & 0.787 & 0.396 & 0.326 & 0.573 & 0.465 & 381.290 & 399.756 & 462.884 & 470.214 & 0.833 & 0.596 & 81.594 & 70.458 & 0.924 & 0.245 \\ 
BCZ-DPS-AD & 2.154 & 146 & 147 & 2.559 & 3.344 & 3.321 & 3.786 & 3.710 & 2.897 & 2.860 & 0.338 & 0.300 & 0.785 & 0.761 & 0.888 & 0.851 & 327.489 & 334.153 & 427.915 & 433.580 & 0.126 & 0.105 & 100.426 & 99.427 & 0.208 & 3.390 \\ 
2BTPA-INN & 1.612 & 165 & 166 & 2.036 & 3.138 & 3.115 & 3.633 & 3.619 & 2.358 & 2.366 & 0.321 & 0.329 & 1.102 & 1.078 & 1.276 & 1.253 & 341.235 & 342.630 & 525.841 & 524.071 & 1.983 & 1.866 & 184.606 & 181.441 & 0.274 & 3.336 \\ 
SpiroAc & 2.708 & 61 & 62 & 3.005 & 3.455 & 3.421 & 4.090 & 4.014 & 3.557 & 3.525 & 0.552 & 0.521 & 0.450 & 0.417 & 0.533 & 0.489 & 303.162 & 308.841 & 348.609 & 351.686 & 0.107 & 0.089 & 45.447 & 42.845 & 0.168 & 3.741 \\ 
BuPCzBCO & 3.105 & 66 & 67 & 3.089 & 3.362 & 3.338 & 3.790 & 3.718 & 3.483 & 3.441 & 0.394 & 0.352 & 0.273 & 0.249 & 0.307 & 0.278 & 327.118 & 333.443 & 355.999 & 360.357 & 0.140 & 0.118 & 28.882 & 26.914 & 0.633 & 0.846 \\ 
AQ-S-CZ & 0.892 & 85 & 86 & 1.422 & 2.370 & 2.347 & 2.807 & 2.752 & 1.684 & 1.667 & 0.262 & 0.245 & 0.948 & 0.925 & 1.123 & 1.084 & 441.712 & 450.540 & 736.080 & 743.569 & 0.186 & 0.160 & 294.368 & 293.029 & 0.140 & 8.374 \\ 
DBP-3TPA & 1.328 & 186 & 187 & 1.360 & 3.034 & 3.000 & 3.272 & 3.272 & 1.467 & 1.483 & 0.107 & 0.123 & 1.674 & 1.640 & 1.805 & 1.788 & 378.878 & 378.971 & 845.167 & 835.955 & 0.007 & 0.008 & 466.288 & 456.984 & 0.289 & 6.609 \\ 
DCzIPN & 2.108 & 83 & 84 & 2.350 & 3.069 & 3.050 & 3.538 & 3.495 & 2.709 & 2.693 & 0.359 & 0.343 & 0.718 & 0.700 & 0.828 & 0.802 & 350.466 & 354.737 & 457.612 & 460.397 & 0.304 & 0.231 & 107.146 & 105.660 & 0.495 & 3.182 \\ 
DMeCzIPN & 1.982 & 89 & 90 & 2.271 & 3.070 & 3.055 & 3.446 & 3.413 & 2.549 & 2.536 & 0.278 & 0.266 & 0.799 & 0.784 & 0.897 & 0.876 & 359.771 & 363.302 & 486.442 & 488.817 & 0.179 & 0.154 & 126.671 & 125.514 & 0.378 & 1.829 \\ 
SAFDPA & 2.581 & 106 & 107 & 2.782 & 3.310 & 3.291 & 3.668 & 3.626 & 3.082 & 3.065 & 0.301 & 0.283 & 0.529 & 0.510 & 0.586 & 0.562 & 338.025 & 341.893 & 402.267 & 404.560 & 0.058 & 0.048 & 64.242 & 62.666 & 0.164 & 3.945 \\ 
t-DABNA & 2.351 & 125 & 126 & 2.503 & 2.648 & 2.622 & 3.136 & 3.053 & 2.964 & 2.914 & 0.461 & 0.411 & 0.145 & 0.120 & 0.172 & 0.139 & 395.408 & 406.080 & 418.366 & 425.503 & 0.471 & 0.381 & 22.958 & 19.424 & 0.587 & 1.225 \\ 
3-AcBPtCN & 1.005 & 102 & 103 & 1.020 & 2.023 & 1.989 & 2.501 & 2.442 & 1.261 & 1.252 & 0.241 & 0.232 & 1.003 & 0.969 & 1.240 & 1.190 & 495.659 & 507.799 & 983.145 & 990.543 & 0.435 & 0.381 & 487.486 & 482.744 & 0.442 & 5.969 \\ 
3-AcBPdCN & 1.114 & 98 & 99 & 1.070 & 2.097 & 2.063 & 2.620 & 2.553 & 1.337 & 1.324 & 0.267 & 0.254 & 1.027 & 0.993 & 1.283 & 1.229 & 473.258 & 485.641 & 927.276 & 936.113 & 0.613 & 0.522 & 454.018 & 450.471 & 0.467 & 5.982 \\ 
11-AcBPdCN & 1.284 & 98 & 99 & 1.197 & 1.915 & 1.873 & 2.502 & 2.411 & 1.564 & 1.541 & 0.367 & 0.344 & 0.718 & 0.676 & 0.938 & 0.870 & 495.481 & 514.223 & 792.801 & 804.662 & 0.447 & 0.358 & 297.320 & 290.440 & 0.538 & 0.464 \\ 
PID-3 & 1.991 & 78 & 79 & 1.810 & 2.487 & 2.427 & 3.362 & 3.273 & 2.448 & 2.442 & 0.637 & 0.631 & 0.677 & 0.617 & 0.915 & 0.832 & 368.737 & 378.751 & 506.559 & 507.785 & 1.762 & 1.414 & 137.822 & 129.034 & 0.778 & 2.473 \\ 
3-ACBPmCN & 0.875 & 94 & 95 & 1.237 & 3.071 & 3.038 & 3.200 & 3.198 & 1.289 & 1.303 & 0.052 & 0.065 & 1.833 & 1.801 & 1.910 & 1.895 & 387.487 & 387.693 & 961.553 & 951.851 & 0.017 & 0.018 & 574.066 & 564.158 & 0.150 & 7.608 \\ 
3-DTPA-BBI & 1.102 & 139 & 140 & 1.466 & 2.289 & 2.250 & 2.868 & 2.813 & 1.836 & 1.833 & 0.370 & 0.367 & 0.824 & 0.784 & 1.032 & 0.980 & 432.332 & 440.754 & 675.243 & 676.550 & 1.790 & 1.518 & 242.911 & 235.796 & 0.294 & 7.113 \\ 
IABTCN & 0.894 & 123 & 124 & 1.401 & 2.242 & 2.203 & 2.857 & 2.798 & 1.785 & 1.779 & 0.384 & 0.379 & 0.841 & 0.802 & 1.072 & 1.019 & 433.936 & 443.086 & 694.648 & 696.862 & 1.607 & 1.333 & 260.712 & 253.776 & 0.418 & 6.936 \\ 
BTZPP & 0.997 & 142 & 143 & 1.458 & 2.917 & 2.872 & 3.483 & 3.451 & 1.741 & 1.752 & 0.283 & 0.294 & 1.459 & 1.414 & 1.743 & 1.700 & 355.959 & 359.218 & 712.342 & 707.774 & 2.957 & 2.627 & 356.383 & 348.556 & 0.256 & 3.507 \\ 
DPimdPPA & 1.838 & 78 & 79 & 1.820 & 2.683 & 2.638 & 3.431 & 3.373 & 2.328 & 2.328 & 0.507 & 0.508 & 0.863 & 0.817 & 1.103 & 1.045 & 361.375 & 367.557 & 532.653 & 532.538 & 2.184 & 1.853 & 171.278 & 164.981 & 0.545 & 5.727 \\ 
BCzPh & 2.953 & 89 & 90 & 2.835 & 3.354 & 3.331 & 3.841 & 3.770 & 3.247 & 3.208 & 0.412 & 0.373 & 0.519 & 0.496 & 0.594 & 0.561 & 322.825 & 328.888 & 381.893 & 386.444 & 0.160 & 0.112 & 59.068 & 57.556 & 0.741 & 0.422 \\ 
TBPM2CN & 1.759 & 149 & 150 & 2.072 & 3.337 & 3.307 & 3.737 & 3.704 & 2.321 & 2.322 & 0.248 & 0.249 & 1.265 & 1.234 & 1.416 & 1.383 & 331.792 & 334.703 & 534.270 & 534.031 & 0.818 & 0.723 & 202.477 & 199.328 & 0.119 & 16.773 \\ 
TPM2CN & 1.837 & 135 & 136 & 2.068 & 3.354 & 3.323 & 3.749 & 3.718 & 2.311 & 2.314 & 0.243 & 0.246 & 1.286 & 1.255 & 1.437 & 1.405 & 330.748 & 333.452 & 536.405 & 535.872 & 0.818 & 0.709 & 205.657 & 202.420 & 0.247 & 12.075 \\ 
PT-BZ-DMAC & 1.383 & 90 & 91 & 2.071 & 3.384 & 3.360 & 3.469 & 3.464 & 2.123 & 2.135 & 0.052 & 0.064 & 1.313 & 1.289 & 1.345 & 1.329 & 357.437 & 357.932 & 583.949 & 580.662 & 0.130 & 0.125 & 226.512 & 222.730 & 0.164 & 6.524 \\ 
PS-BZ-DMAC & 1.920 & 96 & 97 & 1.999 & 2.607 & 2.569 & 3.389 & 3.304 & 2.599 & 2.571 & 0.599 & 0.572 & 0.608 & 0.570 & 0.790 & 0.733 & 365.843 & 375.255 & 477.112 & 482.272 & 1.156 & 0.970 & 111.269 & 107.017 & 0.443 & 4.949 \\ 
2PCzBN-tPh & 2.099 & 161 & 162 & 2.393 & 3.411 & 3.389 & 3.755 & 3.727 & 2.635 & 2.632 & 0.241 & 0.239 & 1.018 & 0.996 & 1.120 & 1.095 & 330.175 & 332.638 & 470.577 & 471.071 & 0.661 & 0.609 & 140.402 & 138.433 & 0.330 & 1.749 \\ 
2PCzBN & 2.149 & 135 & 136 & 2.558 & 3.404 & 3.383 & 3.826 & 3.794 & 2.875 & 2.869 & 0.317 & 0.311 & 0.846 & 0.825 & 0.951 & 0.925 & 324.049 & 326.790 & 431.272 & 432.212 & 0.742 & 0.656 & 107.223 & 105.422 & 0.337 & 1.215 \\ 
TPA-2 & 0.594 & 137 & 138 & 0.746 & 2.130 & 2.108 & 2.453 & 2.448 & 0.859 & 0.866 & 0.113 & 0.120 & 1.384 & 1.362 & 1.594 & 1.582 & 505.521 & 506.430 & 1443.327 & 1431.459 & 0.048 & 0.081 & 937.805 & 925.029 & 0.380 & 6.413 \\ 
36DTPAFM & 0.789 & 131 & 132 & 1.242 & 2.243 & 2.205 & 2.648 & 2.629 & 1.466 & 1.481 & 0.224 & 0.239 & 1.001 & 0.963 & 1.182 & 1.148 & 468.254 & 471.566 & 845.764 & 837.166 & 0.342 & 0.325 & 377.510 & 365.600 & 0.308 & 6.338 \\ 
AQTC & 1.140 & 58 & 59 & 1.321 & 2.812 & 2.761 & 3.279 & 3.278 & 1.541 & 1.568 & 0.219 & 0.247 & 1.491 & 1.440 & 1.738 & 1.709 & 378.116 & 378.254 & 804.763 & 790.487 & 0.005 & 0.005 & 426.647 & 412.233 & 0.452 & 1.408 \\ 
3TPAFM & 0.744 & 86 & 87 & 1.373 & 2.173 & 2.144 & 2.475 & 2.447 & 1.563 & 1.567 & 0.191 & 0.194 & 0.800 & 0.771 & 0.911 & 0.880 & 501.027 & 506.678 & 793.037 & 791.461 & 0.231 & 0.220 & 292.010 & 284.783 & 0.361 & 8.772 \\ 
BBPA & 2.116 & 91 & 92 & 1.898 & 2.225 & 2.154 & 3.175 & 3.001 & 2.709 & 2.645 & 0.810 & 0.746 & 0.327 & 0.256 & 0.466 & 0.356 & 390.563 & 413.129 & 457.732 & 468.795 & 0.416 & 0.288 & 67.169 & 55.665 & 0.931 & 0.049 \\ 
DMPA & 2.149 & 85 & 86 & 1.900 & 2.263 & 2.192 & 3.223 & 3.059 & 2.706 & 2.651 & 0.806 & 0.752 & 0.363 & 0.292 & 0.517 & 0.408 & 384.722 & 405.283 & 458.209 & 467.636 & 0.445 & 0.317 & 73.487 & 62.353 & 0.927 & 0.008 \\ 
PXZ-NAI & 0.945 & 83 & 84 & 1.534 & 1.525 & 1.508 & 1.834 & 1.798 & 1.845 & 1.829 & 0.311 & 0.295 & -0.009 & -0.026 & -0.011 & -0.031 & 675.995 & 689.529 & 671.882 & 677.874 & 0.223 & 0.186 & -4.113 & -11.655 & 0.418 & 4.495 \\ 
PTZ-NAI & 0.739 & 83 & 84 & 1.476 & 1.878 & 1.870 & 2.027 & 2.014 & 1.593 & 1.589 & 0.117 & 0.113 & 0.403 & 0.395 & 0.435 & 0.425 & 611.513 & 615.612 & 778.316 & 780.238 & 0.115 & 0.105 & 166.803 & 164.626 & 0.314 & 5.274 \\ 
AI-4Cz & 1.299 & 161 & 162 & 1.647 & 2.355 & 2.341 & 2.682 & 2.645 & 1.876 & 1.861 & 0.229 & 0.214 & 0.708 & 0.694 & 0.806 & 0.784 & 462.334 & 468.732 & 660.958 & 666.148 & 0.052 & 0.049 & 198.624 & 197.417 & 0.382 & 1.460 \\ 
DAcIPN & 1.861 & 101 & 102 & 1.966 & 2.881 & 2.855 & 3.369 & 3.322 & 2.299 & 2.287 & 0.333 & 0.321 & 0.915 & 0.889 & 1.070 & 1.035 & 368.015 & 373.233 & 539.288 & 542.055 & 0.113 & 0.107 & 171.273 & 168.822 & 0.271 & 4.161 \\ 
TCz1 & 2.718 & 115 & 116 & 2.803 & 3.163 & 3.139 & 3.637 & 3.562 & 3.224 & 3.180 & 0.421 & 0.377 & 0.360 & 0.336 & 0.414 & 0.382 & 340.859 & 348.084 & 384.607 & 389.866 & 0.047 & 0.037 & 43.748 & 41.782 & 0.487 & 1.544 \\ 
MBF & 0.908 & 92 & 93 & 1.645 & 2.307 & 2.294 & 2.624 & 2.598 & 1.871 & 1.863 & 0.226 & 0.218 & 0.662 & 0.649 & 0.753 & 0.735 & 472.573 & 477.285 & 662.713 & 665.519 & 0.857 & 0.758 & 190.140 & 188.234 & 0.340 & 7.954 \\ 
MPA & 1.327 & 84 & 85 & 1.955 & 2.752 & 2.721 & 3.114 & 3.075 & 2.212 & 2.209 & 0.257 & 0.254 & 0.797 & 0.766 & 0.902 & 0.866 & 398.164 & 403.227 & 560.497 & 561.210 & 0.017 & 0.014 & 162.334 & 157.983 & 0.153 & 9.322 \\ 
3,3-NHC & 2.612 & 85 & 86 & 2.256 & 3.239 & 3.192 & 4.179 & 4.093 & 2.911 & 2.892 & 0.655 & 0.636 & 0.983 & 0.937 & 1.268 & 1.201 & 296.670 & 302.910 & 425.956 & 428.672 & 0.466 & 0.414 & 129.286 & 125.762 & 0.113 & 6.055 \\ 
3CP-DPS-DMAC & 2.250 & 107 & 108 & 2.815 & 3.359 & 3.335 & 3.804 & 3.729 & 3.188 & 3.148 & 0.373 & 0.333 & 0.544 & 0.520 & 0.616 & 0.581 & 325.931 & 332.460 & 388.872 & 393.851 & 0.158 & 0.127 & 62.941 & 61.391 & 0.240 & 4.026 \\ 
3CP-DPS-PXZ & 2.203 & 101 & 102 & 2.550 & 2.761 & 2.730 & 3.129 & 3.091 & 2.890 & 2.887 & 0.340 & 0.337 & 0.211 & 0.179 & 0.240 & 0.203 & 396.204 & 401.152 & 429.046 & 429.386 & 0.013 & 0.011 & 32.842 & 28.234 & 0.347 & 3.958 \\ 
3CzAnN & 2.085 & 100 & 101 & 1.848 & 2.250 & 2.180 & 3.259 & 3.112 & 2.677 & 2.639 & 0.829 & 0.791 & 0.402 & 0.332 & 0.582 & 0.474 & 380.425 & 398.394 & 463.112 & 469.896 & 0.757 & 0.547 & 82.687 & 71.502 & 0.864 & 1.262 \\ 
DPQ-DMAC & 1.072 & 91 & 92 & 1.438 & 2.906 & 2.898 & 3.018 & 3.009 & 1.494 & 1.493 & 0.056 & 0.055 & 1.468 & 1.460 & 1.525 & 1.516 & 410.789 & 412.072 & 830.105 & 830.349 & 0.110 & 0.105 & 419.316 & 418.277 & 0.257 & 5.546 \\ 
DPAA & 2.156 & 61 & 62 & 1.902 & 2.257 & 2.183 & 3.315 & 3.129 & 2.794 & 2.726 & 0.892 & 0.824 & 0.355 & 0.281 & 0.521 & 0.403 & 373.998 & 396.192 & 443.732 & 454.774 & 0.401 & 0.286 & 69.734 & 58.582 & 0.937 & 0.000 \\ 
t3Cz-SO & 2.148 & 176 & 177 & 2.456 & 3.188 & 3.168 & 3.634 & 3.568 & 2.800 & 2.766 & 0.344 & 0.310 & 0.732 & 0.712 & 0.835 & 0.802 & 341.150 & 347.450 & 442.875 & 448.182 & 0.244 & 0.206 & 101.725 & 100.732 & 0.249 & 7.403 \\ 
Cz-SO & 2.722 & 68 & 69 & 2.982 & 3.421 & 3.398 & 3.873 & 3.802 & 3.376 & 3.336 & 0.394 & 0.354 & 0.439 & 0.416 & 0.497 & 0.466 & 320.149 & 326.120 & 367.297 & 371.654 & 0.261 & 0.224 & 47.148 & 45.534 & 0.394 & 4.761 \\ 
DPQ-PXZ & 1.083 & 85 & 86 & 1.416 & 2.336 & 2.325 & 2.558 & 2.536 & 1.551 & 1.545 & 0.135 & 0.129 & 0.920 & 0.909 & 1.007 & 0.991 & 484.597 & 488.858 & 799.329 & 802.423 & 0.223 & 0.201 & 314.732 & 313.565 & 0.347 & 5.470 \\ 
pCzAnN & 2.098 & 100 & 101 & 1.848 & 2.259 & 2.189 & 3.287 & 3.128 & 2.690 & 2.642 & 0.842 & 0.794 & 0.410 & 0.340 & 0.597 & 0.486 & 377.173 & 396.318 & 460.870 & 469.255 & 0.711 & 0.503 & 83.697 & 72.937 & 0.859 & 1.501 \\ 
3-BHH & 2.640 & 77 & 78 & 2.790 & 3.172 & 3.129 & 4.150 & 4.056 & 3.649 & 3.616 & 0.859 & 0.826 & 0.383 & 0.339 & 0.501 & 0.440 & 298.757 & 305.719 & 339.773 & 342.901 & 0.146 & 0.129 & 41.016 & 37.183 & 0.191 & 5.275 \\ 
DPP-PXZ & 0.900 & 85 & 86 & 1.034 & 1.817 & 1.802 & 2.097 & 2.063 & 1.193 & 1.184 & 0.159 & 0.149 & 0.783 & 0.768 & 0.904 & 0.879 & 591.274 & 600.990 & 1038.948 & 1047.478 & 0.225 & 0.193 & 447.674 & 446.488 & 0.471 & 4.536 \\ 
APPT-PXZ & 1.074 & 97 & 98 & 1.374 & 1.687 & 1.674 & 1.958 & 1.930 & 1.594 & 1.584 & 0.220 & 0.210 & 0.313 & 0.300 & 0.363 & 0.346 & 633.380 & 642.538 & 777.782 & 782.761 & 0.308 & 0.270 & 144.401 & 140.223 & 0.354 & 5.297 \\ 
HITPE & 2.597 & 133 & 134 & 1.833 & 3.114 & 3.078 & 3.881 & 3.828 & 2.284 & 2.280 & 0.451 & 0.447 & 1.281 & 1.245 & 1.596 & 1.548 & 319.497 & 323.905 & 542.740 & 543.866 & 1.052 & 0.880 & 223.243 & 219.961 & 0.784 & 3.338 \\ 
DV-3CzCN & 2.165 & 184 & 185 & 2.465 & 3.341 & 3.318 & 3.803 & 3.771 & 2.805 & 2.801 & 0.340 & 0.336 & 0.876 & 0.853 & 0.997 & 0.970 & 326.060 & 328.801 & 441.983 & 442.617 & 0.191 & 0.165 & 115.924 & 113.817 & 0.327 & 1.817 \\ 
SF-DPSO & 2.818 & 152 & 153 & 2.720 & 3.794 & 3.761 & 4.499 & 4.461 & 3.225 & 3.226 & 0.505 & 0.506 & 1.074 & 1.041 & 1.274 & 1.235 & 275.600 & 277.942 & 384.473 & 384.356 & 2.115 & 1.936 & 108.873 & 106.415 & 0.571 & 1.629 \\ 
BDQ-tBuCz & 1.394 & 160 & 161 & 1.475 & 2.472 & 2.448 & 2.786 & 2.752 & 1.662 & 1.659 & 0.187 & 0.183 & 0.997 & 0.973 & 1.123 & 1.094 & 445.074 & 450.475 & 745.897 & 747.558 & 0.347 & 0.302 & 300.824 & 297.083 & 0.569 & 1.437 \\ 
BDQDMAC & 1.166 & 130 & 131 & 1.354 & 2.527 & 2.514 & 2.664 & 2.651 & 1.428 & 1.428 & 0.074 & 0.074 & 1.173 & 1.160 & 1.237 & 1.224 & 465.371 & 467.600 & 868.449 & 868.292 & 0.131 & 0.119 & 403.078 & 400.692 & 0.428 & 1.518 \\ 
BDQPCz & 1.552 & 140 & 141 & 1.546 & 3.091 & 3.054 & 3.437 & 3.426 & 1.719 & 1.734 & 0.173 & 0.188 & 1.545 & 1.509 & 1.718 & 1.692 & 360.755 & 361.892 & 721.426 & 715.108 & 0.133 & 0.156 & 360.671 & 353.216 & 0.591 & 0.496 \\ 
4-SCZ & 2.800 & 74 & 75 & 2.637 & 3.120 & 3.090 & 3.675 & 3.594 & 3.106 & 3.067 & 0.469 & 0.430 & 0.483 & 0.453 & 0.569 & 0.526 & 337.409 & 344.995 & 399.209 & 404.207 & 0.186 & 0.154 & 61.800 & 59.213 & 0.745 & 1.167 \\ 
Py-TPA & 0.623 & 152 & 153 & 1.076 & 2.704 & 2.680 & 3.040 & 3.012 & 1.210 & 1.209 & 0.134 & 0.134 & 1.628 & 1.604 & 1.830 & 1.803 & 407.896 & 411.607 & 1025.047 & 1025.190 & 0.637 & 0.595 & 617.151 & 613.583 & 0.277 & 8.777 \\ 
DPACPhTPI & 2.215 & 155 & 156 & 2.312 & 3.401 & 3.372 & 3.768 & 3.728 & 2.562 & 2.556 & 0.250 & 0.244 & 1.088 & 1.060 & 1.206 & 1.171 & 329.054 & 332.611 & 483.883 & 485.044 & 0.402 & 0.364 & 154.829 & 152.432 & 0.099 & 9.175 \\ 
oPTBC & 1.624 & 88 & 89 & 2.169 & 2.560 & 2.553 & 2.711 & 2.698 & 2.297 & 2.292 & 0.128 & 0.123 & 0.391 & 0.385 & 0.414 & 0.406 & 457.304 & 459.507 & 539.822 & 540.983 & 0.091 & 0.080 & 82.519 & 81.475 & 0.300 & 3.364 \\ 
mPTBC & 1.519 & 88 & 89 & 2.089 & 2.671 & 2.661 & 2.949 & 2.926 & 2.307 & 2.297 & 0.218 & 0.208 & 0.582 & 0.572 & 0.643 & 0.628 & 420.399 & 423.776 & 537.511 & 539.718 & 0.278 & 0.246 & 117.111 & 115.942 & 0.299 & 5.329 \\ 
P3C & 1.982 & 99 & 100 & 1.802 & 2.598 & 2.531 & 3.496 & 3.411 & 2.425 & 2.428 & 0.623 & 0.626 & 0.796 & 0.729 & 1.071 & 0.983 & 354.615 & 363.473 & 511.188 & 510.604 & 1.113 & 0.953 & 156.573 & 147.131 & 0.893 & 1.604 \\ 
DBCP & 1.524 & 96 & 97 & 2.027 & 2.711 & 2.680 & 2.820 & 2.814 & 2.109 & 2.129 & 0.081 & 0.102 & 0.684 & 0.653 & 0.711 & 0.685 & 439.660 & 440.551 & 587.979 & 582.368 & 0.052 & 0.048 & 148.319 & 141.817 & 0.198 & 5.572 \\ 
NAQ3 & 1.426 & 115 & 116 & 1.523 & 2.118 & 2.097 & 2.516 & 2.476 & 1.809 & 1.799 & 0.286 & 0.276 & 0.595 & 0.573 & 0.707 & 0.677 & 492.744 & 500.744 & 685.191 & 689.183 & 0.470 & 0.404 & 192.448 & 188.439 & 0.528 & 2.367 \\ 
mCP-BP-DMAC & 1.541 & 127 & 128 & 2.169 & 2.751 & 2.719 & 3.115 & 3.078 & 2.457 & 2.455 & 0.287 & 0.286 & 0.581 & 0.550 & 0.658 & 0.622 & 398.010 & 402.860 & 504.632 & 504.950 & 0.017 & 0.014 & 106.622 & 102.090 & 0.256 & 6.193 \\ 
BFCZPZ3 & 2.229 & 107 & 108 & 2.326 & 3.248 & 3.225 & 3.685 & 3.649 & 2.639 & 2.632 & 0.314 & 0.306 & 0.922 & 0.899 & 1.046 & 1.017 & 336.420 & 339.785 & 469.749 & 471.102 & 0.677 & 0.597 & 133.329 & 131.317 & 0.504 & 0.007 \\ 
BTCZPZ1 & 1.982 & 107 & 108 & 2.154 & 3.086 & 3.065 & 3.458 & 3.418 & 2.414 & 2.403 & 0.259 & 0.248 & 0.932 & 0.911 & 1.044 & 1.016 & 358.595 & 362.707 & 513.680 & 516.001 & 0.774 & 0.673 & 155.085 & 153.294 & 0.485 & 1.336 \\ 
BFCZPZ2 & 2.172 & 107 & 108 & 2.180 & 3.166 & 3.142 & 3.590 & 3.551 & 2.471 & 2.464 & 0.292 & 0.284 & 0.987 & 0.962 & 1.119 & 1.088 & 345.370 & 349.114 & 501.681 & 503.243 & 1.679 & 1.480 & 156.311 & 154.130 & 0.518 & 0.613 \\ 
CZ9CZPZ & 1.865 & 135 & 136 & 2.152 & 3.199 & 3.176 & 3.669 & 3.624 & 2.468 & 2.456 & 0.316 & 0.304 & 1.047 & 1.024 & 1.201 & 1.168 & 337.951 & 342.101 & 502.337 & 504.833 & 1.513 & 1.309 & 164.386 & 162.732 & 0.277 & 2.453 \\ 
BFCZPZ1 & 2.130 & 107 & 108 & 2.218 & 3.086 & 3.063 & 3.475 & 3.434 & 2.497 & 2.486 & 0.279 & 0.269 & 0.868 & 0.845 & 0.978 & 0.948 & 356.820 & 361.028 & 496.496 & 498.656 & 0.906 & 0.786 & 139.676 & 137.628 & 0.587 & 0.117 \\ 
TPBPPI-PY & 2.589 & 152 & 153 & 2.421 & 3.493 & 3.463 & 3.894 & 3.857 & 2.699 & 2.696 & 0.278 & 0.275 & 1.072 & 1.042 & 1.195 & 1.161 & 318.357 & 321.486 & 459.356 & 459.887 & 0.267 & 0.248 & 140.999 & 138.401 & 0.458 & 5.189 \\ 
TPBPPI-PBI & 2.461 & 187 & 188 & 2.457 & 3.540 & 3.512 & 3.871 & 3.831 & 2.687 & 2.680 & 0.230 & 0.223 & 1.083 & 1.055 & 1.184 & 1.151 & 320.282 & 323.659 & 461.400 & 462.643 & 0.193 & 0.179 & 141.118 & 138.984 & 0.268 & 8.468 \\ 
PTZ-2PTO & 2.924 & 87 & 88 & 2.563 & 3.433 & 3.405 & 3.825 & 3.794 & 2.855 & 2.855 & 0.293 & 0.293 & 0.870 & 0.842 & 0.970 & 0.938 & 324.159 & 326.799 & 434.246 & 434.199 & 0.461 & 0.408 & 110.087 & 107.400 & 0.579 & 2.397 \\ 
4F-m-$\nu$-DABNA & 2.053 & 237 & 238 & 2.219 & 2.860 & 2.841 & 3.203 & 3.163 & 2.485 & 2.470 & 0.266 & 0.251 & 0.641 & 0.622 & 0.718 & 0.693 & 387.112 & 391.946 & 499.006 & 501.881 & 1.039 & 0.917 & 111.895 & 109.936 & 0.223 & 4.884 \\ 
m-$\nu$-DABNA & 2.204 & 225 & 226 & 2.288 & 2.793 & 2.773 & 3.147 & 3.104 & 2.578 & 2.561 & 0.290 & 0.274 & 0.506 & 0.485 & 0.570 & 0.543 & 393.951 & 399.369 & 481.024 & 484.061 & 0.881 & 0.772 & 87.073 & 84.691 & 0.530 & 0.629 \\ 
TPA-PyI & 2.203 & 117 & 118 & 2.241 & 3.372 & 3.345 & 3.822 & 3.800 & 2.541 & 2.546 & 0.299 & 0.305 & 1.131 & 1.104 & 1.282 & 1.254 & 324.379 & 326.257 & 488.027 & 486.966 & 1.801 & 1.642 & 163.648 & 160.709 & 0.324 & 8.790 \\ 
4F-$\nu$-DABNA & 2.112 & 213 & 214 & 2.234 & 2.836 & 2.816 & 3.187 & 3.147 & 2.511 & 2.496 & 0.277 & 0.262 & 0.602 & 0.582 & 0.677 & 0.651 & 388.994 & 394.001 & 493.846 & 496.727 & 0.974 & 0.855 & 104.851 & 102.726 & 0.231 & 4.663 \\ 
CBPTZ & 1.866 & 145 & 146 & 2.221 & 3.415 & 3.393 & 3.864 & 3.805 & 2.513 & 2.491 & 0.292 & 0.270 & 1.194 & 1.172 & 1.351 & 1.314 & 320.845 & 325.854 & 493.368 & 497.754 & 0.360 & 0.285 & 172.523 & 171.900 & 0.061 & 8.723 \\ 
CBPBM & 2.486 & 138 & 139 & 2.410 & 3.419 & 3.396 & 3.905 & 3.839 & 2.752 & 2.724 & 0.342 & 0.314 & 1.010 & 0.987 & 1.153 & 1.115 & 317.542 & 322.943 & 450.581 & 455.149 & 0.066 & 0.046 & 133.040 & 132.207 & 0.265 & 4.548 \\ 
CBPPY & 2.647 & 103 & 104 & 2.521 & 3.456 & 3.433 & 3.932 & 3.868 & 2.868 & 2.841 & 0.347 & 0.319 & 0.935 & 0.912 & 1.064 & 1.028 & 315.361 & 320.530 & 432.312 & 436.474 & 0.363 & 0.271 & 116.951 & 115.944 & 0.434 & 1.988 \\ 
N-B & 2.706 & 63 & 64 & 2.754 & 3.965 & 3.949 & 4.207 & 4.195 & 2.922 & 2.925 & 0.168 & 0.171 & 1.211 & 1.196 & 1.285 & 1.270 & 294.709 & 295.552 & 424.307 & 423.878 & 0.172 & 0.158 & 129.597 & 128.326 & 0.530 & 1.599 \\ 
DPACpBr & 3.185 & 85 & 86 & 2.993 & 3.541 & 3.517 & 4.019 & 3.983 & 3.397 & 3.389 & 0.404 & 0.396 & 0.548 & 0.525 & 0.622 & 0.594 & 308.472 & 311.307 & 364.978 & 365.877 & 0.403 & 0.358 & 56.506 & 54.570 & 0.615 & 1.282 \\ 
DPCN & 1.433 & 125 & 126 & 2.134 & 3.351 & 3.319 & 3.833 & 3.795 & 2.441 & 2.439 & 0.307 & 0.306 & 1.217 & 1.186 & 1.393 & 1.355 & 323.423 & 326.713 & 507.972 & 508.254 & 0.312 & 0.285 & 184.549 & 181.541 & 0.012 & 11.374 \\ 
BZC-PXZ & 1.318 & 78 & 79 & 1.889 & 2.463 & 2.450 & 2.761 & 2.732 & 2.118 & 2.106 & 0.229 & 0.218 & 0.574 & 0.561 & 0.644 & 0.626 & 448.974 & 453.772 & 585.411 & 588.664 & 0.269 & 0.232 & 136.437 & 134.891 & 0.073 & 6.678 \\ 
CzBN & 2.249 & 73 & 74 & 2.779 & 3.347 & 3.328 & 3.708 & 3.669 & 3.079 & 3.063 & 0.300 & 0.284 & 0.568 & 0.550 & 0.629 & 0.606 & 334.360 & 337.914 & 402.709 & 404.764 & 0.244 & 0.223 & 68.349 & 66.850 & 0.342 & 3.467 \\ 
2CzBN & 2.307 & 79 & 80 & 2.675 & 3.329 & 3.309 & 3.683 & 3.648 & 2.960 & 2.950 & 0.285 & 0.275 & 0.654 & 0.634 & 0.724 & 0.699 & 336.603 & 339.822 & 418.890 & 420.318 & 0.230 & 0.203 & 82.287 & 80.496 & 0.410 & 3.923 \\ 
TPA-DPPI & 2.157 & 166 & 167 & 2.189 & 3.458 & 3.429 & 3.879 & 3.842 & 2.456 & 2.453 & 0.266 & 0.264 & 1.269 & 1.240 & 1.423 & 1.389 & 319.662 & 322.691 & 504.914 & 505.497 & 0.129 & 0.060 & 185.252 & 182.806 & 0.067 & 9.978 \\ 
ANQDC-PSTA & 0.865 & 144 & 145 & 1.227 & 1.943 & 1.930 & 2.156 & 2.134 & 1.361 & 1.357 & 0.134 & 0.130 & 0.716 & 0.703 & 0.795 & 0.777 & 575.119 & 580.994 & 910.799 & 913.995 & 0.308 & 0.282 & 335.680 & 333.001 & 0.211 & 7.926 \\ 
pDPAPQ-PXZ & 1.156 & 107 & 108 & 1.418 & 1.786 & 1.773 & 2.032 & 2.007 & 1.614 & 1.606 & 0.196 & 0.188 & 0.368 & 0.355 & 0.418 & 0.402 & 610.158 & 617.605 & 768.395 & 772.154 & 0.291 & 0.261 & 158.236 & 154.549 & 0.362 & 5.054 \\ 
m-CZ-DPS-DMAC & 2.572 & 137 & 138 & 2.552 & 3.348 & 3.328 & 3.836 & 3.777 & 2.925 & 2.897 & 0.372 & 0.345 & 0.796 & 0.775 & 0.912 & 0.880 & 323.187 & 328.226 & 423.949 & 427.936 & 0.122 & 0.095 & 100.762 & 99.710 & 0.152 & 4.945 \\ 
pDPBPZ-PXZ & 0.891 & 112 & 113 & 1.233 & 2.768 & 2.737 & 2.990 & 2.975 & 1.332 & 1.340 & 0.099 & 0.107 & 1.535 & 1.504 & 1.658 & 1.635 & 414.718 & 416.740 & 930.846 & 925.110 & 0.410 & 0.386 & 516.128 & 508.370 & 0.244 & 7.913 \\ 
DDPhCz-DPPZ & 1.183 & 167 & 168 & 1.322 & 2.681 & 2.664 & 2.988 & 2.960 & 1.474 & 1.469 & 0.151 & 0.147 & 1.359 & 1.342 & 1.515 & 1.491 & 414.899 & 418.866 & 841.356 & 843.888 & 0.724 & 0.659 & 426.457 & 425.022 & 0.362 & 6.293 \\ 
DCz-DPPZ & 1.339 & 111 & 112 & 1.355 & 2.579 & 2.559 & 2.965 & 2.924 & 1.558 & 1.548 & 0.202 & 0.193 & 1.224 & 1.204 & 1.407 & 1.376 & 418.216 & 424.052 & 796.045 & 800.832 & 0.712 & 0.624 & 377.829 & 376.780 & 0.584 & 0.176 \\ 
Oxd-bCZ & 2.003 & 129 & 130 & 2.215 & 3.379 & 3.345 & 3.856 & 3.813 & 2.528 & 2.525 & 0.313 & 0.310 & 1.164 & 1.130 & 1.328 & 1.288 & 321.544 & 325.153 & 490.524 & 491.083 & 2.210 & 1.638 & 168.980 & 165.929 & 0.287 & 2.630 \\ 
Fene & 1.671 & 90 & 91 & 1.966 & 2.739 & 2.714 & 3.014 & 3.002 & 2.163 & 2.175 & 0.197 & 0.209 & 0.773 & 0.748 & 0.851 & 0.827 & 411.429 & 412.992 & 573.287 & 570.065 & 0.069 & 0.070 & 161.857 & 157.073 & 0.265 & 3.944 \\ 
Fens & 1.650 & 90 & 91 & 2.146 & 2.738 & 2.710 & 3.182 & 3.164 & 2.494 & 2.505 & 0.348 & 0.359 & 0.592 & 0.564 & 0.688 & 0.658 & 389.593 & 391.909 & 497.033 & 494.892 & 0.029 & 0.115 & 107.440 & 102.984 & 0.142 & 4.554 \\ 
Yad & 1.898 & 102 & 103 & 2.178 & 2.799 & 2.771 & 3.316 & 3.242 & 2.580 & 2.548 & 0.402 & 0.370 & 0.621 & 0.593 & 0.736 & 0.693 & 373.931 & 382.467 & 480.537 & 486.537 & 0.293 & 0.237 & 106.607 & 104.070 & 0.186 & 3.761 \\ 
DTPCZPYTZ & 1.931 & 159 & 160 & 1.866 & 2.716 & 2.653 & 3.617 & 3.529 & 2.486 & 2.482 & 0.619 & 0.616 & 0.850 & 0.787 & 1.131 & 1.046 & 342.782 & 351.349 & 498.822 & 499.449 & 1.679 & 1.408 & 156.040 & 148.099 & 0.360 & 8.969 \\ 
TPADSO2 & 1.687 & 91 & 92 & 2.190 & 3.041 & 3.014 & 3.586 & 3.539 & 2.583 & 2.572 & 0.392 & 0.382 & 0.851 & 0.824 & 1.004 & 0.967 & 345.716 & 350.327 & 480.045 & 482.049 & 1.207 & 1.077 & 134.329 & 131.722 & 0.267 & 8.376 \\ 
B4PyPPM & 2.183 & 113 & 114 & 2.223 & 3.989 & 3.975 & 3.960 & 3.958 & 2.206 & 2.213 & -0.016 & -0.009 & 1.767 & 1.752 & 1.754 & 1.745 & 313.099 & 313.210 & 561.942 & 560.154 & 0.010 & 0.010 & 248.843 & 246.944 & 0.466 & 1.341 \\ 
mAP & 2.753 & 93 & 94 & 3.094 & 3.385 & 3.353 & 4.082 & 4.027 & 3.731 & 3.716 & 0.637 & 0.622 & 0.291 & 0.259 & 0.351 & 0.311 & 303.764 & 307.921 & 332.306 & 333.679 & 0.094 & 0.059 & 28.542 & 25.758 & 0.251 & 1.788 \\ 
DBBPZ-DPXZ & 1.025 & 145 & 146 & 1.253 & 2.782 & 2.769 & 3.015 & 2.997 & 1.358 & 1.356 & 0.105 & 0.103 & 1.529 & 1.516 & 1.657 & 1.641 & 411.265 & 413.667 & 913.055 & 914.358 & 0.631 & 0.590 & 501.790 & 500.692 & 0.305 & 6.540 \\ 
DPIBPZ-DPXZ & 0.764 & 145 & 146 & 1.087 & 2.531 & 2.521 & 2.781 & 2.761 & 1.194 & 1.190 & 0.107 & 0.103 & 1.444 & 1.434 & 1.587 & 1.570 & 445.794 & 449.104 & 1038.238 & 1041.651 & 0.650 & 0.594 & 592.445 & 592.546 & 0.358 & 6.717 \\ 
m-DTPACO & 1.764 & 115 & 116 & 2.122 & 2.793 & 2.769 & 3.253 & 3.218 & 2.472 & 2.466 & 0.350 & 0.344 & 0.671 & 0.647 & 0.781 & 0.752 & 381.115 & 385.331 & 501.554 & 502.764 & 0.047 & 0.044 & 120.439 & 117.433 & 0.304 & 5.961 \\ 
mDPBPZ-DPXZ & 0.902 & 145 & 146 & 1.181 & 2.684 & 2.673 & 2.923 & 2.905 & 1.287 & 1.284 & 0.105 & 0.102 & 1.503 & 1.492 & 1.637 & 1.621 & 424.110 & 426.811 & 963.600 & 965.690 & 0.639 & 0.591 & 539.490 & 538.880 & 0.323 & 6.621 \\ 
p-DTPACO & 1.699 & 115 & 116 & 1.886 & 2.713 & 2.685 & 3.354 & 3.306 & 2.331 & 2.322 & 0.445 & 0.437 & 0.827 & 0.799 & 1.023 & 0.984 & 369.705 & 374.982 & 531.925 & 533.851 & 1.513 & 1.343 & 162.220 & 158.869 & 0.421 & 2.546 \\ 
2TDBA-SBA & 1.969 & 208 & 209 & 2.389 & 3.075 & 3.055 & 3.559 & 3.486 & 2.766 & 2.726 & 0.377 & 0.337 & 0.685 & 0.666 & 0.793 & 0.760 & 348.319 & 355.653 & 448.197 & 454.776 & 0.244 & 0.203 & 99.878 & 99.123 & 0.088 & 8.582 \\ 
TPA-APm & 0.762 & 91 & 92 & 0.695 & 2.530 & 2.495 & 2.636 & 2.635 & 0.724 & 0.734 & 0.029 & 0.039 & 1.834 & 1.800 & 1.912 & 1.901 & 470.296 & 470.493 & 1711.487 & 1688.984 & 0.000 & 0.000 & 1241.190 & 1218.491 & 0.544 & 0.160 \\ 
TPA-AP & 1.472 & 91 & 92 & 1.601 & 2.976 & 2.927 & 3.519 & 3.498 & 1.892 & 1.913 & 0.292 & 0.312 & 1.376 & 1.326 & 1.626 & 1.585 & 352.368 & 354.463 & 655.194 & 648.151 & 0.218 & 0.195 & 302.826 & 293.687 & 0.178 & 11.245 \\ 
TDBA-SBA & 1.909 & 162 & 163 & 2.534 & 3.075 & 3.055 & 3.561 & 3.486 & 2.935 & 2.892 & 0.401 & 0.358 & 0.541 & 0.521 & 0.626 & 0.594 & 348.182 & 355.612 & 422.440 & 428.705 & 0.279 & 0.227 & 74.258 & 73.092 & 0.024 & 10.295 \\ 
TPA-APy & 1.230 & 91 & 92 & 1.218 & 2.779 & 2.777 & 2.745 & 2.743 & 1.203 & 1.203 & -0.015 & -0.015 & 1.561 & 1.559 & 1.542 & 1.540 & 451.706 & 451.969 & 1030.393 & 1030.363 & 0.003 & 0.003 & 578.687 & 578.394 & 0.538 & 2.305 \\ 
TPD4PA & 2.113 & 142 & 143 & 2.399 & 2.887 & 2.866 & 3.288 & 3.231 & 2.732 & 2.704 & 0.334 & 0.306 & 0.488 & 0.468 & 0.556 & 0.527 & 377.058 & 383.686 & 453.789 & 458.502 & 0.256 & 0.221 & 76.731 & 74.817 & 0.345 & 6.033 \\ 
o-Ac2BBP & 1.242 & 131 & 132 & 1.560 & 3.106 & 3.099 & 3.233 & 3.226 & 1.624 & 1.624 & 0.064 & 0.064 & 1.546 & 1.538 & 1.609 & 1.601 & 383.484 & 384.364 & 763.383 & 763.287 & 0.067 & 0.064 & 379.899 & 378.923 & 0.149 & 5.789 \\ 
TPA-PyF2 & 2.613 & 185 & 186 & 2.890 & 3.485 & 3.463 & 3.941 & 3.899 & 3.268 & 3.254 & 0.378 & 0.364 & 0.595 & 0.573 & 0.673 & 0.645 & 314.617 & 317.998 & 379.417 & 381.063 & 0.047 & 0.038 & 64.801 & 63.065 & 0.129 & 4.154 \\ 
o-Px2BBP & 1.152 & 119 & 120 & 1.520 & 2.681 & 2.671 & 2.980 & 2.963 & 1.689 & 1.686 & 0.169 & 0.166 & 1.161 & 1.151 & 1.290 & 1.277 & 416.096 & 418.470 & 733.978 & 735.301 & 0.322 & 0.285 & 317.881 & 316.831 & 0.311 & 4.634 \\ 
D-BP-PXZ & 1.271 & 133 & 134 & 1.650 & 2.799 & 2.769 & 3.167 & 3.132 & 1.867 & 1.866 & 0.217 & 0.216 & 1.149 & 1.119 & 1.300 & 1.266 & 391.475 & 395.901 & 664.140 & 664.519 & 0.023 & 0.020 & 272.664 & 268.619 & 0.255 & 5.731 \\ 
BTD-PXZ & 0.976 & 55 & 56 & 1.758 & 2.569 & 2.551 & 2.820 & 2.796 & 1.929 & 1.926 & 0.172 & 0.168 & 0.811 & 0.794 & 0.890 & 0.870 & 439.691 & 443.434 & 642.574 & 643.704 & 0.128 & 0.110 & 202.883 & 200.270 & 0.347 & 5.322 \\ 
tBuCzDBA & 1.279 & 180 & 181 & 1.706 & 2.944 & 2.918 & 3.124 & 3.124 & 1.811 & 1.826 & 0.104 & 0.120 & 1.238 & 1.212 & 1.313 & 1.297 & 396.876 & 396.927 & 684.781 & 678.867 & 0.000 & 0.000 & 287.905 & 281.940 & 0.154 & 0.521 \\ 
5-Cz-Sac & 2.077 & 73 & 74 & 2.574 & 3.414 & 3.392 & 3.854 & 3.796 & 2.906 & 2.881 & 0.332 & 0.306 & 0.840 & 0.818 & 0.948 & 0.915 & 321.728 & 326.635 & 426.688 & 430.418 & 0.242 & 0.247 & 104.960 & 103.782 & 0.358 & 4.433 \\ 
6-Cz-Sac & 2.135 & 73 & 74 & 2.549 & 3.315 & 3.293 & 3.784 & 3.728 & 2.909 & 2.886 & 0.360 & 0.337 & 0.766 & 0.744 & 0.875 & 0.842 & 327.680 & 332.558 & 426.212 & 429.647 & 0.557 & 0.473 & 98.532 & 97.090 & 0.429 & 4.507 \\ 
DiCz-Sac & 1.999 & 103 & 104 & 2.349 & 3.242 & 3.222 & 3.596 & 3.560 & 2.606 & 2.596 & 0.256 & 0.247 & 0.893 & 0.872 & 0.990 & 0.964 & 344.793 & 348.241 & 475.853 & 477.557 & 0.221 & 0.194 & 131.060 & 129.316 & 0.432 & 4.012 \\ 
2CM & 2.944 & 135 & 136 & 2.906 & 3.061 & 3.035 & 3.562 & 3.474 & 3.383 & 3.326 & 0.476 & 0.420 & 0.154 & 0.129 & 0.179 & 0.147 & 348.084 & 356.943 & 366.529 & 372.738 & 0.155 & 0.119 & 18.444 & 15.794 & 0.580 & 2.482 \\ 
CzoB & 2.272 & 93 & 94 & 2.528 & 3.301 & 3.285 & 3.429 & 3.419 & 2.625 & 2.630 & 0.097 & 0.103 & 0.774 & 0.758 & 0.803 & 0.788 & 361.628 & 362.675 & 472.314 & 471.372 & 0.050 & 0.047 & 110.686 & 108.696 & 0.348 & 2.986 \\ 
CzBroB & 2.152 & 96 & 97 & 2.395 & 3.276 & 3.267 & 3.393 & 3.383 & 2.480 & 2.480 & 0.086 & 0.085 & 0.881 & 0.872 & 0.913 & 0.903 & 365.412 & 366.524 & 499.925 & 500.008 & 0.056 & 0.052 & 134.513 & 133.484 & 0.364 & 2.947 \\ 
PxCN & 1.196 & 113 & 114 & 1.896 & 2.852 & 2.821 & 3.237 & 3.202 & 2.152 & 2.152 & 0.256 & 0.256 & 0.956 & 0.925 & 1.085 & 1.050 & 382.998 & 387.257 & 576.090 & 576.225 & 0.017 & 0.014 & 193.091 & 188.968 & 0.165 & 2.760 \\ 
AcCN & 1.224 & 125 & 126 & 1.973 & 3.387 & 3.357 & 3.723 & 3.719 & 2.168 & 2.186 & 0.196 & 0.213 & 1.414 & 1.384 & 1.555 & 1.533 & 333.004 & 333.380 & 571.754 & 567.246 & 0.195 & 0.189 & 238.750 & 233.866 & 0.094 & 7.388 \\ 
CzCNoB & 1.841 & 97 & 98 & 2.125 & 3.002 & 2.994 & 3.120 & 3.108 & 2.209 & 2.206 & 0.084 & 0.081 & 0.877 & 0.869 & 0.911 & 0.902 & 397.411 & 398.907 & 561.362 & 562.105 & 0.051 & 0.046 & 163.951 & 163.198 & 0.341 & 3.376 \\ 
CNPP-TPA & 0.775 & 140 & 141 & 1.266 & 2.686 & 2.663 & 3.226 & 3.204 & 1.521 & 1.523 & 0.255 & 0.257 & 1.420 & 1.397 & 1.705 & 1.680 & 384.292 & 387.015 & 815.136 & 813.974 & 0.781 & 0.730 & 430.844 & 426.959 & 0.382 & 8.480 \\ 
SPAC-FO & 0.996 & 153 & 154 & 1.502 & 2.436 & 2.427 & 2.661 & 2.641 & 1.641 & 1.635 & 0.138 & 0.133 & 0.934 & 0.924 & 1.020 & 1.006 & 465.966 & 469.459 & 755.645 & 758.342 & 0.137 & 0.118 & 289.680 & 288.883 & 0.303 & 3.763 \\ 
DMAC-FO & 1.220 & 111 & 112 & 1.493 & 2.018 & 1.977 & 2.537 & 2.471 & 1.877 & 1.866 & 0.384 & 0.373 & 0.525 & 0.484 & 0.660 & 0.605 & 488.646 & 501.737 & 660.586 & 664.303 & 0.250 & 0.215 & 171.940 & 162.566 & 0.246 & 5.710 \\ 
6AcBIQ & 0.916 & 89 & 90 & 1.617 & 2.215 & 2.204 & 2.353 & 2.342 & 1.717 & 1.718 & 0.100 & 0.101 & 0.598 & 0.587 & 0.635 & 0.624 & 526.987 & 529.440 & 721.996 & 721.656 & 0.100 & 0.095 & 195.009 & 192.217 & 0.308 & 4.629 \\ 
PtB & 2.112 & 103 & 104 & 1.933 & 2.676 & 2.611 & 3.522 & 3.462 & 2.544 & 2.564 & 0.611 & 0.631 & 0.743 & 0.678 & 0.978 & 0.899 & 351.988 & 358.077 & 487.315 & 483.576 & 0.716 & 0.642 & 135.327 & 125.499 & 0.678 & 3.836 \\ 
BCPBT & 1.315 & 170 & 171 & 1.744 & 2.860 & 2.807 & 3.660 & 3.564 & 2.232 & 2.214 & 0.488 & 0.470 & 1.116 & 1.064 & 1.428 & 1.350 & 338.755 & 347.918 & 555.513 & 560.125 & 1.499 & 1.203 & 216.758 & 212.207 & 0.144 & 0.565 \\ 
InDM & 2.639 & 78 & 79 & 2.592 & 3.378 & 3.358 & 4.048 & 3.966 & 3.105 & 3.061 & 0.513 & 0.470 & 0.787 & 0.766 & 0.943 & 0.905 & 306.308 & 312.578 & 399.316 & 404.982 & 0.037 & 0.047 & 93.008 & 92.403 & 0.344 & 4.069 \\ 
PnB & 2.122 & 103 & 104 & 1.927 & 2.685 & 2.620 & 3.537 & 3.476 & 2.539 & 2.557 & 0.612 & 0.630 & 0.758 & 0.693 & 0.998 & 0.919 & 350.545 & 356.645 & 488.382 & 484.852 & 0.704 & 0.636 & 137.837 & 128.206 & 0.674 & 3.867 \\ 
BANE & 2.118 & 121 & 122 & 1.787 & 2.252 & 2.181 & 3.171 & 3.056 & 2.516 & 2.504 & 0.729 & 0.717 & 0.465 & 0.394 & 0.655 & 0.552 & 391.019 & 405.707 & 492.799 & 495.236 & 1.061 & 0.819 & 101.780 & 89.529 & 0.912 & 0.708 \\ 
CBM & 1.817 & 69 & 70 & 1.887 & 2.451 & 2.402 & 3.213 & 3.149 & 2.473 & 2.473 & 0.586 & 0.586 & 0.565 & 0.516 & 0.740 & 0.676 & 385.919 & 393.738 & 501.434 & 501.409 & 1.266 & 1.064 & 115.515 & 107.671 & 0.575 & 1.703 \\ 
DCzBNPh-1 & 2.217 & 111 & 112 & 2.483 & 3.467 & 3.445 & 3.915 & 3.859 & 2.804 & 2.782 & 0.321 & 0.298 & 0.984 & 0.962 & 1.111 & 1.077 & 316.682 & 321.269 & 442.114 & 445.697 & 0.563 & 0.470 & 125.432 & 124.428 & 0.317 & 1.007 \\ 
MCZ-P2-DTM & 1.728 & 120 & 121 & 2.106 & 3.226 & 3.207 & 3.642 & 3.606 & 2.378 & 2.368 & 0.272 & 0.262 & 1.120 & 1.100 & 1.265 & 1.237 & 340.391 & 343.866 & 521.422 & 523.511 & 1.130 & 0.997 & 181.031 & 179.646 & 0.343 & 7.543 \\ 
DBTO-PTZ & 1.548 & 103 & 104 & 1.940 & 2.900 & 2.870 & 3.213 & 3.199 & 2.149 & 2.162 & 0.209 & 0.223 & 0.961 & 0.930 & 1.064 & 1.037 & 385.883 & 387.523 & 577.049 & 573.388 & 0.028 & 0.029 & 191.166 & 185.865 & 0.254 & 5.317 \\ 
$\alpha$-DMAC-DBP & 1.035 & 90 & 91 & 1.251 & 2.464 & 2.455 & 2.565 & 2.557 & 1.302 & 1.303 & 0.051 & 0.052 & 1.213 & 1.204 & 1.263 & 1.254 & 483.388 & 484.957 & 952.232 & 951.834 & 0.053 & 0.049 & 468.844 & 466.877 & 0.356 & 3.698 \\ 
$\alpha$-2DMAC-DBP & 0.950 & 129 & 130 & 1.135 & 2.372 & 2.360 & 2.493 & 2.483 & 1.193 & 1.194 & 0.058 & 0.059 & 1.237 & 1.225 & 1.300 & 1.289 & 497.329 & 499.252 & 1039.468 & 1038.163 & 0.093 & 0.087 & 542.139 & 538.911 & 0.410 & 1.841 \\ 
$\beta$-DI-DBP & 1.249 & 141 & 142 & 1.362 & 2.984 & 2.955 & 3.264 & 3.261 & 1.489 & 1.502 & 0.127 & 0.141 & 1.623 & 1.594 & 1.775 & 1.759 & 379.877 & 380.203 & 832.628 & 825.217 & 0.022 & 0.031 & 452.751 & 445.014 & 0.110 & 7.473 \\ 
DIC-TRZ & 1.924 & 103 & 104 & 2.246 & 3.050 & 3.027 & 3.520 & 3.458 & 2.592 & 2.566 & 0.346 & 0.320 & 0.804 & 0.781 & 0.928 & 0.892 & 352.238 & 358.564 & 478.356 & 483.211 & 0.297 & 0.250 & 126.118 & 124.647 & 0.188 & 4.611 \\ 
PO-TPA & 0.374 & 193 & 194 & 0.630 & 1.295 & 1.244 & 1.984 & 1.874 & 0.965 & 0.949 & 0.336 & 0.319 & 0.665 & 0.614 & 1.019 & 0.925 & 624.763 & 661.637 & 1284.428 & 1306.760 & 0.829 & 0.608 & 659.665 & 645.123 & 0.530 & 6.575 \\ 
DMAC-Cz-TTR & 1.198 & 154 & 155 & 1.901 & 3.406 & 3.375 & 3.821 & 3.765 & 2.133 & 2.121 & 0.231 & 0.220 & 1.505 & 1.473 & 1.688 & 1.644 & 324.523 & 329.272 & 581.356 & 584.426 & 0.437 & 0.390 & 256.832 & 255.153 & 0.065 & 8.786 \\ 
DCzPO & 2.627 & 121 & 122 & 2.825 & 3.310 & 3.287 & 3.823 & 3.756 & 3.263 & 3.229 & 0.438 & 0.403 & 0.485 & 0.462 & 0.560 & 0.527 & 324.303 & 330.096 & 379.962 & 384.028 & 0.310 & 0.151 & 55.659 & 53.931 & 0.280 & 0.946 \\ 
IQ-oTPA & 0.725 & 132 & 133 & 1.109 & 2.706 & 2.705 & 2.701 & 2.700 & 1.107 & 1.107 & -0.002 & -0.002 & 1.597 & 1.596 & 1.594 & 1.593 & 459.065 & 459.201 & 1119.922 & 1119.923 & 0.003 & 0.002 & 660.858 & 660.722 & 0.171 & 9.839 \\ 
2C & 1.202 & 67 & 68 & 1.604 & 2.650 & 2.585 & 3.441 & 3.380 & 2.083 & 2.098 & 0.479 & 0.494 & 1.046 & 0.981 & 1.358 & 1.282 & 360.283 & 366.774 & 595.217 & 590.964 & 1.274 & 1.107 & 234.934 & 224.190 & 0.322 & 7.282 \\ 
C-H & 1.172 & 70 & 71 & 1.603 & 2.678 & 2.610 & 3.513 & 3.449 & 2.102 & 2.118 & 0.499 & 0.515 & 1.076 & 1.008 & 1.411 & 1.332 & 352.930 & 359.437 & 589.822 & 585.468 & 1.113 & 0.965 & 236.892 & 226.031 & 0.296 & 7.485 \\ 
PSPP & 1.730 & 71 & 72 & 2.387 & 2.792 & 2.760 & 3.161 & 3.120 & 2.703 & 2.699 & 0.316 & 0.312 & 0.405 & 0.373 & 0.458 & 0.422 & 392.181 & 397.322 & 458.657 & 459.392 & 0.013 & 0.011 & 66.476 & 62.071 & 0.141 & 6.102 \\ 
2DN & 0.916 & 146 & 147 & 1.284 & 1.800 & 1.762 & 2.361 & 2.265 & 1.684 & 1.650 & 0.400 & 0.367 & 0.516 & 0.478 & 0.677 & 0.615 & 525.179 & 547.343 & 736.410 & 751.201 & 0.178 & 0.129 & 211.231 & 203.857 & 0.193 & 5.338 \\ 
PSPBP & 1.682 & 104 & 105 & 2.145 & 2.930 & 2.899 & 3.315 & 3.279 & 2.427 & 2.427 & 0.282 & 0.281 & 0.784 & 0.754 & 0.887 & 0.852 & 374.043 & 378.116 & 510.809 & 510.925 & 0.015 & 0.011 & 136.766 & 132.809 & 0.169 & 5.268 \\ 
2PN & 0.748 & 134 & 135 & 1.063 & 1.961 & 1.949 & 2.159 & 2.141 & 1.170 & 1.167 & 0.107 & 0.105 & 0.898 & 0.887 & 0.988 & 0.974 & 574.347 & 579.041 & 1059.445 & 1062.002 & 0.212 & 0.183 & 485.098 & 482.961 & 0.349 & 3.194 \\ 
pCbz-PYR & 2.539 & 131 & 132 & 2.644 & 3.488 & 3.468 & 3.853 & 3.820 & 2.921 & 2.912 & 0.277 & 0.268 & 0.844 & 0.824 & 0.933 & 0.908 & 321.744 & 324.566 & 424.474 & 425.717 & 1.070 & 0.951 & 102.730 & 101.151 & 0.515 & 1.105 \\ 
PPI-An-NPIM & 2.093 & 168 & 169 & 1.840 & 2.258 & 2.189 & 3.318 & 3.171 & 2.703 & 2.664 & 0.864 & 0.825 & 0.419 & 0.350 & 0.615 & 0.506 & 373.638 & 391.019 & 458.637 & 465.350 & 0.898 & 0.648 & 84.999 & 74.331 & 0.897 & 0.437 \\ 
2PS-2FPh & 2.218 & 87 & 88 & 2.339 & 2.833 & 2.803 & 3.204 & 3.161 & 2.645 & 2.637 & 0.306 & 0.298 & 0.494 & 0.464 & 0.559 & 0.523 & 386.955 & 392.281 & 468.699 & 470.135 & 0.051 & 0.043 & 81.744 & 77.854 & 0.133 & 5.872 \\ 
9CzTPE & 2.203 & 111 & 112 & 1.745 & 2.899 & 2.852 & 3.582 & 3.546 & 2.156 & 2.170 & 0.411 & 0.425 & 1.154 & 1.107 & 1.427 & 1.377 & 346.093 & 349.596 & 575.098 & 571.401 & 2.158 & 1.916 & 229.005 & 221.805 & 0.771 & 2.888 \\ 
2CzTPE & 2.236 & 117 & 118 & 1.744 & 2.890 & 2.842 & 3.614 & 3.574 & 2.181 & 2.193 & 0.437 & 0.449 & 1.146 & 1.098 & 1.433 & 1.381 & 343.104 & 346.916 & 568.544 & 565.352 & 2.616 & 2.289 & 225.440 & 218.436 & 0.892 & 0.203 \\ 
FTAT-FBO & 3.500 & 94 & 95 & 3.330 & 5.176 & 5.135 & 5.140 & 5.110 & 3.306 & 3.314 & -0.024 & -0.016 & 1.847 & 1.805 & 1.833 & 1.796 & 241.233 & 242.631 & 375.008 & 374.163 & 0.000 & 0.000 & 133.774 & 131.533 & 0.061 & 7.967 \\ 
DmPy-PPI & 2.710 & 138 & 139 & 2.436 & 3.478 & 3.450 & 3.835 & 3.796 & 2.685 & 2.680 & 0.250 & 0.244 & 1.043 & 1.014 & 1.150 & 1.116 & 323.313 & 326.627 & 461.722 & 462.645 & 0.341 & 0.311 & 138.409 & 136.018 & 0.706 & 3.612 \\ 
mCP-BmPy & 2.674 & 171 & 172 & 2.882 & 3.379 & 3.357 & 3.777 & 3.712 & 3.221 & 3.187 & 0.339 & 0.305 & 0.497 & 0.475 & 0.555 & 0.525 & 328.287 & 333.982 & 384.891 & 388.995 & 0.332 & 0.279 & 56.604 & 55.013 & 0.092 & 7.799 \\ 
mCP-Py & 3.015 & 143 & 144 & 2.965 & 3.388 & 3.366 & 3.807 & 3.743 & 3.331 & 3.296 & 0.366 & 0.331 & 0.424 & 0.402 & 0.476 & 0.446 & 325.691 & 331.278 & 372.249 & 376.154 & 0.328 & 0.278 & 46.558 & 44.876 & 0.409 & 6.035 \\ 
mCP-Ph & 3.063 & 143 & 144 & 2.970 & 3.390 & 3.368 & 3.809 & 3.744 & 3.338 & 3.303 & 0.368 & 0.332 & 0.419 & 0.397 & 0.471 & 0.441 & 325.461 & 331.146 & 371.394 & 375.406 & 0.308 & 0.260 & 45.933 & 44.261 & 0.589 & 3.366 \\ 
DMTAC & 2.070 & 116 & 117 & 1.914 & 2.429 & 2.376 & 3.120 & 3.046 & 2.459 & 2.453 & 0.544 & 0.539 & 0.515 & 0.462 & 0.661 & 0.592 & 397.436 & 407.093 & 504.302 & 505.390 & 0.267 & 0.252 & 106.866 & 98.298 & 0.774 & 1.238 \\ 
IPTAC & 2.074 & 128 & 129 & 1.923 & 2.426 & 2.374 & 3.116 & 3.042 & 2.470 & 2.465 & 0.547 & 0.541 & 0.503 & 0.451 & 0.646 & 0.578 & 397.870 & 407.508 & 501.877 & 503.016 & 0.261 & 0.249 & 104.007 & 95.508 & 0.779 & 1.129 \\ 
TBTAC & 2.073 & 134 & 135 & 1.923 & 2.430 & 2.379 & 3.121 & 3.048 & 2.469 & 2.463 & 0.546 & 0.541 & 0.508 & 0.456 & 0.652 & 0.584 & 397.296 & 406.786 & 502.210 & 503.288 & 0.259 & 0.252 & 104.914 & 96.503 & 0.780 & 1.168 \\ 
p2Cz2Trz & 1.620 & 159 & 160 & 1.670 & 3.096 & 3.085 & 3.300 & 3.276 & 1.780 & 1.774 & 0.110 & 0.104 & 1.426 & 1.415 & 1.519 & 1.502 & 375.755 & 378.404 & 696.441 & 698.881 & 0.149 & 0.131 & 320.685 & 320.477 & 0.382 & 0.016 \\ 
m2Cz2Trz & 1.934 & 159 & 160 & 1.984 & 3.367 & 3.349 & 3.666 & 3.644 & 2.160 & 2.158 & 0.176 & 0.174 & 1.383 & 1.365 & 1.506 & 1.485 & 338.228 & 340.279 & 573.999 & 574.445 & 0.216 & 0.202 & 235.771 & 234.165 & 0.461 & 2.725 \\ 
2,4-CzPyCl3 & 2.351 & 84 & 85 & 2.619 & 3.446 & 3.425 & 3.845 & 3.796 & 2.923 & 2.904 & 0.303 & 0.284 & 0.826 & 0.805 & 0.922 & 0.892 & 322.498 & 326.584 & 424.196 & 426.953 & 0.610 & 0.516 & 101.699 & 100.369 & 0.415 & 3.609 \\ 
DMAC-PCN & 1.025 & 104 & 105 & 1.929 & 3.397 & 3.365 & 3.597 & 3.591 & 2.042 & 2.058 & 0.113 & 0.129 & 1.469 & 1.436 & 1.555 & 1.533 & 344.707 & 345.302 & 607.182 & 602.483 & 0.213 & 0.202 & 262.475 & 257.181 & 0.045 & 8.167 \\ 
2PXZP & 1.332 & 119 & 120 & 1.802 & 2.749 & 2.718 & 3.118 & 3.081 & 2.045 & 2.043 & 0.242 & 0.241 & 0.946 & 0.916 & 1.073 & 1.038 & 397.627 & 402.363 & 606.370 & 606.739 & 0.021 & 0.018 & 208.743 & 204.376 & 0.176 & 8.411 \\ 
2,4,6-CzPyCl2 & 2.482 & 111 & 112 & 2.598 & 3.452 & 3.428 & 3.842 & 3.801 & 2.891 & 2.880 & 0.294 & 0.283 & 0.854 & 0.830 & 0.951 & 0.920 & 322.665 & 326.206 & 428.792 & 430.445 & 0.545 & 0.479 & 106.127 & 104.240 & 0.458 & 2.014 \\ 
1PXZP & 1.312 & 72 & 73 & 1.939 & 2.720 & 2.708 & 2.958 & 2.938 & 2.109 & 2.104 & 0.169 & 0.165 & 0.781 & 0.769 & 0.849 & 0.834 & 419.163 & 422.002 & 588.002 & 589.286 & 0.380 & 0.341 & 168.839 & 167.284 & 0.302 & 6.463 \\ 
3,6-T2C & 1.438 & 166 & 167 & 1.837 & 3.286 & 3.260 & 3.735 & 3.699 & 2.088 & 2.084 & 0.251 & 0.247 & 1.449 & 1.423 & 1.647 & 1.615 & 331.988 & 335.174 & 593.859 & 594.869 & 1.268 & 1.097 & 261.871 & 259.695 & 0.120 & 12.872 \\ 
3,6-TC & 1.619 & 162 & 163 & 1.987 & 3.287 & 3.261 & 3.722 & 3.687 & 2.250 & 2.246 & 0.263 & 0.259 & 1.300 & 1.274 & 1.472 & 1.441 & 333.112 & 336.301 & 551.028 & 551.987 & 1.337 & 1.154 & 217.916 & 215.686 & 0.176 & 12.562 \\ 
Ph-CF3 & 2.876 & 92 & 93 & 2.769 & 3.404 & 3.373 & 3.866 & 3.817 & 3.145 & 3.133 & 0.376 & 0.364 & 0.634 & 0.604 & 0.721 & 0.684 & 320.704 & 324.796 & 394.180 & 395.678 & 1.151 & 0.887 & 73.476 & 70.883 & 0.652 & 0.849 \\ 
arylene & 2.858 & 92 & 93 & 2.770 & 3.390 & 3.360 & 3.855 & 3.809 & 3.150 & 3.140 & 0.380 & 0.370 & 0.620 & 0.590 & 0.705 & 0.669 & 321.594 & 325.520 & 393.601 & 394.881 & 1.205 & 0.945 & 72.007 & 69.361 & 0.649 & 0.851 \\ 
TS-1 & 2.710 & 68 & 69 & 2.982 & 3.421 & 3.399 & 3.874 & 3.803 & 3.376 & 3.337 & 0.394 & 0.355 & 0.440 & 0.417 & 0.498 & 0.466 & 320.067 & 326.034 & 367.240 & 371.594 & 0.263 & 0.226 & 47.174 & 45.560 & 0.395 & 4.787 \\ 
3,6-MeCzOXD & 1.893 & 113 & 114 & 2.262 & 3.364 & 3.341 & 3.684 & 3.664 & 2.477 & 2.480 & 0.215 & 0.219 & 1.102 & 1.079 & 1.207 & 1.184 & 336.530 & 338.394 & 500.531 & 499.878 & 0.247 & 0.224 & 164.002 & 161.484 & 0.250 & 4.926 \\ 
p-PO15NCzDPA & 2.126 & 125 & 126 & 1.865 & 2.260 & 2.189 & 3.215 & 3.050 & 2.654 & 2.599 & 0.789 & 0.734 & 0.394 & 0.324 & 0.561 & 0.451 & 385.607 & 406.452 & 467.155 & 476.959 & 0.645 & 0.466 & 81.548 & 70.506 & 0.931 & 0.026 \\ 
2,7-MeCzOXD & 1.940 & 113 & 114 & 2.266 & 3.480 & 3.460 & 3.756 & 3.739 & 2.446 & 2.449 & 0.179 & 0.183 & 1.214 & 1.194 & 1.310 & 1.290 & 330.105 & 331.615 & 506.978 & 506.340 & 0.176 & 0.162 & 176.873 & 174.725 & 0.249 & 4.368 \\ 
BPCN-Cz2Ph & 2.184 & 91 & 92 & 2.547 & 3.411 & 3.389 & 3.846 & 3.783 & 2.872 & 2.843 & 0.325 & 0.297 & 0.864 & 0.842 & 0.974 & 0.940 & 322.380 & 327.732 & 431.728 & 436.051 & 0.163 & 0.137 & 109.348 & 108.319 & 0.231 & 7.364 \\ 
o-CzOXD & 2.039 & 101 & 102 & 2.357 & 3.380 & 3.356 & 3.724 & 3.698 & 2.597 & 2.596 & 0.240 & 0.240 & 1.024 & 1.000 & 1.128 & 1.102 & 332.888 & 335.256 & 477.499 & 477.509 & 0.289 & 0.256 & 144.611 & 142.254 & 0.253 & 4.740 \\ 
BPCN-2Cz & 2.056 & 107 & 108 & 2.502 & 3.363 & 3.340 & 3.845 & 3.776 & 2.861 & 2.828 & 0.359 & 0.327 & 0.861 & 0.839 & 0.984 & 0.948 & 322.447 & 328.331 & 433.413 & 438.381 & 0.174 & 0.142 & 110.966 & 110.051 & 0.160 & 10.653 \\ 
Cbz-MI & 0.717 & 152 & 153 & 0.957 & 2.426 & 2.407 & 2.846 & 2.812 & 1.123 & 1.118 & 0.166 & 0.161 & 1.469 & 1.450 & 1.724 & 1.694 & 435.567 & 440.864 & 1104.173 & 1108.847 & 0.001 & 0.001 & 668.606 & 667.983 & 0.066 & 11.149 \\ 
DBFDPO & 3.430 & 99 & 100 & 3.299 & 4.011 & 3.979 & 4.357 & 4.304 & 3.584 & 3.569 & 0.285 & 0.270 & 0.712 & 0.680 & 0.774 & 0.736 & 284.537 & 288.034 & 345.977 & 347.435 & 0.064 & 0.059 & 61.440 & 59.401 & 0.629 & 1.781 \\ 
XCBP & 1.893 & 84 & 85 & 2.435 & 3.384 & 3.359 & 3.462 & 3.460 & 2.491 & 2.508 & 0.056 & 0.073 & 0.949 & 0.924 & 0.971 & 0.952 & 358.181 & 358.367 & 497.745 & 494.369 & 0.001 & 0.001 & 139.565 & 136.002 & 0.095 & 10.411 \\ 
Cbz-PYR & 2.754 & 75 & 76 & 2.791 & 3.503 & 3.481 & 3.874 & 3.831 & 3.087 & 3.072 & 0.296 & 0.280 & 0.712 & 0.690 & 0.788 & 0.759 & 320.017 & 323.642 & 401.672 & 403.649 & 0.753 & 0.652 & 81.655 & 80.006 & 0.499 & 0.975 \\ 
tCbz-mPYRs & 2.521 & 132 & 133 & 2.724 & 3.409 & 3.387 & 3.819 & 3.774 & 3.051 & 3.035 & 0.327 & 0.311 & 0.685 & 0.664 & 0.768 & 0.739 & 324.685 & 328.539 & 406.362 & 408.580 & 0.624 & 0.536 & 81.677 & 80.041 & 0.422 & 2.459 \\ 
PCBP & 1.911 & 78 & 79 & 2.341 & 3.401 & 3.377 & 3.495 & 3.494 & 2.406 & 2.422 & 0.065 & 0.081 & 1.060 & 1.036 & 1.089 & 1.072 & 354.717 & 354.879 & 515.242 & 511.916 & 0.001 & 0.001 & 160.525 & 157.037 & 0.191 & 9.788 \\ 
MeCZ-TRZ & 1.807 & 165 & 166 & 2.087 & 3.509 & 3.486 & 3.957 & 3.907 & 2.354 & 2.339 & 0.267 & 0.252 & 1.421 & 1.399 & 1.603 & 1.568 & 313.353 & 317.347 & 526.692 & 530.015 & 0.605 & 0.485 & 213.339 & 212.669 & 0.229 & 1.372 \\ 
3ca & 2.136 & 80 & 81 & 1.930 & 2.676 & 2.627 & 3.501 & 3.414 & 2.525 & 2.508 & 0.595 & 0.578 & 0.746 & 0.697 & 0.977 & 0.906 & 354.119 & 363.164 & 491.106 & 494.390 & 1.396 & 1.116 & 136.987 & 131.226 & 0.788 & 1.147 \\ 
2MeCZ-TRZ & 1.742 & 174 & 175 & 2.048 & 3.488 & 3.466 & 3.934 & 3.886 & 2.310 & 2.297 & 0.262 & 0.248 & 1.440 & 1.417 & 1.624 & 1.589 & 315.161 & 319.070 & 536.667 & 539.850 & 0.738 & 0.576 & 221.507 & 220.780 & 0.247 & 0.686 \\ 
CZ-TRZ & 1.893 & 156 & 157 & 2.135 & 3.501 & 3.479 & 3.963 & 3.909 & 2.416 & 2.399 & 0.282 & 0.264 & 1.367 & 1.344 & 1.547 & 1.510 & 312.839 & 317.168 & 513.117 & 516.846 & 0.560 & 0.446 & 200.279 & 199.678 & 0.257 & 0.222 \\ 
DMAC-AQ & 1.240 & 77 & 78 & 1.308 & 1.604 & 1.557 & 2.207 & 2.113 & 1.800 & 1.774 & 0.492 & 0.466 & 0.296 & 0.250 & 0.407 & 0.339 & 561.701 & 586.852 & 688.813 & 698.922 & 0.309 & 0.237 & 127.112 & 112.070 & 0.497 & 4.228 \\ 
DTPTCzDP-CN & 1.156 & 149 & 150 & 1.726 & 2.784 & 2.767 & 3.187 & 3.139 & 1.975 & 1.958 & 0.249 & 0.232 & 1.058 & 1.041 & 1.211 & 1.181 & 389.068 & 395.018 & 627.645 & 633.170 & 0.783 & 0.616 & 238.578 & 238.153 & 0.328 & 7.650 \\ 
mP2MPC & 2.729 & 132 & 133 & 2.582 & 3.387 & 3.363 & 3.777 & 3.734 & 2.880 & 2.867 & 0.298 & 0.284 & 0.805 & 0.781 & 0.898 & 0.867 & 328.218 & 332.050 & 430.521 & 432.526 & 0.282 & 0.258 & 102.304 & 100.476 & 0.035 & 12.165 \\ 
XPhos & 2.938 & 94 & 95 & 2.158 & 3.049 & 3.000 & 4.165 & 4.039 & 2.949 & 2.906 & 0.790 & 0.748 & 0.890 & 0.841 & 1.216 & 1.133 & 297.688 & 306.945 & 420.482 & 426.602 & 0.514 & 0.394 & 122.794 & 119.657 & 0.694 & 1.418 \\ 
TPXZ-as-TAZ & 1.256 & 156 & 157 & 1.286 & 2.699 & 2.689 & 2.926 & 2.909 & 1.394 & 1.391 & 0.108 & 0.105 & 1.413 & 1.403 & 1.532 & 1.518 & 423.791 & 426.268 & 889.485 & 891.469 & 0.491 & 0.455 & 465.695 & 465.201 & 0.161 & 6.823 \\ 
2Trz6CNDBT & 2.307 & 77 & 78 & 2.367 & 3.545 & 3.527 & 3.892 & 3.842 & 2.598 & 2.578 & 0.231 & 0.211 & 1.179 & 1.160 & 1.294 & 1.264 & 318.603 & 322.716 & 477.287 & 480.913 & 0.157 & 0.143 & 158.684 & 158.197 & 0.456 & 2.123 \\ 
TPAPyPI & 1.865 & 149 & 150 & 2.017 & 2.727 & 2.658 & 3.678 & 3.618 & 2.721 & 2.745 & 0.704 & 0.728 & 0.710 & 0.642 & 0.958 & 0.873 & 337.069 & 342.697 & 455.734 & 451.719 & 0.049 & 0.559 & 118.664 & 109.022 & 0.016 & 9.837 \\ 
TPACzPI & 2.312 & 157 & 158 & 2.279 & 3.388 & 3.366 & 3.767 & 3.721 & 2.535 & 2.520 & 0.255 & 0.241 & 1.108 & 1.086 & 1.232 & 1.201 & 329.159 & 333.210 & 489.170 & 491.990 & 0.616 & 0.149 & 160.012 & 158.780 & 0.391 & 8.558 \\ 
NA-TNA & 1.014 & 121 & 122 & 1.410 & 2.336 & 2.283 & 3.006 & 2.952 & 1.814 & 1.823 & 0.404 & 0.414 & 0.926 & 0.873 & 1.192 & 1.129 & 412.497 & 419.958 & 683.607 & 680.003 & 2.393 & 2.083 & 271.110 & 260.045 & 0.300 & 10.594 \\ 
CzPrSBI & 1.729 & 70 & 71 & 2.431 & 3.301 & 3.275 & 3.787 & 3.705 & 2.789 & 2.750 & 0.358 & 0.319 & 0.870 & 0.844 & 0.998 & 0.955 & 327.368 & 334.676 & 444.503 & 450.915 & 0.056 & 0.045 & 117.134 & 116.239 & 0.118 & 3.511 \\ 
m-CzCNDMT & 2.979 & 117 & 118 & 2.962 & 3.481 & 3.458 & 3.909 & 3.851 & 3.326 & 3.299 & 0.364 & 0.337 & 0.519 & 0.496 & 0.583 & 0.553 & 317.168 & 321.920 & 372.752 & 375.880 & 0.106 & 0.094 & 55.584 & 53.960 & 0.470 & 6.916 \\ 
DTXO-TPA2 & 2.329 & 115 & 116 & 2.359 & 2.776 & 2.744 & 3.269 & 3.233 & 2.779 & 2.780 & 0.420 & 0.421 & 0.416 & 0.385 & 0.490 & 0.453 & 379.215 & 383.460 & 446.111 & 446.002 & 0.593 & 0.514 & 66.896 & 62.542 & 0.543 & 0.652 \\ 
24PQ-Cz & 1.818 & 112 & 113 & 1.902 & 3.305 & 3.267 & 3.740 & 3.734 & 2.153 & 2.175 & 0.251 & 0.272 & 1.402 & 1.364 & 1.587 & 1.559 & 331.500 & 332.032 & 575.846 & 570.122 & 0.029 & 0.044 & 244.347 & 238.090 & 0.315 & 7.136 \\ 
SFPC & 2.611 & 101 & 102 & 2.410 & 3.396 & 3.377 & 3.820 & 3.764 & 2.711 & 2.686 & 0.301 & 0.276 & 0.985 & 0.967 & 1.108 & 1.078 & 324.591 & 329.395 & 457.277 & 461.543 & 0.481 & 0.379 & 132.686 & 132.148 & 0.313 & 6.550 \\ 
2CzMC & 2.522 & 63 & 64 & 2.659 & 3.072 & 3.033 & 3.686 & 3.619 & 3.190 & 3.173 & 0.531 & 0.514 & 0.413 & 0.373 & 0.496 & 0.446 & 336.411 & 342.640 & 388.686 & 390.767 & 0.191 & 0.168 & 52.275 & 48.127 & 0.529 & 3.649 \\ 
PPI-PIM-2 & 2.225 & 148 & 149 & 2.290 & 3.419 & 3.391 & 3.829 & 3.789 & 2.564 & 2.559 & 0.274 & 0.269 & 1.129 & 1.101 & 1.264 & 1.231 & 323.845 & 327.178 & 483.543 & 484.505 & 0.499 & 0.450 & 159.698 & 157.326 & 0.104 & 11.681 \\ 
4CzMC & 2.630 & 63 & 64 & 2.722 & 3.134 & 3.097 & 3.738 & 3.677 & 3.246 & 3.232 & 0.524 & 0.510 & 0.413 & 0.375 & 0.492 & 0.446 & 331.695 & 337.152 & 382.006 & 383.645 & 0.400 & 0.367 & 50.311 & 46.493 & 0.571 & 3.220 \\ 
PPI-PIM-1 & 2.237 & 148 & 149 & 2.197 & 3.454 & 3.426 & 3.845 & 3.807 & 2.446 & 2.442 & 0.249 & 0.244 & 1.257 & 1.229 & 1.399 & 1.365 & 322.464 & 325.700 & 506.872 & 507.807 & 0.562 & 0.498 & 184.407 & 182.108 & 0.232 & 10.811 \\ 
CzTPA & 2.954 & 76 & 77 & 3.044 & 3.356 & 3.334 & 3.778 & 3.721 & 3.427 & 3.398 & 0.383 & 0.354 & 0.312 & 0.289 & 0.351 & 0.323 & 328.183 & 333.183 & 361.785 & 364.868 & 0.130 & 0.092 & 33.603 & 31.685 & 0.331 & 3.588 \\ 
SFX-bPy & 2.340 & 84 & 85 & 2.406 & 3.466 & 3.421 & 4.073 & 4.024 & 2.828 & 2.830 & 0.422 & 0.424 & 1.060 & 1.015 & 1.246 & 1.194 & 304.375 & 308.104 & 438.483 & 438.106 & 0.541 & 0.494 & 134.108 & 130.001 & 0.468 & 0.588 \\ 
t–BuCz2BP & 1.841 & 142 & 143 & 2.192 & 3.204 & 3.184 & 3.694 & 3.674 & 2.526 & 2.529 & 0.334 & 0.337 & 1.013 & 0.993 & 1.168 & 1.146 & 335.673 & 337.455 & 490.835 & 490.329 & 0.071 & 0.201 & 155.162 & 152.875 & 0.350 & 2.896 \\ 
SAF-2CzB & 2.267 & 211 & 212 & 2.293 & 3.406 & 3.384 & 3.853 & 3.796 & 2.593 & 2.572 & 0.301 & 0.279 & 1.113 & 1.091 & 1.259 & 1.224 & 321.828 & 326.592 & 478.062 & 482.062 & 0.938 & 0.733 & 156.234 & 155.470 & 0.173 & 3.529 \\ 
F-2CzB & 2.435 & 173 & 174 & 2.332 & 3.423 & 3.401 & 3.869 & 3.815 & 2.636 & 2.616 & 0.304 & 0.284 & 1.091 & 1.069 & 1.233 & 1.199 & 320.422 & 325.008 & 470.337 & 473.989 & 1.069 & 0.816 & 149.915 & 148.981 & 0.480 & 1.084 \\ 
SAF-CzB & 2.376 & 143 & 144 & 2.472 & 3.381 & 3.359 & 3.792 & 3.725 & 2.771 & 2.741 & 0.300 & 0.270 & 0.910 & 0.887 & 1.020 & 0.984 & 327.006 & 332.826 & 447.374 & 452.293 & 0.255 & 0.206 & 120.368 & 119.467 & 0.168 & 3.893 \\ 
BPy-TP2 & 2.244 & 98 & 99 & 2.180 & 3.586 & 3.546 & 3.880 & 3.852 & 2.359 & 2.369 & 0.179 & 0.188 & 1.406 & 1.366 & 1.521 & 1.484 & 319.522 & 321.836 & 525.500 & 523.446 & 0.000 & 0.000 & 205.978 & 201.610 & 0.543 & 0.387 \\ 
Cz–AQ & 1.100 & 68 & 69 & 1.512 & 2.301 & 2.283 & 2.654 & 2.615 & 1.744 & 1.732 & 0.232 & 0.220 & 0.789 & 0.771 & 0.910 & 0.883 & 467.125 & 474.073 & 710.733 & 715.693 & 0.272 & 0.235 & 243.609 & 241.620 & 0.372 & 5.600 \\ 
-ph-pCzAnBzt & 2.049 & 115 & 116 & 1.863 & 2.256 & 2.186 & 3.211 & 3.045 & 2.651 & 2.595 & 0.788 & 0.732 & 0.393 & 0.322 & 0.559 & 0.449 & 386.171 & 407.240 & 467.644 & 477.705 & 0.604 & 0.425 & 81.473 & 70.466 & 0.047 & 13.011 \\ 
PyI & 2.482 & 44 & 45 & 2.291 & 2.848 & 2.786 & 3.748 & 3.691 & 3.016 & 3.036 & 0.724 & 0.744 & 0.556 & 0.495 & 0.732 & 0.655 & 330.792 & 335.919 & 411.126 & 408.423 & 0.007 & 0.281 & 80.334 & 72.505 & 0.908 & 0.669 \\ 
DVCz-2CzCN & 2.104 & 231 & 232 & 2.492 & 3.436 & 3.414 & 3.770 & 3.734 & 2.734 & 2.726 & 0.242 & 0.233 & 0.944 & 0.922 & 1.036 & 1.008 & 328.862 & 332.068 & 453.412 & 454.901 & 0.297 & 0.101 & 124.550 & 122.833 & 0.005 & 9.348 \\ 
ATDBT & 2.123 & 107 & 108 & 1.876 & 2.291 & 2.220 & 3.301 & 3.134 & 2.704 & 2.649 & 0.827 & 0.773 & 0.415 & 0.344 & 0.598 & 0.485 & 375.539 & 395.560 & 458.561 & 467.998 & 0.609 & 0.420 & 83.022 & 72.438 & 0.882 & 1.164 \\ 
DPhBCz & 2.952 & 89 & 90 & 2.835 & 3.353 & 3.330 & 3.842 & 3.771 & 3.248 & 3.210 & 0.413 & 0.375 & 0.518 & 0.496 & 0.594 & 0.561 & 322.741 & 328.775 & 381.756 & 386.249 & 0.198 & 0.110 & 59.015 & 57.474 & 0.740 & 0.407 \\ 
AcHPM & 1.456 & 121 & 122 & 1.880 & 3.403 & 3.372 & 3.563 & 3.559 & 1.968 & 1.984 & 0.088 & 0.104 & 1.523 & 1.492 & 1.594 & 1.575 & 348.006 & 348.349 & 629.905 & 624.836 & 0.156 & 0.151 & 281.899 & 276.488 & 0.161 & 2.776 \\ 
PhCO-DMAC & 1.446 & 73 & 74 & 2.185 & 3.319 & 3.312 & 3.416 & 3.412 & 2.249 & 2.251 & 0.064 & 0.066 & 1.134 & 1.127 & 1.167 & 1.161 & 362.909 & 363.430 & 551.225 & 550.852 & 0.040 & 0.050 & 188.316 & 187.422 & 0.195 & 6.203 \\ 
Diphenylsulfane & 2.381 & 99 & 100 & 2.427 & 4.122 & 4.089 & 4.118 & 4.117 & 2.424 & 2.443 & -0.002 & 0.017 & 1.695 & 1.663 & 1.694 & 1.674 & 301.064 & 301.137 & 511.411 & 507.477 & 0.005 & 0.005 & 210.347 & 206.340 & 0.450 & 0.621 \\ 
2BrCPT & 2.229 & 93 & 94 & 2.276 & 3.365 & 3.342 & 3.811 & 3.741 & 2.578 & 2.548 & 0.302 & 0.272 & 1.089 & 1.066 & 1.234 & 1.194 & 325.324 & 331.393 & 481.024 & 486.634 & 0.483 & 0.383 & 155.700 & 155.241 & 0.361 & 6.463 \\ 
DCbz-Ph-Bz & 2.489 & 124 & 125 & 2.484 & 3.405 & 3.381 & 3.883 & 3.821 & 2.833 & 2.807 & 0.349 & 0.323 & 0.921 & 0.897 & 1.050 & 1.014 & 319.284 & 324.473 & 437.676 & 441.706 & 0.278 & 0.203 & 118.392 & 117.233 & 0.207 & 6.986 \\ 
DDPA-Ph-Bz & 2.195 & 126 & 127 & 2.398 & 3.459 & 3.432 & 3.846 & 3.817 & 2.666 & 2.668 & 0.268 & 0.270 & 1.061 & 1.033 & 1.180 & 1.149 & 322.380 & 324.796 & 465.004 & 464.709 & 0.061 & 0.061 & 142.623 & 139.914 & 0.218 & 6.705 \\ 
IDAC-MCO & 1.663 & 99 & 100 & 2.280 & 2.831 & 2.808 & 3.353 & 3.271 & 2.700 & 2.656 & 0.420 & 0.375 & 0.551 & 0.528 & 0.652 & 0.615 & 369.793 & 379.052 & 459.121 & 466.827 & 0.134 & 0.106 & 89.328 & 87.775 & 0.287 & 7.273 \\ 
diarylbiindole & 2.237 & 93 & 94 & 2.003 & 2.666 & 2.598 & 3.643 & 3.540 & 2.737 & 2.728 & 0.734 & 0.726 & 0.663 & 0.595 & 0.906 & 0.811 & 340.354 & 350.277 & 453.016 & 454.418 & 0.175 & 0.664 & 112.661 & 104.141 & 0.937 & 0.129 \\ 
CNDSB & 2.255 & 61 & 62 & 1.902 & 2.838 & 2.785 & 3.750 & 3.681 & 2.513 & 2.514 & 0.611 & 0.612 & 0.936 & 0.883 & 1.237 & 1.167 & 330.607 & 336.850 & 493.373 & 493.161 & 2.372 & 1.972 & 162.766 & 156.311 & 0.876 & 0.003 \\ 
TMAB & 1.996 & 162 & 163 & 2.614 & 3.474 & 3.454 & 4.042 & 3.960 & 3.042 & 2.998 & 0.427 & 0.384 & 0.860 & 0.839 & 1.000 & 0.962 & 306.740 & 313.076 & 407.612 & 413.553 & 0.084 & 0.068 & 100.872 & 100.477 & 0.077 & 7.554 \\ 
MOF & 2.854 & 127 & 128 & 1.975 & 4.313 & 4.287 & 4.828 & 4.785 & 2.211 & 2.205 & 0.236 & 0.230 & 2.338 & 2.311 & 2.617 & 2.580 & 256.792 & 259.088 & 560.678 & 562.204 & 0.038 & 0.036 & 303.886 & 303.115 & 0.124 & 7.220 \\ 
DICzTrz & 1.729 & 120 & 121 & 2.040 & 3.303 & 3.279 & 3.581 & 3.551 & 2.212 & 2.209 & 0.172 & 0.169 & 1.262 & 1.239 & 1.369 & 1.342 & 346.209 & 349.104 & 560.446 & 561.180 & 0.143 & 0.089 & 214.237 & 212.076 & 0.156 & 7.221 \\ 
PXZ2PTO & 2.322 & 87 & 88 & 2.610 & 2.780 & 2.748 & 3.144 & 3.106 & 2.951 & 2.949 & 0.342 & 0.339 & 0.171 & 0.139 & 0.193 & 0.157 & 394.327 & 399.215 & 420.099 & 420.457 & 0.011 & 0.010 & 25.772 & 21.242 & 0.356 & 4.220 \\ 
SPBP-DPAC & 2.095 & 124 & 125 & 2.222 & 2.618 & 2.584 & 3.289 & 3.220 & 2.792 & 2.769 & 0.570 & 0.547 & 0.396 & 0.362 & 0.497 & 0.451 & 376.943 & 385.068 & 444.078 & 447.741 & 0.943 & 0.787 & 67.135 & 62.673 & 0.486 & 4.334 \\ 
PX-TRZ & 1.568 & 94 & 95 & 1.985 & 3.704 & 3.670 & 4.176 & 4.134 & 2.238 & 2.236 & 0.253 & 0.251 & 1.719 & 1.685 & 1.938 & 1.898 & 296.933 & 299.928 & 554.039 & 554.582 & 0.068 & 0.015 & 257.107 & 254.654 & 0.205 & 7.143 \\ 
C2MPI & 3.068 & 120 & 121 & 3.072 & 3.563 & 3.540 & 4.051 & 4.007 & 3.492 & 3.477 & 0.420 & 0.405 & 0.492 & 0.468 & 0.559 & 0.530 & 306.073 & 309.411 & 355.073 & 356.579 & 0.041 & 0.031 & 49.000 & 47.167 & 0.249 & 5.105 \\ 
p-PCzTPD & 1.522 & 137 & 138 & 1.819 & 2.837 & 2.794 & 3.432 & 3.393 & 2.201 & 2.209 & 0.382 & 0.390 & 1.017 & 0.975 & 1.231 & 1.184 & 361.291 & 365.369 & 563.365 & 561.227 & 2.217 & 1.956 & 202.074 & 195.859 & 0.396 & 3.634 \\ 
m-PCzTPD & 1.413 & 137 & 138 & 1.935 & 2.926 & 2.880 & 3.590 & 3.553 & 2.375 & 2.387 & 0.439 & 0.452 & 0.990 & 0.945 & 1.215 & 1.166 & 345.360 & 348.976 & 522.127 & 519.442 & 0.041 & 0.059 & 176.767 & 170.466 & 0.132 & 6.046 \\ 
o-PCzTPD & 1.698 & 137 & 138 & 2.123 & 3.335 & 3.298 & 3.756 & 3.710 & 2.391 & 2.388 & 0.268 & 0.265 & 1.212 & 1.175 & 1.365 & 1.322 & 330.070 & 334.207 & 518.462 & 519.136 & 0.028 & 0.030 & 188.392 & 184.929 & 0.149 & 3.288 \\ 
CPBzFC & 1.742 & 80 & 81 & 2.044 & 3.228 & 3.190 & 3.803 & 3.751 & 2.409 & 2.404 & 0.365 & 0.360 & 1.183 & 1.146 & 1.395 & 1.347 & 325.991 & 330.510 & 514.726 & 515.766 & 0.988 & 0.913 & 188.735 & 185.256 & 0.264 & 7.345 \\ 
SiCz2Py2 & 2.659 & 148 & 149 & 2.817 & 3.390 & 3.368 & 3.833 & 3.765 & 3.185 & 3.149 & 0.367 & 0.332 & 0.573 & 0.550 & 0.648 & 0.615 & 323.482 & 329.342 & 389.335 & 393.699 & 0.263 & 0.225 & 65.853 & 64.357 & 0.087 & 8.728 \\ 
SiCz1Py3 & 2.641 & 132 & 133 & 2.831 & 3.367 & 3.343 & 3.807 & 3.735 & 3.201 & 3.163 & 0.370 & 0.332 & 0.536 & 0.512 & 0.606 & 0.572 & 325.674 & 331.952 & 387.306 & 392.005 & 0.187 & 0.158 & 61.632 & 60.053 & 0.098 & 8.531 \\ 
SiCz3Py1 & 2.676 & 164 & 165 & 2.812 & 3.416 & 3.393 & 3.899 & 3.831 & 3.210 & 3.175 & 0.398 & 0.363 & 0.603 & 0.581 & 0.689 & 0.656 & 318.022 & 323.634 & 386.252 & 390.456 & 0.190 & 0.157 & 68.230 & 66.822 & 0.104 & 8.687 \\ 
POBBPE & 3.332 & 90 & 91 & 3.338 & 4.415 & 4.396 & 4.796 & 4.746 & 3.626 & 3.604 & 0.288 & 0.266 & 1.077 & 1.058 & 1.170 & 1.142 & 258.500 & 261.228 & 341.906 & 343.997 & 0.023 & 0.021 & 83.406 & 82.768 & 0.428 & 3.811 \\ 
CzppT & 2.745 & 159 & 160 & 2.634 & 3.511 & 3.488 & 4.051 & 3.986 & 3.039 & 3.010 & 0.405 & 0.376 & 0.877 & 0.854 & 1.012 & 0.976 & 306.096 & 311.057 & 408.013 & 411.910 & 0.585 & 0.377 & 101.917 & 100.853 & 0.468 & 2.437 \\ 
SBDBQ-PXZ & 1.255 & 85 & 86 & 1.529 & 2.505 & 2.494 & 2.702 & 2.683 & 1.649 & 1.645 & 0.120 & 0.115 & 0.976 & 0.965 & 1.052 & 1.038 & 458.912 & 462.162 & 751.755 & 753.786 & 0.199 & 0.182 & 292.843 & 291.624 & 0.316 & 5.414 \\ 
DBQ-3PXZ & 1.098 & 151 & 152 & 1.333 & 2.546 & 2.536 & 2.728 & 2.711 & 1.428 & 1.425 & 0.096 & 0.092 & 1.213 & 1.203 & 1.300 & 1.287 & 454.438 & 457.270 & 867.994 & 870.145 & 0.221 & 0.205 & 413.557 & 412.875 & 0.145 & 7.942 \\ 
P4CzCN–BCz & 3.202 & 66 & 67 & 3.010 & 3.751 & 3.698 & 4.623 & 4.597 & 3.710 & 3.741 & 0.700 & 0.732 & 0.741 & 0.689 & 0.914 & 0.856 & 268.184 & 269.683 & 334.232 & 331.378 & 0.001 & 0.002 & 66.048 & 61.695 & 0.099 & 7.233 \\ 
NAP-1,5-DPA & 2.140 & 110 & 111 & 2.183 & 2.463 & 2.427 & 2.930 & 2.883 & 2.597 & 2.593 & 0.414 & 0.410 & 0.279 & 0.244 & 0.332 & 0.290 & 423.183 & 430.083 & 477.349 & 478.138 & 0.594 & 0.509 & 54.166 & 48.056 & 0.646 & 0.239 \\ 
3DPA3CN & 1.562 & 162 & 163 & 1.867 & 2.867 & 2.846 & 3.203 & 3.183 & 2.086 & 2.088 & 0.219 & 0.221 & 1.000 & 0.979 & 1.117 & 1.095 & 387.076 & 389.508 & 594.428 & 593.698 & 1.400 & 1.283 & 207.352 & 204.191 & 0.247 & 3.602 \\ 
TPA-AN-NA & 1.893 & 101 & 102 & 1.801 & 2.281 & 2.211 & 3.232 & 3.078 & 2.551 & 2.507 & 0.750 & 0.706 & 0.480 & 0.410 & 0.681 & 0.571 & 383.603 & 402.860 & 485.942 & 494.589 & 0.772 & 0.528 & 102.339 & 91.729 & 0.399 & 6.181 \\ 
OCzBN & 2.119 & 127 & 128 & 2.394 & 3.123 & 3.097 & 3.720 & 3.672 & 2.852 & 2.839 & 0.458 & 0.445 & 0.728 & 0.702 & 0.868 & 0.833 & 333.309 & 337.611 & 434.691 & 436.664 & 0.341 & 0.207 & 101.382 & 99.053 & 0.358 & 1.196 \\ 
BBCz & 3.021 & 47 & 48 & 2.969 & 3.341 & 3.306 & 3.810 & 3.759 & 3.386 & 3.377 & 0.416 & 0.407 & 0.372 & 0.336 & 0.424 & 0.382 & 325.435 & 329.798 & 366.174 & 367.151 & 0.001 & 0.001 & 40.739 & 37.353 & 0.728 & 0.753 \\ 
IQ-Se & 2.177 & 119 & 120 & 1.439 & 2.715 & 2.676 & 3.532 & 3.443 & 1.872 & 1.852 & 0.433 & 0.413 & 1.276 & 1.237 & 1.660 & 1.592 & 351.041 & 360.053 & 662.389 & 669.611 & 0.530 & 0.391 & 311.348 & 309.558 & 0.495 & 3.115 \\ 
dTolmp & 3.339 & 98 & 99 & 3.093 & 4.987 & 4.955 & 5.033 & 5.005 & 3.121 & 3.124 & 0.029 & 0.031 & 1.895 & 1.862 & 1.912 & 1.881 & 246.328 & 247.701 & 397.234 & 396.869 & 0.001 & 0.000 & 150.906 & 149.168 & 0.372 & 2.750 \\ 
SiTCNCz & 2.240 & 122 & 123 & 2.314 & 3.630 & 3.612 & 4.042 & 3.989 & 2.577 & 2.556 & 0.263 & 0.242 & 1.316 & 1.298 & 1.465 & 1.433 & 306.717 & 310.800 & 481.127 & 485.088 & 0.396 & 0.344 & 174.410 & 174.288 & 0.374 & 3.638 \\ 
dpmb & 3.049 & 83 & 84 & 2.505 & 4.829 & 4.790 & 4.955 & 4.927 & 2.571 & 2.577 & 0.065 & 0.071 & 2.324 & 2.285 & 2.384 & 2.350 & 250.230 & 251.658 & 482.323 & 481.156 & 0.001 & 0.001 & 232.092 & 229.498 & 0.543 & 1.641 \\ 
3CzBN & 2.282 & 109 & 110 & 2.527 & 3.344 & 3.319 & 3.750 & 3.724 & 2.834 & 2.835 & 0.307 & 0.308 & 0.817 & 0.792 & 0.916 & 0.889 & 330.633 & 332.978 & 437.548 & 437.368 & 0.347 & 0.321 & 106.914 & 104.391 & 0.403 & 0.448 \\ 
TCB & 1.469 & 109 & 110 & 2.171 & 3.342 & 3.319 & 3.685 & 3.680 & 2.394 & 2.407 & 0.223 & 0.236 & 1.171 & 1.148 & 1.291 & 1.273 & 336.475 & 336.868 & 517.959 & 515.088 & 0.005 & 0.291 & 181.485 & 178.221 & 0.118 & 12.845 \\ 
CPzPyC & 1.964 & 89 & 90 & 1.925 & 3.302 & 3.286 & 3.605 & 3.573 & 2.102 & 2.094 & 0.176 & 0.168 & 1.377 & 1.360 & 1.503 & 1.479 & 343.923 & 347.003 & 589.862 & 592.189 & 0.216 & 0.202 & 245.939 & 245.186 & 0.338 & 4.845 \\ 
CPzPzC & 1.614 & 89 & 90 & 1.570 & 3.034 & 3.011 & 3.467 & 3.426 & 1.795 & 1.787 & 0.225 & 0.216 & 1.463 & 1.441 & 1.672 & 1.639 & 357.571 & 361.881 & 690.732 & 693.897 & 0.300 & 0.261 & 333.161 & 332.016 & 0.538 & 0.074 \\ 
CPzPC & 2.058 & 89 & 90 & 2.130 & 3.335 & 3.317 & 3.701 & 3.658 & 2.364 & 2.349 & 0.234 & 0.219 & 1.205 & 1.187 & 1.337 & 1.308 & 335.011 & 338.958 & 524.429 & 527.745 & 0.437 & 0.419 & 189.418 & 188.786 & 0.401 & 4.282 \\ 
CBIQD & 1.921 & 60 & 61 & 2.191 & 2.750 & 2.694 & 3.744 & 3.637 & 2.983 & 2.958 & 0.792 & 0.767 & 0.559 & 0.503 & 0.761 & 0.679 & 331.154 & 340.859 & 415.589 & 419.119 & 0.058 & 0.422 & 84.435 & 78.259 & 0.176 & 6.746 \\ 
PXZ-QL & 2.147 & 57 & 58 & 2.343 & 2.726 & 2.705 & 3.174 & 3.118 & 2.727 & 2.700 & 0.385 & 0.358 & 0.383 & 0.362 & 0.446 & 0.418 & 390.686 & 397.627 & 454.605 & 459.152 & 0.323 & 0.268 & 63.919 & 61.524 & 0.481 & 3.640 \\ 
SBA & 3.143 & 64 & 65 & 3.064 & 3.459 & 3.427 & 4.089 & 4.034 & 3.622 & 3.606 & 0.558 & 0.543 & 0.396 & 0.363 & 0.468 & 0.427 & 303.184 & 307.379 & 342.350 & 343.795 & 0.061 & 0.051 & 39.166 & 36.417 & 0.716 & 0.120 \\ 
TATP-BP & 1.674 & 214 & 215 & 2.053 & 3.462 & 3.431 & 3.679 & 3.657 & 2.183 & 2.189 & 0.129 & 0.135 & 1.408 & 1.377 & 1.497 & 1.468 & 336.959 & 339.051 & 568.051 & 566.442 & 0.123 & 0.110 & 231.092 & 227.391 & 0.138 & 7.448 \\ 
Pd-1 & 1.649 & 121 & 122 & 1.190 & 2.501 & 2.460 & 2.916 & 2.888 & 1.387 & 1.397 & 0.197 & 0.207 & 1.311 & 1.271 & 1.529 & 1.491 & 425.215 & 429.278 & 893.851 & 887.637 & 0.336 & 0.298 & 468.636 & 458.359 & 0.512 & 5.380 \\ 
C3F7 & 2.272 & 93 & 94 & 2.527 & 3.303 & 3.286 & 3.431 & 3.421 & 2.626 & 2.631 & 0.098 & 0.104 & 0.776 & 0.759 & 0.806 & 0.790 & 361.333 & 362.368 & 472.229 & 471.201 & 0.049 & 0.046 & 110.896 & 108.833 & 0.347 & 2.988 \\ 
BuCzCF3oB & 1.859 & 129 & 130 & 2.182 & 2.978 & 2.971 & 3.106 & 3.094 & 2.276 & 2.272 & 0.094 & 0.090 & 0.796 & 0.789 & 0.831 & 0.821 & 399.138 & 400.763 & 544.819 & 545.643 & 0.071 & 0.065 & 145.682 & 144.879 & 0.317 & 3.469 \\ 
phenazasiline & 1.311 & 57 & 58 & 1.400 & 3.167 & 3.137 & 3.191 & 3.190 & 1.410 & 1.423 & 0.011 & 0.024 & 1.767 & 1.737 & 1.781 & 1.766 & 388.568 & 388.714 & 879.174 & 871.145 & 0.007 & 0.007 & 490.606 & 482.431 & 0.547 & 0.104 \\ 
D–A–D & 1.311 & 57 & 58 & 1.400 & 3.167 & 3.136 & 3.191 & 3.189 & 1.410 & 1.423 & 0.011 & 0.024 & 1.767 & 1.737 & 1.780 & 1.766 & 388.580 & 388.738 & 879.114 & 871.112 & 0.007 & 0.007 & 490.534 & 482.374 & 0.547 & 0.104 \\ 
pzpy & 2.133 & 131 & 132 & 1.863 & 2.259 & 2.188 & 3.220 & 3.053 & 2.656 & 2.600 & 0.793 & 0.737 & 0.396 & 0.325 & 0.564 & 0.453 & 385.068 & 406.093 & 466.827 & 476.841 & 0.631 & 0.455 & 81.759 & 70.748 & 0.933 & 0.009 \\ 
m-PO-ABN & 2.103 & 104 & 105 & 1.844 & 2.254 & 2.183 & 3.210 & 3.049 & 2.627 & 2.576 & 0.782 & 0.732 & 0.409 & 0.339 & 0.583 & 0.473 & 386.256 & 406.599 & 471.999 & 481.271 & 0.618 & 0.431 & 85.743 & 74.672 & 0.893 & 0.716 \\ 
PO-ABN & 2.094 & 104 & 105 & 1.842 & 2.250 & 2.180 & 3.203 & 3.043 & 2.622 & 2.571 & 0.780 & 0.729 & 0.408 & 0.338 & 0.581 & 0.471 & 387.148 & 407.494 & 472.903 & 482.183 & 0.693 & 0.472 & 85.755 & 74.689 & 0.888 & 0.668 \\ 
p-PO-ABN & 2.064 & 104 & 105 & 1.793 & 2.266 & 2.196 & 3.212 & 3.070 & 2.541 & 2.507 & 0.748 & 0.714 & 0.473 & 0.403 & 0.671 & 0.564 & 386.039 & 403.831 & 487.980 & 494.634 & 1.016 & 0.712 & 101.941 & 90.803 & 0.881 & 0.131 \\ 
teracridan & 3.374 & 100 & 101 & 2.928 & 3.684 & 3.654 & 4.217 & 4.156 & 3.352 & 3.330 & 0.423 & 0.402 & 0.756 & 0.726 & 0.865 & 0.826 & 294.024 & 298.347 & 369.918 & 372.341 & 0.026 & 0.020 & 75.894 & 73.994 & 0.697 & 0.832 \\ 
PTPC & 2.375 & 192 & 193 & 2.340 & 3.490 & 3.462 & 3.832 & 3.794 & 2.569 & 2.564 & 0.229 & 0.225 & 1.150 & 1.122 & 1.263 & 1.230 & 323.566 & 326.799 & 482.592 & 483.489 & 0.346 & 0.316 & 159.026 & 156.690 & 0.171 & 16.069 \\ 
TPTI & 2.390 & 53 & 54 & 2.260 & 2.550 & 2.518 & 3.215 & 3.094 & 2.849 & 2.777 & 0.589 & 0.517 & 0.290 & 0.258 & 0.366 & 0.317 & 385.667 & 400.776 & 435.158 & 446.497 & 0.181 & 0.142 & 49.491 & 45.720 & 0.764 & 0.003 \\ 
BDBTCz-Trz & 1.807 & 147 & 148 & 2.134 & 3.406 & 3.385 & 3.797 & 3.747 & 2.379 & 2.362 & 0.245 & 0.228 & 1.272 & 1.251 & 1.418 & 1.385 & 326.541 & 330.925 & 521.138 & 524.971 & 0.773 & 0.631 & 194.597 & 194.046 & 0.285 & 8.412 \\ 
BDBFCz-Trz & 1.841 & 147 & 148 & 2.153 & 3.381 & 3.360 & 3.763 & 3.713 & 2.397 & 2.379 & 0.244 & 0.226 & 1.228 & 1.207 & 1.367 & 1.334 & 329.447 & 333.919 & 517.284 & 521.142 & 0.785 & 0.642 & 187.837 & 187.223 & 0.316 & 7.406 \\ 
HAP-3MF & 1.933 & 91 & 92 & 1.993 & 3.158 & 3.146 & 3.244 & 3.225 & 2.047 & 2.043 & 0.054 & 0.050 & 1.165 & 1.153 & 1.197 & 1.182 & 382.243 & 384.495 & 605.751 & 606.851 & 0.000 & 0.000 & 223.508 & 222.356 & 0.378 & 0.944 \\ 
FlCz & 2.148 & 95 & 96 & 2.149 & 3.394 & 3.357 & 3.731 & 3.726 & 2.362 & 2.385 & 0.213 & 0.236 & 1.246 & 1.209 & 1.369 & 1.341 & 332.344 & 332.754 & 525.022 & 519.955 & 0.204 & 0.266 & 192.678 & 187.201 & 0.406 & 7.229 \\ 
SFCz & 2.102 & 116 & 117 & 2.129 & 3.420 & 3.396 & 3.762 & 3.756 & 2.342 & 2.355 & 0.213 & 0.226 & 1.291 & 1.267 & 1.420 & 1.401 & 329.552 & 330.105 & 529.441 & 526.576 & 0.217 & 0.324 & 199.888 & 196.471 & 0.378 & 7.825 \\ 
o-TPA-AP-TPA & 1.825 & 159 & 160 & 1.756 & 2.199 & 2.131 & 3.107 & 2.989 & 2.481 & 2.464 & 0.725 & 0.707 & 0.443 & 0.375 & 0.625 & 0.525 & 399.099 & 414.760 & 499.693 & 503.196 & 0.825 & 0.590 & 100.593 & 88.436 & 0.150 & 8.511 \\ 
p-TPA-AP-TPA & 1.871 & 159 & 160 & 1.714 & 2.291 & 2.220 & 3.243 & 3.122 & 2.426 & 2.409 & 0.713 & 0.696 & 0.577 & 0.507 & 0.817 & 0.712 & 382.290 & 397.182 & 510.998 & 514.633 & 1.380 & 0.950 & 128.709 & 117.451 & 0.386 & 7.202 \\ 
TNPZ & 1.190 & 177 & 178 & 1.303 & 3.052 & 3.023 & 3.277 & 3.275 & 1.399 & 1.412 & 0.096 & 0.109 & 1.749 & 1.720 & 1.877 & 1.863 & 378.381 & 378.555 & 886.016 & 877.999 & 0.007 & 0.007 & 507.635 & 499.444 & 0.279 & 8.417 \\ 
m-TPA-AP-TPA & 1.921 & 159 & 160 & 1.779 & 2.274 & 2.203 & 3.199 & 3.067 & 2.504 & 2.477 & 0.724 & 0.698 & 0.494 & 0.424 & 0.695 & 0.590 & 387.560 & 404.239 & 495.214 & 500.444 & 0.943 & 0.662 & 107.655 & 96.205 & 0.071 & 11.940 \\ 
5,6PXZ-PIDO & 0.751 & 127 & 128 & 1.418 & 2.913 & 2.883 & 3.295 & 3.260 & 1.603 & 1.603 & 0.186 & 0.185 & 1.495 & 1.466 & 1.691 & 1.657 & 376.337 & 380.366 & 773.349 & 773.633 & 0.000 & 0.000 & 397.012 & 393.267 & 0.089 & 9.067 \\ 
TRZ-3SO2 & 2.269 & 126 & 127 & 2.303 & 4.139 & 4.132 & 4.122 & 4.120 & 2.293 & 2.296 & -0.010 & -0.007 & 1.836 & 1.829 & 1.829 & 1.824 & 300.787 & 300.896 & 540.605 & 539.913 & 0.001 & 0.001 & 239.818 & 239.017 & 0.401 & 0.255 \\ 
35tCzBPym & 1.270 & 142 & 143 & 1.763 & 3.082 & 3.071 & 3.350 & 3.321 & 1.916 & 1.906 & 0.154 & 0.143 & 1.319 & 1.309 & 1.434 & 1.415 & 370.069 & 373.390 & 647.015 & 650.597 & 0.066 & 0.057 & 276.946 & 277.207 & 0.177 & 6.315 \\ 
35CzBPym & 1.444 & 94 & 95 & 1.865 & 3.215 & 3.205 & 3.474 & 3.444 & 2.016 & 2.005 & 0.150 & 0.139 & 1.350 & 1.340 & 1.459 & 1.440 & 356.851 & 359.959 & 615.112 & 618.482 & 0.061 & 0.053 & 258.262 & 258.523 & 0.186 & 6.050 \\ 
25CzBPym & 1.396 & 94 & 95 & 1.829 & 2.891 & 2.884 & 3.038 & 3.022 & 1.922 & 1.917 & 0.093 & 0.088 & 1.062 & 1.055 & 1.116 & 1.105 & 408.125 & 410.245 & 645.072 & 646.764 & 0.065 & 0.059 & 236.948 & 236.519 & 0.257 & 4.348 \\ 
25tCzBPym & 1.250 & 142 & 143 & 1.725 & 2.790 & 2.783 & 2.939 & 2.923 & 1.817 & 1.812 & 0.092 & 0.087 & 1.065 & 1.058 & 1.122 & 1.111 & 421.916 & 424.110 & 682.502 & 684.182 & 0.068 & 0.061 & 260.586 & 260.072 & 0.241 & 4.706 \\ 
BPBiPA & 2.133 & 131 & 132 & 1.863 & 2.259 & 2.188 & 3.219 & 3.053 & 2.655 & 2.599 & 0.792 & 0.736 & 0.396 & 0.325 & 0.564 & 0.454 & 385.116 & 406.146 & 466.999 & 477.019 & 0.631 & 0.454 & 81.883 & 70.873 & 0.933 & 0.009 \\ 
BTZ–DMAC & 0.896 & 100 & 101 & 1.466 & 2.670 & 2.646 & 2.875 & 2.861 & 1.579 & 1.585 & 0.113 & 0.119 & 1.204 & 1.180 & 1.297 & 1.276 & 431.204 & 433.345 & 785.365 & 781.992 & 0.166 & 0.156 & 354.160 & 348.647 & 0.312 & 1.828 \\ 
BTZ–DPA & 1.107 & 84 & 85 & 1.421 & 2.008 & 1.959 & 2.609 & 2.524 & 1.846 & 1.831 & 0.425 & 0.410 & 0.587 & 0.538 & 0.763 & 0.693 & 475.290 & 491.221 & 671.655 & 677.230 & 0.597 & 0.475 & 196.365 & 186.009 & 0.561 & 2.079 \\ 
2F & 1.015 & 130 & 131 & 1.533 & 2.883 & 2.862 & 3.329 & 3.254 & 1.770 & 1.742 & 0.237 & 0.210 & 1.350 & 1.330 & 1.559 & 1.512 & 372.381 & 381.021 & 700.450 & 711.580 & 0.137 & 0.109 & 328.069 & 330.559 & 0.120 & 11.549 \\ 
PFBP-2a & 1.108 & 119 & 120 & 1.603 & 2.932 & 2.919 & 3.225 & 3.205 & 1.763 & 1.760 & 0.160 & 0.157 & 1.328 & 1.316 & 1.461 & 1.445 & 384.495 & 386.870 & 703.076 & 704.451 & 0.345 & 0.313 & 318.581 & 317.581 & 0.399 & 6.071 \\ 
PFBP-2b & 1.304 & 179 & 180 & 1.422 & 2.938 & 2.929 & 3.281 & 3.255 & 1.588 & 1.580 & 0.166 & 0.158 & 1.516 & 1.506 & 1.693 & 1.674 & 377.851 & 380.962 & 780.543 & 784.479 & 0.000 & 0.000 & 402.692 & 403.517 & 0.451 & 0.030 \\ 
PXZ-PPO & 2.329 & 63 & 64 & 2.308 & 2.901 & 2.872 & 3.577 & 3.522 & 2.847 & 2.831 & 0.538 & 0.523 & 0.593 & 0.563 & 0.731 & 0.691 & 346.586 & 352.008 & 435.552 & 437.913 & 0.144 & 0.547 & 88.966 & 85.905 & 0.571 & 3.502 \\ 
PXZ-BOO & 1.592 & 63 & 64 & 2.223 & 2.626 & 2.614 & 2.925 & 2.897 & 2.477 & 2.464 & 0.254 & 0.241 & 0.402 & 0.391 & 0.448 & 0.433 & 423.849 & 427.945 & 500.551 & 503.118 & 0.273 & 0.236 & 76.703 & 75.173 & 0.389 & 4.773 \\ 
PPZTPI & 1.653 & 127 & 128 & 2.111 & 2.262 & 2.232 & 2.494 & 2.463 & 2.327 & 2.330 & 0.216 & 0.219 & 0.151 & 0.121 & 0.167 & 0.133 & 497.190 & 503.285 & 532.854 & 532.114 & 0.000 & 0.000 & 35.664 & 28.829 & 0.239 & 7.335 \\ 
PPZPPI & 1.625 & 115 & 116 & 2.087 & 2.264 & 2.233 & 2.497 & 2.466 & 2.302 & 2.305 & 0.215 & 0.217 & 0.176 & 0.146 & 0.195 & 0.161 & 496.533 & 502.795 & 538.492 & 537.937 & 0.000 & 0.000 & 41.960 & 35.142 & 0.236 & 7.350 \\ 
Pra-2DMAC & 2.639 & 93 & 94 & 2.929 & 3.369 & 3.337 & 3.972 & 3.917 & 3.453 & 3.439 & 0.524 & 0.510 & 0.439 & 0.408 & 0.518 & 0.479 & 312.177 & 316.488 & 359.014 & 360.536 & 0.022 & 0.023 & 46.837 & 44.047 & 0.249 & 3.653 \\ 
BAPCN & 1.806 & 81 & 82 & 2.119 & 2.566 & 2.531 & 3.140 & 3.064 & 2.593 & 2.565 & 0.474 & 0.446 & 0.447 & 0.413 & 0.547 & 0.499 & 394.804 & 404.635 & 478.121 & 483.419 & 0.302 & 0.241 & 83.317 & 78.784 & 0.377 & 7.881 \\ 
BACN & 2.051 & 67 & 68 & 2.244 & 2.439 & 2.403 & 3.007 & 2.924 & 2.767 & 2.730 & 0.523 & 0.486 & 0.195 & 0.160 & 0.240 & 0.194 & 412.319 & 424.023 & 448.133 & 454.164 & 0.229 & 0.184 & 35.815 & 30.142 & 0.603 & 3.871 \\ 
BDQC-2 & 1.290 & 141 & 142 & 1.577 & 2.987 & 2.963 & 3.339 & 3.307 & 1.762 & 1.760 & 0.186 & 0.183 & 1.410 & 1.386 & 1.576 & 1.547 & 371.366 & 374.926 & 703.467 & 704.528 & 0.290 & 0.274 & 332.101 & 329.602 & 0.097 & 6.836 \\ 
NIDPA-1 & 1.895 & 115 & 116 & 2.038 & 2.443 & 2.412 & 2.932 & 2.859 & 2.446 & 2.415 & 0.408 & 0.377 & 0.405 & 0.374 & 0.486 & 0.444 & 422.880 & 433.663 & 506.982 & 513.355 & 0.195 & 0.153 & 84.102 & 79.692 & 0.539 & 3.382 \\ 
NIDPA-2 & 1.893 & 115 & 116 & 2.113 & 2.580 & 2.559 & 3.014 & 2.945 & 2.469 & 2.431 & 0.356 & 0.318 & 0.467 & 0.447 & 0.546 & 0.514 & 411.320 & 421.070 & 502.257 & 510.097 & 0.373 & 0.303 & 90.936 & 89.026 & 0.470 & 3.597 \\ 
SABIQ & 1.122 & 93 & 94 & 1.301 & 2.430 & 2.365 & 2.846 & 2.845 & 1.523 & 1.565 & 0.223 & 0.264 & 1.129 & 1.064 & 1.322 & 1.280 & 435.705 & 435.843 & 813.837 & 792.316 & 0.001 & 0.001 & 378.132 & 356.473 & 0.326 & 3.599 \\ 
Perylene & 1.889 & 46 & 47 & 1.699 & 2.155 & 2.083 & 3.251 & 3.078 & 2.562 & 2.511 & 0.863 & 0.812 & 0.456 & 0.384 & 0.688 & 0.568 & 381.408 & 402.755 & 483.863 & 493.854 & 0.864 & 0.602 & 102.456 & 91.099 & 0.946 & 0.000 \\ 
SAIP & 1.695 & 75 & 76 & 1.983 & 3.407 & 3.377 & 3.566 & 3.565 & 2.075 & 2.093 & 0.093 & 0.111 & 1.425 & 1.394 & 1.491 & 1.472 & 347.645 & 347.743 & 597.478 & 592.278 & 0.003 & 0.003 & 249.832 & 244.535 & 0.265 & 3.500 \\ 
FAC & 2.709 & 61 & 62 & 3.004 & 3.461 & 3.428 & 4.090 & 4.015 & 3.550 & 3.518 & 0.546 & 0.514 & 0.457 & 0.424 & 0.540 & 0.497 & 303.125 & 308.810 & 349.271 & 352.388 & 0.108 & 0.089 & 46.146 & 43.578 & 0.170 & 3.739 \\ 
phenylperylene & 1.833 & 60 & 61 & 1.619 & 2.128 & 2.061 & 3.113 & 2.968 & 2.368 & 2.332 & 0.750 & 0.713 & 0.509 & 0.442 & 0.744 & 0.636 & 398.292 & 417.765 & 523.480 & 531.733 & 0.723 & 0.511 & 125.188 & 113.968 & 0.937 & 0.186 \\ 
ImPy-2 & 2.408 & 65 & 66 & 2.279 & 2.656 & 2.621 & 3.276 & 3.187 & 2.811 & 2.771 & 0.532 & 0.492 & 0.377 & 0.342 & 0.465 & 0.416 & 378.474 & 389.043 & 441.099 & 447.375 & 0.307 & 0.243 & 62.625 & 58.332 & 0.661 & 3.229 \\ 
ImPy-1 & 2.388 & 59 & 60 & 2.295 & 2.665 & 2.630 & 3.295 & 3.203 & 2.837 & 2.796 & 0.542 & 0.501 & 0.370 & 0.334 & 0.458 & 0.407 & 376.291 & 387.100 & 436.979 & 443.477 & 0.314 & 0.248 & 60.688 & 56.377 & 0.562 & 4.139 \\ 
ImPy-3 & 1.938 & 72 & 73 & 1.864 & 2.534 & 2.478 & 3.162 & 3.103 & 2.326 & 2.333 & 0.462 & 0.469 & 0.670 & 0.615 & 0.836 & 0.769 & 392.144 & 399.627 & 533.039 & 531.396 & 0.864 & 0.708 & 140.894 & 131.769 & 0.637 & 4.028 \\ 
BTaz-Ar-PXZ & 1.507 & 69 & 70 & 2.060 & 2.766 & 2.734 & 3.046 & 3.027 & 2.268 & 2.280 & 0.208 & 0.221 & 0.706 & 0.675 & 0.778 & 0.747 & 407.053 & 409.581 & 546.648 & 543.759 & 0.444 & 0.399 & 139.595 & 134.178 & 0.312 & 6.168 \\ 
FSF4A & 2.518 & 125 & 126 & 2.540 & 3.090 & 3.065 & 3.443 & 3.418 & 2.830 & 2.832 & 0.290 & 0.292 & 0.550 & 0.525 & 0.613 & 0.586 & 360.126 & 362.728 & 438.155 & 437.765 & 0.342 & 0.306 & 78.029 & 75.037 & 0.554 & 2.301 \\ 
TPA-L-BN & 2.082 & 73 & 74 & 2.760 & 3.411 & 3.388 & 3.914 & 3.874 & 3.168 & 3.156 & 0.408 & 0.396 & 0.650 & 0.628 & 0.747 & 0.718 & 316.731 & 320.050 & 391.365 & 392.811 & 0.083 & 0.063 & 74.634 & 72.761 & 0.110 & 4.316 \\ 
IpCm-PhBzAc & 1.615 & 105 & 106 & 2.426 & 3.073 & 3.041 & 3.732 & 3.670 & 2.947 & 2.928 & 0.521 & 0.501 & 0.647 & 0.615 & 0.785 & 0.742 & 332.192 & 337.841 & 420.731 & 423.499 & 0.966 & 0.908 & 88.539 & 85.658 & 0.036 & 8.324 \\ 
DphAn-Br & 2.578 & 67 & 68 & 2.530 & 3.660 & 3.659 & 3.650 & 3.649 & 2.523 & 2.523 & -0.007 & -0.007 & 1.130 & 1.129 & 1.127 & 1.126 & 339.711 & 339.813 & 491.484 & 491.484 & 0.000 & 0.000 & 151.773 & 151.671 & 0.536 & 0.193 \\ 
5-DBFBI & 2.884 & 82 & 83 & 2.743 & 3.570 & 3.542 & 4.093 & 4.051 & 3.146 & 3.138 & 0.402 & 0.394 & 0.826 & 0.798 & 0.948 & 0.913 & 302.895 & 306.081 & 394.141 & 395.151 & 1.426 & 1.246 & 91.245 & 89.070 & 0.668 & 2.524 \\ 
4-DBFBI & 2.649 & 82 & 83 & 2.669 & 3.713 & 3.686 & 4.196 & 4.155 & 3.016 & 3.009 & 0.347 & 0.340 & 1.044 & 1.017 & 1.180 & 1.146 & 295.496 & 298.405 & 411.090 & 412.062 & 0.424 & 0.375 & 115.594 & 113.657 & 0.329 & 5.152 \\ 
DMACMNPTO & 2.429 & 99 & 100 & 3.033 & 3.350 & 3.317 & 3.954 & 3.897 & 3.581 & 3.564 & 0.547 & 0.530 & 0.317 & 0.284 & 0.374 & 0.334 & 313.551 & 318.137 & 346.269 & 347.914 & 0.019 & 0.018 & 32.718 & 29.778 & 0.027 & 7.734 \\ 
1CzSO & 2.031 & 145 & 146 & 2.333 & 3.441 & 3.420 & 3.879 & 3.827 & 2.630 & 2.611 & 0.297 & 0.278 & 1.108 & 1.087 & 1.249 & 1.217 & 319.638 & 323.947 & 471.445 & 474.941 & 0.388 & 0.335 & 151.808 & 150.994 & 0.354 & 4.930 \\ 
DpAn-BzAc & 1.355 & 119 & 120 & 2.171 & 2.986 & 2.958 & 3.527 & 3.466 & 2.564 & 2.543 & 0.393 & 0.372 & 0.816 & 0.788 & 0.963 & 0.923 & 351.549 & 357.736 & 483.643 & 487.557 & 0.174 & 0.149 & 132.094 & 129.821 & 0.030 & 7.529 \\ 
BzITz & 1.977 & 98 & 99 & 2.141 & 3.303 & 3.284 & 3.701 & 3.673 & 2.398 & 2.394 & 0.257 & 0.253 & 1.163 & 1.143 & 1.303 & 1.279 & 335.029 & 337.583 & 517.015 & 517.897 & 0.860 & 0.782 & 181.986 & 180.314 & 0.367 & 6.254 \\ 
TPXZ–as-TAZ & 1.254 & 156 & 157 & 1.441 & 2.832 & 2.812 & 2.885 & 2.881 & 1.468 & 1.476 & 0.027 & 0.036 & 1.391 & 1.371 & 1.417 & 1.405 & 429.755 & 430.336 & 844.651 & 839.731 & 0.041 & 0.040 & 414.896 & 409.395 & 0.106 & 1.926 \\ 
TPA-CN-N4-2PY & 2.253 & 94 & 95 & 2.359 & 3.150 & 3.115 & 3.735 & 3.695 & 2.797 & 2.797 & 0.438 & 0.439 & 0.791 & 0.757 & 0.938 & 0.897 & 331.979 & 335.573 & 443.300 & 443.234 & 0.829 & 0.687 & 111.321 & 107.661 & 0.404 & 5.466 \\ 
TPA-CN-N4 & 1.341 & 51 & 52 & 1.395 & 3.133 & 3.083 & 3.215 & 3.214 & 1.431 & 1.454 & 0.036 & 0.059 & 1.739 & 1.689 & 1.784 & 1.760 & 385.619 & 385.763 & 866.345 & 852.866 & 0.007 & 0.007 & 480.726 & 467.103 & 0.564 & 0.044 \\ 
6,7-DCNQx-DICz & 0.709 & 150 & 151 & 1.238 & 3.148 & 3.128 & 3.201 & 3.198 & 1.259 & 1.266 & 0.021 & 0.028 & 1.910 & 1.890 & 1.942 & 1.932 & 387.378 & 387.644 & 984.750 & 979.197 & 0.018 & 0.018 & 597.372 & 591.553 & 0.074 & 9.615 \\ 
PBICT & 2.079 & 149 & 150 & 2.126 & 3.091 & 3.068 & 3.589 & 3.529 & 2.469 & 2.445 & 0.342 & 0.319 & 0.965 & 0.942 & 1.121 & 1.083 & 345.418 & 351.379 & 502.256 & 506.991 & 0.530 & 0.428 & 156.838 & 155.612 & 0.288 & 4.034 \\ 
DCBNPE & 0.955 & 110 & 111 & 1.183 & 1.843 & 1.819 & 2.225 & 2.189 & 1.429 & 1.424 & 0.246 & 0.241 & 0.659 & 0.635 & 0.796 & 0.765 & 557.207 & 566.422 & 867.741 & 870.649 & 0.281 & 0.233 & 310.533 & 304.227 & 0.381 & 0.477 \\ 
TPA-BT-Q & 3.060 & 120 & 121 & 2.994 & 3.481 & 3.458 & 4.057 & 4.020 & 3.490 & 3.480 & 0.496 & 0.486 & 0.487 & 0.465 & 0.568 & 0.540 & 305.575 & 308.426 & 355.295 & 356.291 & 0.508 & 0.434 & 49.719 & 47.865 & 0.670 & 0.991 \\ 
D5 & 2.723 & 100 & 101 & 2.729 & 3.400 & 3.377 & 3.869 & 3.801 & 3.106 & 3.072 & 0.377 & 0.343 & 0.671 & 0.648 & 0.764 & 0.729 & 320.414 & 326.154 & 399.177 & 403.544 & 0.289 & 0.236 & 78.763 & 77.390 & 0.176 & 10.371 \\ 
D6 & 2.689 & 86 & 87 & 2.705 & 3.384 & 3.361 & 3.829 & 3.757 & 3.060 & 3.024 & 0.355 & 0.319 & 0.679 & 0.656 & 0.768 & 0.733 & 323.828 & 330.000 & 405.140 & 409.994 & 0.199 & 0.164 & 81.312 & 79.994 & 0.239 & 7.057 \\ 
PxPYM & 1.476 & 109 & 110 & 1.839 & 2.772 & 2.740 & 3.127 & 3.106 & 2.075 & 2.085 & 0.236 & 0.245 & 0.932 & 0.901 & 1.052 & 1.021 & 396.483 & 399.164 & 597.458 & 594.705 & 0.507 & 0.015 & 200.975 & 195.541 & 0.294 & 6.248 \\ 
D1–D6 & 2.688 & 86 & 87 & 2.705 & 3.384 & 3.360 & 3.829 & 3.757 & 3.061 & 3.025 & 0.356 & 0.320 & 0.679 & 0.655 & 0.768 & 0.732 & 323.812 & 330.000 & 405.057 & 409.919 & 0.198 & 0.163 & 81.245 & 79.919 & 0.239 & 7.038 \\ 
DTPCZTZ & 2.327 & 123 & 124 & 2.419 & 3.442 & 3.419 & 3.869 & 3.803 & 2.720 & 2.691 & 0.301 & 0.272 & 1.022 & 1.000 & 1.149 & 1.112 & 320.431 & 325.991 & 455.815 & 460.693 & 0.201 & 0.164 & 135.385 & 134.702 & 0.277 & 9.463 \\ 
DHPZ-2BI & 1.611 & 132 & 133 & 2.004 & 2.316 & 2.286 & 2.553 & 2.522 & 2.209 & 2.211 & 0.205 & 0.208 & 0.312 & 0.282 & 0.344 & 0.311 & 485.679 & 491.513 & 561.203 & 560.635 & 0.000 & 0.000 & 75.524 & 69.122 & 0.269 & 2.540 \\ 
DHPZ-2BN & 1.498 & 70 & 71 & 1.944 & 2.256 & 2.247 & 2.520 & 2.492 & 2.172 & 2.156 & 0.228 & 0.212 & 0.312 & 0.303 & 0.348 & 0.336 & 491.942 & 497.549 & 570.795 & 575.150 & 0.000 & 0.000 & 78.853 & 77.601 & 0.354 & 0.051 \\ 
SAF-2NP & 0.996 & 111 & 112 & 1.257 & 2.524 & 2.513 & 2.703 & 2.688 & 1.346 & 1.344 & 0.089 & 0.087 & 1.267 & 1.256 & 1.357 & 1.343 & 458.657 & 461.319 & 921.121 & 922.357 & 0.221 & 0.208 & 462.464 & 461.037 & 0.311 & 5.805 \\ 
BTPO & 3.062 & 62 & 63 & 3.199 & 3.636 & 3.612 & 4.098 & 4.048 & 3.605 & 3.585 & 0.406 & 0.386 & 0.438 & 0.414 & 0.493 & 0.463 & 302.541 & 306.255 & 343.954 & 345.850 & 0.056 & 0.187 & 41.413 & 39.595 & 0.508 & 2.192 \\ 
PyDCN–DMAC & 1.519 & 104 & 105 & 2.178 & 3.368 & 3.336 & 3.860 & 3.851 & 2.495 & 2.514 & 0.318 & 0.336 & 1.190 & 1.158 & 1.364 & 1.337 & 321.244 & 321.970 & 496.850 & 493.227 & 0.053 & 0.036 & 175.606 & 171.257 & 0.069 & 9.804 \\ 
PyDCN & 2.430 & 65 & 66 & 2.641 & 3.856 & 3.814 & 4.487 & 4.449 & 3.073 & 3.080 & 0.432 & 0.439 & 1.215 & 1.173 & 1.414 & 1.368 & 276.300 & 278.704 & 403.423 & 402.490 & 0.573 & 0.531 & 127.123 & 123.786 & 0.295 & 0.928 \\ 
PXZ-OXD & 1.588 & 74 & 75 & 2.186 & 2.777 & 2.746 & 3.096 & 3.078 & 2.437 & 2.451 & 0.251 & 0.265 & 0.591 & 0.560 & 0.659 & 0.627 & 400.453 & 402.768 & 508.665 & 505.859 & 0.435 & 0.394 & 108.213 & 103.091 & 0.291 & 6.770 \\ 
TCz-3PA-TCz & 2.040 & 179 & 180 & 2.026 & 3.190 & 3.159 & 3.657 & 3.631 & 2.322 & 2.328 & 0.296 & 0.302 & 1.165 & 1.134 & 1.335 & 1.303 & 339.023 & 341.488 & 533.962 & 532.601 & 2.489 & 2.272 & 194.939 & 191.113 & 0.568 & 0.109 \\ 
NAI–BiFA & 1.419 & 148 & 149 & 1.637 & 1.926 & 1.885 & 2.546 & 2.468 & 2.163 & 2.142 & 0.526 & 0.506 & 0.290 & 0.249 & 0.383 & 0.325 & 487.072 & 502.449 & 573.239 & 578.749 & 0.755 & 0.617 & 86.167 & 76.301 & 0.528 & 3.705 \\ 
NAI–PhBiFA & 1.031 & 162 & 163 & 1.617 & 2.589 & 2.551 & 3.064 & 3.033 & 1.914 & 1.922 & 0.297 & 0.305 & 0.972 & 0.934 & 1.150 & 1.111 & 404.582 & 408.757 & 647.728 & 644.957 & 1.239 & 1.137 & 243.146 & 236.200 & 0.301 & 7.870 \\ 
pDTCz-2DPyS & 1.957 & 146 & 147 & 2.072 & 3.277 & 3.259 & 3.732 & 3.698 & 2.359 & 2.351 & 0.287 & 0.279 & 1.205 & 1.186 & 1.372 & 1.346 & 332.246 & 335.301 & 525.484 & 527.258 & 0.128 & 0.116 & 193.238 & 191.957 & 0.485 & 3.617 \\ 
2SPBAC-BP & 1.589 & 172 & 173 & 1.935 & 2.812 & 2.780 & 3.396 & 3.345 & 2.338 & 2.328 & 0.402 & 0.393 & 0.876 & 0.844 & 1.059 & 1.016 & 365.057 & 370.700 & 530.397 & 532.466 & 0.090 & 0.115 & 165.341 & 161.767 & 0.252 & 3.448 \\ 
SPBAC-PH & 2.513 & 84 & 85 & 2.590 & 2.712 & 2.676 & 3.326 & 3.241 & 3.175 & 3.136 & 0.586 & 0.547 & 0.123 & 0.087 & 0.150 & 0.105 & 372.784 & 382.490 & 390.440 & 395.318 & 0.258 & 0.210 & 17.656 & 12.828 & 0.620 & 2.925 \\ 
DFPBI & 2.313 & 122 & 123 & 2.221 & 3.092 & 3.063 & 3.555 & 3.528 & 2.553 & 2.558 & 0.333 & 0.337 & 0.871 & 0.842 & 1.002 & 0.970 & 348.760 & 351.459 & 485.580 & 484.717 & 1.704 & 1.532 & 136.820 & 133.258 & 0.580 & 5.484 \\ 
TDPA–TRZ & 2.012 & 150 & 151 & 2.118 & 2.942 & 2.913 & 3.488 & 3.459 & 2.510 & 2.515 & 0.393 & 0.397 & 0.825 & 0.795 & 0.978 & 0.944 & 355.439 & 358.408 & 493.882 & 493.015 & 1.617 & 1.486 & 138.443 & 134.607 & 0.446 & 0.679 \\ 
DMAC-11-DPPZ & 1.119 & 90 & 91 & 1.319 & 2.769 & 2.756 & 2.919 & 2.907 & 1.390 & 1.391 & 0.071 & 0.072 & 1.450 & 1.437 & 1.529 & 1.516 & 424.720 & 426.473 & 891.850 & 891.295 & 0.159 & 0.150 & 467.131 & 464.823 & 0.262 & 5.725 \\ 
PXZ-11-DPPZ & 1.087 & 84 & 85 & 1.304 & 2.227 & 2.215 & 2.451 & 2.428 & 1.435 & 1.430 & 0.131 & 0.126 & 0.923 & 0.911 & 1.015 & 0.998 & 505.893 & 510.559 & 863.794 & 867.026 & 0.250 & 0.221 & 357.901 & 356.467 & 0.329 & 5.709 \\ 
PXZ-10-DPPZ & 0.965 & 84 & 85 & 1.202 & 2.033 & 2.024 & 2.188 & 2.173 & 1.293 & 1.291 & 0.091 & 0.089 & 0.831 & 0.822 & 0.894 & 0.882 & 566.681 & 570.593 & 958.577 & 960.637 & 0.086 & 0.075 & 391.895 & 390.044 & 0.385 & 3.809 \\ 
CCC & 3.293 & 47 & 48 & 3.034 & 3.696 & 3.645 & 4.290 & 4.267 & 3.521 & 3.551 & 0.487 & 0.517 & 0.662 & 0.611 & 0.769 & 0.715 & 289.034 & 290.586 & 352.137 & 349.133 & 0.010 & 0.012 & 63.103 & 58.547 & 0.916 & 0.597 \\ 
CzmPPC & 2.379 & 99 & 100 & 2.412 & 4.101 & 4.069 & 4.228 & 4.227 & 2.486 & 2.506 & 0.074 & 0.094 & 1.689 & 1.656 & 1.741 & 1.721 & 293.273 & 293.343 & 498.647 & 494.777 & 0.008 & 0.008 & 205.374 & 201.434 & 0.443 & 0.568 \\ 
C2FLA-1 & 2.228 & 105 & 106 & 2.145 & 3.228 & 3.187 & 3.884 & 3.840 & 2.580 & 2.584 & 0.435 & 0.439 & 1.084 & 1.043 & 1.304 & 1.256 & 319.226 & 322.876 & 480.562 & 479.868 & 2.956 & 2.568 & 161.336 & 156.993 & 0.650 & 6.627 \\ 
MDP3FL & 2.202 & 177 & 178 & 2.169 & 3.284 & 3.258 & 3.707 & 3.689 & 2.447 & 2.456 & 0.279 & 0.287 & 1.116 & 1.089 & 1.259 & 1.234 & 334.487 & 336.046 & 506.613 & 504.837 & 4.064 & 3.766 & 172.126 & 168.791 & 0.534 & 0.804 \\ 
C3FLA-2 & 2.078 & 167 & 168 & 1.972 & 3.240 & 3.201 & 3.743 & 3.720 & 2.278 & 2.292 & 0.306 & 0.320 & 1.268 & 1.230 & 1.465 & 1.429 & 331.252 & 333.255 & 544.265 & 541.050 & 5.170 & 4.730 & 213.013 & 207.795 & 0.724 & 1.065 \\ 
9CzFDPEPO & 2.598 & 188 & 189 & 2.870 & 3.415 & 3.392 & 3.892 & 3.823 & 3.271 & 3.235 & 0.400 & 0.365 & 0.545 & 0.522 & 0.621 & 0.588 & 318.594 & 324.294 & 379.078 & 383.250 & 0.168 & 0.142 & 60.484 & 58.956 & 0.056 & 10.993 \\ 
9CzFDPESPO & 2.756 & 154 & 155 & 2.940 & 3.370 & 3.347 & 3.803 & 3.733 & 3.317 & 3.279 & 0.377 & 0.339 & 0.431 & 0.407 & 0.486 & 0.454 & 326.000 & 332.121 & 373.764 & 378.139 & 0.178 & 0.150 & 47.764 & 46.018 & 0.032 & 15.442 \\ 
CTM & 1.998 & 80 & 81 & 2.390 & 3.336 & 3.315 & 3.563 & 3.560 & 2.553 & 2.567 & 0.163 & 0.177 & 0.946 & 0.925 & 1.010 & 0.993 & 347.967 & 348.270 & 485.646 & 483.009 & 0.009 & 0.012 & 137.678 & 134.739 & 0.327 & 6.048 \\ 
tCTM & 1.830 & 104 & 105 & 2.303 & 3.251 & 3.231 & 3.621 & 3.597 & 2.565 & 2.564 & 0.262 & 0.261 & 0.948 & 0.928 & 1.056 & 1.033 & 342.394 & 344.697 & 483.288 & 483.501 & 0.274 & 0.497 & 140.894 & 138.804 & 0.326 & 6.319 \\ 
PSBC & 2.135 & 161 & 162 & 2.174 & 3.414 & 3.392 & 3.792 & 3.744 & 2.415 & 2.400 & 0.241 & 0.226 & 1.240 & 1.217 & 1.377 & 1.344 & 326.937 & 331.154 & 513.342 & 516.568 & 0.016 & 0.001 & 186.405 & 185.413 & 0.297 & 7.069 \\ 
26DAcBPy & 1.044 & 131 & 132 & 1.580 & 2.816 & 2.803 & 3.137 & 3.115 & 1.760 & 1.756 & 0.180 & 0.176 & 1.236 & 1.223 & 1.377 & 1.359 & 395.282 & 397.959 & 704.548 & 705.944 & 0.253 & 0.235 & 309.266 & 307.985 & 0.165 & 6.957 \\ 
25DAcBPy & 1.007 & 131 & 132 & 1.258 & 2.561 & 2.525 & 3.233 & 3.203 & 1.588 & 1.596 & 0.330 & 0.338 & 1.303 & 1.266 & 1.645 & 1.607 & 383.448 & 387.051 & 780.692 & 776.706 & 0.240 & 0.328 & 397.244 & 389.654 & 0.211 & 7.076 \\ 
26DPXZBPy & 0.939 & 119 & 120 & 1.454 & 2.521 & 2.511 & 2.813 & 2.798 & 1.622 & 1.620 & 0.169 & 0.166 & 1.067 & 1.057 & 1.191 & 1.178 & 440.676 & 443.181 & 764.270 & 765.444 & 0.014 & 0.015 & 323.594 & 322.263 & 0.292 & 6.794 \\ 
BTITrz & 1.750 & 98 & 99 & 2.060 & 3.420 & 3.399 & 3.800 & 3.776 & 2.288 & 2.289 & 0.229 & 0.229 & 1.361 & 1.339 & 1.512 & 1.488 & 326.231 & 328.305 & 541.791 & 541.759 & 0.710 & 0.671 & 215.560 & 213.455 & 0.305 & 6.669 \\ 
mTPA–PPI & 2.396 & 113 & 114 & 2.517 & 3.385 & 3.360 & 3.749 & 3.711 & 2.787 & 2.780 & 0.270 & 0.263 & 0.868 & 0.843 & 0.961 & 0.931 & 330.748 & 334.099 & 444.815 & 445.990 & 0.595 & 0.502 & 114.067 & 111.891 & 0.209 & 8.898 \\ 
PPI & 2.839 & 68 & 69 & 2.599 & 3.411 & 3.381 & 3.784 & 3.739 & 2.883 & 2.874 & 0.284 & 0.275 & 0.813 & 0.782 & 0.902 & 0.865 & 327.611 & 331.571 & 430.084 & 431.391 & 0.197 & 0.184 & 102.474 & 99.821 & 0.785 & 1.376 \\ 
CzTPA-m-Trz & 1.553 & 146 & 147 & 2.016 & 3.063 & 3.050 & 3.430 & 3.391 & 2.257 & 2.241 & 0.242 & 0.226 & 1.048 & 1.034 & 1.173 & 1.150 & 361.417 & 365.660 & 549.244 & 553.206 & 0.044 & 0.036 & 187.827 & 187.546 & 0.032 & 8.469 \\ 
TPA–2PPITPA & 2.309 & 242 & 243 & 2.115 & 3.482 & 3.459 & 3.846 & 3.822 & 2.336 & 2.337 & 0.221 & 0.222 & 1.366 & 1.344 & 1.509 & 1.485 & 322.405 & 324.413 & 530.661 & 530.468 & 1.234 & 1.092 & 208.255 & 206.055 & 0.494 & 3.779 \\ 
TPA–2SPPITPA & 1.841 & 252 & 253 & 1.747 & 2.818 & 2.777 & 3.441 & 3.409 & 2.134 & 2.145 & 0.386 & 0.397 & 1.071 & 1.030 & 1.307 & 1.264 & 360.346 & 363.750 & 581.122 & 578.118 & 0.440 & 0.491 & 220.776 & 214.368 & 0.332 & 7.920 \\ 
2Cz2tCzBn & 1.976 & 187 & 188 & 2.343 & 2.992 & 2.980 & 3.269 & 3.229 & 2.560 & 2.539 & 0.217 & 0.196 & 0.649 & 0.637 & 0.709 & 0.690 & 379.261 & 383.935 & 484.272 & 488.258 & 0.465 & 0.407 & 105.011 & 104.323 & 0.378 & 0.214 \\ 
2tCz2CzBn & 1.939 & 187 & 188 & 2.343 & 3.011 & 2.999 & 3.303 & 3.261 & 2.570 & 2.548 & 0.227 & 0.205 & 0.668 & 0.655 & 0.733 & 0.713 & 375.414 & 380.250 & 482.419 & 486.589 & 0.432 & 0.376 & 107.005 & 106.339 & 0.347 & 2.328 \\ 
PmPmP & 1.100 & 90 & 91 & 1.703 & 2.761 & 2.730 & 3.124 & 3.085 & 1.927 & 1.924 & 0.224 & 0.221 & 1.058 & 1.027 & 1.197 & 1.160 & 396.889 & 401.946 & 643.489 & 644.301 & 0.015 & 0.013 & 246.600 & 242.355 & 0.211 & 8.617 \\ 
PLQYs & 1.896 & 145 & 146 & 2.114 & 2.803 & 2.732 & 3.333 & 3.290 & 2.513 & 2.546 & 0.400 & 0.432 & 0.690 & 0.618 & 0.820 & 0.744 & 371.934 & 376.852 & 493.279 & 487.034 & 0.031 & 0.026 & 121.345 & 110.183 & 0.318 & 0.080 \\ 
PXZ-ND & 1.922 & 90 & 91 & 1.905 & 2.592 & 2.568 & 3.025 & 2.978 & 2.223 & 2.209 & 0.318 & 0.304 & 0.687 & 0.662 & 0.801 & 0.768 & 409.906 & 416.390 & 557.667 & 561.177 & 0.883 & 0.751 & 147.761 & 144.788 & 0.541 & 1.532 \\ 
CPPyC & 2.583 & 89 & 90 & 2.687 & 3.393 & 3.369 & 3.820 & 3.753 & 3.026 & 2.993 & 0.338 & 0.306 & 0.705 & 0.682 & 0.794 & 0.759 & 324.591 & 330.395 & 409.786 & 414.212 & 0.422 & 0.339 & 85.195 & 83.817 & 0.274 & 5.374 \\ 
DMAC-ND & 2.126 & 102 & 103 & 2.087 & 2.756 & 2.728 & 3.258 & 3.196 & 2.468 & 2.445 & 0.380 & 0.358 & 0.669 & 0.641 & 0.791 & 0.751 & 380.518 & 387.923 & 502.455 & 507.085 & 0.957 & 0.805 & 121.937 & 119.162 & 0.546 & 1.035 \\ 
PrDPhAc & 2.613 & 137 & 138 & 2.422 & 3.105 & 3.075 & 3.786 & 3.715 & 2.952 & 2.926 & 0.531 & 0.505 & 0.684 & 0.653 & 0.833 & 0.789 & 327.507 & 333.712 & 419.962 & 423.717 & 0.619 & 0.509 & 92.456 & 90.004 & 0.691 & 0.063 \\ 
2Mi2SB & 2.467 & 133 & 134 & 2.802 & 4.115 & 4.089 & 4.683 & 4.632 & 3.188 & 3.174 & 0.387 & 0.372 & 1.313 & 1.287 & 1.494 & 1.458 & 264.771 & 267.651 & 388.871 & 390.638 & 0.135 & 0.123 & 124.101 & 122.986 & 0.282 & 0.705 \\ 
BFDMAc-NAI & 1.026 & 117 & 118 & 1.642 & 2.103 & 2.090 & 2.267 & 2.253 & 1.771 & 1.770 & 0.128 & 0.128 & 0.460 & 0.448 & 0.496 & 0.483 & 546.909 & 550.307 & 700.220 & 700.449 & 0.118 & 0.109 & 153.311 & 150.142 & 0.328 & 4.465 \\ 
HPIPXZ & 2.492 & 60 & 61 & 2.359 & 3.160 & 3.119 & 3.718 & 3.661 & 2.776 & 2.769 & 0.417 & 0.410 & 0.801 & 0.760 & 0.942 & 0.892 & 333.461 & 338.681 & 446.614 & 447.719 & 0.633 & 0.578 & 113.153 & 109.039 & 0.734 & 3.042 \\ 
3BPy-mDTC & 1.503 & 142 & 143 & 1.980 & 3.235 & 3.225 & 3.490 & 3.462 & 2.136 & 2.126 & 0.156 & 0.146 & 1.255 & 1.245 & 1.354 & 1.336 & 355.245 & 358.150 & 580.344 & 583.243 & 0.084 & 0.075 & 225.099 & 225.094 & 0.195 & 5.937 \\ 
2BPy-mDTC & 1.318 & 142 & 143 & 1.722 & 3.172 & 3.163 & 3.328 & 3.319 & 1.807 & 1.807 & 0.085 & 0.085 & 1.450 & 1.441 & 1.521 & 1.512 & 372.560 & 373.559 & 686.117 & 686.027 & 0.034 & 0.037 & 313.557 & 312.468 & 0.216 & 4.714 \\ 
BP-mDTC & 1.716 & 142 & 143 & 2.166 & 3.381 & 3.362 & 3.667 & 3.637 & 2.349 & 2.343 & 0.183 & 0.177 & 1.215 & 1.196 & 1.318 & 1.294 & 338.126 & 340.906 & 527.820 & 529.121 & 0.137 & 0.131 & 189.693 & 188.215 & 0.208 & 4.527 \\ 
Cz2ICz & 2.348 & 104 & 105 & 2.552 & 3.137 & 3.118 & 3.490 & 3.434 & 2.839 & 2.811 & 0.287 & 0.259 & 0.585 & 0.566 & 0.651 & 0.624 & 355.205 & 360.996 & 436.671 & 441.131 & 0.389 & 0.337 & 81.466 & 80.135 & 0.423 & 1.750 \\ 
Ac-BPCN & 1.273 & 98 & 99 & 1.209 & 1.936 & 1.894 & 2.544 & 2.454 & 1.589 & 1.566 & 0.380 & 0.357 & 0.727 & 0.685 & 0.956 & 0.888 & 487.321 & 505.254 & 780.450 & 791.532 & 0.443 & 0.353 & 293.129 & 286.279 & 0.501 & 1.009 \\ 
5CzICz & 2.479 & 74 & 75 & 2.705 & 3.199 & 3.179 & 3.582 & 3.521 & 3.029 & 2.996 & 0.324 & 0.291 & 0.494 & 0.474 & 0.553 & 0.525 & 346.112 & 352.128 & 409.323 & 413.861 & 0.242 & 0.212 & 63.212 & 61.733 & 0.370 & 5.479 \\ 
DCPDAPM & 2.071 & 133 & 134 & 2.026 & 2.712 & 2.678 & 3.404 & 3.338 & 2.544 & 2.526 & 0.517 & 0.500 & 0.685 & 0.651 & 0.860 & 0.812 & 364.263 & 371.410 & 487.448 & 490.781 & 1.013 & 0.864 & 123.185 & 119.370 & 0.479 & 4.320 \\ 
SPFS-PXZ & 2.153 & 133 & 134 & 2.448 & 2.911 & 2.882 & 3.296 & 3.262 & 2.771 & 2.771 & 0.324 & 0.323 & 0.464 & 0.434 & 0.525 & 0.491 & 376.109 & 380.110 & 447.355 & 447.502 & 0.012 & 0.010 & 71.247 & 67.392 & 0.355 & 2.138 \\ 
DPS-PXZ & 1.940 & 104 & 105 & 2.354 & 2.901 & 2.870 & 3.287 & 3.251 & 2.667 & 2.666 & 0.313 & 0.312 & 0.547 & 0.516 & 0.620 & 0.585 & 377.219 & 381.384 & 464.836 & 464.996 & 0.005 & 0.004 & 87.617 & 83.611 & 0.350 & 2.883 \\ 
TX-CzPh & 1.810 & 80 & 81 & 2.235 & 2.904 & 2.877 & 3.620 & 3.510 & 2.787 & 2.727 & 0.552 & 0.492 & 0.668 & 0.642 & 0.833 & 0.783 & 342.479 & 353.251 & 444.852 & 454.657 & 0.175 & 0.137 & 102.373 & 101.405 & 0.240 & 7.655 \\ 
bpipH & 1.859 & 57 & 58 & 2.350 & 3.224 & 3.192 & 3.850 & 3.776 & 2.805 & 2.780 & 0.456 & 0.430 & 0.875 & 0.843 & 1.044 & 0.997 & 322.062 & 328.305 & 441.949 & 446.058 & 0.523 & 0.471 & 119.887 & 117.754 & 0.165 & 6.271 \\ 
Tri-PXZ-PCN & 0.968 & 164 & 165 & 1.403 & 2.581 & 2.570 & 2.872 & 2.851 & 1.562 & 1.557 & 0.158 & 0.153 & 1.177 & 1.167 & 1.310 & 1.294 & 431.700 & 434.925 & 793.895 & 796.511 & 0.519 & 0.465 & 362.195 & 361.585 & 0.091 & 8.260 \\ 
ACID–BPPZ & 0.884 & 138 & 139 & 1.381 & 2.841 & 2.818 & 3.166 & 3.159 & 1.539 & 1.548 & 0.158 & 0.167 & 1.460 & 1.437 & 1.627 & 1.610 & 391.587 & 392.541 & 805.385 & 800.812 & 0.194 & 0.167 & 413.798 & 408.271 & 0.169 & 8.057 \\ 
C-BPyIA & 2.058 & 175 & 176 & 1.808 & 2.263 & 2.193 & 3.260 & 3.108 & 2.605 & 2.562 & 0.797 & 0.754 & 0.455 & 0.386 & 0.656 & 0.546 & 380.261 & 398.907 & 476.016 & 484.000 & 0.972 & 0.684 & 95.755 & 85.093 & 0.820 & 0.083 \\ 
N-BPyIA & 2.018 & 175 & 176 & 1.871 & 2.254 & 2.184 & 3.212 & 3.044 & 2.667 & 2.608 & 0.795 & 0.737 & 0.383 & 0.312 & 0.545 & 0.435 & 386.003 & 407.360 & 464.938 & 475.316 & 0.744 & 0.513 & 78.935 & 67.956 & 0.120 & 8.851 \\ 
2-TA-AN & 2.117 & 66 & 67 & 1.920 & 2.309 & 2.236 & 3.410 & 3.230 & 2.835 & 2.773 & 0.916 & 0.853 & 0.389 & 0.316 & 0.575 & 0.457 & 363.579 & 383.900 & 437.268 & 447.129 & 0.389 & 0.271 & 73.689 & 63.229 & 0.633 & 4.086 \\ 
ANOP-MeFAC & 0.424 & 110 & 111 & 0.853 & 1.691 & 1.669 & 2.022 & 1.988 & 1.019 & 1.015 & 0.166 & 0.163 & 0.839 & 0.816 & 1.002 & 0.972 & 613.328 & 623.820 & 1216.553 & 1221.049 & 0.279 & 0.249 & 603.225 & 597.229 & 0.387 & 7.311 \\ 
ANOP-DMAC & 0.428 & 83 & 84 & 0.882 & 1.812 & 1.795 & 2.073 & 2.047 & 1.009 & 1.006 & 0.127 & 0.124 & 0.930 & 0.913 & 1.064 & 1.042 & 598.062 & 605.569 & 1228.994 & 1232.677 & 0.212 & 0.186 & 630.932 & 627.108 & 0.349 & 7.385 \\ 
4PyCNICz & 1.420 & 121 & 122 & 1.954 & 3.370 & 3.345 & 3.757 & 3.708 & 2.178 & 2.166 & 0.224 & 0.212 & 1.416 & 1.391 & 1.579 & 1.542 & 330.009 & 334.360 & 569.170 & 572.329 & 0.136 & 0.134 & 239.161 & 237.969 & 0.106 & 8.249 \\ 
2PyCNBCz & 1.387 & 135 & 136 & 1.885 & 3.360 & 3.336 & 3.794 & 3.759 & 2.128 & 2.124 & 0.244 & 0.239 & 1.475 & 1.451 & 1.666 & 1.635 & 326.782 & 329.824 & 582.531 & 583.807 & 1.559 & 1.344 & 255.749 & 253.983 & 0.193 & 11.765 \\ 
CzA-PPO & 1.634 & 148 & 149 & 1.663 & 1.897 & 1.843 & 2.384 & 2.332 & 2.090 & 2.104 & 0.427 & 0.442 & 0.234 & 0.180 & 0.294 & 0.228 & 520.068 & 531.573 & 593.358 & 589.189 & 0.275 & 0.244 & 73.290 & 57.616 & 0.575 & 2.691 \\ 
2PyCNICz & 1.426 & 121 & 122 & 1.926 & 3.350 & 3.324 & 3.726 & 3.679 & 2.142 & 2.131 & 0.216 & 0.206 & 1.424 & 1.398 & 1.584 & 1.547 & 332.790 & 337.014 & 578.804 & 581.689 & 0.141 & 0.130 & 246.014 & 244.675 & 0.164 & 8.192 \\ 
TAA-PPO & 1.634 & 118 & 119 & 1.672 & 1.894 & 1.840 & 2.392 & 2.338 & 2.112 & 2.125 & 0.439 & 0.453 & 0.222 & 0.168 & 0.280 & 0.213 & 518.350 & 530.255 & 587.156 & 583.485 & 0.277 & 0.244 & 68.806 & 53.230 & 0.578 & 2.695 \\ 
pSFIAc2 & 2.278 & 163 & 164 & 2.309 & 2.655 & 2.632 & 3.090 & 3.008 & 2.687 & 2.640 & 0.378 & 0.331 & 0.346 & 0.322 & 0.403 & 0.369 & 401.243 & 412.127 & 461.386 & 469.671 & 0.411 & 0.332 & 60.143 & 57.545 & 0.669 & 0.310 \\ 
TBN-TPA & 2.370 & 179 & 180 & 2.500 & 2.670 & 2.647 & 3.130 & 3.053 & 2.931 & 2.884 & 0.430 & 0.383 & 0.170 & 0.147 & 0.199 & 0.169 & 396.179 & 406.146 & 423.067 & 429.974 & 0.439 & 0.354 & 26.888 & 23.828 & 0.587 & 0.717 \\ 
CzBPDCb & 2.733 & 89 & 90 & 2.888 & 3.282 & 3.256 & 3.792 & 3.711 & 3.336 & 3.291 & 0.449 & 0.404 & 0.394 & 0.369 & 0.455 & 0.420 & 326.997 & 334.081 & 371.641 & 376.719 & 0.118 & 0.101 & 44.644 & 42.638 & 0.052 & 8.933 \\ 
{[2,1-b]IF} & 0.583 & 107 & 108 & 0.666 & 0.305 & 0.192 & 0.736 & 0.625 & 1.610 & 2.168 & 0.944 & 1.502 & -0.361 & -0.474 & -0.873 & -1.543 & 1683.653 & 1984.382 & 770.234 & 571.927 & 0.007 & 0.003 & -913.419 & -1412.456 & 0.578 & 2.989 \\ 
cyclohexanone & 3.113 & 79 & 80 & 2.829 & 3.780 & 3.742 & 4.521 & 4.458 & 3.384 & 3.370 & 0.555 & 0.541 & 0.951 & 0.913 & 1.137 & 1.088 & 274.229 & 278.122 & 366.376 & 367.872 & 0.380 & 0.390 & 92.147 & 89.749 & 0.823 & 0.345 \\ 
thio-ether & 0.583 & 107 & 108 & 0.666 & 0.304 & 0.192 & 0.736 & 0.625 & 1.610 & 2.167 & 0.944 & 1.501 & -0.361 & -0.474 & -0.874 & -1.542 & 1684.339 & 1985.335 & 769.991 & 572.163 & 0.007 & 0.003 & -914.349 & -1413.172 & 0.578 & 2.989 \\ 
ICz-2 & 2.341 & 69 & 70 & 1.606 & 3.895 & 3.856 & 4.135 & 4.125 & 1.705 & 1.718 & 0.099 & 0.112 & 2.289 & 2.250 & 2.430 & 2.407 & 299.812 & 300.597 & 727.092 & 721.658 & 0.055 & 0.056 & 427.280 & 421.062 & 0.484 & 1.786 \\ 
DDCzTrz & 1.729 & 177 & 178 & 2.029 & 3.529 & 3.512 & 3.867 & 3.835 & 2.223 & 2.215 & 0.194 & 0.186 & 1.500 & 1.483 & 1.644 & 1.620 & 320.629 & 323.313 & 557.667 & 559.674 & 0.161 & 0.167 & 237.038 & 236.361 & 0.263 & 3.426 \\ 
B-O-dpa & 2.409 & 75 & 76 & 2.603 & 2.678 & 2.653 & 3.224 & 3.131 & 3.133 & 3.073 & 0.530 & 0.470 & 0.075 & 0.050 & 0.090 & 0.059 & 384.602 & 395.926 & 395.710 & 403.497 & 0.369 & 0.289 & 11.108 & 7.571 & 0.602 & 1.617 \\ 
B-dpa-SpiroAC & 2.223 & 118 & 119 & 2.364 & 2.515 & 2.492 & 2.955 & 2.884 & 2.777 & 2.735 & 0.413 & 0.371 & 0.151 & 0.129 & 0.177 & 0.149 & 419.617 & 429.978 & 446.422 & 453.370 & 0.567 & 0.461 & 26.805 & 23.392 & 0.567 & 1.427 \\ 
DCz-OTP & 2.971 & 103 & 104 & 2.897 & 3.405 & 3.382 & 3.882 & 3.815 & 3.303 & 3.268 & 0.406 & 0.371 & 0.508 & 0.485 & 0.580 & 0.547 & 319.358 & 324.983 & 375.399 & 379.409 & 0.136 & 0.116 & 56.042 & 54.426 & 0.366 & 3.952 \\ 
B-dpa-Cz & 2.193 & 88 & 89 & 2.348 & 2.550 & 2.526 & 3.040 & 2.962 & 2.799 & 2.754 & 0.451 & 0.406 & 0.202 & 0.178 & 0.241 & 0.209 & 407.883 & 418.512 & 442.954 & 450.219 & 0.605 & 0.482 & 35.071 & 31.707 & 0.585 & 1.683 \\ 
c-D2T & 1.578 & 234 & 235 & 2.029 & 3.348 & 3.327 & 3.767 & 3.699 & 2.283 & 2.256 & 0.254 & 0.227 & 1.319 & 1.297 & 1.483 & 1.442 & 329.176 & 335.192 & 543.040 & 549.463 & 0.112 & 0.156 & 213.863 & 214.270 & 0.070 & 6.193 \\ 
DPXZ-DPPM & 0.789 & 136 & 137 & 1.078 & 2.610 & 2.599 & 2.863 & 2.844 & 1.182 & 1.179 & 0.104 & 0.101 & 1.532 & 1.521 & 1.680 & 1.664 & 433.102 & 435.981 & 1048.679 & 1051.321 & 0.547 & 0.503 & 615.577 & 615.340 & 0.313 & 7.337 \\ 
CBPMCN & 1.963 & 102 & 103 & 2.241 & 3.439 & 3.416 & 3.877 & 3.826 & 2.526 & 2.510 & 0.286 & 0.269 & 1.198 & 1.175 & 1.351 & 1.316 & 319.786 & 324.049 & 490.740 & 493.970 & 0.552 & 0.442 & 170.954 & 169.921 & 0.179 & 6.121 \\ 
CPBPMCN & 1.923 & 116 & 117 & 2.212 & 3.471 & 3.446 & 3.875 & 3.831 & 2.469 & 2.459 & 0.257 & 0.247 & 1.260 & 1.234 & 1.406 & 1.372 & 319.959 & 323.609 & 502.217 & 504.185 & 0.415 & 0.381 & 182.258 & 180.577 & 0.095 & 10.578 \\ 
TPB-AC & 1.929 & 106 & 107 & 2.284 & 3.419 & 3.395 & 3.900 & 3.872 & 2.605 & 2.605 & 0.321 & 0.321 & 1.135 & 1.111 & 1.295 & 1.267 & 317.892 & 320.215 & 475.891 & 475.990 & 1.063 & 0.954 & 157.999 & 155.775 & 0.185 & 10.966 \\ 
Me-DMAC & 1.312 & 82 & 83 & 2.142 & 3.396 & 3.364 & 3.616 & 3.609 & 2.281 & 2.299 & 0.139 & 0.156 & 1.254 & 1.221 & 1.335 & 1.310 & 342.896 & 343.532 & 543.543 & 539.389 & 0.143 & 0.135 & 200.647 & 195.857 & 0.044 & 7.726 \\ 
iTPBI-CN & 2.351 & 124 & 125 & 2.540 & 3.741 & 3.714 & 4.220 & 4.195 & 2.865 & 2.869 & 0.325 & 0.329 & 1.201 & 1.174 & 1.355 & 1.326 & 293.787 & 295.566 & 432.742 & 432.116 & 0.158 & 0.155 & 138.955 & 136.549 & 0.220 & 3.371 \\ 
TCP & 3.067 & 105 & 106 & 3.054 & 3.419 & 3.395 & 3.925 & 3.863 & 3.506 & 3.475 & 0.452 & 0.421 & 0.365 & 0.341 & 0.419 & 0.388 & 315.851 & 320.953 & 353.642 & 356.811 & 0.325 & 0.274 & 37.791 & 35.858 & 0.458 & 1.995 \\ 
CDBP-BP-PXZ & 1.575 & 147 & 148 & 2.173 & 2.768 & 2.737 & 3.135 & 3.098 & 2.461 & 2.459 & 0.288 & 0.286 & 0.595 & 0.564 & 0.674 & 0.638 & 395.534 & 400.259 & 503.828 & 504.136 & 0.024 & 0.018 & 108.294 & 103.877 & 0.252 & 6.243 \\ 
CDBP-BP-DMAC & 1.602 & 153 & 154 & 2.232 & 3.251 & 3.226 & 3.599 & 3.594 & 2.471 & 2.487 & 0.239 & 0.255 & 1.018 & 0.994 & 1.127 & 1.107 & 344.535 & 344.956 & 501.735 & 498.563 & 0.184 & 0.197 & 157.201 & 153.607 & 0.149 & 6.338 \\ 
3CzPhpPM & 2.145 & 101 & 102 & 2.216 & 3.411 & 3.389 & 3.820 & 3.757 & 2.482 & 2.457 & 0.266 & 0.241 & 1.195 & 1.173 & 1.338 & 1.300 & 324.566 & 330.009 & 499.569 & 504.699 & 0.430 & 0.339 & 175.003 & 174.691 & 0.302 & 7.404 \\ 
SFI23pPM & 2.149 & 130 & 131 & 2.204 & 3.418 & 3.395 & 3.821 & 3.765 & 2.464 & 2.445 & 0.260 & 0.241 & 1.214 & 1.190 & 1.357 & 1.320 & 324.456 & 329.264 & 503.099 & 507.074 & 0.278 & 0.222 & 178.643 & 177.810 & 0.286 & 7.681 \\ 
3PCzPFP & 2.190 & 75 & 76 & 2.715 & 3.368 & 3.345 & 3.816 & 3.741 & 3.076 & 3.037 & 0.361 & 0.322 & 0.653 & 0.630 & 0.740 & 0.704 & 324.949 & 331.385 & 403.094 & 408.258 & 0.149 & 0.124 & 78.146 & 76.874 & 0.171 & 7.544 \\ 
SFI34pPM & 2.084 & 130 & 131 & 2.187 & 3.385 & 3.364 & 3.751 & 3.694 & 2.423 & 2.401 & 0.236 & 0.214 & 1.199 & 1.177 & 1.328 & 1.293 & 330.545 & 335.655 & 511.766 & 516.392 & 0.340 & 0.275 & 181.221 & 180.737 & 0.284 & 7.791 \\ 
SBA-2DPS & 2.223 & 138 & 139 & 2.547 & 3.448 & 3.418 & 3.939 & 3.930 & 2.910 & 2.929 & 0.363 & 0.382 & 0.901 & 0.871 & 1.029 & 1.002 & 314.745 & 315.441 & 426.062 & 423.340 & 0.115 & 0.070 & 111.318 & 107.898 & 0.171 & 7.211 \\ 
2DMAC-BP-F & 1.405 & 132 & 133 & 1.227 & 2.386 & 2.355 & 3.004 & 2.929 & 1.545 & 1.526 & 0.318 & 0.299 & 1.159 & 1.128 & 1.459 & 1.403 & 412.744 & 423.342 & 802.533 & 812.479 & 0.932 & 0.779 & 389.788 & 389.137 & 0.546 & 0.232 \\ 
DCA & 2.092 & 77 & 78 & 1.853 & 2.260 & 2.189 & 3.285 & 3.106 & 2.693 & 2.629 & 0.840 & 0.776 & 0.407 & 0.336 & 0.592 & 0.477 & 377.448 & 399.176 & 460.396 & 471.604 & 0.448 & 0.321 & 82.947 & 72.427 & 0.152 & 1.697 \\ 
DPFPhe & 2.333 & 113 & 114 & 2.095 & 2.476 & 2.427 & 3.173 & 3.095 & 2.684 & 2.671 & 0.589 & 0.576 & 0.381 & 0.332 & 0.488 & 0.424 & 390.785 & 400.634 & 461.888 & 464.178 & 0.192 & 0.144 & 71.104 & 63.544 & 0.156 & 6.889 \\ 
DFPFPhe & 2.158 & 119 & 120 & 2.069 & 2.505 & 2.464 & 3.160 & 3.086 & 2.610 & 2.592 & 0.541 & 0.522 & 0.436 & 0.395 & 0.550 & 0.495 & 392.318 & 401.724 & 474.950 & 478.398 & 0.138 & 0.106 & 82.632 & 76.674 & 0.060 & 6.515 \\ 
3ai & 2.157 & 98 & 99 & 1.995 & 2.518 & 2.460 & 3.593 & 3.408 & 2.848 & 2.764 & 0.852 & 0.769 & 0.522 & 0.465 & 0.745 & 0.644 & 345.072 & 363.782 & 435.412 & 448.556 & 0.799 & 0.546 & 90.340 & 84.774 & 0.244 & 7.537 \\ 
DNFPh & 2.124 & 131 & 132 & 1.960 & 2.192 & 2.139 & 2.957 & 2.879 & 2.644 & 2.637 & 0.684 & 0.678 & 0.232 & 0.179 & 0.313 & 0.241 & 419.248 & 430.695 & 468.937 & 470.113 & 0.126 & 0.084 & 49.689 & 39.418 & 0.104 & 5.903 \\ 
pCzAnBzt & 2.014 & 95 & 96 & 1.805 & 2.278 & 2.208 & 3.293 & 3.130 & 2.609 & 2.559 & 0.804 & 0.754 & 0.473 & 0.403 & 0.684 & 0.571 & 376.554 & 396.103 & 475.253 & 484.498 & 0.652 & 0.463 & 98.699 & 88.395 & 0.544 & 6.115 \\ 
DPE-DPXZ & 1.920 & 99 & 100 & 2.200 & 2.839 & 2.807 & 3.226 & 3.188 & 2.500 & 2.499 & 0.300 & 0.299 & 0.639 & 0.607 & 0.726 & 0.689 & 384.376 & 388.848 & 495.919 & 496.087 & 0.003 & 0.003 & 111.543 & 107.239 & 0.349 & 0.312 \\ 
3CzAnBzt & 2.018 & 95 & 96 & 1.798 & 2.253 & 2.183 & 3.258 & 3.108 & 2.601 & 2.561 & 0.803 & 0.762 & 0.455 & 0.384 & 0.657 & 0.547 & 380.506 & 398.958 & 476.695 & 484.193 & 0.709 & 0.513 & 96.189 & 85.235 & 0.715 & 3.456 \\ 
TABD-COOH & 2.129 & 83 & 84 & 1.478 & 2.635 & 2.591 & 3.346 & 3.293 & 1.877 & 1.879 & 0.399 & 0.401 & 1.157 & 1.113 & 1.469 & 1.415 & 370.522 & 376.474 & 660.558 & 659.934 & 0.575 & 0.483 & 290.036 & 283.460 & 0.734 & 1.950 \\ 
ADN & 2.127 & 79 & 80 & 1.860 & 2.258 & 2.186 & 3.252 & 3.083 & 2.678 & 2.622 & 0.819 & 0.762 & 0.398 & 0.326 & 0.573 & 0.460 & 381.267 & 402.220 & 462.899 & 472.831 & 0.596 & 0.421 & 81.632 & 70.611 & 0.933 & 0.026 \\ 
Et3SiH & 2.847 & 164 & 165 & 2.298 & 3.408 & 3.376 & 4.170 & 4.122 & 2.812 & 2.806 & 0.514 & 0.508 & 1.110 & 1.078 & 1.359 & 1.316 & 297.296 & 300.750 & 440.952 & 441.848 & 0.407 & 0.358 & 143.656 & 141.098 & 0.666 & 0.758 \\ 
DPE-DDMAc & 2.012 & 111 & 112 & 2.327 & 3.388 & 3.357 & 3.793 & 3.789 & 2.605 & 2.627 & 0.278 & 0.300 & 1.061 & 1.030 & 1.188 & 1.162 & 326.868 & 327.178 & 475.876 & 471.914 & 0.234 & 0.234 & 149.008 & 144.735 & 0.213 & 0.533 \\ 
mCz-TAn-CN & 2.080 & 119 & 120 & 1.811 & 2.325 & 2.259 & 3.290 & 3.140 & 2.563 & 2.517 & 0.751 & 0.706 & 0.514 & 0.448 & 0.727 & 0.623 & 376.840 & 394.892 & 483.808 & 492.594 & 0.523 & 0.380 & 106.968 & 97.703 & 0.799 & 1.938 \\ 
indenoacridine & 1.177 & 49 & 50 & 1.221 & 1.053 & 0.918 & 2.157 & 1.938 & 2.503 & 2.578 & 1.281 & 1.356 & -0.169 & -0.303 & -0.346 & -0.640 & 574.826 & 639.786 & 495.431 & 481.019 & 0.557 & 0.365 & -79.395 & -158.768 & 0.801 & 1.680 \\ 
MPAc & 3.339 & 68 & 69 & 3.104 & 3.762 & 3.744 & 4.251 & 4.186 & 3.508 & 3.470 & 0.404 & 0.366 & 0.658 & 0.641 & 0.743 & 0.716 & 291.631 & 296.202 & 353.429 & 357.327 & 0.089 & 0.075 & 61.798 & 61.125 & 0.483 & 2.087 \\ 
TBAc & 2.806 & 126 & 127 & 1.411 & 3.098 & 3.047 & 3.834 & 3.779 & 1.746 & 1.750 & 0.335 & 0.339 & 1.687 & 1.636 & 2.088 & 2.029 & 323.364 & 328.070 & 710.162 & 708.567 & 0.023 & 0.036 & 386.798 & 380.497 & 0.477 & 0.882 \\ 
poCz-SO & 3.316 & 99 & 100 & 3.280 & 3.538 & 3.513 & 3.968 & 3.893 & 3.680 & 3.635 & 0.399 & 0.355 & 0.257 & 0.233 & 0.288 & 0.258 & 312.452 & 318.480 & 336.943 & 341.084 & 0.059 & 0.050 & 24.491 & 22.604 & 0.680 & 0.377 \\ 
H4TCPE & 3.245 & 95 & 96 & 2.684 & 4.248 & 4.215 & 4.704 & 4.666 & 2.972 & 2.972 & 0.288 & 0.287 & 1.564 & 1.530 & 1.731 & 1.694 & 263.583 & 265.724 & 417.128 & 417.229 & 0.015 & 0.014 & 153.545 & 151.505 & 0.564 & 2.960 \\ 
CbBPCb & 2.969 & 89 & 90 & 2.982 & 3.445 & 3.424 & 3.917 & 3.848 & 3.389 & 3.351 & 0.408 & 0.370 & 0.464 & 0.442 & 0.527 & 0.497 & 316.569 & 322.188 & 365.807 & 369.944 & 0.134 & 0.115 & 49.238 & 47.757 & 0.217 & 6.867 \\ 
TMOE & 2.541 & 86 & 87 & 1.772 & 2.947 & 2.909 & 3.715 & 3.655 & 2.233 & 2.226 & 0.462 & 0.454 & 1.176 & 1.138 & 1.482 & 1.429 & 333.704 & 339.246 & 555.171 & 557.095 & 0.737 & 0.609 & 221.467 & 217.849 & 0.899 & 0.027 \\ 
FAPbCl3 & 3.494 & 71 & 72 & 2.949 & 4.223 & 4.182 & 4.599 & 4.577 & 3.211 & 3.227 & 0.262 & 0.278 & 1.274 & 1.233 & 1.387 & 1.350 & 269.601 & 270.897 & 386.084 & 384.192 & 0.000 & 0.000 & 116.482 & 113.295 & 0.896 & 0.083 \\ 
DBT-SADF & 1.750 & 97 & 98 & 2.448 & 3.455 & 3.427 & 3.646 & 3.636 & 2.583 & 2.598 & 0.135 & 0.150 & 1.007 & 0.979 & 1.063 & 1.038 & 340.102 & 340.963 & 480.005 & 477.250 & 0.021 & 0.020 & 139.903 & 136.287 & 0.205 & 5.244 \\ 
mPXTMP & 2.762 & 84 & 85 & 2.661 & 3.485 & 3.457 & 3.902 & 3.867 & 2.979 & 2.976 & 0.318 & 0.316 & 0.824 & 0.796 & 0.923 & 0.890 & 317.745 & 320.646 & 416.198 & 416.575 & 0.002 & 0.002 & 98.453 & 95.929 & 0.673 & 0.903 \\ 
APDC-tPh & 1.510 & 87 & 88 & 1.534 & 2.595 & 2.550 & 3.190 & 3.151 & 1.886 & 1.896 & 0.352 & 0.362 & 1.061 & 1.016 & 1.304 & 1.255 & 388.702 & 393.476 & 657.412 & 653.970 & 0.100 & 0.119 & 268.711 & 260.494 & 0.254 & 6.383 \\ 
POZDBPHZ & 0.996 & 117 & 118 & 1.259 & 2.880 & 2.850 & 3.076 & 3.064 & 1.344 & 1.353 & 0.086 & 0.095 & 1.621 & 1.591 & 1.731 & 1.710 & 403.122 & 404.701 & 922.341 & 916.275 & 0.449 & 0.422 & 519.219 & 511.574 & 0.242 & 3.729 \\ 
CPTBF & 3.047 & 143 & 144 & 2.957 & 3.402 & 3.379 & 3.900 & 3.833 & 3.390 & 3.354 & 0.433 & 0.397 & 0.445 & 0.422 & 0.510 & 0.479 & 317.892 & 323.457 & 365.734 & 369.609 & 0.256 & 0.217 & 47.842 & 46.152 & 0.364 & 4.552 \\ 
trimesitylboron & 2.743 & 72 & 73 & 2.743 & 3.724 & 3.705 & 4.044 & 4.026 & 2.978 & 2.980 & 0.236 & 0.238 & 0.981 & 0.962 & 1.065 & 1.046 & 306.603 & 307.951 & 416.267 & 415.997 & 0.183 & 0.165 & 109.664 & 108.046 & 0.635 & 0.694 \\ 
CMP & 4.138 & 60 & 61 & 3.112 & 4.899 & 4.858 & 5.074 & 5.044 & 3.223 & 3.232 & 0.111 & 0.120 & 1.787 & 1.745 & 1.850 & 1.812 & 244.376 & 245.786 & 384.667 & 383.616 & 0.002 & 0.002 & 140.291 & 137.831 & 0.833 & 0.384 \\ 
CH3OH–CHCl3 & 2.310 & 85 & 86 & 2.049 & 2.717 & 2.647 & 3.688 & 3.631 & 2.781 & 2.811 & 0.732 & 0.762 & 0.668 & 0.598 & 0.907 & 0.820 & 336.174 & 341.470 & 445.769 & 441.061 & 0.015 & 0.511 & 109.595 & 99.591 & 0.938 & 0.173 \\ 
s-triazine & 3.730 & 68 & 69 & 3.371 & 4.977 & 4.936 & 5.028 & 4.998 & 3.406 & 3.414 & 0.034 & 0.043 & 1.606 & 1.564 & 1.622 & 1.584 & 246.592 & 248.058 & 364.050 & 363.160 & 0.004 & 0.004 & 117.458 & 115.102 & 0.571 & 1.431 \\ 
{[BMIM][PF6]} & 3.287 & 70 & 71 & 2.969 & 3.800 & 3.761 & 4.562 & 4.504 & 3.565 & 3.556 & 0.596 & 0.586 & 0.830 & 0.792 & 0.997 & 0.948 & 271.758 & 275.288 & 347.754 & 348.702 & 0.300 & 0.324 & 75.996 & 73.414 & 0.855 & 0.353 \\ 
1SBFN & 2.878 & 81 & 82 & 2.458 & 3.339 & 3.287 & 4.217 & 4.145 & 3.105 & 3.099 & 0.646 & 0.641 & 0.880 & 0.829 & 1.112 & 1.045 & 294.024 & 299.132 & 399.334 & 400.017 & 0.918 & 0.750 & 105.310 & 100.885 & 0.914 & 0.360 \\ 
2SBFN & 2.865 & 81 & 82 & 2.536 & 3.388 & 3.335 & 4.200 & 4.163 & 3.143 & 3.165 & 0.607 & 0.629 & 0.852 & 0.799 & 1.056 & 0.998 & 295.215 & 297.803 & 394.421 & 391.678 & 0.091 & 0.148 & 99.206 & 93.875 & 0.905 & 0.915 \\ 
F2PA & 2.512 & 90 & 91 & 2.508 & 3.056 & 3.027 & 3.544 & 3.512 & 2.908 & 2.909 & 0.400 & 0.401 & 0.548 & 0.519 & 0.635 & 0.603 & 349.882 & 353.070 & 426.337 & 426.209 & 1.101 & 0.967 & 76.455 & 73.139 & 0.628 & 1.908 \\ 
TSBFB & 3.015 & 186 & 187 & 2.694 & 3.729 & 3.691 & 4.456 & 4.419 & 3.220 & 3.225 & 0.526 & 0.531 & 1.035 & 0.997 & 1.237 & 1.194 & 278.222 & 280.564 & 385.073 & 384.409 & 1.477 & 1.309 & 106.851 & 103.845 & 0.846 & 1.293 \\ 
DPPP & 2.161 & 149 & 150 & 1.921 & 2.615 & 2.550 & 3.469 & 3.361 & 2.548 & 2.533 & 0.627 & 0.611 & 0.694 & 0.629 & 0.921 & 0.829 & 357.447 & 368.847 & 486.585 & 489.548 & 0.685 & 0.544 & 129.138 & 120.701 & 0.916 & 0.014 \\ 
TPA-NZP & 0.995 & 90 & 91 & 1.196 & 1.852 & 1.768 & 2.837 & 2.681 & 1.831 & 1.813 & 0.635 & 0.618 & 0.657 & 0.572 & 1.006 & 0.868 & 437.072 & 462.438 & 677.211 & 683.752 & 1.054 & 0.737 & 240.139 & 221.314 & 0.426 & 5.825 \\ 
mTPA-PPI & 2.406 & 113 & 114 & 2.521 & 3.383 & 3.357 & 3.748 & 3.710 & 2.793 & 2.786 & 0.272 & 0.265 & 0.862 & 0.836 & 0.955 & 0.924 & 330.792 & 334.207 & 443.850 & 445.039 & 0.561 & 0.476 & 113.058 & 110.831 & 0.214 & 8.830 \\ 
BSBFB & 3.042 & 129 & 130 & 2.703 & 3.700 & 3.663 & 4.503 & 4.461 & 3.290 & 3.292 & 0.586 & 0.589 & 0.997 & 0.960 & 1.213 & 1.169 & 275.367 & 277.904 & 376.880 & 376.590 & 1.412 & 1.216 & 101.513 & 98.685 & 0.884 & 0.895 \\ 
BN-DBC-Ph2 & 1.129 & 88 & 89 & 1.279 & 1.844 & 1.806 & 2.450 & 2.382 & 1.700 & 1.687 & 0.420 & 0.408 & 0.565 & 0.527 & 0.750 & 0.695 & 506.079 & 520.548 & 729.519 & 735.034 & 0.301 & 0.269 & 223.440 & 214.486 & 0.534 & 4.168 \\ 
TCbTrz & 1.853 & 147 & 148 & 2.106 & 3.315 & 3.291 & 3.811 & 3.762 & 2.420 & 2.407 & 0.315 & 0.301 & 1.210 & 1.186 & 1.390 & 1.355 & 325.358 & 329.605 & 512.248 & 515.193 & 0.288 & 0.246 & 186.890 & 185.588 & 0.128 & 6.930 \\ 
Xm-mCP & 1.890 & 110 & 111 & 2.466 & 3.286 & 3.259 & 3.805 & 3.803 & 2.856 & 2.878 & 0.389 & 0.412 & 0.820 & 0.793 & 0.949 & 0.925 & 325.845 & 326.034 & 434.177 & 430.819 & 0.002 & 0.004 & 108.331 & 104.785 & 0.031 & 7.839 \\ 
Xp-mCP & 1.878 & 110 & 111 & 2.329 & 3.297 & 3.268 & 3.877 & 3.833 & 2.738 & 2.731 & 0.410 & 0.402 & 0.968 & 0.940 & 1.139 & 1.102 & 319.794 & 323.465 & 452.762 & 454.028 & 0.007 & 0.179 & 132.968 & 130.563 & 0.122 & 7.859 \\ 
ethylacetate & 2.417 & 108 & 109 & 2.195 & 3.159 & 3.139 & 3.331 & 3.321 & 2.315 & 2.323 & 0.119 & 0.128 & 0.964 & 0.943 & 1.016 & 0.998 & 372.258 & 373.300 & 535.648 & 533.730 & 0.009 & 0.008 & 163.390 & 160.429 & 0.260 & 6.470 \\ 
3DMACIPN & 1.225 & 143 & 144 & 1.527 & 2.568 & 2.559 & 2.771 & 2.754 & 1.648 & 1.644 & 0.121 & 0.117 & 1.041 & 1.031 & 1.123 & 1.110 & 447.419 & 450.180 & 752.327 & 754.142 & 0.110 & 0.098 & 304.909 & 303.961 & 0.274 & 2.429 \\ 
ICZ & 2.627 & 62 & 63 & 2.666 & 2.777 & 2.745 & 3.343 & 3.234 & 3.210 & 3.141 & 0.544 & 0.475 & 0.110 & 0.079 & 0.133 & 0.093 & 370.910 & 383.377 & 386.272 & 394.769 & 0.118 & 0.091 & 15.362 & 11.392 & 0.692 & 0.045 \\ 
BDAVBi & 2.070 & 129 & 130 & 1.697 & 2.829 & 2.786 & 3.480 & 3.450 & 2.087 & 2.101 & 0.391 & 0.404 & 1.132 & 1.089 & 1.393 & 1.349 & 356.266 & 359.385 & 593.964 & 590.035 & 2.144 & 1.992 & 237.698 & 230.650 & 0.628 & 2.363 \\ 
DPVBi & 2.499 & 95 & 96 & 1.988 & 3.172 & 3.131 & 3.816 & 3.786 & 2.391 & 2.403 & 0.403 & 0.416 & 1.185 & 1.143 & 1.425 & 1.382 & 324.898 & 327.507 & 518.557 & 515.884 & 2.267 & 2.014 & 193.660 & 188.377 & 0.903 & 0.016 \\ 
CBTD2 & 1.198 & 158 & 159 & 1.542 & 2.794 & 2.743 & 3.507 & 3.446 & 1.935 & 1.937 & 0.393 & 0.395 & 1.253 & 1.202 & 1.572 & 1.509 & 353.523 & 359.813 & 640.726 & 640.223 & 2.261 & 1.920 & 287.203 & 280.410 & 0.317 & 1.914 \\ 
MeOCzPCN & 1.955 & 103 & 104 & 2.225 & 2.823 & 2.800 & 3.451 & 3.388 & 2.721 & 2.693 & 0.495 & 0.467 & 0.597 & 0.575 & 0.730 & 0.696 & 359.270 & 365.908 & 455.682 & 460.434 & 0.023 & 0.018 & 96.411 & 94.526 & 0.478 & 1.121 \\ 
Na-DMAC & 1.086 & 122 & 123 & 1.793 & 3.102 & 3.058 & 3.538 & 3.531 & 2.046 & 2.071 & 0.252 & 0.278 & 1.308 & 1.264 & 1.493 & 1.460 & 350.416 & 351.081 & 606.072 & 598.628 & 0.310 & 0.300 & 255.656 & 247.547 & 0.053 & 8.245 \\ 
3Py-DMAC & 1.334 & 104 & 105 & 1.623 & 2.662 & 2.636 & 3.165 & 3.117 & 1.930 & 1.920 & 0.307 & 0.296 & 1.038 & 1.013 & 1.234 & 1.197 & 391.772 & 397.755 & 642.314 & 645.874 & 1.128 & 0.984 & 250.541 & 248.119 & 0.178 & 6.638 \\ 
6tBPA & 1.645 & 167 & 168 & 1.603 & 1.845 & 1.788 & 2.389 & 2.311 & 2.076 & 2.072 & 0.473 & 0.469 & 0.242 & 0.185 & 0.313 & 0.239 & 519.088 & 536.449 & 597.299 & 598.370 & 0.455 & 0.371 & 78.211 & 61.921 & 0.694 & 0.015 \\ 
C-O & 2.918 & 100 & 101 & 2.889 & 3.114 & 3.089 & 3.703 & 3.618 & 3.435 & 3.384 & 0.546 & 0.495 & 0.225 & 0.200 & 0.268 & 0.234 & 334.839 & 342.649 & 360.944 & 366.362 & 0.139 & 0.122 & 26.105 & 23.713 & 0.675 & 1.696 \\ 
IDFL-2DPA & 1.937 & 128 & 129 & 2.139 & 2.751 & 2.733 & 3.071 & 3.021 & 2.389 & 2.365 & 0.249 & 0.226 & 0.611 & 0.593 & 0.682 & 0.656 & 403.726 & 410.353 & 519.032 & 524.177 & 0.298 & 0.260 & 115.307 & 113.824 & 0.453 & 2.739 \\ 
ACRF & 1.528 & 83 & 84 & 2.200 & 3.276 & 3.276 & 3.277 & 3.276 & 2.200 & 2.200 & 0.000 & 0.000 & 1.077 & 1.076 & 1.077 & 1.076 & 378.381 & 378.427 & 563.548 & 563.514 & 0.000 & 0.000 & 185.167 & 185.086 & 0.133 & 3.752 \\ 
TPSi-F & 3.432 & 104 & 105 & 3.073 & 3.828 & 3.790 & 4.637 & 4.576 & 3.722 & 3.710 & 0.649 & 0.637 & 0.755 & 0.717 & 0.915 & 0.866 & 267.357 & 270.950 & 333.086 & 334.159 & 0.330 & 0.318 & 65.729 & 63.208 & 0.821 & 1.476 \\ 
PAB & 2.394 & 108 & 109 & 2.534 & 2.688 & 2.666 & 3.138 & 3.064 & 2.957 & 2.911 & 0.424 & 0.378 & 0.155 & 0.133 & 0.181 & 0.152 & 395.093 & 404.675 & 419.242 & 425.863 & 0.372 & 0.301 & 24.149 & 21.189 & 0.565 & 1.099 \\ 
2tPAB & 2.372 & 156 & 157 & 2.506 & 2.682 & 2.660 & 3.125 & 3.052 & 2.920 & 2.875 & 0.414 & 0.369 & 0.176 & 0.154 & 0.205 & 0.177 & 396.737 & 406.279 & 424.632 & 431.279 & 0.417 & 0.337 & 27.895 & 24.999 & 0.582 & 0.831 \\ 
pDTPA-DTPZ & 1.023 & 137 & 138 & 1.209 & 2.442 & 2.399 & 2.978 & 2.906 & 1.474 & 1.465 & 0.265 & 0.256 & 1.233 & 1.190 & 1.504 & 1.442 & 416.334 & 426.605 & 840.971 & 846.545 & 0.690 & 0.515 & 424.638 & 419.940 & 0.356 & 2.474 \\ 
oDTPA-DTPZ & 1.095 & 137 & 138 & 1.288 & 2.549 & 2.508 & 3.070 & 2.993 & 1.552 & 1.538 & 0.263 & 0.249 & 1.261 & 1.220 & 1.519 & 1.456 & 403.818 & 414.192 & 799.122 & 806.341 & 0.035 & 0.025 & 395.305 & 392.149 & 0.297 & 8.004 \\ 
oTPAPO-DTPZ & 0.939 & 126 & 127 & 1.248 & 2.510 & 2.469 & 3.021 & 2.942 & 1.502 & 1.488 & 0.254 & 0.239 & 1.262 & 1.221 & 1.519 & 1.455 & 410.408 & 421.385 & 825.241 & 833.441 & 0.050 & 0.037 & 414.833 & 412.056 & 0.226 & 8.847 \\ 
BPZPP & 1.232 & 145 & 146 & 1.283 & 2.636 & 2.611 & 2.950 & 2.923 & 1.436 & 1.437 & 0.153 & 0.153 & 1.353 & 1.328 & 1.514 & 1.486 & 420.257 & 424.182 & 863.177 & 863.075 & 0.173 & 0.152 & 442.920 & 438.893 & 0.385 & 6.727 \\ 
BIPOCz & 2.839 & 114 & 115 & 2.531 & 3.411 & 3.384 & 3.893 & 3.822 & 2.889 & 2.858 & 0.358 & 0.327 & 0.880 & 0.853 & 1.004 & 0.963 & 318.472 & 324.430 & 429.209 & 433.778 & 0.042 & 0.037 & 110.737 & 109.348 & 0.783 & 1.429 \\ 
tDPAC-BN & 2.368 & 186 & 187 & 2.494 & 2.651 & 2.628 & 3.124 & 3.048 & 2.939 & 2.893 & 0.445 & 0.399 & 0.157 & 0.134 & 0.185 & 0.155 & 396.826 & 406.772 & 421.814 & 428.554 & 0.433 & 0.348 & 24.988 & 21.782 & 0.597 & 0.971 \\ 
tDMAC-BN & 2.285 & 164 & 165 & 2.394 & 2.602 & 2.582 & 3.007 & 2.943 & 2.766 & 2.729 & 0.372 & 0.335 & 0.208 & 0.188 & 0.241 & 0.215 & 412.360 & 421.242 & 448.239 & 454.357 & 0.467 & 0.381 & 35.879 & 33.115 & 0.574 & 0.960 \\ 
2ICz-OXD & 1.867 & 161 & 162 & 2.206 & 3.371 & 3.347 & 3.796 & 3.744 & 2.484 & 2.468 & 0.278 & 0.262 & 1.165 & 1.141 & 1.311 & 1.276 & 326.661 & 331.137 & 499.121 & 502.312 & 0.312 & 0.290 & 172.460 & 171.176 & 0.209 & 7.554 \\ 
SIR-B & 1.391 & 126 & 127 & 2.013 & 3.083 & 3.082 & 3.086 & 3.085 & 2.014 & 2.014 & 0.002 & 0.002 & 1.071 & 1.070 & 1.071 & 1.071 & 401.803 & 401.894 & 615.539 & 615.479 & 0.001 & 0.000 & 213.737 & 213.586 & 0.151 & 4.184 \\ 
SIR-C & 1.404 & 154 & 155 & 2.025 & 3.111 & 3.110 & 3.110 & 3.110 & 2.025 & 2.025 & -0.001 & -0.000 & 1.086 & 1.085 & 1.085 & 1.085 & 398.650 & 398.676 & 612.349 & 612.251 & 0.001 & 0.001 & 213.699 & 213.575 & 0.153 & 4.201 \\ 
SIR-A & 1.394 & 98 & 99 & 2.056 & 3.131 & 3.130 & 3.131 & 3.130 & 2.056 & 2.056 & 0.000 & 0.000 & 1.075 & 1.074 & 1.075 & 1.074 & 396.014 & 396.078 & 603.031 & 603.012 & 0.000 & 0.000 & 207.017 & 206.934 & 0.150 & 4.352 \\ 
TRZ3DPA & 2.013 & 150 & 151 & 2.121 & 2.936 & 2.907 & 3.485 & 3.457 & 2.518 & 2.523 & 0.397 & 0.401 & 0.815 & 0.786 & 0.967 & 0.934 & 355.724 & 358.688 & 492.397 & 491.511 & 1.631 & 1.498 & 136.672 & 132.823 & 0.412 & 0.638 \\ 
BO3N & 1.761 & 117 & 118 & 1.688 & 2.046 & 1.968 & 2.989 & 2.901 & 2.467 & 2.489 & 0.778 & 0.800 & 0.358 & 0.280 & 0.523 & 0.413 & 414.760 & 427.325 & 502.630 & 498.217 & 0.141 & 0.084 & 87.870 & 70.892 & 0.391 & 4.927 \\ 
BPPyA & 1.810 & 143 & 144 & 1.749 & 2.231 & 2.175 & 2.767 & 2.707 & 2.169 & 2.177 & 0.420 & 0.428 & 0.482 & 0.426 & 0.598 & 0.530 & 448.163 & 457.979 & 571.628 & 569.540 & 1.031 & 0.864 & 123.466 & 111.560 & 0.770 & 0.105 \\ 
SiCN2Cz & 2.412 & 138 & 139 & 2.465 & 3.656 & 3.637 & 4.077 & 4.033 & 2.749 & 2.734 & 0.284 & 0.269 & 1.191 & 1.171 & 1.328 & 1.299 & 304.077 & 307.439 & 450.964 & 453.482 & 0.550 & 0.460 & 146.887 & 146.042 & 0.367 & 3.792 \\ 
PhPC & 2.109 & 91 & 92 & 1.869 & 2.255 & 2.183 & 3.308 & 3.141 & 2.743 & 2.690 & 0.873 & 0.821 & 0.385 & 0.313 & 0.565 & 0.451 & 374.812 & 394.741 & 452.080 & 460.913 & 0.602 & 0.423 & 77.267 & 66.172 & 0.848 & 1.693 \\ 
1MOBI & 1.935 & 107 & 108 & 1.709 & 2.389 & 2.337 & 3.141 & 3.063 & 2.247 & 2.240 & 0.538 & 0.530 & 0.680 & 0.628 & 0.894 & 0.823 & 394.741 & 404.807 & 551.829 & 553.562 & 2.527 & 2.038 & 157.088 & 148.755 & 0.820 & 0.010 \\ 
3BrBI & 2.006 & 101 & 102 & 1.751 & 2.747 & 2.692 & 3.502 & 3.459 & 2.232 & 2.251 & 0.481 & 0.499 & 0.996 & 0.940 & 1.269 & 1.208 & 354.069 & 358.450 & 555.374 & 550.887 & 3.885 & 3.403 & 201.305 & 192.437 & 0.795 & 0.183 \\ 
DMBFTX & 2.225 & 108 & 109 & 2.385 & 2.823 & 2.795 & 3.500 & 3.382 & 2.957 & 2.885 & 0.572 & 0.500 & 0.438 & 0.411 & 0.543 & 0.497 & 354.241 & 366.622 & 419.312 & 429.785 & 0.207 & 0.155 & 65.071 & 63.163 & 0.085 & 2.206 \\ 
SBF-AnCN & 2.057 & 108 & 109 & 1.803 & 2.248 & 2.179 & 3.178 & 3.022 & 2.549 & 2.500 & 0.745 & 0.697 & 0.445 & 0.376 & 0.629 & 0.522 & 390.170 & 410.272 & 486.493 & 495.858 & 0.684 & 0.491 & 96.323 & 85.586 & 0.878 & 1.062 \\ 
DMF-AnCN & 2.058 & 87 & 88 & 1.808 & 2.251 & 2.182 & 3.190 & 3.032 & 2.563 & 2.513 & 0.755 & 0.705 & 0.443 & 0.374 & 0.628 & 0.520 & 388.629 & 408.865 & 483.808 & 493.420 & 0.669 & 0.476 & 95.179 & 84.555 & 0.863 & 1.313 \\ 
DPF-AnCN & 2.042 & 109 & 110 & 1.803 & 2.241 & 2.172 & 3.167 & 3.013 & 2.548 & 2.501 & 0.745 & 0.698 & 0.438 & 0.369 & 0.619 & 0.512 & 391.537 & 411.511 & 486.607 & 495.681 & 0.702 & 0.503 & 95.070 & 84.170 & 0.872 & 1.171 \\ 
DPA & 2.158 & 61 & 62 & 1.902 & 2.258 & 2.184 & 3.317 & 3.131 & 2.794 & 2.726 & 0.892 & 0.824 & 0.356 & 0.282 & 0.523 & 0.405 & 373.795 & 395.989 & 443.696 & 454.760 & 0.399 & 0.284 & 69.901 & 58.770 & 0.937 & 0.000 \\ 
TPA–DAP–TPA & 1.836 & 191 & 192 & 1.729 & 2.300 & 2.233 & 3.206 & 3.111 & 2.410 & 2.409 & 0.681 & 0.680 & 0.571 & 0.504 & 0.796 & 0.702 & 386.713 & 398.522 & 514.418 & 514.593 & 2.129 & 1.610 & 127.704 & 116.071 & 0.286 & 11.358 \\ 
AcDbp & 0.957 & 129 & 130 & 1.255 & 3.141 & 3.116 & 3.186 & 3.184 & 1.272 & 1.282 & 0.018 & 0.028 & 1.887 & 1.861 & 1.913 & 1.902 & 389.202 & 389.373 & 974.461 & 967.006 & 0.025 & 0.026 & 585.259 & 577.633 & 0.178 & 3.618 \\ 
4-Ac & 3.063 & 90 & 91 & 2.820 & 3.252 & 3.220 & 3.945 & 3.884 & 3.421 & 3.401 & 0.601 & 0.581 & 0.433 & 0.400 & 0.525 & 0.482 & 314.258 & 319.251 & 362.471 & 364.517 & 0.021 & 0.017 & 48.213 & 45.266 & 0.690 & 1.507 \\ 
czpzpy & 2.583 & 57 & 58 & 2.573 & 3.105 & 3.078 & 3.631 & 3.555 & 3.008 & 2.972 & 0.435 & 0.399 & 0.533 & 0.505 & 0.623 & 0.584 & 341.507 & 348.740 & 412.210 & 417.226 & 0.371 & 0.303 & 70.702 & 68.486 & 0.509 & 2.817 \\ 
NyDPO & 1.202 & 118 & 119 & 1.510 & 2.859 & 2.829 & 3.227 & 3.210 & 1.705 & 1.714 & 0.195 & 0.204 & 1.349 & 1.318 & 1.523 & 1.496 & 384.161 & 386.232 & 727.376 & 723.470 & 0.958 & 0.029 & 343.215 & 337.238 & 0.217 & 0.257 \\ 
1MPA & 2.990 & 140 & 141 & 2.897 & 3.745 & 3.726 & 4.137 & 4.116 & 3.201 & 3.200 & 0.304 & 0.303 & 0.848 & 0.829 & 0.937 & 0.916 & 299.674 & 301.254 & 387.355 & 387.484 & 0.554 & 0.498 & 87.680 & 86.229 & 0.542 & 2.458 \\ 
LEt & 2.883 & 101 & 102 & 2.664 & 4.856 & 4.826 & 5.020 & 4.993 & 2.753 & 2.756 & 0.090 & 0.092 & 2.193 & 2.162 & 2.266 & 2.237 & 246.990 & 248.316 & 450.309 & 449.874 & 0.003 & 0.003 & 203.319 & 201.558 & 0.525 & 1.917 \\ 
DC-TC & 1.357 & 147 & 148 & 1.653 & 2.656 & 2.655 & 2.665 & 2.663 & 1.658 & 1.658 & 0.006 & 0.005 & 1.003 & 1.002 & 1.007 & 1.005 & 465.249 & 465.546 & 747.674 & 747.785 & 0.001 & 0.001 & 282.425 & 282.239 & 0.296 & 6.206 \\ 
DC-ACR & 1.084 & 117 & 118 & 1.347 & 2.851 & 2.839 & 2.928 & 2.927 & 1.383 & 1.388 & 0.037 & 0.041 & 1.504 & 1.493 & 1.545 & 1.538 & 423.385 & 423.646 & 896.235 & 893.137 & 0.001 & 0.001 & 472.849 & 469.491 & 0.233 & 6.271 \\ 
1G-F1 & 2.902 & 75 & 76 & 2.691 & 4.336 & 4.289 & 5.152 & 5.124 & 3.198 & 3.215 & 0.507 & 0.524 & 1.645 & 1.597 & 1.955 & 1.909 & 240.634 & 241.982 & 387.711 & 385.621 & 0.000 & 0.000 & 147.078 & 143.639 & 0.459 & 2.130 \\ 
P–Cu–C & 2.899 & 91 & 92 & 2.435 & 4.399 & 4.362 & 4.939 & 4.921 & 2.734 & 2.746 & 0.299 & 0.312 & 1.964 & 1.927 & 2.205 & 2.174 & 251.041 & 251.970 & 453.560 & 451.449 & 0.000 & 0.001 & 202.519 & 199.480 & 0.404 & 1.991 \\ 
BPCP-2CPC & 1.293 & 233 & 234 & 2.036 & 2.933 & 2.915 & 3.253 & 3.227 & 2.259 & 2.254 & 0.223 & 0.218 & 0.896 & 0.878 & 0.994 & 0.973 & 381.115 & 384.221 & 548.882 & 549.978 & 0.206 & 0.182 & 167.768 & 165.757 & 0.023 & 16.401 \\ 
2H-Qz & 1.347 & 113 & 114 & 1.753 & 2.741 & 2.710 & 3.105 & 3.066 & 1.986 & 1.984 & 0.233 & 0.231 & 0.988 & 0.956 & 1.119 & 1.082 & 399.331 & 404.345 & 624.340 & 624.914 & 0.015 & 0.013 & 225.009 & 220.570 & 0.197 & 7.500 \\ 
PPINCN-Cz & 1.571 & 191 & 192 & 1.811 & 2.798 & 2.735 & 3.588 & 3.565 & 2.322 & 2.361 & 0.511 & 0.550 & 0.987 & 0.924 & 1.266 & 1.204 & 345.572 & 347.782 & 533.899 & 525.234 & 0.248 & 0.286 & 188.327 & 177.452 & 0.132 & 11.852 \\ 
PPINCN & 1.720 & 103 & 104 & 1.837 & 2.721 & 2.655 & 3.597 & 3.537 & 2.429 & 2.447 & 0.592 & 0.611 & 0.884 & 0.818 & 1.169 & 1.089 & 344.659 & 350.545 & 510.538 & 506.585 & 0.873 & 0.797 & 165.879 & 156.040 & 0.189 & 4.545 \\ 
BDAPM & 2.265 & 156 & 157 & 2.427 & 2.943 & 2.914 & 3.379 & 3.347 & 2.786 & 2.787 & 0.359 & 0.360 & 0.517 & 0.488 & 0.593 & 0.560 & 366.893 & 370.478 & 444.994 & 444.900 & 1.169 & 1.058 & 78.101 & 74.422 & 0.503 & 1.710 \\ 
12AcCz-PM & 2.123 & 126 & 127 & 2.218 & 3.082 & 3.054 & 3.557 & 3.523 & 2.559 & 2.558 & 0.342 & 0.341 & 0.865 & 0.837 & 0.998 & 0.965 & 348.574 & 351.898 & 484.469 & 484.646 & 1.086 & 0.984 & 135.896 & 132.748 & 0.407 & 5.933 \\ 
23AcCz-PM & 1.622 & 126 & 127 & 2.017 & 3.198 & 3.170 & 3.601 & 3.586 & 2.271 & 2.281 & 0.254 & 0.265 & 1.181 & 1.153 & 1.330 & 1.304 & 344.305 & 345.793 & 545.941 & 543.482 & 0.267 & 0.276 & 201.636 & 197.689 & 0.143 & 7.498 \\ 
CDDPI & 2.301 & 118 & 119 & 2.157 & 3.045 & 3.008 & 3.513 & 3.480 & 2.488 & 2.496 & 0.331 & 0.339 & 0.888 & 0.851 & 1.025 & 0.985 & 352.930 & 356.235 & 498.302 & 496.776 & 0.626 & 0.565 & 145.373 & 140.541 & 0.532 & 1.965 \\ 
DDBP & 2.143 & 134 & 135 & 2.085 & 3.174 & 3.130 & 3.728 & 3.699 & 2.449 & 2.463 & 0.365 & 0.378 & 1.089 & 1.046 & 1.279 & 1.235 & 332.540 & 335.210 & 506.176 & 503.310 & 1.408 & 1.269 & 173.636 & 168.100 & 0.389 & 6.383 \\ 
CCDD & 1.340 & 126 & 127 & 1.968 & 2.856 & 2.836 & 3.303 & 3.230 & 2.276 & 2.241 & 0.308 & 0.273 & 0.888 & 0.868 & 1.027 & 0.988 & 375.425 & 383.900 & 544.847 & 553.205 & 0.312 & 0.239 & 169.422 & 169.305 & 0.254 & 8.300 \\ 
DPNC & 1.812 & 140 & 141 & 2.256 & 2.717 & 2.696 & 3.178 & 3.100 & 2.640 & 2.595 & 0.383 & 0.339 & 0.460 & 0.439 & 0.539 & 0.505 & 390.121 & 399.910 & 469.717 & 477.764 & 0.084 & 0.065 & 79.596 & 77.854 & 0.228 & 6.223 \\ 
LiPr & 2.895 & 113 & 114 & 2.765 & 4.822 & 4.793 & 4.994 & 4.966 & 2.864 & 2.866 & 0.099 & 0.100 & 2.057 & 2.027 & 2.130 & 2.101 & 248.266 & 249.651 & 432.891 & 432.651 & 0.003 & 0.003 & 184.624 & 183.000 & 0.523 & 1.917 \\ 
Spiro-CN & 1.155 & 140 & 141 & 1.799 & 2.941 & 2.910 & 3.382 & 3.358 & 2.068 & 2.076 & 0.270 & 0.277 & 1.143 & 1.111 & 1.314 & 1.283 & 366.579 & 369.209 & 599.425 & 597.344 & 1.580 & 1.460 & 232.847 & 228.134 & 0.050 & 3.232 \\ 
TMDBP & 3.217 & 65 & 66 & 3.124 & 3.358 & 3.322 & 3.953 & 3.907 & 3.677 & 3.674 & 0.553 & 0.549 & 0.234 & 0.198 & 0.276 & 0.233 & 313.670 & 317.371 & 337.173 & 337.495 & 0.190 & 0.233 & 23.504 & 20.124 & 0.751 & 0.569 \\ 
ACRSA & 1.588 & 80 & 81 & 2.170 & 3.244 & 3.243 & 3.243 & 3.243 & 2.170 & 2.170 & -0.000 & 0.000 & 1.073 & 1.073 & 1.073 & 1.073 & 382.266 & 382.325 & 571.314 & 571.296 & 0.000 & 0.000 & 189.047 & 188.971 & 0.163 & 4.360 \\ 
CAPI & 1.959 & 139 & 140 & 1.816 & 2.196 & 2.129 & 2.938 & 2.873 & 2.430 & 2.450 & 0.614 & 0.634 & 0.380 & 0.313 & 0.508 & 0.423 & 421.988 & 431.550 & 510.281 & 506.018 & 0.415 & 0.397 & 88.294 & 74.468 & 0.662 & 2.251 \\ 
PhCzSPOTz & 2.326 & 93 & 94 & 2.362 & 3.608 & 3.589 & 4.019 & 3.963 & 2.631 & 2.608 & 0.269 & 0.246 & 1.246 & 1.227 & 1.388 & 1.355 & 308.472 & 312.870 & 471.234 & 475.397 & 0.384 & 0.340 & 162.762 & 162.527 & 0.490 & 1.533 \\ 
CCAPI & 1.519 & 143 & 144 & 1.745 & 2.198 & 2.133 & 2.931 & 2.862 & 2.327 & 2.341 & 0.582 & 0.596 & 0.453 & 0.388 & 0.604 & 0.520 & 422.952 & 433.254 & 532.734 & 529.573 & 0.455 & 0.416 & 109.781 & 96.320 & 0.048 & 9.833 \\ 
2CzCbPy & 2.355 & 105 & 106 & 2.630 & 3.246 & 3.224 & 3.703 & 3.640 & 3.001 & 2.970 & 0.371 & 0.340 & 0.616 & 0.594 & 0.702 & 0.670 & 334.794 & 340.569 & 413.157 & 417.435 & 0.332 & 0.266 & 78.363 & 76.866 & 0.343 & 5.284 \\ 
CzCbPy & 2.434 & 75 & 76 & 2.665 & 3.242 & 3.220 & 3.736 & 3.663 & 3.070 & 3.032 & 0.405 & 0.367 & 0.577 & 0.554 & 0.665 & 0.631 & 331.908 & 338.449 & 403.801 & 408.864 & 0.234 & 0.186 & 71.893 & 70.415 & 0.356 & 5.246 \\ 
DCE & 5.023 & 80 & 81 & 3.589 & 5.220 & 5.178 & 5.988 & 5.985 & 4.117 & 4.149 & 0.528 & 0.560 & 1.631 & 1.589 & 1.871 & 1.836 & 207.041 & 207.144 & 301.121 & 298.830 & 0.013 & 0.014 & 94.080 & 91.686 & 0.887 & 0.213 \\ 
PICFOCz & 2.227 & 125 & 126 & 2.427 & 3.361 & 3.330 & 3.783 & 3.712 & 2.732 & 2.705 & 0.305 & 0.278 & 0.934 & 0.904 & 1.051 & 1.007 & 327.749 & 333.982 & 453.882 & 458.358 & 0.214 & 0.096 & 126.133 & 124.375 & 0.016 & 6.884 \\ 
dpmt & 2.870 & 81 & 82 & 2.582 & 4.041 & 3.995 & 5.090 & 5.061 & 3.253 & 3.271 & 0.670 & 0.689 & 1.459 & 1.413 & 1.838 & 1.790 & 243.565 & 244.980 & 381.195 & 379.036 & 0.001 & 0.002 & 137.630 & 134.056 & 0.530 & 1.700 \\ 
BICFOCz & 2.287 & 126 & 127 & 2.430 & 3.429 & 3.406 & 3.887 & 3.816 & 2.754 & 2.723 & 0.324 & 0.293 & 0.999 & 0.975 & 1.132 & 1.093 & 319.004 & 324.898 & 450.163 & 455.284 & 0.076 & 0.062 & 131.158 & 130.386 & 0.013 & 7.377 \\ 
19a & 2.106 & 79 & 80 & 1.917 & 2.325 & 2.255 & 3.408 & 3.233 & 2.810 & 2.749 & 0.894 & 0.832 & 0.408 & 0.338 & 0.598 & 0.485 & 363.761 & 383.448 & 441.161 & 451.054 & 0.253 & 0.170 & 77.400 & 67.606 & 0.941 & 0.009 \\ 
BTPBFCz & 2.034 & 105 & 106 & 2.113 & 3.339 & 3.318 & 3.763 & 3.709 & 2.382 & 2.362 & 0.269 & 0.249 & 1.225 & 1.205 & 1.381 & 1.347 & 329.474 & 334.279 & 520.527 & 524.877 & 0.172 & 0.150 & 191.053 & 190.597 & 0.196 & 4.624 \\ 
Ph-OBNA & 2.435 & 79 & 80 & 2.646 & 3.074 & 3.054 & 3.466 & 3.414 & 2.984 & 2.958 & 0.338 & 0.312 & 0.427 & 0.408 & 0.482 & 0.457 & 357.716 & 363.153 & 415.508 & 419.217 & 0.168 & 0.141 & 57.793 & 56.063 & 0.542 & 3.079 \\ 
HPVAnt & 2.024 & 70 & 71 & 1.848 & 2.286 & 2.210 & 3.395 & 3.214 & 2.745 & 2.688 & 0.897 & 0.840 & 0.437 & 0.362 & 0.650 & 0.526 & 365.153 & 385.763 & 451.592 & 461.279 & 0.308 & 0.205 & 86.438 & 75.516 & 0.931 & 0.937 \\ 
BTPBFCz-D3 & 1.777 & 165 & 166 & 1.945 & 3.375 & 3.354 & 3.753 & 3.708 & 2.162 & 2.150 & 0.218 & 0.206 & 1.430 & 1.409 & 1.590 & 1.558 & 330.378 & 334.360 & 573.342 & 576.540 & 0.073 & 0.068 & 242.964 & 242.180 & 0.134 & 7.785 \\ 
ICBNTrz4 & 1.681 & 113 & 114 & 2.026 & 3.251 & 3.234 & 3.587 & 3.561 & 2.236 & 2.231 & 0.210 & 0.205 & 1.224 & 1.208 & 1.351 & 1.330 & 345.639 & 348.172 & 554.480 & 555.709 & 0.805 & 0.731 & 208.841 & 207.537 & 0.327 & 7.126 \\ 
1PCTRz & 1.636 & 131 & 132 & 2.103 & 3.345 & 3.321 & 3.808 & 3.745 & 2.394 & 2.371 & 0.291 & 0.268 & 1.242 & 1.218 & 1.414 & 1.374 & 325.563 & 331.039 & 517.852 & 522.816 & 0.366 & 0.251 & 192.289 & 191.777 & 0.172 & 10.039 \\ 
DMACN-B & 2.823 & 133 & 134 & 2.800 & 3.221 & 3.204 & 3.718 & 3.648 & 3.233 & 3.187 & 0.433 & 0.387 & 0.421 & 0.404 & 0.486 & 0.460 & 333.434 & 339.897 & 383.528 & 388.971 & 0.050 & 0.043 & 50.094 & 49.074 & 0.316 & 3.895 \\ 
CzSO-1CO & 2.160 & 100 & 101 & 2.285 & 2.852 & 2.810 & 3.703 & 3.603 & 2.966 & 2.930 & 0.681 & 0.645 & 0.568 & 0.525 & 0.737 & 0.673 & 334.821 & 344.104 & 418.046 & 423.190 & 0.332 & 0.264 & 83.225 & 79.085 & 0.095 & 3.517 \\ 
PPO21 & 3.028 & 113 & 114 & 3.035 & 3.389 & 3.366 & 3.816 & 3.744 & 3.418 & 3.376 & 0.383 & 0.341 & 0.354 & 0.331 & 0.398 & 0.368 & 324.906 & 331.172 & 362.775 & 367.284 & 0.188 & 0.161 & 37.869 & 36.112 & 0.535 & 2.953 \\ 
OXD-7 & 2.747 & 91 & 92 & 2.649 & 3.410 & 3.367 & 4.242 & 4.203 & 3.294 & 3.306 & 0.646 & 0.658 & 0.762 & 0.719 & 0.948 & 0.897 & 292.298 & 294.969 & 376.380 & 375.007 & 2.063 & 1.831 & 84.081 & 80.038 & 0.265 & 4.815 \\ 
TCZ1 & 2.717 & 115 & 116 & 2.793 & 3.157 & 3.134 & 3.632 & 3.557 & 3.213 & 3.169 & 0.421 & 0.377 & 0.364 & 0.341 & 0.419 & 0.387 & 341.319 & 348.613 & 385.859 & 391.196 & 0.049 & 0.039 & 44.540 & 42.583 & 0.489 & 1.520 \\ 
APPT & 1.544 & 64 & 65 & 1.643 & 2.913 & 2.862 & 3.319 & 3.289 & 1.872 & 1.888 & 0.229 & 0.245 & 1.270 & 1.219 & 1.447 & 1.401 & 373.514 & 376.955 & 662.261 & 656.684 & 0.009 & 0.007 & 288.747 & 279.730 & 0.347 & 2.172 \\ 
ANQDC & 1.386 & 54 & 55 & 1.497 & 2.863 & 2.812 & 3.402 & 3.400 & 1.779 & 1.810 & 0.282 & 0.313 & 1.366 & 1.315 & 1.623 & 1.590 & 364.488 & 364.649 & 697.069 & 684.857 & 0.006 & 0.006 & 332.581 & 320.208 & 0.500 & 0.685 \\ 
ECDPTT & 1.578 & 129 & 130 & 1.688 & 3.117 & 3.085 & 3.742 & 3.694 & 2.026 & 2.021 & 0.339 & 0.333 & 1.429 & 1.397 & 1.716 & 1.673 & 331.305 & 335.664 & 611.833 & 613.480 & 0.354 & 0.169 & 280.529 & 277.816 & 0.155 & 10.587 \\ 
1CM & 2.856 & 84 & 85 & 2.955 & 3.059 & 3.034 & 3.570 & 3.477 & 3.448 & 3.386 & 0.493 & 0.432 & 0.105 & 0.079 & 0.122 & 0.090 & 347.275 & 356.615 & 359.562 & 366.130 & 0.082 & 0.064 & 12.286 & 9.515 & 0.527 & 4.557 \\ 
NPE-AcDPS & 2.408 & 138 & 139 & 2.645 & 3.402 & 3.370 & 3.859 & 3.824 & 3.001 & 3.001 & 0.356 & 0.356 & 0.756 & 0.725 & 0.858 & 0.823 & 321.261 & 324.226 & 413.139 & 413.092 & 0.429 & 0.346 & 91.878 & 88.865 & 0.212 & 4.177 \\ 
DMAC-Cz & 2.303 & 109 & 110 & 2.783 & 3.357 & 3.325 & 3.913 & 3.840 & 3.244 & 3.214 & 0.461 & 0.431 & 0.574 & 0.542 & 0.669 & 0.626 & 316.828 & 322.876 & 382.151 & 385.746 & 0.064 & 0.055 & 65.324 & 62.870 & 0.146 & 2.589 \\ 
VBC-PTZ & 1.673 & 96 & 97 & 1.661 & 2.354 & 2.309 & 3.038 & 2.986 & 2.143 & 2.148 & 0.482 & 0.487 & 0.694 & 0.648 & 0.895 & 0.839 & 408.138 & 415.177 & 578.588 & 577.265 & 1.276 & 1.090 & 170.450 & 162.088 & 0.416 & 5.034 \\ 
t-BuPCz & 3.136 & 83 & 84 & 2.956 & 3.476 & 3.452 & 3.888 & 3.819 & 3.306 & 3.270 & 0.350 & 0.314 & 0.520 & 0.496 & 0.582 & 0.549 & 318.914 & 324.676 & 375.028 & 379.212 & 0.043 & 0.038 & 56.114 & 54.535 & 0.633 & 0.484 \\ 
4BPy-mDTC & 1.442 & 142 & 143 & 1.859 & 3.187 & 3.177 & 3.440 & 3.412 & 2.006 & 1.996 & 0.148 & 0.138 & 1.328 & 1.318 & 1.434 & 1.415 & 360.419 & 363.409 & 617.947 & 621.098 & 0.080 & 0.072 & 257.528 & 257.690 & 0.196 & 6.037 \\ 
DC–TC & 3.054 & 120 & 121 & 3.043 & 3.475 & 3.452 & 4.052 & 4.015 & 3.548 & 3.539 & 0.505 & 0.496 & 0.432 & 0.409 & 0.503 & 0.476 & 306.013 & 308.802 & 349.433 & 350.325 & 0.391 & 0.363 & 43.420 & 41.523 & 0.669 & 0.987 \\ 
DFDBQPXZ & 0.749 & 124 & 125 & 1.203 & 2.935 & 2.905 & 3.324 & 3.289 & 1.363 & 1.362 & 0.160 & 0.159 & 1.732 & 1.702 & 1.961 & 1.927 & 372.975 & 376.978 & 909.753 & 910.212 & 0.000 & 0.000 & 536.778 & 533.235 & 0.161 & 7.982 \\ 
DPE & 1.930 & 99 & 100 & 2.202 & 2.848 & 2.816 & 3.234 & 3.198 & 2.501 & 2.500 & 0.299 & 0.298 & 0.646 & 0.614 & 0.734 & 0.698 & 383.354 & 387.741 & 495.820 & 495.949 & 0.010 & 0.010 & 112.467 & 108.207 & 0.358 & 0.030 \\ 
CBZ & 1.549 & 111 & 112 & 2.323 & 3.689 & 3.655 & 3.949 & 3.916 & 2.487 & 2.489 & 0.164 & 0.166 & 1.366 & 1.331 & 1.462 & 1.426 & 313.995 & 316.625 & 498.564 & 498.066 & 0.161 & 0.138 & 184.569 & 181.440 & 0.047 & 7.439 \\ 
tBuCz2 & 2.583 & 139 & 140 & 2.763 & 3.259 & 3.236 & 3.716 & 3.649 & 3.151 & 3.115 & 0.388 & 0.352 & 0.496 & 0.474 & 0.566 & 0.534 & 333.614 & 339.804 & 393.499 & 398.082 & 0.042 & 0.034 & 59.885 & 58.278 & 0.402 & 2.287 \\ 
26DCzPPy & 2.460 & 103 & 104 & 2.698 & 3.410 & 3.387 & 3.869 & 3.808 & 3.062 & 3.033 & 0.364 & 0.335 & 0.712 & 0.689 & 0.808 & 0.775 & 320.414 & 325.597 & 404.973 & 408.760 & 0.002 & 0.002 & 84.559 & 83.163 & 0.232 & 5.779 \\ 
mCBP & 2.946 & 89 & 90 & 2.983 & 3.423 & 3.400 & 3.906 & 3.840 & 3.404 & 3.369 & 0.421 & 0.386 & 0.440 & 0.417 & 0.502 & 0.471 & 317.379 & 322.884 & 364.216 & 368.010 & 0.144 & 0.123 & 46.836 & 45.127 & 0.442 & 2.706 \\ 
benzoxazole & 2.197 & 80 & 81 & 1.964 & 2.882 & 2.842 & 3.541 & 3.483 & 2.413 & 2.407 & 0.449 & 0.443 & 0.918 & 0.878 & 1.128 & 1.076 & 350.109 & 355.959 & 513.817 & 515.115 & 0.332 & 0.285 & 163.707 & 159.156 & 0.588 & 1.891 \\ 
dbG2TAZ & 2.603 & 49 & 50 & 2.385 & 3.043 & 2.993 & 3.650 & 3.598 & 2.860 & 2.867 & 0.475 & 0.482 & 0.659 & 0.608 & 0.790 & 0.731 & 339.664 & 344.640 & 433.478 & 432.473 & 0.038 & 0.036 & 93.814 & 87.833 & 0.870 & 0.043 \\ 
V–TPA & 2.553 & 161 & 162 & 2.643 & 3.437 & 3.414 & 3.826 & 3.794 & 2.942 & 2.937 & 0.299 & 0.294 & 0.794 & 0.771 & 0.884 & 0.857 & 324.074 & 326.816 & 421.460 & 422.194 & 1.043 & 0.907 & 97.386 & 95.378 & 0.032 & 12.759 \\ 
CCDC & 1.677 & 124 & 125 & 2.217 & 3.231 & 3.210 & 3.417 & 3.415 & 2.344 & 2.358 & 0.128 & 0.142 & 1.015 & 0.994 & 1.073 & 1.057 & 362.835 & 363.015 & 528.899 & 525.772 & 0.002 & 0.002 & 166.064 & 162.757 & 0.199 & 8.775 \\ 
PXZPDO & 1.351 & 108 & 109 & 1.708 & 2.739 & 2.708 & 3.119 & 3.082 & 1.945 & 1.945 & 0.237 & 0.236 & 1.031 & 0.999 & 1.174 & 1.138 & 397.513 & 402.233 & 637.387 & 637.584 & 0.025 & 0.022 & 239.874 & 235.352 & 0.166 & 7.117 \\ 
DMAC-BP & 1.663 & 112 & 113 & 1.949 & 2.698 & 2.662 & 3.412 & 3.345 & 2.464 & 2.448 & 0.516 & 0.500 & 0.749 & 0.714 & 0.947 & 0.897 & 363.409 & 370.633 & 503.129 & 506.378 & 1.120 & 0.960 & 139.720 & 135.745 & 0.162 & 6.480 \\ 
SBTF & 2.289 & 131 & 132 & 2.022 & 2.829 & 2.779 & 3.570 & 3.497 & 2.552 & 2.544 & 0.530 & 0.522 & 0.807 & 0.757 & 1.018 & 0.953 & 347.334 & 354.565 & 485.916 & 487.334 & 1.463 & 1.206 & 138.582 & 132.769 & 0.911 & 0.768 \\ 
3-DPM & 1.152 & 104 & 105 & 1.627 & 2.514 & 2.502 & 2.755 & 2.732 & 1.783 & 1.776 & 0.156 & 0.149 & 0.887 & 0.875 & 0.972 & 0.955 & 450.017 & 453.872 & 695.405 & 697.987 & 0.020 & 0.017 & 245.388 & 244.115 & 0.251 & 4.807 \\ 
4-DPM & 1.521 & 104 & 105 & 1.668 & 2.226 & 2.189 & 2.850 & 2.817 & 2.135 & 2.147 & 0.467 & 0.479 & 0.558 & 0.521 & 0.715 & 0.670 & 435.048 & 440.066 & 580.674 & 577.452 & 1.299 & 1.160 & 145.627 & 137.386 & 0.415 & 2.840 \\ 
2CzPy & 2.617 & 89 & 90 & 2.603 & 3.401 & 3.378 & 3.883 & 3.816 & 2.971 & 2.940 & 0.368 & 0.338 & 0.799 & 0.775 & 0.912 & 0.876 & 319.308 & 324.906 & 417.336 & 421.668 & 0.136 & 0.112 & 98.027 & 96.762 & 0.431 & 4.035 \\ 
2PBCzPy & 2.360 & 177 & 178 & 2.356 & 3.488 & 3.467 & 3.974 & 3.913 & 2.685 & 2.659 & 0.328 & 0.303 & 1.132 & 1.111 & 1.290 & 1.253 & 311.981 & 316.884 & 461.840 & 466.235 & 0.172 & 0.141 & 149.860 & 149.351 & 0.282 & 8.491 \\ 
2BFCzPy & 2.569 & 121 & 122 & 2.560 & 3.429 & 3.405 & 3.845 & 3.797 & 2.871 & 2.855 & 0.311 & 0.295 & 0.869 & 0.845 & 0.975 & 0.942 & 322.414 & 326.558 & 431.875 & 434.301 & 0.432 & 0.379 & 109.462 & 107.743 & 0.438 & 4.408 \\ 
CNTPA-CZ & 2.513 & 110 & 111 & 2.694 & 3.074 & 3.046 & 3.727 & 3.675 & 3.267 & 3.251 & 0.573 & 0.557 & 0.380 & 0.351 & 0.460 & 0.424 & 332.638 & 337.335 & 379.499 & 381.340 & 0.713 & 0.613 & 46.861 & 44.005 & 0.432 & 5.424 \\ 
CNTPA-PXZ & 1.938 & 116 & 117 & 2.458 & 2.851 & 2.820 & 3.242 & 3.206 & 2.795 & 2.795 & 0.337 & 0.336 & 0.393 & 0.362 & 0.447 & 0.411 & 382.396 & 386.689 & 443.514 & 443.618 & 0.014 & 0.011 & 61.118 & 56.928 & 0.100 & 6.811 \\ 
BMZ-TZ & 1.885 & 120 & 121 & 1.760 & 3.381 & 3.378 & 3.373 & 3.372 & 1.756 & 1.757 & -0.004 & -0.003 & 1.621 & 1.618 & 1.618 & 1.615 & 367.557 & 367.709 & 706.243 & 705.784 & 0.008 & 0.007 & 338.686 & 338.074 & 0.573 & 1.557 \\ 
TPAPm & 1.745 & 109 & 110 & 2.024 & 2.727 & 2.699 & 3.369 & 3.341 & 2.500 & 2.506 & 0.476 & 0.482 & 0.703 & 0.675 & 0.869 & 0.835 & 368.015 & 371.055 & 495.866 & 494.737 & 2.082 & 1.913 & 127.851 & 123.682 & 0.405 & 1.677 \\ 
CzPm & 1.710 & 107 & 108 & 2.086 & 3.329 & 3.306 & 3.814 & 3.775 & 2.389 & 2.382 & 0.304 & 0.296 & 1.243 & 1.221 & 1.424 & 1.394 & 325.094 & 328.400 & 518.875 & 520.610 & 1.503 & 1.257 & 193.782 & 192.210 & 0.295 & 2.150 \\ 
TCPZ & 1.506 & 148 & 149 & 1.150 & 1.371 & 1.314 & 2.054 & 1.939 & 1.724 & 1.697 & 0.574 & 0.547 & 0.221 & 0.164 & 0.331 & 0.242 & 603.594 & 639.456 & 719.357 & 730.627 & 0.368 & 0.266 & 115.764 & 91.170 & 0.773 & 1.230 \\ 
TrisCz-Trz & 1.916 & 147 & 148 & 2.069 & 3.417 & 3.395 & 3.781 & 3.764 & 2.289 & 2.294 & 0.220 & 0.225 & 1.348 & 1.326 & 1.492 & 1.470 & 327.914 & 329.386 & 541.624 & 540.489 & 0.106 & 0.108 & 213.710 & 211.103 & 0.330 & 2.790 \\ 
PTZ–TAZ & 1.516 & 107 & 108 & 1.935 & 2.825 & 2.816 & 3.100 & 3.088 & 2.122 & 2.122 & 0.188 & 0.187 & 0.891 & 0.881 & 0.977 & 0.966 & 400.001 & 401.451 & 584.151 & 584.298 & 0.893 & 0.837 & 184.150 & 182.847 & 0.334 & 1.569 \\ 
DDMA-TXO2 & 2.348 & 124 & 125 & 2.587 & 3.402 & 3.370 & 3.952 & 3.888 & 3.005 & 2.984 & 0.418 & 0.397 & 0.815 & 0.784 & 0.947 & 0.904 & 313.725 & 318.930 & 412.627 & 415.564 & 0.037 & 0.024 & 98.901 & 96.634 & 0.221 & 4.339 \\ 
UGH3 & 3.606 & 105 & 106 & 3.458 & 5.189 & 5.145 & 5.214 & 5.187 & 3.475 & 3.486 & 0.017 & 0.028 & 1.731 & 1.687 & 1.740 & 1.701 & 237.773 & 239.043 & 356.815 & 355.692 & 0.000 & 0.000 & 119.042 & 116.650 & 0.603 & 0.903 \\ 
\end{longtable}

